Optimization and Evaluation of Nested Queries and Procedures

Many database applications perform complex data retrieval and update tasks. Nested queries, and queries that invoke user-defined functions, which are written using a mix of procedural and SQL constructs, are often used in such applications. A straight-forward evaluation of such queries involves repeated execution of parameterized sub-queries or blocks containing queries and procedural code. An important problem that arises while optimizing nested queries as well as queries with joins, aggregates and set operations is the problem of finding an optimal sort order from a factorial number of possible sort orders. We show that even a special case of this problem is NP-Hard, and present practical heuristics that are effective and easy to incorporate in existing query optimizers. We also consider iterative execution of queries and updates inside complex procedural blocks such as user-defined functions and stored procedures. Parameter batching is an important means of improving performance as it enables set-orientated processing. The key challenge to parameter batching lies in rewriting a given procedure/function to process a batch of parameter values. We propose a solution, based on program analysis and rewrite rules, to automate the generation of batched forms of procedures and replace iterative database calls within imperative loops with a single call to the batched form. We present experimental results for the proposed techniques, and the results show significant gains in performance.

==> abstract.tex <==
Many database applications perform complex data retrieval and update tasks.
Nested queries, and queries that invoke user-defined functions, which are
written using a mix of procedural and {\small SQL} constructs, are often
used in such applications.  A straight-forward evaluation of such queries
involves repeated execution of parameterized sub-queries or blocks
containing queries and procedural code. Repeated execution of queries and
updates also happens when external batch programs call database stored
procedures repeatedly with different parameter bindings. 

Iterative execution of queries and updates is often inefficient due to lack
of opportunities for sharing of work, random IO, and network round-trip
delays.  Query decorrelation is an important technique which addresses the
problem of iterative evaluation of nested queries, by rewriting them using
set operations such as joins and outer-joins.  Thereby, decorrelation
enables the use of set-oriented plans with reduced random IO, which are
often more efficient than the alternative iterative plans. However,
decorrelation is not applicable to complex nested blocks such as
user-defined functions and stored procedures. 

The focus of this thesis is to develop query evaluation, optimization and
program transformation techniques to improve the performance of repeatedly
invoked tasks such as parameterized database queries, updates,
stored-procedures and user-defined functions. 

To do so, we first propose enhancements to iterative query execution plans
which improve their efficiency by exploiting sorted parameter bindings and
state retention. For several queries, even when decorrelation is applicable,
an iterative plan can be the most efficient alternative. Hence, speeding up
the execution of iterative plans and their inclusion in the optimizer's
search space of alternative plans is important.  We show how to extend a
cost-based query optimizer so that the effects of sorted parameter bindings
and state retention of plans are taken into account. 

An important problem that arises while optimizing nested queries as well as
queries with joins, aggregates and set operations is the problem of finding
an optimal sort order from a factorial number of possible sort orders. Our
second contribution is to show that even a special case of this problem is
NP-Hard, and present practical heuristics that are effective and easy to
incorporate in existing query optimizers.

We then consider iterative execution of queries and updates inside complex
procedural blocks such as user-defined functions and stored procedures.
Parameter batching is an important means of improving performance as it
enables set-orientated processing. The key challenge to parameter batching
lies in rewriting a given procedure/function to process a batch of parameter
values.  Our third contribution is a solution, based on program analysis and
rewrite rules, to automate the generation of batched forms of procedures and
replace iterative database calls within  imperative loops with a single call
to the batched form.

We present experimental results for all the proposed techniques, and the
results show significant gains in performance.  \\

\noindent
{\bf Keywords:} Query optimization, Nested queries, Stored procedures,
                User-defined functions, Program transformation, 
                Parameter batching.


==> ack.tex <==
I have been very fortunate to have Prof. Sudarshan as my advisor. I am
indebted to Sudarshan for motivating me to take up research in database
systems, for guiding me at every stage and for his constant encouragement.
It is only due to his patience and understanding that I could cross the
hurdles of returning to academic life after a long gap.  His guidance and
appreciation were essential to drive things till the finishing line. 

I thank Prof. Sunita Sarawagi, Prof. N.L. Sarda and Prof. Krithi Ramamritham
for their feedback at various stages, and Prof. Ajit Diwan and Dr. Sobhan
Babu for extending their help and collaborating on parts of this thesis.
Thanks to Prasan Roy for the extensible Volcano implementation, it was a joy
working with his code; to Ramanujam H. S. and C.  Santosh Kumar for
assisting me in parts of the implementation. I thank Yogesh Murarka for the
several discussions, which educated me on the techniques and terminology
used in compilers and gave me clarity on several issues, and Sobhan, Shetal
and Aru for painstakingly reviewing parts of this thesis and my technical 
papers. 

I thank all my friends at IIT Bombay for making my days here so joyful.
%that now it's a hard time to leave the campus.  
Special thanks to Shetal, Sundar, Sita madam, my music teacher Shakuntala
madam and Puru for being so nice to me, and for feeding me often with great
food!, and to Sobhan for introducing me to the mountains and marathons.
Infolab has always been a great place to work and I thank all the
labmates, past and present, for having created such a wonderful environment.
The members of {\small CSE} office staff, particularly Vijay Ambre, have
provided timely help in all administrative tasks.

I thank Trivikram Nayak and my earlier colleagues at Aztecsoft, particularly
Govi, for all the help during the initial years. I am highly grateful to
Bell Laboratories for supporting me through a Ph.D. fellowship. 

Finally, I thank all my family members, especially my little nieces, for their
understanding through all these years.
%the state-retention techniques and extensions to external sorting. 
%the {\em NP-Hardness} proof and the 1/2-approximation algorithm presented in
%\refchap{chap:eio} are joint works with Ajit A. Diwan and Ch. Sobhan Babu.
%I thank Cesar Galindo-Legaria and Goetz Graefe for their
%feedback and clarifications.



==> appendices/bpo_extra_rules.tex <==
\chapter{Additional Transformation Rules}
\label{appen:extra-rules}
In \refchap{chap:concl}, we mentioned that our program transformation
techniques can be extended to build a single dataflow for queries with UDF
invocations, and thereby avoid materialization of parameter batches.  In
this section, we present a few additional program transformation rules, which
are useful for future work in this direction.

Rule 7 in \reffig{fig:rule-arith} and Rule 8 in \reffig{fig:rule-inline} are
useful in replacing loops containing simple expressions and assignment with
relational operators and avoiding materialization of intermediate results.

Batched forms of procedures are relation valued, {\em i.e.,} they return
sets of tuples. For example, the batched form of
\reffig{fig:trivial-batched-form} constructs the table to be returned
iteratively.  Rule 9 in \reffig{fig:rule-return} is useful to convert such
code into a set valued expression. The example in Appendix
\ref{step-by-step-trans} illustrates the use of Rule 9.

\begin{figure}[!h]
\begin{minipage}{0.5\textwidth}
{\bf Rule 7}
%{\scriptsize
\begin{transrule}
for each t by ref in r [order by key] loop \\
\>    t.b = {\em arith-expr}$(t.a_1, t.a_2, \ldots, t.a_n)$;  \\
end loop; \\
\hspace{10mm} {\large $\Updownarrow$}
\end{transrule}
%}
\vspace{-15pt}
{\small
\begin{transrule}
%$r = \Pi_{\{r.*-b\}, \textit{arith-expr}(t.a_1, t.a_2, \ldots, t.a_n)\ as\ b}(r)$ 
$r = \Pi_{A, \textit{arith-expr}(t.a_1, t.a_2, \ldots, t.a_n)\ as\ b}(r)$, 
\\
where {\em A=schema(r)}$-$$\{b\}$
\end{transrule}
}
\end{minipage}
\caption{Loops with Arithmetic Expressions and Assignment}
\label{fig:rule-arith}
\end{figure}

\newpage 

\begin{figure}[!h]
\begin{minipage}{0.5\textwidth}
{\bf Rule 8}
%{\scriptsize
\begin{transrule}
{\small Let expr1 be a side-effect free expression ({\em e.g.,} a query).} \\
\\
table r1 = expr1(); \\
table r2 = expr2(r1); \\
%\ \ \ {\large $\Leftrightarrow$}\ \ \  table r2 = expr2(expr1); \\
{\em dead}(r1)  // r1 unused hereafter \\
\hspace{10mm} {\large $\Updownarrow$} \\
table r2 = expr2(expr1);
\end{transrule}
%}
\end{minipage}
\caption{Rule for Avoiding Materialization}
\label{fig:rule-inline}
\end{figure}

\begin{figure}[!h]
\begin{minipage}{0.5\textwidth}
{\bf Rule 9}
%\scriptsize{
\begin{transrule}
table result; \\
for each t [by ref] in r [order by key] loop \\
%\>    result.addRecord($(t.a_1, t.a_2, \ldots, t.a_n)$);  \\
\>    result.addRecord($(c_1, c_2, \ldots, c_n)$);  \\
\>    // where each $c_i$ is a function of attributes of {\em t}. \\
end loop; \\
return result;\\
\hspace{10mm} {\large $\Updownarrow$} \\
return select $c_1, c_2, \ldots, c_n$ from r;
\end{transrule}
%}
\end{minipage}
\caption{Rule for {\em return} Statement}
\label{fig:rule-return}
\end{figure}

\noindent
We omit a formal proof of correctness for these transformation rules,
as their correctness is straight-forward to infer.



==> appendices/bpo_javamapping.tex <==
\chapter{API and Code Patterns}
As mentioned in \refsec{sec:perf:chap:bpo}, we implemented the transformation
rules for Java because tools for Java program analysis are available 
in public domain. We make use of the {\em SOOT} optimization framework 
for obtaining data dependence information. To simplify the task of 
recognizing query execution statements and code patterns that match
a rule, our current implementation requires that queries and updates 
be performed using our API layer built on top of JDBC. During rewrite,
we recognize these calls and transform them for batched bindings when 
possible. In this section, we give the details of our API layer and
the Java code patterns, which map to constructs described earlier,
in this thesis.
{\em SOOT} uses an intermediate code representation called {\em Jimple}. 
Our implementation works on {\em Jimple} and transforms it back to Java. 
Recognizing {\em Jimple} code patterns corresponding to each of our 
API calls and Java code patters is relatively straight forward and 
we omit the details.

\eat{
This mapping, used in our implementation, employs a custom API layer 
built on top of JDBC and is designed for easy recognition of program 
fragments that match the rule antecedents. It is possible to define 
alternative mappings - {\em e.g.}, a mapping that helps rewrite programs 
that directly make use of JDBC API. Mappings to languages like PL/SQL or
TSQL are more direct as the language constructs used in this thesis are
similar to the ones in those languages ({\em e.g.}, cursor loops).
}

\begin{itemize}
\item{\bf Query/Update Execution Statements}:
The class {\em DBI} in our implementation provides various methods for 
executing queries and updates.

{\small
\begin{itemize}
\item {\em Record executeScalarQuery(int queryId, Record params)}
%\item {\em Record executeScalarQuery(int queryId, \\ \hspace*{37mm} Record params)}
\item {\em Table executeQuery(int queryId, Record params)}
\item {\em int executeUpdate(int queryId, Record params)}
\end{itemize}
}

The {\em queryId} specifies a parameterized SQL query or update 
statement in a query registry. Unlike JDBC, where the query string 
is directly specified in the program, we make use of a registry.
The query registry, in addition to the query string, also contains 
the manually written batched form for the query.
Unlike position-based parameters 
in JDBC, we use named parameters. The {\em Record} class is used
to pass parameters as name-value pairs and also to obtain the
result of a scalar query. The class {\em Table} implements a 
tuple set and is used to retrieve query results, and for constructing
parameter batches.
% Sample entries in the registry
%SELECT city, state, zip FROM contactinfo WHERE emp-id=[empid]
%SELECT empid, city, state, zip FROM [batchtable] b, contactinfo c WHERE c.emp-id=b.empid

\begin{figure}[ht]
\begin{center}
\begin{tabular}{lcl}
\begin{minipage}{0.6\textwidth}
\scriptsize{
\ordinalg{
\\
%{\bf In Java} \\
Table res = DBI.executeQuery($\ldots$); \\
Iterator resIter = res.iterator(); \\
xxx\=xxx\=xxx\=\kill
while(resIter.hasNext()) $\{$ \\
    \> Record r = (Record) resIter.next(); \\
    \> $\ldots$ \\
$\}$ \\
}
}
\end{minipage}
&
\begin{minipage}{0.1\textwidth}
$\Longrightarrow$ \\
\end{minipage}
&
\begin{minipage}{0.3\textwidth}
\scriptsize{
\ordinalg{
%\noindent {\bf A Cursor Loop} \\
for each r in {\em query} \\
\> $\ldots$ \\
end loop; 
}
}
\end{minipage}
\end{tabular}
\end{center}
\caption{Pattern for Cursor Loops}
\label{fig:cursorloop}
\end{figure}


\item{\bf Looping Statements}:
{\em while} loops have a direct mapping to Java. Unlike some of
the procedural languages offered by database systems (e.g., PL/SQL), 
Java does not have cursor loops. Each cursor loop maps to a sequence 
of statements in Java. \reffig{fig:cursorloop} shows the code pattern.

\item{\bf Batched Execution}:
The class {\em Table} in our implemen\-tation can be used for constructing 
parameter batches row by row using the method {\em addRecord(Record r)}. The
DBI class has methods for executing batched forms of queries by passing
a batch of parameters and also for merging back the results. These methods 
are used by the transformed program (generated code).

{\small
\begin{itemize}
%\item {\em Table executeBatchedQuery(int queryId, \\ \hspace*{8mm}Table paramBatch)}
\item {\em Table executeBatchedQuery(int queryId, Table paramBatch, FilterPred pred)}
%\item {\em void executeBatchedUpdate(int queryId, \\ \hspace*{8mm}Table paramBatch)}
\item {\em void executeBatchedUpdate(int queryId, Table paramBatch, FilterPred pred)}
\end{itemize}
}

\item{\bf Other Constructs}:
Control flow, assignment and \- other constructs in the simple procedural
language used in this thesis have a direct mapping to Java. Conditional
statements, generated when control-dependencies are converted to
flow-dependencies, are Java {\em if} statements, where the {\em if-block}
contains a single statement and the predicate is a boolean variable.

\end{itemize}


==> appendices/bpo_proof_rule_correctness.tex <==
\chapter{Correctness of Transformation Rules}
\label{appendix3}

In this section, we give a formal proof of correctness of all the
program transformation rules presented in \refchap{chap:bpo}.

The {\em program state} $G$ comprises of values for all variables accessible 
at a program position $p$ and the {\em system state} $S$ comprises of the 
state of all external resources like database and file system. 
Let $P_L$ be a program fragment that matches the LHS of a rule and 
$P_R$ be the program fragment instantiated by the corresponding RHS.
Let $p$ be the position in the program at which $P_L$ 
begins. Let $(G,S)$ be the pair of {\em any} valid program and system 
states at $p$. To prove the correctness of a transformation rule, 
we must show the following. If the execution of $P_L$ on $(G,S)$ 
results in the state $(G', S')$ then the execution of $P_R$ on $(G, S)$ 
will also result in the state $(G', S')$.

\begin{itemize}
\item {\bf Rule 1A(i):}
%\noindent %{\bf Program State} \\
In Rule 1A(i), both $P_L$ and $P_R$ do not modify the program state 
(as we use a call by value semantics and there are no global variables). 

%\noindent {\bf System State} \\
Consider the multiset $S=\Pi^{d}_{c_{1}, c_{2}, \ldots, c_{m}}$ with 
which $qb$ is invoked.  Let $S'$ be the multiset of tuples
constructed from parameters passed to each invocation of $q$ inside
the loop. We can see that $S$ is multiset equivalent to $S'$. Now the 
equivalence of the two program fragments
follows directly from the definition of {\em batch-safe} 
operation (when an operation is batch-safe the final system state 
depends only on the set of parameters and not the order of 
invocations).
       
\item{\bf Rule 1A(ii):}
Proof is similar to that of Rule 1A(i).

\item{\bf Rule 1B:} 
%\noindent
The only program state $P_L$ and $P_R$ modify is the table $r$.
Let the initial state (state at the point where $P_L/P_R$ begins) 
of the table be $r_{init}$. Let $r'$ be the state 
the table reaches if $P_L$ is executed and
$r''$ be the state the table reaches if $P_R$ is executed. 
We show $r'$ and $r''$ to be multiset equivalent.

\vspace*{5pt}
Since $q$ is a scalar query, from the definition of {\em batched forms}
it follows that, during merge, each tuple in $r_{init}$ matches with exactly one 
tuple in the result of the batched invocation, 
$qb(\Pi_{c_{r1}, \ldots, c_{rm}}(r))$.
As a result, {\em (i)} cardinalities of $r', r''$ 
and $r_{init}$ are equal, i.e., $|r'|=|r''|=|r_{init}|$ and {\em (ii)} For each tuple
$t \in r_{init}$, there exists a distinct tuple $t' \in r'$ and a distinct tuple
$t'' \in r''$ such that $t$, $t'$ and $t''$ have the same values for all 
attributes except (possibly) the updated attributes {\em viz.,} 
$c_{w1}, c_{w2}, \ldots, c_{wn}$.  

\vspace*{5pt}
Let $t_r$ be the tuple in the result
of the batched invocation $(qb)$ that matches (during merge) with tuple 
$t$ of $r_{init}$. Let $(v_1, v_2, \ldots, v_m)$ be the values of attributes
$c_{r1}, c_{r2}, \ldots, c_{rm}$ of $t$. Therefore, attributes 
$c_{r1}, c_{r2}, \ldots, c_{rm}$
of $t_r$ must also have the values $(v_1, v_2, \ldots, v_m)$. Let 
$(w_1, w_2, \ldots, w_n)$ be the values of the remaining attributes
(named $c_{w1'}, c_{w2'}, \ldots, c_{wn'}$) of $t_r$. From the definition
of {\em batched forms}, we have 
$(w_1, w_2, \ldots, w_n) = q(v_1, v_2, \ldots, v_m)$. {\em i.e.,} the
tuple resulting from the merge ($t''$ in $r''$) has values assigned from
$q(v_1, v_2, \ldots, v_m)$ for its attributes $c_{w1}, c_{w2}, \ldots, c_{wn}$.
From the LHS of the rule, it is clear that the corresponding tuple
$t' \in r'$ also has the values of $q(v_1, v_2, \ldots, v_m)$ assigned 
for its attributes $c_{w1}, c_{w2}, \ldots,$ $c_{wn}$. This makes 
$t' = t''$ and hence $r'=r''$.

\eat{Further, there exists a 
one-to-one correspondence between the tuples of $r$, $r'$ and $r''$, 
where the corresponding tuples have the same value for the merge 
attributes.

Let $t'$ be any tuple in $r'$ and $t''$ be its corresponding tuple in
$r''$ ({\em i.e.,} $t'$  and $t''$ have the same value for the merge attributes).
From the definition of {\em batch-safe} operation and the semantics
of equi-join it is easy to see that $t'$ and $t''$ will have the
same values for all attributes. This makes $r'$ and $r''$ multiset 
equivalent.
}

\vspace*{5pt}
%\noindent {\bf System State} \\
Since $q$ is a {\em pure} function the system state remains 
unaffected by both $P_L$ and $P_R$.

\eat{
We can see that $qb$ is invoked with the same set of tuples with 
which $q$ gets invoked over all the iterations of the loop. Hence
from the definition of a batch-safe operation, the final system 
state in both the cases must be the same.
}
    
\item{\bf Rule 1C:}
Proof is similar to the proof for 1B.


\item{\bf Rule 1D:} 
The equivalence directly follows from the definition of batch-safe
operation.


\item{\bf Rule 2:} 
Let $P_L$ be the program fragment matching the LHS of the rule and $P_R$ be
the program fragment instantiated by the RHS.  Let us call the {\em while}
loop in $P_L$ as $L$, the first ({\em while}) loop of $P_R$, which contains
$ss_1'$, as $L_1$, the cursor loop after that, which contains $s'$, as
$L_2$, and the last cursor loop of $P_R$, which contains $ss_2$, as $L_3$.

First, we note that there exists a one-to-one correspondence between
statements in $ss_1$ of $L$ and statements in $ss_1'$ of $L_1$. The
correspondence follows from the construction of $ss_1'$. For every statement
$s_x$ in $ss_1$, the corresponding statement $s_x'$ in $ss_1'$ performs
exactly the same set of operations. 

Let $v$ be the value of a variable $a$ at statement $s_x$ in $ss_1$ in the
$i^{th}$ iteration of $L$.  As there are no loop-carried flow dependence
edges crossing the split boundaries, it is evident that the statement that
assigns value $v$ to variable $a$ must also appear in $L_1$ or must precede
$L_1$. Therefore, we can see that $v$ will be the value of $a$ at $s_x'$
(the statement corresponding to $s_x$) in the $i^{th}$ iteration of $L_1$. 

Similarly, we can see that values read by statement $s'$ in the $i^{th}$
iteration of $L_2$ are same as the value read by statement $s$ in the
corresponding iteration of $L$.

Now, consider a statement $s_y$ in $ss_2$ of loop $L$. Let $v$ be the value
of a variable $a$ read by $s_y$ in the $i^{th}$ iteration of $L$.  We now
prove by induction on $i$ that $v$ will be the value read by the
corresponding statement $s_y'$ in $L_3$.

Let $i=1$ (the first iteration). In this case, the assignment of $v$ to $a$
must be performed by a statement that precedes $s_y$ in $L$. Therefore, we
can observe that in the $i^{th}$ iteration of $L_3$, either a statement in
$ss_r$ or a statement that precedes $s_y'$ in $ss_2$ will assign $v$ to $a$.
And hence, $s_y'$ will read the value $v$ from $a$.

Now consider the $k^{th}$ iteration ($i=k$). In this case, $s_y$ will read
the value of $a$ which is either assigned by a preceding statement in the
$k^{th}$ iteration of $L$, or a the value of $a$, which was present at the
end of previous ($(k-1)^{th}$) iteration. In the former case, we will again
have a statement that precedes $s_y'$, which assigns value $v$ to $a$. In
the later case, we know by the induction hypothesis that the value of $a$ at the
end of $(k-1)^{th}$ iteration for both $L$ and $L_3$ will be the same. Since
$a$ was not assigned in the $k^{th}$ iteration by any statement preceding 
$s_y$, no statement in $ss_r$ will overwrite $a$. And hence, we see that 
$v$ will be the value read by $s_y'$ in the $k^{th}$ iteration.

Since there are no inter-statement dependencies involving external system
state, the output and change in system state produced by any statement $s_x$
and the corresponding statement $s_x'$ will be the same. Further, for every
non local variable $gv$, if the last assignment in $P_L$ was made by a
statement $s_x$ in the $i^{th}$ iteration of $L$, then in $P_R$ the last
assignment will be made by the corresponding statement $s_x'$ in the
$i^{th}$ iteration of $L_1$, $L_2$ or $L_2$. The only additional change
introduced by $P_R$ to the program state is the new variable {\em loopkey},
which is not used after the point where $P_R$ ends and hence does not affect
the program. Hence, the execution of both the $P_L$ and $P_R$ result in
equivalent program and system states.


\item{\bf Rules 3, 4 and 5:} 
The equivalence of these rules is straight forward to infer.

\item{\bf Rule 6A:} 
As in the proof for {\em Rule 1A}, we can observe that the multiset
of parameters passed to {\em qb} in $P_R$ is equivalent to the multiset 
of parameters passed over all the iterations of $P_L$. Hence, from 
the definition of the batch-safe operation, the equivalence holds.

\item{\bf Rule 6B:} 
\noindent The proof is similar to that of {\em Rule 1B}.

%\item{\bf Rules 7, 8 and 9:} 
%The equivalence of these rules is straight forward to infer.
\end{itemize}



==> appendices/bpo_queries.tex <==
%\chapter{Procedures used in Experiments}
\chapter{Procedures Used in Experiments}
\label{appendix1}
%\section*{Procedure for Experiment 2}
This section gives pseudocode for the additional procedures used for
performance evaluation in \refsec{sec:perf:chap:bpo}. \reffig{fig:nicproc}
shows the procedure for Experiment-3 and the procedure for Experiment-2 is
given in \reffig{fig:proc2}. The functionality implemented by these
procedures was explained earlier, in \refsec{sec:perf:chap:bpo}.

%\section*{Value Range Expansion: Exp 3}
\begin{figure}[ht]
\begin{minipage}{1.0\textwidth}
\scriptsize{
\ordinalg{
PROCEDURE expand-issued-forms(DATE issuedate) \\
DECLARE \\
    \> INT num; \\
BEGIN \\
    \> FOR EACH irec IN SELECT agent$\_$id, start$\_$no, end$\_$no, issue$\_$date \\
    \> \> \> \> \> FROM issued$\_$forms WHERE issue$\_$date = issuedate LOOP \\
    \> \> num := irec.start$\_$no; \\
    \> \> WHILE (num $<=$ irec.end$\_$no) LOOP \\
    \> \> \> INSERT INTO forms-master VALUES (num, irec.agent$\_$id, irec.issue$\_$date, 'NEW'); \\
    \> \> \> num := num + 1; \\
    \> \> END LOOP; \\
    \> END LOOP; \\
END; \\
}
}
\end{minipage}
\caption{Procedure for Experiment 3}
\label{fig:nicproc}
\end{figure}


\begin{figure}[ht]
\begin{minipage}{1.0\textwidth}
\scriptsize{
\ordinalg{
PROCEDURE emp-upload(VARCHAR filename) \\
DECLARE \\
    \> // Data types of local variables omitted for brevity. \\
    \> empid, clientid, iempid, optcode, optinfo, termcode, taxinfo, \\
    \> city, state, zip, operation, curtaxinfo, curcity, curstate, curzip\\
BEGIN \\
\>    fd := open(filename); \\
\>    linestr := readline(fd); \\
\>    WHILE (linestr $!=$ null) LOOP \\
\>  \>  tokenize linestr and extract empid, clientid, optcode, $\ldots$ zip \\
\>  \>  // some validation and pre-processing code  \\
\>  \>  if(optcode == 0) \\
\>  \>   \> optinfo = ... ; \\
\> \>  $\ldots$ \\
\\
\> \>   SELECT internl-empid into iempid, tax-info into curtaxinfo, \\
\> \>   FROM options WHERE client-id=clientid AND emp-id=empid; \\
\\
\> \>   // If options has no record for the employee \\
\> \>   if(iempid == null) $\{$ \\ 
\> \> \>    operation := 1;  // we must insert \\
\> \> \>    iempid := gen-new-id(); \\
\> \>   $\}$ \\
\> \>   else $\{$ \\
\> \> \>    operation := 2;  // we must update \\
\\
\> \> \>    SELECT city into curcity, state into curstate, zip into curzip \\
\> \> \>    FROM contactinfo  WHERE internal-empid=iempid; \\
\\      
\> \> \>    // Retain the current values if new ones are blank \\
\> \> \>    if(taxinfo == $""$) \\
\>  \> \>  \>   taxinfo := curtaxinfo; \\
\> \> \>    if(city == $""$) \\
\> \> \> \>     city := curcity; \\
\> \> \>    $\ldots$ \\
\> \> \>    $\ldots$ \\
\eat{
\> \> \>    if(state == "") \\
\> \> \> \>     state := curstate; \\
\> \> \>   if(zip  == "") \\
\> \> \> \>    zip := curzip; \\
}
\> \> $\}$ \\
\> \>  if(operation == 1) $\{$ \\
\> \> \>  INSERT INTO options VALUES (iempid, clientid, ... optinfo, ... taxinfo); \\
\> \> \>  INSERT INTO contactinfo VALUES(iempid, city, state, zip); \\
\> \>  $\}$ \\
\> \>   else $\{$ \\
\> \> \>    UPDATE options set option-info=optinfo, $\ldots$ tax-info=taxinfo \\
\> \> \>    WHERE internal-empid=iempid; \\
\> \> \>    UPDATE contactinfo SET city=city, state=state, zip=zip \\
\> \> \>    WHERE internal-empid=iempid; \\
\> \>  $\}$ \\
\> \>   linestr := readline(fd); \\
\>  END LOOP; \\
END; \\
}
}
\end{minipage}
\caption{Procedure for Experiment 2}
\label{fig:proc2}
\end{figure}




==> appendices/bpo_step_by_step_trans.tex <==
\chapter{Transformation Examples}
\label{step-by-step-trans}
In this section, we illustrate the transformation of the UDFs in
\refex{ex:udf-count-offers} and \refex{ex:udf-travcat} as the rules get
applied following the batching procedure in \reffig{fig:control-algo}. We
call these two UDFs as UDF-1 and UDF-2 respectively. Here, we assume that
every query needs to be batched (when possible) and with respect to all the
loops enclosing it.

\input{chapters/bpo/examples/udf1-batched.tex}
\input{chapters/bpo/examples/udf2-batched.tex}


==> appendices/eio_proof_optorder.tex <==
\onlythesis{\chapter{Optimality with Minimal Favorable Orders}}
\onlyjournal{\section{Proof of Optimality with Minimal Favorable Orders}}
\label{appen:proof-opt-order}
\newcommand{\fmin}{\text{\em ford-min}} 
\newcommand{\st}{\text{such that}}
The notion of {\em minimal favorable orders}, introduced in
\refsec{sec:favord:chap:eio}, served as the basis for our heuristics for
selecting sort orders. Since it is hard to compute the exact set of minimal
favorable orders, we used a heuristic approach to compute them
approximately. However, it is interesting to study the properties of minimal
favorable orders.  In this section we give a proof of
Theorem~\ref{theorem:optorder} stated earlier in \refsec{subsec:plangen}.
The theorem essentially states the following: to identify an optimal sort
order, it is sufficient to consider only the minimal favorable orders and
not the full set of favorable orders. Below, we repeat the formal statement
of the theorem and present a proof.  The proof makes use of notation
introduced in Sections~\ref{subsec:extsort} and \ref{subsec:favord}. \\

%\begin{theorem}
\noindent{\bf Theorem 3}
{\em
The set $\mathcal{I}(e,o)$ computed with exact ford-min contains an optimal
sort order $o_p$ for the optimization goal $e=(e_l \Join e_r)$ with $(o)$ as
the required output sort order.
}
%\end{theorem}

\noindent We prove Theorem~\ref{theorem:optorder} under the following
assumption: If $o_1$, $o_2$ are two sort orders on the same set of
attributes ({\em i.e.,} attrs$(o_1)$ $=$ attrs$(o_2)$), then the {\small
CPU} cost of sorting the result of an expression {\em e} to obtain $o_1$
will be same as that for $o_2$, {\em i.e.,} cpu-cost$(e, o_1)=$cpu-cost$(e,
o_2)$.

\begin{proof}
Consider the optimization goal for a join expression $(e=e_l\Join e_r$, with
$(o)$ as the sort order required on the result of $e$. Let $S$ be the set of
join attributes and $o'$ be any sort order on $S$.  The cost of the best
merge-join plan for $e$, when $o'$ is chosen as the sort order for 
$e_l$, $e_r$, is given by:
\begin{eqnarray}
\label{optproof:eqn1}
PC(e, o, o') & = &cbp(e_l, o') + cbp(e_r, o') + coe(e, o', o) + 
                            CM(e_l, e_r), \nonumber \\
              &  & \text{where } CM(e_l, e_r) \text{ is the cost of merging}.
\end{eqnarray}

\noindent
In Equation~\ref{optproof:eqn1}, we note that $CM(e_l, e_r)$ is independent
of the sort order $o'$. \\

\noindent
Let $o_b$ be an {\em optimal sort order} for $el \Join e_r$. Assume 
$o_b \notin \mathcal{I}(e)$.  We show that $\exists o_p\in \mathcal{I}(e)$ 
such that {\em PC}$(o_p)=${\em PC}$(o_b)$. \\

\noindent {\bf Case 1:} Suppose $o_b$ is such that $o_b \notin ford(e_l) \cup
ford(e_r)$. 
\begin{eqnarray}
\label{optproof:eqn2}
PC(e, o, o_b) &=& cbp(e_l, o_b) + cbp(e_r, o_b) + coe(e, o_b, o) + \nonumber \\
              & & CM(e_l, e_r) \\
\label{optproof:eqn3}
              & & \text{Since, } o_b \notin ford(e_l) \cup ford(e_r) 
                  \text{ we can write} \nonumber \\ 
              &=& cbp(e_l, \epsilon) + coe(e_l, \epsilon, o_b) + 
                  cbp(e_r, \epsilon) + \nonumber \\
              & & coe(e_r, \epsilon, o_b) + coe(e, o_b, o) + CM(e_l, e_r)
\end{eqnarray}


Let $o_p$ be a sort order in $\mathcal{I}(e)$ such that $o \wedge S \leq o_p$,
where $o$ is the required output sort order in the optimization goal.
The existence of such a sort order in $\mathcal{I}(e)$ directly follows from
the construction of $\mathcal{I}(e)$, specifically, steps 1 and 2 in 
\refsec{subsec:plangen}.

Since both $o_b$ and $o_p$ are sort orders on the same attribute
set $S$, we have
\begin{equation}
\label{optproof:eqn4}
coe(e_l, \epsilon, o_b)=coe(e_l, \epsilon, o_p) \text{ and }
coe(e_r, \epsilon, o_b)=coe(e_r, \epsilon, o_p)
\end{equation}

\noindent Substituting Equation~\ref{optproof:eqn4} in
Equation~\ref{optproof:eqn3} we get:
\begin{eqnarray}
\label{optproof:eqn5}
PC(e, o, o_b) &=& cbp(e_l, \epsilon) + coe(e_l, \epsilon, o_p) + 
                  cbp(e_r, \epsilon) + \nonumber \\
              & & coe(e_r, \epsilon, o_p) + coe(e, o_b, o) + 
                  CM(e_l, e_r) \\
\label{optproof:eqn6}
              &\geq& cbp(e_l, o_p) + cbp(e_r, o_p) + 
                     coe(e, o_b, o) + \nonumber \\
              & &    CM(e_l, e_r)
\end{eqnarray}

\noindent 
As $(o \wedge S) \leq o_p$, we have $(o_b \wedge o) \leq (o_p \wedge o)$ 
(because $o_b$ is a permutation of $S$). Therefore, 
$coe(e, o_b, o) \geq coe(e, o_p, o)$. From this, we can rewrite 
Equation~\ref{optproof:eqn6} as:
\begin{eqnarray}
PC(e, o, o_b) &\geq& cbp(e_l, o_p) + cbp(e_r, o_p) + 
                     coe(e, o_p, o) + CM(e_l, e_r) \nonumber \\
              &\geq& PC(e, o, o_p). \nonumber
\end{eqnarray}

\noindent
By assumption $o_b$ is an optimal sort order. So we conclude \-
$PC(e, o, o_b)= PC(e, o, o_p)$. In other words, $\mathcal{I}(e)$
contains a sort order $o_p$ having the same plan cost as the
optimal sort order $o_b$. \\

\noindent {\bf Case 2:} Suppose $o_b$ is such that $o_b \in ford(e_l)$ or
$ford(e_r)$ but not both. \\ Without loss of generality we assume $o_b \in
ford(e_l)$. This implies one of the following:

\eat{
\begin{equation}
\exists o' \in \fmin(e_l) \ \st \ o_b \leq o' \text{ and }
        cbp(e_l, o_b) = cbp(e_l, o') 
\end{equation}
or
\begin{equation}
\exists o' \in \fmin(e_l) \ \st\ o' \leq o_b \text{ and }
        cbp(e_l, o') + coe(e_l, o', o_b) = cbp(e_l, o_b)
\end{equation}
}

\begin{enumerate}[(i)]
\onlythesis{\addtolength{\itemsep}{-3mm}}
    \item $\exists o' \in$ {\em ford-min}$(e_l)$ such that $o_b \leq o'$ and
          $cbp(e_l, o_b) = cbp(e_l, o')$ or
   \item  $\exists o' \in$ {\em ford-min}$(e_l)$ such that $o' \leq o_b$ and
          $cbp(e_l, o') + coe(e_l, o', o_b) = cbp(e_l, o_b)$.
\end{enumerate}
\noindent We now consider, each of these cases separately.

\noindent {\bf Case 2-A}: Suppose condition (i), repeated below as 
Equation~\ref{optproof:eqn21}, holds.
%In this case, we know the following condition holds.
\begin{equation}
\label{optproof:eqn21}
\exists o' \in \fmin(e_l) \ \st\ o_b \leq o' \text{ and } 
                cbp(e_l, o_b) = cbp(e_l, o')
\end{equation}
%
\noindent
$o' \in \fmin(e_l)$ implies $(o' \wedge S) \in \fmin(e_l, S)$. Therefore,
from the construction of set $\mathcal{I}(e)$, we know:
\begin{equation}
\label{optproof:eqn23}
\exists o_p \in \mathcal{I}(e) \ \st\ (o' \wedge S) \leq o_p 
\end{equation}
%
\begin{equation}
\label{optproof:eqn24}
\text{Since } o_b \leq o', \text{ we know } (o_b \wedge S) \leq (o' \wedge S)
\end{equation}
%
Substituting Equation~\ref{optproof:eqn24} in Equation~\ref{optproof:eqn23},
we get $(o_b \wedge S) \leq o_p$. Since both $o_b$ and $o_p$ are permutations
of the same attribute set $S$, we must have $o_b=o_p$. {\em i.e.,} the
optimal sort order $o_b$ must be in $\mathcal{I}(e)$.

\noindent
{\bf Case 2-B}: Suppose condition (ii), repeated below as 
Equation~\ref{optproof:eqn25}, holds.
\onecolonly{
\begin{equation}
\label{optproof:eqn25}
\exists o' \in \fmin(e_l) \ \st \ o' \leq o_b \text{ and } 
                cbp(e_l, o') + coe(e_l, o', o_b) = cbp(e_l, o_b)
\end{equation}
}
\twocolonly{
\begin{eqnarray}
\label{optproof:eqn25}
\exists o' \in \fmin(e_l) \ \st \ o' \leq o_b \text{ and } \nonumber \\
                cbp(e_l, o') + coe(e_l, o', o_b) = cbp(e_l, o_b)
\end{eqnarray}
}
The plan cost for $e$, with $o_b$ as as the chosen sort order, is given by:
%
\onecolonly{
\begin{eqnarray}
\label{optproof:eqn26}
\hspace*{-8mm}
PC(e, o_b) &=& cbp(e_l, o_b) + cbp (e_r, o_b) + 
               coe (e, o_b, o) + CM(e_l, e_r) \nonumber \\
           & & \text{Substituting for $cbp(e_l, o_b)$ from 
                     Equation~\ref{optproof:eqn25}, we get} \nonumber \\
           &=& cbp(e_l, o') + coe(e_l, o', o_b) + cbp(e_r, o_b) + 
               coe(e, o_b, o) + CM(e_l, e_r) 
\end{eqnarray}
}
\twocolonly{
\begin{eqnarray}
\label{optproof:eqn26}
PC(e, o_b) &=& cbp(e_l, o_b) + cbp (e_r, o_b) + 
               coe (e, o_b, o) + CM(e_l, e_r) \nonumber \\
           & & \text{Substituting for $cbp(e_l, o_b)$ from 
                    Equation~\ref{optproof:eqn25}, we get} \nonumber \\
           &=& cbp(e_l, o') + coe(e_l, o', o_b) + cbp(e_r, o_b) + \nonumber \\
           & & coe(e, o_b, o) + CM(e_l, e_r) 
\end{eqnarray}
}
%
$o' \in \fmin(e_l)$ implies $\exists o_p \in \mathcal{I}(e) \ \st\ (o'
\wedge S) \leq o_p$.  Since $o' \leq o_b$, we know {\em attrs}$(o')
\subseteq S$.  Therefore, we have $o' \wedge S = o'$. And hence, $o' \leq
o_p$.  Also, since both $o_p$ and $o_b$ are permutations of $S$, we have
$|o_b|=|o_p|$.

\noindent
Since, $o_b \notin ford(e_r)$,  we have $cbp(e_r, o_b) =
cbp(e_r, o_p)$. Substituting this in Equation~\ref{optproof:eqn26}, we get:
%
\onecolonly{
\begin{equation}
\label{optproof:eqn27}
PC(e, o_b) = cbp(e_l, o') + coe(e_l, o', o_b) + cbp(e_r, o_p) + 
             coe(e, o_b, o) + CM(e_l, e_r) 
\end{equation}
}
\twocolonly{
\begin{eqnarray}
\label{optproof:eqn27}
PC(e, o_b) &=& cbp(e_l, o') + coe(e_l, o', o_b) + cbp(e_r, o_p) + \nonumber \\
           & & coe(e, o_b, o) + CM(e_l, e_r) 
\end{eqnarray}
}
%
Since $o' \leq o_b$ and $o' \leq o_p$ and $|o_b|=|o_p|$ we can write 
Equation~\ref{optproof:eqn27} as:
\onecolonly{
\begin{eqnarray}
\label{optproof:eqn28}
PC(e, o_b)   &=&   cbp(e_l, o') + coe(e_l, o', o_p) + cbp(e_r, o_p) + 
                   coe(e, o_b, o) + CM(e_l, e_r) \nonumber \\
           &\geq&  cbp(e_l, o_p) + cbp(e_r, o_p) + coe(e, o_b, o) + CM(e_l, e_r)
\end{eqnarray}
}
\twocolonly{
\begin{eqnarray}
\label{optproof:eqn28}
PC(e, o_b) &=& cbp(e_l, o') + coe(e_l, o', o_p) + cbp(e_r, o_p) + \nonumber \\
           & & coe(e, o_b, o) + CM(e_l, e_r) \nonumber \\
           &\geq&  cbp(e_l, o_p) + cbp(e_r, o_p) + \nonumber \\
           & &     coe(e, o_b, o) + CM(e_l, e_r)
\end{eqnarray}
}
%
\noindent Now, we show that $coe(e, o_b, o) \geq coe(e, o_p, o)$ to 
complete the proof.

\noindent
{\bf Case (a)}: Suppose, $o' \leq o$.  \\
Since $\mathcal{I}(e)$ contains a sort order
which subsumes, $o \wedge S$, it is possible to choose $o_p$ from
$\mathcal{I}(e)$ such that $(o \wedge S) \leq o_p$. This implies, $|o_b
\wedge o| \leq |o_p \wedge o|$.  Hence, $coe(e, o_b, o) \geq coe(e, o_p,
o)$. Substituting this in Equation~\ref{optproof:eqn28}, we get:
%
\begin{eqnarray}
\label{optproof:eqn29}
PC(e, o_b)  &\geq&  cbp(e_l, o_p) + cbp(e_r, o_p) + coe(e, o_p, o) + CM(e_l, e_r) \nonumber \\
            &\geq&  PC(e, o_p) \nonumber
\end{eqnarray}
%
\noindent
{\bf Case (b)}: Suppose, $o' \nleq o$.  \\
Now, $o' \wedge  o = o_b \wedge  o = o_p \wedge o$ (because $o' \leq o_b$
and $o' \leq o_p$). Therefore, $coe(e, o_b, o) = coe(e, o_p, o)$.
Substituting this in Equation~\ref{optproof:eqn28}, we get:
\begin{eqnarray}
\label{optproof:eqn30}
PC(e, o_b)  &\geq&  cbp(e_l, o_p) + cbp(e_r, o_p) + 
                    coe(e, o_p, o) + CM(e_l, e_r) \nonumber \\
            &\geq&  PC(e, o_p) \nonumber
\end{eqnarray}

\noindent {\bf Case 3:} Suppose $o_b$ is present in both {\em ford}$(e_l)$ 
                        and {\em ford}$(e_r)$ \\
This implies one of the following:
\begin{enumerate}[(i)]
    \item $\exists o' \in$ {\em ford-min}$(e_l)$ $\cup$ {\em ford-min}$(e_r)$ 
          such that $o_b \leq o'$.  In this case the proof can proceed as in 
          Case 2-A.

    \item $\exists o_1 \in$ {\em ford-min}$(e_l)$ and $\exists o_2 \in$ {\em ford-min}$(e_r)$
          such that {\em (a)} $o_1 \leq o_b$ and $o_2 \leq o_b$ and 
          {\em (b)} $cbp(e_l, o_1) + coe(e_l, o_1, o_b) = cbp(e_l, o_b)$ and
          {\em (c)} $cbp(e_r, o_2) + coe(e_r, o_2, o_b) = cbp(e_r, o_b)$. \\
          \\
          Since $o_1 \leq o_b$ and $o_2 \leq o_b$, either $o_1 \leq o_2$ or $o_2
          \leq o_1$. Hence, $\exists o_p \in \mathcal{I}(e)$ such that $o_1 \leq
          o_p$ and $o_2 \leq o_p$.  Choosing such an $o_p$, and proceeding as in
          Case 2-B we can prove $PC(e, o_b) \geq PC(e, o_p)$
\end{enumerate}
This completes the proof of Theorem~\ref{theorem:optorder}.
\end{proof}



==> appendices/extra-rules.tex <==
\subsection*{Extra Rules}
\label{extra-rules}
%This appendix provides few additional transformation rules.
Rule 7 in \reffig{fig:rule-arith} and Rule 8 in \reffig{fig:rule-inline} are
useful in replacing loops containing simple expressions and assignment with
relational operators and avoiding materialization of intermediate results.
As mentioned in \refchap{chap:concl} these rules can be used to
build a single dataflow for queries, which invoke UDFs that run inside the
database.  The {\em trivial batched form} (see
\reffig{fig:trivial-batched-form}) constructs the {\em return table}
iteratively.  Rule 9 in \reffig{fig:rule-return} is useful to convert this
into a set valued expression. The example in Appendix
\ref{step-by-step-trans} illustrates the use of this rule.

\begin{figure}[ht]
\begin{minipage}{0.5\textwidth}
{\bf Rule 7}
{\scriptsize
\begin{transrule}
FOR EACH t BY REF IN r [ORDER BY key] LOOP \\
\>    t.b = {\em arith-expr}$(t.a_1, t.a_2, \ldots t.a_n)$;  \\
END LOOP; \\
\hspace{10mm} {\large $\Updownarrow$}
\end{transrule}
}
\vspace{-15pt}
{\small
\begin{transrule}
%$r = \Pi_{\{r.*-b\}, \textit{arith-expr}(t.a_1, t.a_2, \ldots t.a_n)\ as\ b}(r)$ 
$r = \Pi_{A, \textit{arith-expr}(t.a_1, t.a_2, \ldots t.a_n)\ as\ b}(r)$, 
\\
where {\em A=schema(r)}$-$$\{b\}$
\end{transrule}
}
\end{minipage}
\caption{Loops with Arithmetic Expressions and Assignment}
\label{fig:rule-arith}
\end{figure}

\begin{figure}[ht]
\begin{minipage}{0.5\textwidth}
{\bf Rule 8}
{\scriptsize
\begin{transrule}
{\small Let expr1 be a side-effect free expression ({\em e.g.,} a query).} \\
\\
TABLE r1 = expr1(); \\
TABLE r2 = expr2(r1);
%\ \ \ {\large $\Leftrightarrow$}\ \ \  TABLE r2 = expr2(expr1); \\
{\em dead}(r1)  // r1 unused hereafter \\
\hspace{10mm} {\large $\Updownarrow$} \\
TABLE r2 = expr2(expr1);
\end{transrule}
}
\end{minipage}
\caption{Rule for Avoiding Materialization}
\label{fig:rule-inline}
\end{figure}

\begin{figure}[ht]
\begin{minipage}{0.5\textwidth}
{\bf Rule 9}
\scriptsize{
\begin{transrule}
TABLE result; \\
FOR EACH t [BY REF] IN r [ORDER BY key] LOOP \\
%\>    result.addRecord($(t.a_1, t.a_2, \ldots t.a_n)$);  \\
\>    result.addRecord($(c_1, c_2, \ldots c_n)$);  \\
\>    // where each $c_i$ is a function of attributes of {\em t}. \\
END LOOP; \\
RETURN result;\\
\hspace{10mm} {\large $\Updownarrow$} \\
RETURN SELECT $c_1, c_2, \ldots c_n$ FROM r;
\end{transrule}
}
\end{minipage}
\caption{Rule for {\small RETURN} Statement}
\label{fig:rule-return}
\end{figure}




==> chapters/bpo/algos/algo_main.tex <==
\begin{figure}[ht]
\begin{minipage}{0.5\textwidth}
\small {
\ordinalg{
{\bf procedure batch(Stmt s, Loop l)} \\
{\bf Inputs:} \\
    \> {\bf s}: \> The query execution statement to be batched \\
    \> {\bf l}: \> A program loop {\em w.r.t.} which the query must be batched ({\em i.e.}, {\bf s} must be pulled out of {\bf l}). \\
    \> \> {\bf s} may  be present directly inside {\bf l} or within a descendant loop of {\bf l}. \\ \\
    \> {\bf Note:} \> \ \ \ We assume the above inputs are provided manually; 
                            cost-based decision \\
    \>\> \ \ \              is a future work.

%    \> {\bf Note:} \> \ \ \ Deciding the above inputs in a cost-based manner
%                            is a future work and \\
%    \>\> \ \ \              we discuss it further in \refchap{chap:concl}.
\\
%{\bf Output:} \\
%    \> {\bf status}: True of the statement could be batched, False otherwise. \\
%\\
{\bf Goal:} \\
  \> Rewrite the program to batch the query execution in statement {\bf s} {\em w.r.t.} loop {\bf l}. \\
\\
%{\bf procedure batch(Stmt s, Loop l)} \\
{\bf begin} \\
%\>  // Check if {\em s} can be batched {\em w.r.t.} {\em l}. If not 
%       return false; \\

%\>  if {\em s} is on a {\em read-write conflict} cycle \\
%\> \>   return false; \\

\>  Let {\bf lp} be the loop which directly encloses {\bf s}. \\
\>  // Batch {\bf s} {\em w.r.t.} {\bf lp}. Let the batched statement 
       be {\bf sb}. \\
\>  {\bf sb} = do-batching({\bf s, lp}); \\

\>  if ({\bf lp} != {\bf l}) \\
\> \>   Let {\bf lpp} be the parent loop of {\bf lp} \\
\> \>   batch({\bf sb}, {\bf lpp}); \\
%\> return;
{\bf end}; \\

\\
{\bf procedure do-batching(Stmt s, Loop l)} \\
{\bf begin} \\
\>  Rewrite {\bf s} using Rule-3 so that {\bf s} is a simple assignment with only the query invocation \\
\>  expression on its RHS. \\
\\
\>  If s is control dependent on any statement inside loop l (other than the loop predicate), \\
\>  convert the control-dependency to flow dependency (using Rule-4). \\
\\
\>  Reorder the statements in {\bf l} to satisfy pre-conditions for Rule-2 (making use of Rule 5). \\ 
\>  {\em reorder(s, l.block);}  \hspace{6mm} // Procedure {\em reorder} is described later (Figures \ref{fig:reorder} and \ref{fig:movedirect}) \\
%\>  shift-back-edges(s, l);   // Uses {\bf Rule-5}. \\
\\  
\>  Applying Rule-2 split the loop {\bf l} at the program points before and after {\bf s}. \\
\\
\>  Batch the query execution using Rule 1 or Rule 6. \\
\\
\>  Return the reference to statement {\bf sb}, the batched form of {\bf s}. \\
end; \\
}
}
\end{minipage}
\caption{Control Algorithm for Rule Application}
\label{fig:control-algo}
\end{figure}



==> chapters/bpo/algos/algo_movedirect.tex <==
\begin{figure}[t]
\begin{minipage}{1.0\textwidth}
{\small
\ordinalg{
{\bf procedure} moveAfter(Stmt $s$, Stmt $t$) \\
{\em External variables used:}\\
\> List {\em srcDeps}, Stmt $s_q$  \hspace{4mm} // Constructed
by procedure {\em reorder} in \reffig{fig:reorder}\\
{\bf begin} \\
\>  if $s$ succeeds $t$ in the basic block \\
\>\>    return; \\

\>  Stmt {\em next} = successor($s$); \\
\>  do $\{$ \\
\>\>    if no flow/anti/output dependence edges between $s$ and {\em next} \\
\>\>\>      /* Reorder the statements by applying Rule-5A */ \\
\>\>\>      swap $s$ and {\em next}; \\
\>\>    else  $\{$\\
\>\>\>      for each $OD_v$ edge from $s$ to {\em next} $\{$  // {\boldmath $OD_v$}: output dependence on variable $v$ \\
\>\>\>\>        /* Shift the OD edge by applying Rule-5C */ \\
\>\>\>\>        Replace writes to $v$ in {\em next} by writes a new variable $v'$; \\
\>\>\>\>        Insert a new statement $as_v'$ that assigns $v'$ to $v$ 
                immediately after {\em next}; \\
\>\>\>\>        {\bf moveAfter}($as_v'$, $t$); \\
\>\>\>      $\}$\\
\\
\>\>\>      for each $AD_v$ edge from $s$ to {\em next} $\{$  // {\boldmath $AD_v$}: anti-dependence on variable $v$ \\
\>\>\>\>        /* Shift the AD edge by applying Rule-5B */ \\
\>\>\>\>        if there exists an $AD_v$ edge from $s_q$ to {\em next} \ \ \ \ // Use a reader stub\\
\>\>\>\>\>          Insert a new statement $as_v'$ that assigns $v$ to a new temp variable $v'$ \\
\>\>\>\>\>          immediately before $s$; \\
\>\>\>\>\>          Replace all read references to $v$ in s by $v'$; \\
\>\>\>\>        else  \ \ \ \ \ \ // Use writer stub \\
%\>\>\>\>        if s is there exists an edge $p \xrightarrow{FD_v} s$ where $p$ is in {\em srcDeps} \\
\>\>\>\>\>          Replace write of $v$ in {\em next} by write to a new temp var $v'$; \\
\>\>\>\>\>          Insert a new statement $as_v$ that assigns $v'$ to $v$ immediately after {\em next}; \\
\>\>\>\>\>          {\bf moveAfter}($as_v$, $t$); \\
\>\>\>     $\}$ \\
\>\>\>      swap $s$ and {\em next}; \\
\>\>   $\}$
\\
\>\>    {\em lastStmt} = {\em next}; \\
\>\>    if ({\em lastStmt} $!=$ $t$) \\
\>\>\>      {\em next}  = successor({\em s}); \\
\> $\}$ \\
\>  while({\em lastStmt} $!=$ $t$) ; \\
{\bf end}
}
}
\end{minipage}
\caption{Procedure {\em moveAfter}}
\label{fig:movedirect}
\end{figure}



==> chapters/bpo/algos/algo_reorder.tex <==
\begin{figure}[t]
\begin{minipage}{1.0\textwidth}
{\small
\ordinalg{
{\bf procedure reorder(BasicBlock $b$, Stmt $s_q$)} \\
// Goal: Reorder the statements within $b$, such that no LCFD edges cross \\
// the program points immediately preceding and succeeding $s_q$. \\
// Assumption: $s_q$ does not lie on a true-dependence cycle in the subgraph \\
// of the DDG induced by statements in $b$. \\
{\bf begin} \\
\>  while there exists an LCFD edge crossing the split boundaries for $s_q$ \\
\>\>    Pick an LCFD edge $(v_1, v_2)$ crossing the split boundaries. \\
\\
%\>\>    if $v_2 = s_q$ or $s_q$ has a true-dependence path from $v_2$ \\
\>\>    if there exists a true-dependence path from $v_1$ to $s_q$ \\
\>\>    /* No true-dependence path from $s_q$ to $v_1$ */ \\
\>\>\>      {\em stmtToMove} = $s_q$; \\
\>\>\>      {\em targetStmt} = $v_1$; \\
\>\>    else  \\
\>\>    /* No true-dependence path from $v_1$ to $s_q$, which implies no 
           true-dependence \\
\>\> \ \ \ \ path from $v_2$ to $s_q$ as there exists an  LCFD edge from 
           $v_1$ to $v_2$ */ \\
\>\>\>      {\em stmtToMove}  = $v_2$; \\
\>\>\>      {\em targetStmt}  = $s_q$; \\
\\
\>\>    // {\bf Move {\em stmtToMove} past the {\em targetStmt}} \\
\>\>    Compute {\em srcDeps}, the set of all statements between 
        {\em stmtToMove} and {\em targetStmt}, \\
\>\>    which have a flow dependence path from {\em stmtToMove}. \\
\\
%\>\>    Let tgtDeps be the set of all statements between stmtToMove and \\
%\>\>    targetStmt from which there is a flow dependency path to the targetStmt. \\
%\>\>    assert(srcDeps $\cap$ tgtDeps = $\phi$); \\
%\\ 
\>\>    while {\em srcDeps} is not empty \\
\>\>\>      Let $v$ be the statement in {\em srcDeps} closest to 
                                        {\em targetStmt} \\
\>\>\>      {\bf moveAfter}($v$, {\em targetStmt}); 
                      \hspace{4mm} // {\bf see \reffig{fig:movedirect}} \\
\\
\>\>    {\bf moveAfter}({\em stmtToMove}, {\em targetStmt}); \\
{\bf end;} 
}
}
\end{minipage}
\caption{Procedure {\em reorder}}
\label{fig:reorder}
\end{figure}


==> chapters/bpo/chap_bpo.tex <==
\chapter{Rewriting Procedures for Batched Bindings}
\label{chap:bpo}
In this chapter we consider parameter batching as a means of improving
performance of iteratively invoked database procedures. Several data
retrieval and update tasks need more expressive power than what standard
{\small SQL} offers. Therefore, many database applications perform queries
and updates from within procedural code that encodes business logic.  Stored
procedures and user-defined functions written using procedural extensions to
{\small SQL} ({\em e.g.}, {\small PL/SQL}~\cite{PLSQL}, {\small
PL/pgSQL}~\cite{PLPGSQL}\nocite{SQLPSM}) are widely used. Other paradigms
that allow mixing of procedural constructs with database access are {\small
SQL} extensions to procedural languages, {\em e.g.}, {\small
SQLJ}~\cite{SQLJ} and Microsoft's language integrated query ({\small
LINQ})~\cite{LINQ}, and application programming interfaces ({\small API})
for database access, {\em e.g.}, {\small JDBC, ODBC}.  Such
procedures/programs can run either inside a database system, as stored
procedures or user-defined functions ({\small UDF}), or outside the database
system.  As queries in {\small SQL} can in turn invoke {\small UDF}s (as
part of {\small WHERE/SELECT} clauses), control can alternate between the
{\small SQL} execution engine and the procedural code. 

We have earlier seen an example (\refex{ex:udf-count-offers} in
\refchap{chap:intro}) of a query that invokes a simple {\small UDF} in its
{\small WHERE} clause. In general, {\small UDF}s/procedures can be more
complex with arbitrary control-flow and looping. Such a {\small UDF} is
shown in \refex{ex:udf-travcat}, where the {\small UDF} counts the number of
items in a given category and all its sub-categories.

\input{chapters/bpo/examples/udf-travcat.tex}

Parameter batching is an important technique to speedup iterative execution
of queries and updates~\cite{GRA03,QPUPDATE}. Parameter batching allows the
choice of efficient set-oriented plans for queries and updates, thus
reducing random IO.  For inserts and updates batching allows efficient
integrity checks and index maintenance.  When the calls span across a
network, batching also helps in reducing network round-trip delays. 

\noindent In this chapter we present our work on automatic rewrite of
iterative programs to fulfill the following needs:

\begin{enumerate}[(a)]
\addtolength{\itemsep}{-4pt}
\item Rewrite {\small UDF}s and stored procedures to accept batched bindings
\item Rewrite programs that repeatedly execute a parameterized
      query or stored procedure to use batched invocation when possible
%\item Unnest queries having complex procedural nested blocks (e.g., queries
%      that invoke {\small UDF}s)
\end{enumerate}

The rest of this chapter is organized as follows.
\refsec{sec:define:chap:bpo} defines the problem, introduces the notion of
{\em batched forms} and {\em batch-safe} operations. We identify the program
transformation goal of pulling expensive operations out of loops as a key
for addressing the two needs mentioned above.  \refsec{sec:prelims:chap:bpo}
describes the background needed for our approach. In
\refsec{sec:rules:chap:bpo} we present the set of program transformation
rules, which together achieve the required program transformation, when the
program satisfies certain conditions. The program transformation rules rely
on the {\em data dependence graph} of the given program and can work with
complex procedures such as the ones shown in \refex{ex:udf-count-offers} and
\refex{ex:udf-travcat}.  We present the results of our experiments in
\refsec{sec:perf:chap:bpo}. The experiments are based on real-life examples
of performance problems.  We discuss related work in
\refsec{sec:relwork:chap:bpo} and summarize in
\refsec{sec:summary:chap:bpo}.

\input{chapters/bpo/sections/sec_define.tex}
\input{chapters/bpo/sections/sec_prelims.tex}
\input{chapters/bpo/sections/sec_rules.tex}
%\clearpage
\input{chapters/bpo/sections/sec_controlalgo.tex}
\input{chapters/bpo/sections/sec_condition.tex}
\input{chapters/bpo/sections/sec_perf.tex}
%\input{chapters/bpo/sections/sec_discuss.tex}
\input{chapters/bpo/sections/sec_relwork.tex}
\input{chapters/bpo/sections/sec_summary.tex}



==> chapters/bpo/examples/case1.tex <==
\begin{figure}[ht]
\begin{center}
\begin{minipage}{1.0\textwidth}
{\small 
\ordinalg{
for each r in \> \> \> SELECT grantid, empid, gnum FROM grantload loop \\ 
\> int internalid = foo(r.grantid, r.empid); \\ %$\lra (s1)
\> {\bf INSERT INTO grants VALUES (internalid, r.empid, r.gnum);} \\ % $\lra$ (s2)
\>  total $+=$ r.gnum; \\ % $\lra$ (s3)
end loop; \\
\\
\>\>\>{\Large $\Downarrow$} \\
\\
\\
TABLE(key, empid, gnum, internalid) t; \\
int loopkey = 0; \\
for each r in \> \> \> SELECT grantid, empid, gnum FROM grantload loop \\
    \> RECORD(key, empid, gnum, internalid) s; \\
    \> s.empid = r.empid; \ \ s.gnum  = r.gnum; \\
    \> int internalid = foo(r.grantid, r.empid); \\
    \> s.internalid = internalid; \\
    \> s.key  = loopkey++; \\
    \> t.addRecord(s); \\
end loop; \\
\\
for each s in t loop order by key \\%  --> (L2)
    \>  {\bf INSERT INTO grants VALUES (s.internalid, s.empid, s.gnum);} \\
end loop; \\
\\
for each s in t loop order by key \\ % --> (L3)
    \>    total += s.gnum; \\
end loop;
}
}
\end{minipage}
\end{center}
\caption{Splitting a {\tt cursor} loop}
\label{fig:loop-split-ex1}
\end{figure}



==> chapters/bpo/examples/case1b.tex <==
\begin{figure}[ht]
\begin{center}
\begin{minipage}{1.0\textwidth}
{\small
\ordinalg{
while (top $>$ 0) loop \\
    \> top $=$ top $-$ 1; \\
    \> curcat $=$ stack[top]; \\
    \> catitems = {\bf SELECT count(itemid) FROM item WHERE category=curcat;} \\
    \> totalcount $+=$ catitems; \\
end loop;\\
\\
\>\>\>\Large{$\Downarrow$} \\
\\
TABLE(key, curcat, catitems) t; \\
int loopkey = 0; \\
while(top $>$ 0) loop \\
    \> RECORD(key, curcat, catitems) r; \\
    \> top = top $-$ 1; \\
    \> curcat = stack[top]; \\
    \> r.curcat = curcat; \\
    \> r.key = loopkey$++$; \\
    \> t.addRecord(r); \\
end loop; \\
\\
for each r by ref in t order by key loop \\
    \> t.catitems = {\bf SELECT count(itemid) FROM item WHERE category=t.curcat;} \\
end loop; \\
\\
for each r in t order by key loop \\
    \> totalcount $+=$ t.catitems; \\
end loop; 
}
}
\end{minipage}
\end{center}
\caption{Splitting a {\tt while} loop}
\label{fig:loop-split-ex2}
\end{figure}



==> chapters/bpo/examples/case3.tex <==
\begin{figure}[t]
\begin{center}
\begin{tabular}{lcl}
\begin{minipage}{0.45\textwidth}
{\small
%\begin{sqlindent}
\ordinalg{
\\
xx\=xx\=xx\=xx\=\kill
for each t by ref in sales loop \\
    \> if (t.brcode $==$ 58)  \\
        \>\> t.brcode = 1; \\
        \>\> {\bf q(t.item, t.qty, t.brcode);} \\
    \> end if \\
end loop;
%\end{sqlindent}
}
}
\end{minipage}
&
\begin{minipage}{0.1\textwidth}
\centerline{\large{$\Longleftrightarrow$}} 
\end{minipage}
&
\begin{minipage}{0.45\textwidth}
{\small 
\ordinalg{
xx\=xx\=xx\=xx\=\kill
for each t by ref in sales loop \\
    \> // {\em Using a control variable remember} \\
    \> // {\em the branching decision} \\
    \> boolean cv = (t.brcode $==$ 58); \\
    \> (cv$==$true)? t.brcode = 1; \\
    \> {\bf (cv$==$true)? q(t.item, t.qty,}\\
    \> \hspace{1.2in}     {\bf t.brcode);} \\
end loop;
}
}
\end{minipage}
\eat{
\\
\begin{minipage}{0.2\textwidth}
\centerline{\large{ $\Updownarrow$}}
\end{minipage}
\\
\begin{minipage}{0.5\textwidth}
{\small
\ordinalg{
for each t by ref in sales loop \\
    \> t.cv = (t.brcode $==$ 58); \\
    \> (t.cv$==$true)? t.brcode = 1; \\
end loop; \\
for each t in sales loop \\
    \> {\bf (t.cv$==$true)? q(t.item, t.qty, t.brcode);} \\
end loop;
}
}
\end{minipage}
}
%\\
%\hline 
\end{tabular}
\end{center}
{\small
{\em Note: After this transformation, we can apply Rule-2 and split the
loop. The conditional invocation of {\bf q} can then be batched using Rule
1C.}
}

\caption{Transforming Control-Dependencies to Flow-Dependencies}
\label{fig:control-to-flow}

\end{figure}


==> chapters/bpo/examples/case3.tex.v13 <==
\begin{figure}[t]
\begin{center}
\begin{tabular}{l}
%\hline
\begin{minipage}{0.5\textwidth}
\scriptsize{
\ordinalg{
\\
for each t by ref in sales loop \\
    \> if (t.brcode $==$ 58)  \\
        \>\> t.brcode = 1; \\
        \>\> {\bf q(t.item, t.qty, t.brcode);} \\
    \> end if
end loop;
}
}
\end{minipage}
\\
\begin{minipage}{0.2\textwidth}
\centerline{\large{$\Updownarrow$}} 
\end{minipage}
\\
\begin{minipage}{0.5\textwidth}
\scriptsize {
\ordinalg{
for each t by ref in sales loop \\
    \> // Remember the branching decision in a boolean valued \\
    \> // control variable (cv) \\
    \> t.cv = (t.brcode $==$ 58); \\
    \> (t.cv$==$true)? t.brcode = 1; \\
    \> {\bf (t.cv$==$true)? q(t.item, t.qty, t.brcode);} \\
end loop;
}
}
\end{minipage}
\\
\begin{minipage}{0.2\textwidth}
\centerline{\large{ $\Updownarrow$}}
\end{minipage}
\\
\begin{minipage}{0.5\textwidth}
\scriptsize {
\ordinalg{
for each t by ref in sales loop \\
    \> t.cv = (t.brcode $==$ 58); \\
    \> (t.cv$==$true)? t.brcode = 1; \\
end loop; \\
for each t in sales loop \\
    \> {\bf (t.cv$==$true)? q(t.item, t.qty, t.brcode);} \\
end loop;
}
}
\end{minipage}
%\\
%\hline 
\end{tabular}
\end{center}
\caption{Splitting a loop after transforming control dependencies to flow-dependencies}
\label{fig:control-to-flow}
\end{figure}



==> chapters/bpo/examples/case4a.tex <==
\begin{figure}[ht]
\begin{center}
\begin{tabular}{lcl}
%\hline
\begin{minipage}{0.25\textwidth}
{\small
\ordinalg{
{\bf (i) Original Code} \\
%1234\=12\=12\=\kill
while (n $>$ 0) loop \\
    \> x = s[$--$n]; \\
    \> {\em // q() is to be batched; print() is not batch-safe}  \\
    \> print({\bf q(x)});  \\
end loop;
}
}
\end{minipage}
&
\begin{minipage}{0.05\textwidth}
\centerline {\Large{$\Leftrightarrow$}}
\end{minipage}
&
\begin{minipage}{0.25\textwidth}
{\small
\ordinalg{
{\bf (ii) After applying Rule-3} \\
%12\=12\=12\=\kill
while (n $>$ 0) loop \\
    \> x = s[$--$n]; \\
    \> {\em // Let T be type-of(q(...))} \\
    \> {\bf T v = q(x);} \\ 
    \> print(v); \\
end loop;
}
}
\end{minipage}
\eat{
&
\begin{minipage}{0.05\textwidth}
\centerline{{\large $\Leftrightarrow$}} %{\scriptsize After loop split} 
\end{minipage}
&
}
\\
\\
\begin{minipage}{0.4\textwidth}
\scriptsize{
\ordinalg{
%\\
{\bf (iii) After splitting the loop} \\
\\
Table(...) t; int loopkey = 0; \\
while (n $>$ 0) loop \\
%   \> ...   // construct the batch $r$ \\
    \> Record($\ldots$) r; \\
    \> x = s[$--$n]; \\
    \> r.x = x; r.key = loopkey++; t.addRecord(r); \\
end loop; \\
\\
{\em // order-by removed with Rule 1D}\\
for each {\em r} by ref in {\em t} loop \\
    \> {\bf r.v = q(r.x);} \\
end loop; \\
\\
{\em // order-by is required} \\
for each {\em r} in {\em t} order by {\em t.key} loop \\
    \> print(r.v); \\
end loop;
}
}
\end{minipage}
%\\
%\hline 
\end{tabular}
\end{center}

\caption{Separating Batch-Safe Operations}
\label{fig:separate-batch-safe}
\end{figure}


==> chapters/bpo/examples/case4a.tex.v3 <==
\begin{figure}[ht]
\begin{center}
\begin{tabular}{lcl}
%\hline
\begin{minipage}{0.25\textwidth}
{\small
\ordinalg{
{\bf (i) Original Code} \\
%1234\=12\=12\=\kill
for each {\em t} in {\em r} order by {\em r.key} loop \\
    {\em // print() is not batch-safe}  \\
    \> print({\bf q(t.c)});  \\
end loop;
}
}
\end{minipage}
&
\begin{minipage}{0.05\textwidth}
\centerline {\Large{$\Leftrightarrow$}}
\end{minipage}
&
\begin{minipage}{0.25\textwidth}
{\small
\ordinalg{
{\bf (ii) After applying Rule-3} \\
%12\=12\=12\=\kill
for each {\em t} in {\em r} order by {\em r.key} loop \\
    \> {\em // Let T be type-of(q(...))} \\
    \> {\bf T v = q(t.c);} \\ 
    \> print(v); \\
end loop;
}
}
\end{minipage}
\eat{
&
\begin{minipage}{0.05\textwidth}
\centerline{{\large $\Leftrightarrow$}} %{\scriptsize After loop split} 
\end{minipage}
&
}
\\
\\
\begin{minipage}{0.4\textwidth}
\scriptsize{
\ordinalg{
%\\
{\bf (iii) After splitting the loop} \\
\\
{\em // order-by removed with Rule 1D}\\
for each {\em t} by ref in {\em r} loop \\
    \> {\bf t.v = q(t.c);} \\
end loop; \\
\\
{\em // order-by is required} \\
for each {\em t} in {\em r} order by {\em r.key} loop \\
    \> print(t.v); \\
end loop;
}
}
\end{minipage}
%\\
%\hline 
\end{tabular}
\end{center}

\caption{Separating Batch-Safe Operation}
\label{fig:separate-batch-safe}
\end{figure}


==> chapters/bpo/examples/case4b.tex <==
\begin{figure}[t]
\begin{center}
\begin{tabular}{l|l|l}
\begin{minipage}{0.1\textwidth}
\scriptsize{
\ordinalg{
xx\=xx\=xx\=\kill
// {\tt some strange } \\
// {\tt logic.} \\
int max = $\ldots$; \\
$\ldots$\\
for r in t loop \\
\> if (r.a $>$ max) $\{$ \\
\>  \>  max = r.a; \\
\> $\}$ \\
\>  {\bf q(max);} \\
end loop; \\
\\
print(max); \\
}
}
\end{minipage}
&
\begin{minipage}{0.2\textwidth}
\scriptsize{
\ordinalg{
xx\=xx\=xx\=\kill
int max = $\ldots$; \\
$\ldots$\\
for r in t loop \\
\> int localmax = max; \\
\> if (r.a $>$ max) $\{$ \\
\>  \> localmax = r.a; \\
\>  \> max = localmax; \\
\> $\}$ \\
\>  {\bf q(localmax);} \\
end loop; \\
\\
print(max); \\
}
}
\end{minipage}
&
\begin{minipage}{0.2\textwidth}
\scriptsize{
\ordinalg{
xx\=xx\=xx\=\kill
int max = $\ldots$; \\
$\ldots$ \\
for r in t loop \\
\>    r.localmax = max; \\
\>    if (r.a $>$ r.localmax) $\{$ \\
\> \>   r.localmax = r.a; \\
\> \>   max = r.localmax; \\
\> $\}$ \\
end loop; \\
\\
for r in t loop \\
\>    {\bf q(r.localmax);} \\
end loop; \\
print(max);
}
}
\end{minipage}
\end{tabular}
\end{center}
%\caption{Splitting a loop after applying an auxillary transformation to satisfy condition (c3)}
\caption{Introducing a Loop Local to Enable Loop Splitting}
%after introducing transformation to satisfy condition (c3)}
\label{fig:case-nonlocal}
\end{figure}


==> chapters/bpo/examples/control-nonbatchable.tex <==
\begin{figure}[t]
\begin{center}
\begin{tabular}{|lclcl|}
\hline
\begin{minipage}{0.48\textwidth}
\scriptsize{
\ordinalg{
\\
while(x < n) loop \\
    \> y = y - 1; \\
    \> x = q(y); \\
end loop; \\
}
}
\end{minipage}
&
\begin{minipage}{0.04\textwidth}
\large{
$\Longrightarrow$ \\
}
\end{minipage}
&
\begin{minipage}{0.48\textwidth}
\scriptsize {
\ordinalg{
\\
for each t in q1(x) loop \\
    \> // Remember the branching decision \\
    \> // in a boolean control variable (cv) \\
    \> t.cv = t.qty $<$ 100; \\
    \> t.cv? t.qty = t.qty + 10; \\
    \> {\bf t.cv? q2(t.itemid);} \\
    \> foo(t.qty);  \\
end loop; \\
}
}
\end{minipage}
&
\begin{minipage}{0.04\textwidth}
\large{
$\Longrightarrow$ \\
}
\end{minipage}
&
\begin{minipage}{0.48\textwidth}
\scriptsize {
\ordinalg{
\\
TABLE(...) r = q1(x); \\
for each t in r by ref order by key loop \\
    \> t.cv = t.qty $<$ 100; \\
    \> t.cv? t.qty = t.qty + 10; \\a
end loop; \\

for each t in r loop \\
    \> {\bf t.cv? q2(t.itemid);} \\
end loop; \\

for each t in r order by key loop \\
    \> foo(t.qty);  \\
end loop; \\
}
}
\end{minipage}
\\
\hline 
\end{tabular}
\end{center}
\caption{Control Dependencies to Data Dependencies}
\label{fig:case3}
\end{figure}

\eat{
\begin{figure}
\begin{center}
\begin{tabular}{|lcl|}
\hline
\begin{minipage}{0.48\textwidth}
\scriptsize{
\ordinalg{
\\
if (qty $>$ 0) $\{$ \\
    \> qty = 0; \\
    \> proc = false; \\
$\}$ \\
else $\{$ \\
    \> proc = true; \\
$\}$ \\
}
}
\end{minipage}
&
\begin{minipage}{0.04\textwidth}
\large{
$\Longrightarrow$ \\
}
\end{minipage}
&
\begin{minipage}{0.48\textwidth}
\scriptsize {
\ordinalg{
\\
boolean cv = qty $>$ 0; \\
cv? qty = 0; \\
cv? proc = false; \\
!cv? proc = true; \\
\\
}
}
\end{minipage}
\\
\hline 
\end{tabular}
\end{center}
\caption{Control Dependencies to Data Dependencies}
\label{fig:case3}
\end{figure}
}


==> chapters/bpo/examples/nonlocal.tex <==
while(top > 0) {
    top = top - 1;
    curcat = stack[top];
    select count(itemid) into catitems from item where categoryid=curcat;
    totalcount += catitems;
}

TABLE (key, curcat, catitems) t;
int loopkey = 0;
while(top > 0) {
    Record r = new Record(type-of(t));
    top = top - 1;
    t.curcat = stack[top];
    t.loopkey = key++;
    t.AddRecord(r);
}

for each r in t order by key {
    select count(itemid) into t.catitems from item where categoryid=t.curcat;
}

for each r in t order by key {
    totalcount += t.catitems;
}
--------

    t = select curcat, count(items) as catitems from t LOJ item;




==> chapters/bpo/examples/reorder-examples.tex <==
\begin{figure}[ht]
\begin{tabular}{lcl}
\begin{minipage}{0.45\textwidth}
{\small
\ordinalg{
%{\bf To move s1 past s3} \\
{\bf while}(category != null) {\bf loop} \\
(s1) \> icount = {\bf q(category)}; \\
(s2) \> sum = sum + icount; \\
(s3) \> category = getParent(category); \\
{\bf end loop};
}
}
\end{minipage}
&
\begin{minipage}{0.15\textwidth}
\begin{center}
{\tiny Move s1 past s3} 
{\large $\Longrightarrow$}
\end{center}
\end{minipage}
&
\begin{minipage}{0.45\textwidth}
{\small
\ordinalg{
{\bf while}(category != null) {\bf loop} \\
(ts1)  category1 = category; \\
(s3)   category = getParent(category); \\
(s1)   icount = {\bf q(category1)}; \\
(s2)   sum = sum + icount; \\
{\bf end loop};
}
}
\end{minipage}
\end{tabular}
\caption{Example-1 of Statement Reordering}
\label{fig:reorder-ex1}
\end{figure}

\begin{figure}[ht]
\begin{tabular}{lcl}
\begin{minipage}{0.42\textwidth}
{\small
\ordinalg{
%{\bf To move s8 past s10-block} \\
{\bf while}(top $>$ 0 ) {\bf loop} \\
(s6)  top = top-1; \\
(s7)  curcat = stack$[$top$]$; \\
(s8)  catitems = {\bf q(curcat)};  \\
(s9)  totalcount = totalcount + catitems; \\
(s10') stack, top = block(curcat, top);  \\
{\bf end loop};
}
}
\end{minipage}
&
\begin{minipage}{0.13\textwidth}
\begin{center}
{\tiny Move s8 past s10'} 
{\large $\Longrightarrow$}
\end{center}

\end{minipage}
&
\begin{minipage}{0.45\textwidth}
{\small
\ordinalg{
{\bf while}(top $>$ 0 ) {\bf loop} \\
(s6)  top = top-1; \\
(s7)  curcat = stack$[$top$]$; \\
(s10') stack, top = block(curcat, top); \\
(s8)  catitems = {\bf q(curcat)};  \\
(s9)  totalcount = totalcount + catitems; \\
{\bf end loop};
}
}
\end{minipage}
\end{tabular}
\caption{Example-2 of Statement Reordering (from the UDF in \refex{ex:udf-travcat})}
\label{fig:reorder-ex2}
\end{figure}

\begin{figure}[h!]
\begin{center}
\begin{tabular}{lclcl}
\begin{minipage}{0.3\textwidth}
\scriptsize{
\ordinalg{
{\bf while}(pred(c)) {\bf loop} \\
%{\bf To move s1 past s4} \\
{\scriptsize (s1)} \> cv1? a = {\bf q(b)}; \\
{\scriptsize (s2)} \> cv2? a,c = f(x); \\
{\scriptsize (s3)} \> d = g(a, b); \\
{\scriptsize (s4)} \> cv3? a,b = h(c); \\
{\bf end loop};
}
}
\end{minipage}
&
\begin{minipage}{0.15\textwidth}
\begin{center}
{\tiny Move s1 past s4} 
{\large $\Longrightarrow$}
\end{center}
\end{minipage}
&
\begin{minipage}{0.3\textwidth}
\scriptsize{
\ordinalg{
{\bf while}(pred(c)) {\bf loop} \\
{\scriptsize (s2)} \> cv2? a3,c = f(x); \\
{\scriptsize (n1)} \> b2 = b; \\
{\scriptsize (n2)} \> b5 = b; \\
{\scriptsize (s4)} \> cv3? a1,b = h(c); \\
{\scriptsize (s1)} \> cv1? a = {\bf q(b5)}; \\
%{\scriptsize (n3)} \> cv1? a = a4; \\
{\scriptsize (n3)} \> cv2? a = a3; \\
{\scriptsize (s3)} \> d = g(a, b2); \\
{\scriptsize (n4)} \> cv3? a = a1;\\
{\bf end loop};
}
}
\end{minipage}
\end{tabular}
\end{center}
\caption{Example-3 of Statement Reordering}
\label{fig:reorder-ex3}
\end{figure}

\begin{figure}[h!]
\centerline{\psfig{file=chapters/bpo/fig/reorder-ex3.eps,height=6cm,width=10cm}}
\caption{Data Dependence Graphs for the Example of \reffig{fig:reorder-ex3}}
\label{fig:reorder-ex3-ddg}
\end{figure}

\begin{figure}[h]
\begin{center}
\begin{minipage}{1.0\textwidth}
\scriptsize{
\ordinalg{
{\em Table(key, a1, $\ldots$, b5, cv1, $\ldots$, cv3) t;} \\
{\em int loopkey = 0;} \\
{\bf while}(pred(c)) {\bf loop} \\
\> {\em Record r;} \\
{\scriptsize (s2)}  \> cv2? a3,c = f(x); \\
{\scriptsize (s2')} \> cv2? r.a3 = a3; \\
{\scriptsize (n1)}  \> b2 = b; \>\> {\scriptsize (n1')} \> r.b2 = b2; \\
{\scriptsize (n2)}  \> b5 = b; \>\> {\scriptsize (n2')} \> r.b5 = b5; \\
{\scriptsize (s4)}  \> cv3? a1,b = h(c); \>\> \> \> {\scriptsize (s4')} \> cv3? r.a1 = a1; \\
                    \> r.key = loopkey++;  \\
                    \> t.addRecord(r);  \\
{\bf end loop} \\
\\
{\bf for each} r by ref in t order by key {\bf loop} \\
{\scriptsize (s1)}  \> r.cv1? r.a = {\bf q(r.b5)}; \\
{\bf end loop;} \\
\\
{\bf for each} r by ref in t order by key {\bf loop} \\
\> boolean cv1, cv2, cv3; \\
\> int a1, a3, b2; \\
\> assigned(r.cv1)? cv1 = r.cv1; \\
\> $\ldots$ \\
%\> assigned(r.cv2)? cv2 = r.cv2; \\
%\> assigned(r.cv3)? cv3 = r.cv3; \\
%\> assigned(r.a1)? a1 = r.a1; \\
%\> assigned(r.a3)? a3 = r.a3; \\
%\> assigned(r.a4)? a4 = r.a4; \\
%\> assigned(r.b2)? b2 = r.b2; \\
\> assigned(r.b5)? b5 = r.b5; \\
\\
%{\scriptsize (n3)}  \> cv1? a = a4; \\
{\scriptsize (n3)}  \> cv2? a = a3; \\
{\scriptsize (s3)}  \> d = g(a, b2); \\
{\scriptsize (n4)}  \> cv3? a = a1;\\
{\bf end loop};
}
}
\end{minipage}
\caption{Loop Splitting Applied to Reordered Code in \reffig{fig:reorder-ex3}}
\label{fig:reorder-ex3-split}
\end{center}
\end{figure}




==> chapters/bpo/examples/simple_example_batched.tex <==
\begin{floatexample}
{\small
\begin{tabbing}
xxxxx\=xxxx\=xxxxxxxxx\=xxxxxxxxx\=\kill \\
    Let r1 = \> \> SELECT DISTINCT itemcode, amount, curcode 
         FROM sellorders WHERE  mkt='NSE'; \\
\\
{\small Now, the query of \refex{ex:udf-count-offers} can be written as:} \\
xxxxxxxxx\=xxxxxxxxx\=xxxxxxxxx\=\kill \\
   SELECT \> orderid FROM sellorder so, {\em count$\_$offers$\_$batched(r1)} br \\
   WHERE  \> so.mkt='NSE' AND so.itemcode=br.itemcode AND so.amount=br.amount AND \\
   \> so.curcode=br.curcode AND br.count$\_$offers $>$ 0; \\
\\
{\small where, {\em count$\_$offers$\_$batched} is the batched form of the UDF} 
{\small {\em count$\_$offers}} {\small defined as follows. For brevity,}
\\ {\small we omit the schema details when it is obvious.} \\
%%\line(1,0){470} \\

%{0.5\textwidth}
%\leaders\hrule 
%\begin{tabbing}
xxxx\=xxxx\=xxxx\=xxxx\=xxxx\=xxxx\=\kill  \\
TABLE {\bf count$\_$offers$\_$batched}(TABLE r1) \\
DECLARE \\
    \> TABLE (itemcode, amount, curcode, cond1,
    amount$\_$usd, count$\_$offers) $r2$;  // A temporary table \\
BEGIN \\
    \> FOR EACH t1 IN r1 LOOP \\
%        \> \> RECORD(...) t2; \\
        \> \> FLOAT amount$\_$usd; BOOLEAN cond1; INT count$\_$offers;\\
        \> \> cond1 := (t1.curcode $==$ "USD"); \\
        \> \> cond1 == true? amount$\_$usd := t1.amount; \\
%        \> \> t2.itemcount = t1.itemcount; t2.amount = t1.amount; \\
%        \> \> t2.curcode = t1.curcode; t2.cond1 = cond1; \\
%        \> \> t2.amount$\_$usd = amount$\_$usd; \\
%        \> \> r2.addRecord(t2); \\
        \> \> {\em // variables below take default values if unassigned} \\
        \> \> r2.addRecord((t1.itemcode, t1.amount, t1.curcode, cond1, amount$\_$usd, count$\_$offers)); \\
    \> END LOOP 
   \\
   \\ 
   \> MERGE INTO r2 USING {\bf q1b(e1)} AS q1b ON (r2.curcode=q1b.curcode) \\
   \> WHEN MATCHED THEN UPDATE SET amount$\_$usd = amount * q1b.exchrate; 
   \\
   \\
{\em //} \> where {\bf e1} is SELECT DISTINCT curcode FROM r2 WHERE cond1=false; \\
%{\em //} \> \> \> \> \> FROM r2 WHERE cond1=false; \\
{\em //} \> {\small and {\bf q1b}, the batched form of query q1, is shown
in \refex{ex:udf-co-batched-queries}.} 
   \\
   \\
   \> MERGE INTO r2 USING {\bf q2b(e2)} AS q2b  \\
   \> ON (r2.itemcode=q2b.itemcode AND r2.amount$\_$usd=q2b.amount$\_$usd) \\
   \> WHEN MATCHED THEN UPDATE SET count$\_$offers = q2b.count$\_$offers; \\
   \\
{\em //} \>  where {\bf e2} is SELECT DISTINCT itemcode, amount$\_$usd FROM r2;\\
{\em //} \> {\small and {\bf q2b}, the batched form of query q2, is shown
in \refex{ex:udf-co-batched-queries}.} 
   \\
   \\
   \> RETURN (SELECT itemcode, amount, curcode, count$\_$offers FROM r2;) \\
END \\
\\
{\small {\bf Note:} MERGE is a SQL:2003 construct.}

\eat{
   $e_2$ = \> {\bf SELECT} itemcode, amount, curcode, amount AS amount$\_$usd \\
               \> {\bf FROM} $e_1$ {\bf WHERE} curcode="USD"; \\
               \> {\bf UNION} \\
               \> {\bf SELECT} itemcode, amount, curcode, \\
               \> \> amount*exch$\_$rate AS amount$\_$usd \\
               \> {\bf FROM} $e_1$ {\bf WHERE} curcode$<>$"USD"; \\
\\
  $e_3$ = \> {\bf SELECT} itemcode, amount, curcode, count(*) 
                  AS count$\_$offers \\ 
               \> {\bf FROM} $e_2$, buyoffers {\bf WHERE} itemid=itemcode AND \\
               \>   \> price $>=$ amount$\_$usd \\
               \> GROUP BY itemcode, amount, curcode; \\
\\
}
\end{tabbing}
}
\caption{Batched Form of the Query in \refex{ex:udf-count-offers}}
\label{ex:udf-co-batched}
\end{floatexample}


==> chapters/bpo/examples/simple_example_batched_queries.tex <==
\begin{floatexample}
{\small 
\begin{tabbing}
xxxx\=xxxx\=xxxx\=xxxx\=xxxx\=xxxx\=\kill 
   {\small {\bf q1b(r):} The batched form of query {\bf q1}, with {\em r}
   as the parameter batch} \\  \\
   \> SELECT r.curcode, c.exchrate 
    FROM r JOIN curexch c ON r.curcode=c.ccode; 
   \\ 
   \\
   {\small {\bf q2b(r):} The batched form of query {\bf q2}, with {\em r} 
   as the parameter batch} \\ \\
   \> SELECT r.itemcode, r.amount$\_$usd, count(b.itemcode) AS count$\_$offers \\
   \> FROM r LEFT OUTER JOIN buyoffers b 
   ON b.itemid = r.itemcode AND \\
      \>\>\>b.price $>=$ r.amount$\_$usd \\
   \> GROUP BY r.itemcode, r.amount$\_$usd; 
\end{tabbing}
}
\caption{Batched Forms of Queries in ~\refex{ex:udf-count-offers}}
\label{ex:udf-co-batched-queries}
\end{floatexample}



==> chapters/bpo/examples/simple_example_loop.tex <==
\begin{floatexample}
{\small 
\ordinalg{
for each t in select orderid, itemcode, amount, curcode from sellorders  where mkt='NSE' loop \\
%  \\
    \> $<$ {\em body of the udf with parameters bound from t} $>$ \\
%    \\
    \> if (return value $>$ 0) \\
    \>   \> output t.orderid; \\
end loop
}
}
\caption{An Iterative Program/Plan for the Query in ~\refex{ex:udf-count-offers}}
\label{ex:udf-co-iter-plan}
\end{floatexample}


\eat{
r = SELECT orderid, ... FROM sellorders WHERE mkt='NSE';
for each t in r  {
    if (t.cc == "usd")
        usd = t.amount;
    else 
        exch = select ...;
        usd = amount * exch;

    int countoffer = select count(*) from ...
    if countoffer > 0;
        return r.orderid;
}

r = SELECT orderid, ..., usd FROM sellorders WHERE mkt='NSE';

for each t in r  {
    if (t.cc == "usd")
        t.usd = t.amount;
    else 
        exch = select ...;
        t.usd = amount * exch;
}
$e_2$ = \> SELECT itemcode, amount, curcode, amount AS amount$\_$usd \\
               \> FROM $e_1$ WHERE curcode="USD"; \\
               \> {\bf UNION} \\
               \> SELECT itemcode, amount, curcode, \\
               \> \> amount*exch$\_$rate AS amount$\_$usd \\
               \> FROM $e_1$ WHERE curcode$<>$"USD"; \\

int countoffer = select count(*) from ...
    if countoffer > 0;
        return r.orderid;

}


==> chapters/bpo/examples/swap-example1.tex <==
\begin{figure}[t]
\begin{center}
\begin{tabular}{|lclcl|}
\hline
\begin{minipage}{0.3\textwidth}
{\small
\ordinalg{
c = a + b; \\
a = d + e; \\
}
}
\end{minipage}
&
\begin{minipage}{0.05\textwidth}
\large{
$\Longrightarrow$ \\
}
\end{minipage}
&
\begin{minipage}{0.3\textwidth}
{\small
\ordinalg{
c = a + b; \\
a' = d + e; \\
a = a'; \\
}
}
\end{minipage}
&
\begin{minipage}{0.05\textwidth}
\Large {
$\Longrightarrow$ \\
}
\end{minipage}
&
\begin{minipage}{0.3\textwidth}
{\small
\ordinalg{
a' = d + e; \\
c = a + b; \\
a = a'; \\
}
}
\end{minipage}
\\
\hline 
\end{tabular}
\end{center}
\caption{{\small Order Reversal by Breaking Anti-Dependency Edges} }
\label{fig:swap-ex1}
\end{figure}


==> chapters/bpo/examples/swap-example2.tex <==
\begin{figure}[t]
\begin{center}
\begin{tabular}{|l|l|l|l|}
\hline
\begin{minipage}{0.5\textwidth}
{\small
\ordinalg{
xxxxx\=xxxxx\=\kill
{\bf c = a + b;} \> \> (s1) \\
e = c + d; \> \>  (s2) \\
a = f + g; \> \>  (s3) \\
{\bf c = a + h;} \> \> (s4) \\
}
}
\end{minipage}
&
\begin{minipage}{0.5\textwidth}
{\small
\ordinalg{
xxxxx\=xxxxx\=\kill
{\bf c = a + b;} \> \> (s1) \\
e = c + d;  \> \> (s2) \\
a' = f + g;  \> \> (s3) \\
a = a'; \> \> (s3') \\
{\bf c' = a + h;} \> \> (s4)  \\
c = c';  \> \> (s4') \\
}
}
\end{minipage}
&
\begin{minipage}{0.5\textwidth}
{\small
\ordinalg{
xxxxx\=xxxxx\=\kill
{\bf c = a + b;}  \> \> (s1) \\
e = c + d;  \> \> (s2) \\
a' = f + g; \> \> (s3) \\
{\bf c' = a' + h;} \> \> (s4) \\
a = a'; \> \> (s3') \\
c = c'; \> \> (s4') \\
}
}
\end{minipage}
&
\begin{minipage}{0.5\textwidth}
{\small
\ordinalg{
xxxxx\=xxxxx\=\kill
a' = f + g; \> \> (s3) \\
{\bf c' = a' + h;} \> \> (s4)  \\
{\bf c = a + b;} \> \> (s1) \\
e = c + d; \> \>  (s2) \\
a = a';  \> \> (s3') \\
c = c'; \> \> (s4') \\
}
}
\end{minipage}
\\
\hline 
\end{tabular}
\end{center}
\caption{{\small Order Reversal when no Flow-Dependency Path Exists} }
\label{fig:swap-ex2}
\end{figure}


==> chapters/bpo/examples/udf-travcat.tex <==
\begin{floatexample}
{\small 
\begin{tabbing}
xx\=xxxxxxxxx\=xxxxxxxxx\=xxxxxxxxx\=\kill \\
\> SELECT * FROM category WHERE count$\_$items(category$\_$id) $>$ f(level);
\end{tabbing}
}
%\end{query}

{\small
\ordinalg{
%\> CREATE FUNCTION count$\_$items(catid INT) RETURNS INT AS \\
\> INT count$\_$items(INT catid) \\
\> DECLARE  \\
\>    \> INT totalcount; INT curcat; INT catitems; INT subcat; \\
\>    \> INT stack$[$100$]$; INT top; RECORD catrec; \\

\> BEGIN \\
s1: \>    \> totalcount := 0; \\
s2: \>    \> top := 0; \\
s3: \>    \> stack$[$top$]$ = catid; \\
s4: \>    \> top := top + 1; \\

s5: \>    \> WHILE top $>$ 0 LOOP  \\
s6: \>    \>  \> top := top $-$ 1; \\
s7: \>    \>  \> curcat := stack$[$top$]$; \\

s8: \>    \> \> catitems := SELECT count(item$\_$id) FROM item 
                            WHERE category$\_$id = curcat; \\
%    \>    \> \> \> \> \> WHERE category$\_$id = curcat; \\
s9: \>    \> \> totalcount := totalcount + catitems; \\

\\
\>    \> \> // Now push all the subcategory ids onto the stack \\
s10: \>    \> \> FOR catrec IN SELECT category$\_$id FROM category \\
    \>     \> \> \> \> \> WHERE parent$\_$category=curcat LOOP \\
s11: \>    \> \> \> stack[top] := catrec.category$\_$id; \\
s12: \>    \> \> \> top := top + 1; \\
\>    \>  \> END LOOP; \\
\>    \> END LOOP; \\
s13: \>    \> RETURN totalcount; \\
\>END;
}
}
\caption{Query with a Complex UDF - Items in a Category and Sub-Categories}
\label{ex:udf-travcat}
\end{floatexample}
%\end{minipage}
%\caption{Query Invoking a Complex UDF}
%\label{fig:sampleudf}
%\end{figure}



==> chapters/bpo/examples/udf1-batched.tex <==
\subsection*{Rewriting UDF-1}
\begin{itemize}
\item{\bf Generate the Trivial Batched Form:}
First, we generate the {\em trivial batched form} of the procedure as explained 
in \refsec{sec:gen-batched-form}. \reffig{fig:step1} shows the resulting 
procedure.

\begin{figure}[ht]
\begin{minipage}{1.0\textwidth}
\scriptsize{
\ordinalg{
TABLE count-offers-batched(TABLE r1)  \\
DECLARE \\
 \> TABLE result; \\
BEGIN \\
 \> FOR EACH t IN r1 LOOP \\
 \> \>  FLOAT amount-usd; \\
 \> \>  INT count-offers;  // The return value named after the function \\
 \> \>  IF (t.curcode == "USD") \\
 \> \> \>   amount-usd := t.amount; \\
 \> \>  ELSE \\
 \> \> \>   amount-usd := t.amount * (SELECT exchrate FROM curexch \\
 \> \> \>            \>\>\>\>\>\>     WHERE ccode = t.curcode);  \\
 \> \>  END IF \\
 \> \> count-offers := SELECT count(*) FROM buyoffers \\
 \> \>                    \> \> \> \ \ WHERE itemid = t.itemcode AND 
                                             price $>=$ amount-usd; \\
 \> \> result.addRecord((t.itemcode, t.amount, t.curcode, count-offers)); \\
 \> END LOOP; \\
 \> RETURN result; \\
END;
}
}
\end{minipage}
\caption{UDF-1: Trivial Batched Form}
\label{fig:step1}
\end{figure}

\item {\bf Isolate the Query Execution:}
We isolate the query (expression) to be batched using Rule-3 and 
convert the control-dependencies to flow-dependencies using Rule-4.
The resulting procedure after applying these two rules is shown 
in \reffig{fig:step2}.

\begin{figure}[t]
\begin{minipage}{0.5\textwidth}
{\small
\ordinalg{
TABLE count-offers-batched(TABLE r1)  \\
DECLARE \\
\>  TABLE result; \\
BEGIN \\
\>  FOR EACH t IN r1 LOOP  \\
\> \> FLOAT amount-usd; INT count-offers;\\
\> \> BOOLEAN cond1;  FLOAT exchrate; \\
%\> \> cond1  BOOLEAN; \\
%\> \> exchrate FLOAT; \\
\> \> cond1 := (t.curcode == "USD"); \\
\> \> cond1 == true?  amount-usd := t.amount; \\
\> \> cond1 == false? exchrate := SELECT exchrate FROM curexch \\
\> \>          \>\>\>\>\>\>\ \    WHERE ccode = t.curcode;  \\
\> \> cond1 == false? amount-usd := t.amount * exchrate; \\
\> \> count-offers := SELECT count(*) FROM buyoffers \\
\> \>       \>\>\>\ \ WHERE itemid = t.itemcode AND price $>=$ amount-usd;\\
\> \> result.addRecord((t.itemcode, t.amount, t.curcode, count-offers)); \\
\>  END LOOP; \\
\>  RETURN result; \\
END; 
}
}
\end{minipage}
\caption{UDF-1: After Applying Rules 3 and 4}
\label{fig:step2}
\end{figure}

\eat{
\begin{figure}[t]
\begin{minipage}{0.5\textwidth}
\scriptsize{
\ordinalg{
TABLE result; \\
FOR EACH t [BY REF] IN r [ORDER BY key] LOOP \\
\>    result.addRecord($(t.a_1, t.a_2, \ldots t.a_n)$);  \\
END LOOP; \\
RETURN result;\\
\hspace{10mm} {\large $\Updownarrow$} \\
RETURN SELECT $a_1, a_2, \ldots a_n$ FROM r;
}
}
\end{minipage}
\caption{Auxiliary Rule for Return Statement}
\label{fig:rule-return}
\end{figure}
}

\item {\bf Split the Loop:}
Split the loop (by applying Rule-2) before and after the query execution 
statements. In this example, the pre-conditions for Rule-2 are directly 
satisfied and we do not need to reorder any statements. However, in some
cases we may need to reorder the statements using Rule-5 to satisfy the
pre-conditions for Rule-2. 
%The resulting program is shown in 
\reffig{fig:step3} shows the resulting program.

\begin{figure}[ht]
\begin{minipage}{1.0\textwidth}
\scriptsize{
\ordinalg{
TABLE count-offers-batched(TABLE r1) \\
DECLARE \\
\>  TABLE result; INT loopkey = 0; \\
\>  TABLE (key, itemcode, amount, curcode, cond1, exchrate, amount-usd, count-offers) r2; \\
BEGIN \\
\>  FOR EACH t IN r1 LOOP  \\
\> \>   FLOAT  amount-usd; BOOLEAN cond1;\\
%\> \>  INT     count-offers; \\
%\> \>  BOOLEAN cond1; \\
\> \>   RECORD  rec; \\
\\       
\> \>   cond1 := (t.curcode == "USD"); \\
\> \>   cond1 == true?  amount-usd := t.amount; \\
        
\> \>   rec.key = loopkey++; \\
\> \>   rec.itemcode   = t.itemcode; \\
\> \>   rec.amount     = t.amount; \\
\> \>   rec.curcode    = t.curcode; \\
\> \>   rec.cond1      = cond1; \\
\> \>   rec.amount-usd = amount-usd; \\
        
\> \>   r2.addRecord(rec); \\
\>  END LOOP; \\
\\
\>  FOR EACH t BY REF IN r2 ORDER BY key LOOP \\
\> \>   t.cond1 == false? t.exchrate :=  \\
\> \>   \> \> \> SELECT exchrate FROM curexch WHERE ccode = t.curcode; \\
\>  END LOOP; \\
\\
\>  FOR EACH t BY REF IN r2 ORDER BY key LOOP \\
\>\>    t.cond1 == false? t.amount-usd := t.amount * t.exchrate; \\
\>  END LOOP; \\
\\
\>  FOR EACH t BY REF IN r2 ORDER BY key LOOP \\
\> \>   t.count-offers := SELECT count(*) FROM buyoffers \\
\> \>   \>\>\>\>          WHERE  itemid = t.itemcode AND 
                                 price $>=$ t.amount-usd; \\
\>  END LOOP; \\
\\
\>  FOR EACH t BY REF IN r2 ORDER BY key LOOP \\
\> \>   result.addRecord((t.itemcode, t.amount, t.curcode, t.count-offers));  \\
\>  END LOOP; \\
\\
\>  RETURN result; \\
END; 
}
}
\end{minipage}
\caption{UDF-1: After Loop Split}
\label{fig:step3}
\end{figure}

\item{\bf Replace Loops with Batched Calls:}
Apply Rule-1D to remove the order-by clauses around batch-safe operations 
and then replace the iterations with batched calls using Rules 1B and 1C.
We further apply Rule 9 (\reffig{fig:rule-return})
for the RETURN statement. The resulting program is given in 
\reffig{fig:final}. 
Earlier, in \refex{ex:udf-co-batched} we had shown this batched 
form with minor simplifications for readability.
%The batched form of UDF-1 shown earlier 
%in \reffig{fig:simpleudf-batched} was slightly simplified 
%for readability.

\begin{figure}[ht]
\begin{minipage}{1.0\textwidth}
\scriptsize{
\ordinalg{
TABLE count-offers-batched(TABLE r1)  \\
DECLARE \\
%\>  TABLE result; \\
\>  TABLE (key, itemcode, amount, curcode, cond1, exchrate, amount-usd, count-offers) r2; \\
\>  INT loopkey = 0; \\
BEGIN \\
\>  FOR EACH t IN r1 LOOP  \\
\> \>   FLOAT   amount-usd; BOOLEAN cond1; \\
\> \>   RECORD  rec; 
\\     
\> \>   cond1 := (t.curcode == "USD"); \\
\> \>   cond1 == true?  amount-usd := t.amount; \\
\> \>   rec.key = loopkey++; \\
\> \>   rec.itemcode   = t.itemcode; \\
\> \>   rec.amount     = t.amount; \\
\> \>   rec.curcode    = t.curcode; \\
\> \>   rec.cond1      = cond1; \\
\> \>   rec.amount-usd = amount-usd; \\
\> \>   r2.addRecord(rec); \\
\>  END LOOP; \\
\\
\>  MERGE INTO r2 USING q1b(b1) AS q1b ON (r2.curcode = q1b.curcode) \\
\>  WHEN MATCHED THEN  UPDATE SET exchrate = q1b.exchrate; \\
\\  
//\>  where the parameter batch {\bf b1} is constructed as: \\
//\>\>  SELECT distinct curcode FROM r2 WHERE cond1=false; \\
//\>  and the batched form {\bf q1b(b1)} is defined as: \\
//\>\>  SELECT b1.curcode, c.exchrate FROM b1 JOIN curexch c ON b1.curcode=c.ccode; \\
\\
\>  FOR EACH t BY REF IN r2 ORDER BY key LOOP \\
\> \>   t.cond1 == false? t.amount-usd := t.amount * t.exchrate; \\
\>  END LOOP; \\
\\
\>  MERGE INTO r2 USING q2b(b2) AS q2b \\
\>  ON (r2.itemcode=q2b.itemcode AND r2.amount-usd=q2b.amount-usd) \\
\>  WHEN MATCHED THEN UPDATE SET count-offers = q2b.count-offers; \\
\\
\>  where {\bf b2}     = SELECT distinct itemcode, amount-usd FROM r2; \\
\>  and {\bf q2b(b2)} = SELECT b2.itemcode, b2.amount-usd, 
                                count(o.itemcode) AS count-offers \\
\>  \> \> \>             FROM b2 LEFT OUTER JOIN buyoffers o 
                                 ON o.itemid = b2.itemcode AND \\
 \>  \> \> \>     \hspace{3in}      o.price $>=$ b2.amount-usd \\
\>  \> \> \>             GROUP BY b2.itemcode, b2.amount-usd; \\
\\
\> RETURN SELECT itemcode, curcode, amount, count-offers FROM r2; \\
%   FOR EACH t BY REF IN r2 ORDER BY key LOOP
%       result.addRecord((t.itemcode, t.amount, t.curcode,t.count-offers));
%   END LOOP;
 %  RETURN result;
END;
}
}
\end{minipage}
\caption{UDF-1: The Final Batched Form}
\label{fig:final}
\end{figure}
\end{itemize}



==> chapters/bpo/examples/udf2-batched.tex <==
\subsection*{Rewriting UDF-2}
UDF-2 (\refex{ex:udf-travcat}) contains two queries, one in statement s8 and
the other in statement s10. As mentioned in
\refsec{sec:batchability:chap:bpo}, we cannot batch the query in statement
s10 due to cyclic flow dependence. However, we can batch the query in
statement s8 with respect to the {\small WHILE} loop (of s5) as well as the
outermost cursor loop, which iterates over all the parameters (in the {\em
trivial batched form}).

In \refex{ex:udf-travcat}, observe that splitting the {\small WHILE} loop 
(of s5) before and after the query execution statement (of s8) is not 
directly possible due to the loop-carried dependencies from s11 and s12
to s5, s6 and s7, which violate pre-condition c1 of Rule-2. We therefore,
reorder of statements by moving statements s8 and s9 past s12 (using
Rule-5). We then split the {\small WHILE} loop and batch the 
query execution. The batched query execution is further pulled out of
the outermost cursor loop in the {\em trivial batched form} using Rule-6.

\reffig{fig:final-udf2} shows the final batched form of UDF-2. The 
functions {\small NEST} and {\small UNNEST} implement the {\em nest} 
and {\em unnest} operations discussed in \refsec{subsec:rule6} and
take the corresponding arguments. {\small NEST} takes as its arguments
the table, columns to be nested and the name for the resulting 
table-valued column. Similarly, the {\small UNNEST} method takes the 
table and the name of the table-valued column that needs to be 
unnested.

\begin{figure}[ht]
\begin{minipage}{1.0\textwidth}
\scriptsize{
\ordinalg{
TABLE count-items-batched(TABLE pb) \\
DECLARE \\
\>  TABLE (key, catid, loop-table2, totalcount) loop-table1; \\
\>  INT   loopkey1 = 0; \\
BEGIN \\
\>  FOR EACH t IN pb LOOP \\
\>\>    INT totalcount := 0; INT top := 0; INT stack$[$100$]$; RECORD rec1; \\
\>\>    stack[top] := t.catid; \\
\>\>    top := top + 1; \\
\\
\>\>   TABLE (key, curcat, catitems) loop-table2; \\
\>\>   int loopkey2 = 0; \\
\>\>   WHILE top $>$ 0 LOOP \\
\>\>\>      RECORD rec2; \\
\>\>\>      top := top - 1; \\
\>\>\>      curcat := stack[top]; \\
%\\
\>\>\>      // Now push all the subcategory ids onto the stack \\
\>\>\>      FOR catrec IN SELECT category-id FROM category \\
\>\>\>      \>\>\>        WHERE parent-category=curcat LOOP \\
\>\>\>\>        stack[top] := catrec.category-id; \\
\>\>\>\>        top := top + 1; \\
\>\>\>      END LOOP; \\
%\\
\>\>\>      rec2.key    = loopkey2++; rec2.curcat = curcat; loop-table2.addRecord(rec2); \\
\>\>    END LOOP; \\
\\
\>\>    rec1.key   = loopkey1++; rec1.catid = t.catid; rec1.loop-table2 = loop-table2; \\
\>\>    loop-table1.addRecord(rec1); \\
\>  END LOOP; \\
\\
\eat{
\>  FOR EACH rec1 IN loop-table1 ORDER BY key LOOP \\
\>\>    MERGE INTO rec1.loop-table2 USING qb(b) AS qbr(curcat, res) ON rec1.loop-table2.curcat = qbr.curcat  \\
\>\>    WHEN MATCHED THEN UPDATE SET catitems = res; \\
\\
\>\>    where the parameter batch {\bf b} is constructed as: \\
\>\>    {\bf SELECT} distinct curcat {\bf FROM} rec1.loop-table2; \\
\>\>    and the batched form {\bf qb(b)} is defined as: \\
\>\>    SELECT b.curcat, count(itemid) AS catitems  
\>\>    FROM b LEFT OUTER JOIN item  ON category-id=curcat  \\
\>\>    GROUP BY curcat; \\
\>  END LOOP; \\
}

\>  temp = {\bf UNNEST}(loop-table1, "loop-table2"); \\
\>  MERGE INTO temp USING qb(b) AS qbr(curcat, res) ON temp.curcat = qbr.curcat  \\
\>  WHEN MATCHED THEN UPDATE SET catitems = res; \\
\\

// \>  where the parameter batch {\bf b} is constructed as: \\
// \>\>  SELECT distinct curcat FROM temp; \\
// \>  and the batched form {\bf qb(b)} is defined as: \\
// \>\>  SELECT b.curcat, count(itemid) AS catitems  \\
// \>\>  FROM b LEFT OUTER JOIN item ON category-id=curcat GROUP BY curcat; \\
\> loop-table1 = {\bf NEST}(temp, schema(loop-table1.loop-table2), "loop-table2");
\\
\\
\>  FOR EACH rec1 BY REF IN loop-table1 ORDER BY key LOOP \\
\>\>    FOR EACH rec2 BY REF IN rec1.loop-table2 ORDER BY key LOOP \\
\>\>\>     rec1.totalcount := rec1.totalcount + rec2.catitems; \\
\>\>    END LOOP; \\
\>  END LOOP; \\
\\
\>  RETURN SELECT catid, totalcount FROM loop-table1; \\
END; \\
}
}
\end{minipage}
\caption{UDF-2: The Final Batched Form}
\label{fig:final-udf2}
\end{figure}



==> chapters/bpo/sections/main-theorem.tex <==
\begin{theorem}
\label{lemma:revorder}
Given a basic block of code $b$ and statement $s$ in $b$ such that 
$s$ does not lie on a true-dependence cycle in the DDG, procedure
reorder terminates reordering the statements of $b$ such that:
    \begin{enumerate}[(a)]
        \addtolength{\itemsep}{-3mm}
        \item No LCFD edges cross the program points that immediately 
              precede and succeed $s$.
        \item Program correctness is preserved ({\em i.e.}, the reordered 
              block is equivalent to the original)
    \end{enumerate}
\end{lemma}

\begin{proof}
Let $C$ be the set of {\small LCFD} edges that cross the split boundaries of
$s$ in the given basic block $b$.  Let $T$ be the set of {\small LCFD} edges
$(v_1, v_2)$ such that both $v_1$ and $v_2$ succeed $s$ in $b$.  For
example, in \reffig{fig:proof-ct-sets}, $C = \{(s_2, s_1), (s_3, s)\}$ and
$T = \{(s_3, s_2)\}$.  We prove the following.

\begin{enumerate}[(1)]
    \addtolength{\itemsep}{-3mm}
    \item Each iteration of the outer {\em while} loop of procedure reorder
          completes.
    \item At the end of each iteration of the outer {\em while} loop of
          procedure reorder, $|C|+|T|$ decreases by at least 1.
    \item All statement reordering performed preserve the program 
          correctness.
\end{enumerate}

{\em Outer WHILE loop of procedure reorder terminates}
Since the termination condition for the outer {\small WHILE} loop of
procedure {\em reorder} is $|C|=0$, proving the above three claims 
proves Lemma~\ref{lemma:revorder}. The following two lemmas are used
in proving the three claims.

In each iteration of the outer {\small WHILE} loop of procedure {\em
reorder}, the last call to procedure {\em moveAfter} is made with $s$ being set
to $stmtToMove$. Post-condition (T.2) of Lemma~\ref{lemma:move-cond}
thus proves that $|C|+|T|$ decreases by at least 1 at the end of each 
iteration of the {\small WHILE} loop. Hence, by proving 
Lemma~\ref{lemma:move-cond} and Lemma~\ref{lemma:terminates} we 
prove Lemma~\ref{lemma:revorder} and hence Theorem\ref{theorem:condn}.\\

{\em Inner WHILE loop terminates}
\noindent {\bf Proof of Lemma~\ref{lemma:terminates}:} \\   
This requires us to show that the inner {\em while} loop of procedure
reorder terminates. The proof directly follows from post condition {\em
(T.1)} of procedure {\em moveAfter} and the termination condition for the inner
{\em while} loop ({\em srcDeps} is empty).
\end{proof}



==> chapters/bpo/sections/notation.tex <==
\subsubsection*{Notation Used in the Transformation Rules}

\begin{itemize}
\addtolength{\itemsep}{-5pt}
{\small
\item $R(s)$       : The read-set of $s$ is the set of variables read by 
                     statement or statement sequence $s$.  

\item $W(s)$       : The write-set of $s$ is the set of variables written by 
                     statement or statement sequence $s$. 

\item $U(s)$       : $R(s) \cup W(s)$. Called the use-set of $s$.
%\item $\curstmt$   : Statement that matches the antecedent of 
%                     the rule (used only when the rule antecedent matches 
%                     exactly one statement).

\item {\em pred}$?$ $s$  : Conditional statement. 
                           Equivalent to {\em if (pred) then s}.

\item {\em LV(s)}  : Set of variables local to the block statement {\em s}.

\item {\em NLV(s)} : Set of variables accessible but not local to the block 
                     statement {\em s}. These are variables defined in an 
                     ancestor block.

\item $|ss|$       : Length of the statement sequence $ss$
\item $ss[i]$      : Stmt at the $i^{th}$ position in sequence $ss$, 
                     $1 \leq i \leq |ss|$.

\item $s_1 + s_2$  : Concatenation (of statement sequences or strings).

\item {\em SUBS}$(s, v, v')$ : Statement obtained by substituting all 
                     occurrences of variable $v$ in statement
                     $s$ by variable $v'$.

\item {\em SUBS}$(s, vs, map)$ : Statement obtained as follows. For each 
                     variable $v \in U(s) \cap vs$, substitute all 
                     occurrences of $v$ in statement $s$ by $map(v)$.

\item $s \cup^* r$  : Disjoint union ({\small UNION ALL}) of relations s and r.

\item $\Pi^{d}_{a_1, a_2, \ldots, a_n}(r)$ : Projection without duplicate elimination
\item $(a_1, a_2, \ldots, a_n)$ : Tuple constructor
\item {\em type-of(e)}  : Data type of expression {\em e}.
}
\end{itemize}


\subsubsection*{Predicates on the DDG}
\begin{itemize}
\addtolength{\itemsep}{-5pt}
{\small
\item $s_1 \fdep s_2$    :  True only if the DDG contains a flow-dependence 
                            edge (either internal or external) from $s_1$ to $s_2$.

\item $s_1 \ta{FD+} s_2$ :  True only if the DDG contains a path from $s_1$ 
                            to $s_2$ having only FD edges.
                            
\item $s_1 \ta{(FD|LFD)+} s_2$ : True only if the DDG contains a path from 
                            $s_1$ to $s_2$ having only FD or LFD edges.

\item {\em indep}$(s_1, s_2)$ : True only if there are no dependencies 
                                between statements $s_1$ and $s_2$.
\item Similarly we have predicates for the existence of other types 
      of dependencies.
}
\end{itemize}

\subsubsection*{Conventions}
\begin{enumerate}
%\item $r_1 \overline{\Join}_{p}$ $r_2$ : $r_1$ $\Join_{p} r_2$ and for each pair of columns with the same name, drop the one coming from $r_1$.

%\item If the parameters to an operations come from attributes of a tuple as 
%in $q(t.a_1, t.a_2, \ldots t.a_n)$, we write it as $q(t)$ for 
%conciseness.

\item Loops of the form ``{\em for each t by ref in r}'' are updatable cursor 
loops. The underlying set {\em r} can be modified by assignments 
to the tuple's attributes. 
\eat{
{\em e.g.,} {\em for each t by ref in r loop} 
$t.a_1 = 10;$ {\em end loop;} does the following:
    \begin{enumerate}
        \item If the {\em schema(r)} does not contain an attribute by name 
               $a_1$, a new attribute $a_1$ is added to the schema of $r$.
        \item Assign $10$ to the attribute $a_1$ of the tuple identified 
              by $t$ in {\em r}. 
              %If the attribute is newly added, tuples
              %other than {\em t} in {\rm r} will have {\em null} for the
              %newly added attribute.
    \end{enumerate}
}

\item Suppose a table-valued expression $e$ has arity $n$. The rename
operator $\rho_{x(a_1, a_2, \ldots, a_n)}(e)$ returns
the result of expression $e$ under the name $x$, and with the attributes 
renamed to $a_1, a_2, \ldots, a_n$.

\item The merge operator $\mathcal{M}_{a_1=b_1, \ldots, a_n=b_n}(r, s)$ 
(based on the {\small SQL:2003} merge construct)
updates relation $r$ by merging in the records of $s$.
For each record in $s$ that matches a record in $r$ on the 
attributes common to $r$ and $s$, the record in $r$ is updated by 
assigning the values of attributes $b_1, \ldots, b_n$ from the $s$ tuple
to the attributes $a_1, \ldots, a_n$ of the $r$ tuple correspondingly.

\item Projection that removes the specified attributes: \\
%$\Pi_{\overline{a_1, a_2, \ldots a_n}}(r)$ is equivalent to $\Pi_{S-\{a_1, a_2, \ldots a_n\}}(r)$, where $S$ is the set of all attributes in {\em schema(r)}
$\Pi_{\bar{a_1}, \bar{a_2}, \ldots, \bar{a_n}}(r)$ is equivalent to
$\Pi_{S-\{a_1, a_2, \ldots, a_n\}}(r)$, where $S$ is the set of all attributes in {\em schema(r)}

\item Multi-assignment from scalar queries: Let $q$ be a query returning 
      exactly one tuple of arity $n$. The assignment 
      $v_1, v_2, \ldots, v_m = q$ (where $m \leq n$) assigns the values of 
      the first $m$ attributes of the returned tuple to the $m$ variables
      on the LHS in that order.

\end{enumerate}

\noindent
In all the rules, unless specified, we assume {\bf q} to be a {\bf batch-safe} operation 
%(which we are interested in batching) 
with {\bf qb} as its batched form.


==> chapters/bpo/sections/proof_prepost_cond.tex <==
\begin{proof}
% -----------------------------------------------
% Proof of pre/post conditions for procedure move.
% -----------------------------------------------
\noindent
First, we prove that all the calls to procedure {\em moveAfter}, made from
procedure {\em reorder} satisfy the three pre-conditions R.1, R.2 and R.3.
We then prove that procedure {\em moveAfter} ensures the post-conditions
whenever the pre-conditions hold.
  
\noindent 
\begin{enumerate}[(R.1)]
\item All calls made to procedure {\em moveAfter} from procedure {\em reorder} 
      have the {\em targetStmt} as parameter $t$. All recursive calls within
      procedure {\em moveAfter} do not change parameter $t$. Hence,
      pre-condition R.1 holds.
      
\item
    \begin{enumerate}[{\em (i)}]
      \item If $s_q$ does not lie on a true-dependence cycle, then procedure
          {\em reorder} picks {\em stmtToMove} and {\em targetStmt} such
          that there exists no true-dependence path from {\em stmtToMove} to
          {\em targetStmt}. This can be observed in \reffig{fig:reorder-cases}.
      \item Each statement $v$ in {\em srcDeps} has a true-dependence path
          from {\em stmtToMove} and hence there cannot be a true-dependence
          path from $v$ to {\em targetStmt} (otherwise, {\em stmtToMove}
          would be on a true-dependence cycle).
      \item Observations {\em (i)} and {\em (ii)} above prove that 
            pre-condition R.2 holds for all calls to procedure {\em moveAfter} 
            made from procedure {\em reorder}.
    \end{enumerate}

\item For all the calls to procedure {\em moveAfter}, which are made from 
      procedure {\em reorder}, this condition is seen to hold from the 
      way we pick statement $v$ (passed as argument $s$ for {\em moveAfter}). 
\end{enumerate}

\noindent
{\bf Post-conditions} \\
%and Pre-conditions for Recursive Calls} \\
\noindent
We now show the following: If the pre-conditions for procedure {\em moveAfter}
are met then, the post-conditions and pre-conditions for all recursive 
calls will be met.

\noindent
{\bf Case I}: $s \neq$ {\em stmtToMove} \\
{\em Case IA}: $t$ immediately follows $s$.

\begin{enumerate}[{IA}.1]
\item {\em No flow/anti/output dependencies exist from $s$ to $t$.} \\
      Procedure {\em moveAfter} swaps $s$ and $t$.  Post-condition {\em (T.1)}
      holds because $s$ no longer lies between {\em stmtToMove} and $t$ and
      is accordingly removed from {\em srcDeps}.  Post-condition {\em (T.2)}
      holds because no changes happen to $C$ and $T$ (because $s$ is a
      statement that lies after {\em stmtToMove}).  The program correctness
      is preserved (Post-condition {\em (T.3)} holds) because no 
      flow/anti/output dependencies exist between $s$ and $t$; the 
      {\em do} loop (and hence the procedure) terminates after the
      first iteration and $s$ is moved past $t$ (Post-condition 
      {\em (T.4)} holds).

\item {\em A single output-dependence edge ($OD_v$) exists from $s$ to
      $t$.}\\ Transformations made by procedure {\em moveAfter} are shown
      pictorially in \reffig{fig:proof-od-wstub}. We first note that the
      recursive call to {\em moveAfter}$(as_v', t)$ satisfies the
      pre-conditions for {\em moveAfter}. $as_v'$ appears after $t$ and
      hence the recursive call terminates. We then swap $s$ and $t$. \\
      Post-conditions {\em (T.1)} and  {\em (T.2)} hold for the same reasons
      stated for Case IA.1. Rewriting the {\small LHS} of $t$ with $v'$
      makes $s$ and $t$ independent and hence the swap preserves
      correctness.  The newly introduced copy-back statement, which assigns
      $v'$ to $v$, ensures later statements see the correct value of $v$.
      Hence, post-condition {\em (T.3)} (correctness) holds. The 
      {\em do} loop (and hence the procedure) terminates after the
      first iteration and $s$ is moved past $t$ (Post-condition 
      {\em (T.4)} holds).

      \begin{figure}[ht]
      \begin{center}
      \includegraphics[width=3in,height=1.6in]{chapters/bpo/fig/proof-OD-wstub.eps}
      \caption{Pictorial Depiction of Reordering with OD Edge}
      \label{fig:proof-od-wstub}
      \end{center}
      \end{figure}

\item {\em A single anti-dependence edge ($AD_v$) exists from $s$ to $t$.}\\
      Assume there exists an $AD_v$ edge from $s_q$ to {\em next}.
      Transformations that procedure {\em moveAfter} makes are shown 
      pictorially in \reffig{fig:proof-ad-rstub}.
      The newly introduced statement $as_v'$, which preserves the value of
      $v$ in $v'$, cannot be part of {\em srcDeps} for the following
      reasons.  Assume $as_v'$ has a true-dependence path from {\em
      stmtToMove}, which in this case must be $s_q$. This implies either
      $s_q$ or some statement having a true-dependence path from $s_q$
      writes $v$.  Let this statement be $p$.  This implies a
      true-dependence cycle involving $s_q$ and $p$ since $s_q$ reads $v$
      and $p$ writes $v$. Since it is given that $s_q$ does not lie on a
      true-dependence cycle, we conclude that $as_v'$ cannot have a
      true-dependence path from $s_q$ and hence not part of {\em srcDeps}.
      Now, it is straight-forward to see that the post conditions hold.

      \begin{figure}[ht]
      \begin{center}
      \includegraphics[width=4in,height=1.6in]{chapters/bpo/fig/proof-AD-rstub.eps}
      \caption{Pictorial Depiction of Reordering with AD Edge (R-Stub)}
      \label{fig:proof-ad-rstub}
      \end{center}
      \end{figure}

      \begin{figure}[ht]
      \begin{center}
      \includegraphics[width=4in,height=1.6in]{chapters/bpo/fig/proof-AD-wstub.eps}
      \caption{Pictorial Depiction of Reordering with AD Edge (W-Stub)}
      \label{fig:proof-ad-wstub}
      \end{center}
      \end{figure}

      Assume there exists no $AD_v$ edge from $s_q$ to {\em next}.
      Transformations that procedure {\em moveAfter} makes are shown 
      pictorially in \reffig{fig:proof-ad-wstub}.
      It is straight-forward to see that the pre-conditions for the
      recursive call hold and that the subsequent swap of $s$ and {\em next}
      will be correct and the transformation satisfies the post-conditions.

\item {\em A flow-dependence edge exists from $s$ to $t$.} \\
      This case is ruled out from pre-condition {\em R.2}.
        
\item {\em Multiple AD and OD edges exist from $s$ to $t$.} \\ Each of the
      AD and OD edges can be treated independently as is done in procedure
      {\em moveAfter}. And we can see that the post-conditions continue to
      hold.

\end{enumerate}

\noindent
{\em Case IB}: $t$ does not immediately follow $s$ (there exist 
               other statements between $s$ and $t$).
\begin{enumerate}[{ }]
\item From pre-condition {\em R.3}, the only possible dependencies between
      $s$ and any statement $u$ between $s$ and $t$ are AD and OD. We can
      keep swapping $s$ and its successor till $s$ is moved past $t$. Each
      swap preserves the pre and post conditions as argued above. 
\end{enumerate}

\noindent
{\bf Case II}: $s =$ {\em stmtToMove} \\
{\em Case IIA}: $t$ immediately follows $s$. 

\begin{enumerate}[{IIA}.1]
\item {\em  No flow/anti/output dependencies exist from $s$ to $t$}. \\
      Procedure {\em moveAfter} swaps $s$ and $t$.  Let $k$ be the number of
      LCFD edges incident on $t$. Now, the change in the number of edges in
      sets $C$ and $T$ is as follows (see also \reffig{fig:reorder-cases}).
      \\
      If {\em stmtToMove}=$s_q$: 
        $|C_{new}| \leq |C_{old}| + k - 1$ and 
        $|T_{new}| \leq |T_{old}| - k$  
        \\
        If {\em stmtToMove} $\neq$ $s_q$:
        $|C_{new}| \leq |C_{old}| - k$ and 
        $|T_{new}| \leq |T_{old}| + k - 1$ 
        \\
      In both the above cases, $|C|+|T|$ decreases by at least 1. Hence we
      can see that post-condition {\em (T.2)} holds. Post-condition {\em
      (T.1)} is satisfied since {\em stmtToMove} is not in {\em srcDeps}.
      The swap preserves the correctness since there are no flow/anti/output
      dependencies from $s$ to $t$ (post-condition {\em (T.3)} holds).
      Post-condition {\em (T.4)} holds as argued in IA.1.

\item {\em A single output-dependence edge ($OD_v$) exists from $s$ to $t$}.\\
      The resulting dependencies after the transformation are pictorially
      shown in \reffig{fig:proof-od-wstub}. It can be seen that, $|C|+|T|$
      decreases after the transformation.

\item {\em A single anti-dependence edge ($AD_v$) exists from $s$ to $t$}.\\
      The AD edge is moved using a reader stub if $s = s_q$ and is moved
      using a writer side stub otherwise. The dependencies after this
      reordering are shown in Figures \ref{fig:proof-ad-rstub} and 
      \ref{fig:proof-ad-wstub}. Again, it can be seen that $|C|+|T|$ decreases
      after the transformation.

\item {\em A flow-dependence edge exists from $s$ to $t$}. \\
      This case is ruled out from pre-condition {\em R.2}.

\item {\em Multiple AD and OD edges exist from $s$ to $t$}. \\
      Each of the AD and OD edges can be treated independently as is done in
      procedure {\em moveAfter}. And we can see that the post-conditions
      continue to hold.
\end{enumerate}

\noindent
{\em Case IIB}: $t$ does not immediately follow $s$ (there exist 
                 other statements between $s$ and $t$). 
\begin{enumerate}[{ }]
\vspace{-2.5mm}
\item This case is similar to {\em Case IB}, except that when $s$ is 
      eventually moved past $t$, $|C|+|T|$ strictly decreases. Hence
      the post-conditions hold. 
\end{enumerate}
This completes the proof of Lemma~\ref{lemma:move-cond}.
\end{proof}


==> chapters/bpo/sections/rules/rule1.tex <==
\begin{trule}
\Rule{Rule 1A: Unconditional invocation with no return value}\\
{\small 1A(i) Basic form}
{\small
\begin{transrule}
123\=\kill
for each {\em t} in {\em r} loop \\ % $\{$ \\
\>  $q(t.c_{1}, t.c_{2}, \ldots, t.c_{m});$ \hspace{1mm} {\large
$\Longleftrightarrow$} \hspace{2mm} $qb(\Pi^{d}_{c_{1}, c_{2}, \ldots, c_{m}}(r))$; \\
end loop; \\ %$\}$ \\

\end{transrule}
}

\noindent
{\small 1A(ii) Form with loop invariant parameters}
{\small
\begin{transrule}
123\=\kill
for each {\em t} in {\em r} loop \\ % $\{$ \\
\>  $q(t.c_{1}, t.c_{2}, \ldots, t.c_{m}, v_1, v_2, \ldots, v_n);$ 
\hspace{1mm} {\large $\Longleftrightarrow$} \hspace{2mm}
$qb(\Pi^{d}_{c_{1}, c_{2}, \ldots, c_{m}}(r) \times \{(v_1, v_2, \ldots, v_n)\})$; \\
end loop; \\ %$\}$ \\
%\hspace{10mm} {\large $\Updownarrow$} \\
%$qb(\Pi^{d}_{c_{1}, c_{2}, \ldots, c_{m}}(r) \times \{(v_1, v_2, \ldots, v_n)\})$; \\
\end{transrule}
}

\Rule{Rule 1B: Unconditional invocation with return value}
{\small
\begin{transrule}
123\=\kill
for each {\em t} by ref in {\em r} loop \\ % $\{$ \\
\>  $t.c_{w1}, t.c_{w2}, \ldots, t.c_{wn} = q(t.c_{r1}, t.c_{r2}, \ldots, t.c_{rm});$ \\
end loop; \\ %$\}$ \\
where $q$ is a {\em pure} function. \\

\hspace{10mm} {\large $\Updownarrow$} \\

$\mathcal{M}_{c_{w1}=c_{w1'}, \ldots, c_{wn}=c{wn'}}(r, e)$ \\
where
{\em e} $=$ $\rho_{x (c_{r1}, \ldots, c_{rm}, c_{w1'}, \ldots,
c_{wn'})}qb(\Pi_{c_{r1}, \ldots, c_{rm}}(r))$; \\
\end{transrule}
}

\Rule{Rule 1C: Conditional Invocation}
{\small
\begin{transrule}
123\=\kill
for each {\em t} by ref in {\em r} loop \\ 
\>  $(t.cv==true)?$ $t.c_{w1}, \ldots, t.c_{wn} = $ 
$ q(t.c_{r1}, \ldots, t.c_{rm});$  \\ %\hspace{10mm} // Conditional statement \\
end loop; \\
where $q$ is a {\em pure} function. \\

\hspace{10mm} {\large $\Updownarrow$} \\

$\mathcal{M}_{c_{w1}=c_{w1'}, \ldots, c_{wn}=c{wn'}}(r, e)$, where \\
{\em e} $=$ $\rho_{x (c_{r1}, \ldots, c_{rm}, c_{w1'}, \ldots, c_{wn'})}
qb(\Pi_{c_{r1}, \ldots, c_{rm}}(\sigma_{cv=true}\ r))$;
\end{transrule}
}
{\small Note that in rules 1B and 1C we use duplicate-eliminating 
projection ($\Pi$) and not ($\Pi^d$).} \\

\eat{
In rules 1B and 1C we omit the form with loop invariant parameters.
The loop invariant forms of these rules can be easily constructed on
the lines of the loop invariant form of rule 1A. 
Also, note that in rules 1B and 1C we deal only with assignments 
to cursor attributes and not variables. The reason for this will
be clear when we describe Rule-2 (splitting a loop) and Rule-3 
(separating batch-safe operations from the non batch-safe). For now,
it suffices to know that the later transformations bring the 
program into a form in which we can apply one of the rules
described in this section.
}
\Rule{Rule 1D: Removal of Order-By}
\\
\\
\begin{tabular}{lcl}
\begin{minipage}{0.45\textwidth}
{\small
\begin{transrule}
123\=12\=\kill
for each {\em t} $[$by ref$]$ in {\em r} order by {\em cols} loop \\ 
    \> {\em batch-safe-operation(t)} \\
end loop; 
\end{transrule}
}
\end{minipage}
&
%\hspace{10mm} {\large $\Updownarrow$} \\
\begin{minipage}{0.1\textwidth}
{\large $\Longleftrightarrow$}
\end{minipage}
&
\begin{minipage}{0.45\textwidth}
{\small
\begin{transrule}
for each {\em t} $[$by ref$]$ in {\em r} loop \\ 
123\=\kill
    \> {\em batch-safe-operation(t)} \\
end loop; 
\end{transrule}
}
\end{minipage}
\end{tabular}
\caption{Batching Simple Set Iteration Loops}
\label{fig:rule1}
\end{trule}



==> chapters/bpo/sections/rules/rule2.tex <==
\begin{trule}
{\small
\begin{sqlindent}
{\bf while $p$ loop} \\
    \> $ss_1;$ \ $s;$ \ $ss_2;$ \\
{\bf end loop;} 
\end{sqlindent}
such that:
\begin{enumerate}[(a)]
\addtolength{\itemsep}{-3mm}
\item No loop-carried flow dependencies ({\em i.e.,} LCFD edges, external or otherwise) cross the points before and after $s$.
\item No loop-carried {\em external} anti or output dependencies cross the points before and after $s$.
\end{enumerate}

\begin{sqlindent}
\hspace{3cm}{\Large{$\Updownarrow$}} \\
{\em Table(T)} \ t; \\ 
int loopkey = 0; \\
%1234\=1234\=12\=1234\=1234\=12345678\=123456789ABC\=\kill
{\bf while $p$  loop} \\
    \> {\em Record(T)} r; \ \  $ss_1'$; \ \ r.key=loopkey++; \ \  
       {\em t.addRecord(r);} \\
{\bf end loop;} 
\\
{\bf for each} r {\bf by ref in} t {\bf order by} t.key {\bf loop} \\
    \>  $s'$ \\
{\bf end loop;} 
\\
{\bf for each} r {\bf by ref in} t {\bf order by} t.key {\bf loop} \\
    \>  $ss_r$; \ $ss_2$ \\
{\bf end loop;} \\
{\bf delete} t; 
\end{sqlindent}
where $T,\ ss_1',\ s'$ and $ss_r$ are constructed as follows.\\
Let {\em SV} (split variables) be the set of variables for which 
either an LCAD or LCOD edge crosses the split boundaries (the edge 
is incident from $ss_2$ to $s$ or $ss_1$, or from $s$ to $ss_1$).
%12\=12\=12\=1234\=1234\=12345678\=123456789ABC\=\kill
\begin{enumerate}
\addtolength{\itemsep}{-2mm}
    \item Table $t$ and record $r$ have attributes corresponding to each
          variable in {\em SV} and a key. 

    \item $ss_1'$ is same as $ss_1$ but with additional assignment
          statements to attributes of $r$. Each write to a split variable $v$
          is followed by an assignment statement $r.v = v;$. If the write is
          conditional, then the newly added statement is also conditional on
          the same guard variable.

    \item The statement $s'$ is same as $s$, except that each reference $v$
          to a variable in set $SV$ is replaced by $r.v$.  Formally,
          $s'=SUBS(s, SV, map:v \rightarrow r.v)$

    \item $ss_r$ is a statement sequence assigning attributes 
          of $r$ to corresponding variables. Each
          assignment in $ss_r$ is conditional; the assignment is made 
          only if the attribute of $r$ is non-null ({\em assigned}).
\end{enumerate}
{\bf Note:} If the all operations in the loop are {\em batch-safe} 
            we can omit the {\em loopkey} and the {\em key} attribute. \\

\Rule{Rule 2A: Splitting a Cursor Loop} \\
\\
The rule for splitting cursor loops is a minor variant of 
Rule 2, and we omit the details for brevity.

\caption{Splitting a WHILE Loop}
\label{fig:rule2}
}
\end{trule}



==> chapters/bpo/sections/rules/rule2b.tex <==
\begin{figure}[t]
\begin{center}
\begin{tabular}{l}
%\hline
\begin{minipage}{0.5\textwidth}
\Rule{Rule 2B: Splitting a Cursor Loop}
The rule for splitting cursor loops is a minor variant of Rule 2A and 
we omit its details for brevity.
\end{minipage}
\end{tabular}
\end{center}
%\caption{Rule 3 Control dependencies to flow-dependencies}
%\caption{Rule 4: Converting control-dependencies to flow-dependencies}
\label{fig:rule2b}
%\vspace{-8mm}
\end{figure}



==> chapters/bpo/sections/rules/rule3.tex <==
\begin{trule}
\begin{transrule}
if $(p)$ $\{$ $ss_1$ $\}$ else $\{$ $ss_2$ $\}$ \\ 
\hspace{10mm} {\large $\Updownarrow$} \\
boolean $cv=p$; \\
{\em ss} \\
\\
where $ss[i]  =  (cv==true)? ss_1[i], 1 \leq i \leq |ss_1|$ and \\
$ss[k+j] = (cv==false)? ss_2[j], 1 \leq j \leq |ss_2|, k=|ss_1|$ 
\end{transrule}
\caption{Converting control-dependencies to flow-dependencies}
\end{trule}



==> chapters/bpo/sections/rules/rule4.tex <==
\begin{tabular}{l}
\\
\hline 
\\
\begin{minipage}{0.5\textwidth}
\scriptsize{
\begin{transrule}
while $p$ $\{$  \\
\>  {\em ss} \\
$\}$ \\

Let $v \in ${\em NLV}$(\curstmt)$ and $\exists s \in ss$ {\em s.t.} 
$v \in W(s)$ ({\em i.e., v be a non-local} \\
{\em variable written by some statement in ss})\\

\hspace{20mm} {\large $\Updownarrow$} \\

while $p$ $\{$ \\ 
    \> {\em type-of}$(v)$ lv; \\
    \> lv=v; \\
    \> $ss'$; \\
$\}$ \\

\noindent where $ss'$ is constructed as follows: \\
For each statement $s$ in $ss$ {\em s.t.} $v \in U(s)$, replace 
all occurrences \\
of $v$ in $s$ by {\em lv} and if $v \in W(s)$, emit an extra statement 
$v = lv;$.
\end{transrule}
}
\end{minipage}
\\
\\
\hline
\\
\end{tabular}

% Old form

\eat{
{\small
\begin{transrule}

while $p$ $\{$  \\
\>  {\em ss} \\
$\}$ \\

Let $v$ be a non-local variable written by one or more statements in {\em ss} \\
{\em i.e.,}  $v \in ${\em NLV}$(\curstmt)$ and $\exists s \in ss$ {\em s.t.} 
$v \in W(s)$ \\

\hspace{20mm} $\Updownarrow$ \\

while $p$ $\{$ \\ 
    \> $lv:${\em type}$(v)$; \\
    \> $lv=v$; \\
    \> $ss'$ where $ss'[i]=SUBS(ss[i], v, lv), 1 \leq i \leq |ss|$ \\
    \> $v=lv$; \\
$\}$ \\
NOTE: This equivalence assumes that all loops are single entry and single exit.
We do not have "exit" like statements.
\end{transrule}
}
}


==> chapters/bpo/sections/rules/rule5.tex <==
\begin{trule}
\Rule{Rule 5A: Reordering Independent Statements} \\
Two statements can be reordered if there exists no dependency between them.

\begin{transrule}
123\=\kill
$s_1; s_2;$ where {\em indep($s_1, s_2$)} \ \ \ 
           {\large $\Longleftrightarrow$} \hspace{2mm} $s_2; s_1;$ 
\end{transrule}

\noindent
\Rule{Rule 5B: Shifting an Anti-Dependence Edge} \\
An anti-dependence edge between two statements can be shifted by using
an extra variable.

\begin{transrule}
123\=\kill
$s_1; s_2;$ \\
where $s_1 \ta{AD_v} s_2$ \\ % \wedge \neg{(s_1 \ta{FD|OD} s_2)}$ \\
    \> {\large $\Updownarrow$}\\
$v'=v; s_1'; s_2;$ 
\end{transrule}
where $s_1'$ is constructed from $s_1$ by replacing all reads of $v$ by 
reads of $v'$. \\

\noindent
\Rule{Rule 5C: Shifting an Output-Dependence Edge}
\begin{transrule}
123\=\kill
$s_1; s_2;$ \\
where $s_1 \ta{OD_v} s_2$ \\ % \wedge \neg{(s_1 \ta{FD|OD} s_2)}$ \\
    \> {\large $\Updownarrow$}\\
$s_1; s_2'; v=v';$ 
\end{transrule}
where $s_2'$ is constructed from $s_2$ by replacing all writes of $v$ by 
write to $v'$.

\caption{Basic Rules that Facilitate Reordering of Statements}
\label{fig:rev-order-rule}
\end{trule}


% ********** Old rule  *****************
\eat{ 
{\small

\begin{transrule}

\> $ss_1; s_a; ss_2; s_b; ss_3;$ \\
$\}$ \\
where $s_a \ta{(AD)} s_b$  \\

$\Longleftrightarrow$ \\

while $p$ $\{$ \\
    \> $ss_1; ss_{cp}; s_a'; ss_2; s_b; ss_3;$ \\
$\}$  \\
where \> {\em (i)} $ss_{cp}$ is {\em s.t.} $\forall v \in R(s_a) \bigcup W(s_b)$, {\em stmt}($v'=v$) $\in ss_{cp}$ and \\
      \> {\em (ii)} $s_a'=SUBS(ss_1, R(s_a) \bigcup W(s_b), m:v \rightarrow v')$ \\
\end{transrule}
}
}


==> chapters/bpo/sections/rules/rule6.tex <==
\begin{trule}
Let $s$ be a table valued attribute of table $r$, and let 
$S=${\em schema}$(r.s)$. 

\begin{transrule}
\Rule{Rule 6A. No Return Value} \\
for each $t$ in $r$ loop  \\ % \> \> \>  \> \> $\mathbf{(s_1)}$ \\
\ \ \ \ $qb((t.c_1, \ldots, t.c_n) \times t.s)$; \\
end loop; \\

\hspace{10mm} {\large $\Updownarrow$} \\

$qb(\Pi^{d}_{A} (\mu_{s}(r)))$ \ where $A=\{c_1, \ldots, c_n\} \cup S$ \\
\end{transrule}

\begin{transrule}
\Rule{Rule 6B: With Return Value} \\

for each $t$ in $r$ loop  \\ % \> \> \>  \> \> $\mathbf{(s_1)}$ \\
\> $\mathcal{M}_{c_{1}=c_{1}', \ldots, c_{n}=c{n}'}(t.s, qb(t.s))$ \\
end loop; \\
where $qb$ is a {\em pure} function. \\

\hspace{10mm} {\large $\Updownarrow$} \\

$rs = \mu_{s}(r)$; \\
$\mathcal{M}_{c_{1}=c_{1}', \ldots, c_{n}=c{n}'}(rs, qb(\Pi_{S}(rs)))$; \\
$r = \nu_{S \rightarrow s}(rs)$;

\end{transrule}

\caption{Batching Across Nested Loops}
\label{fig:rule6}
\end{trule}



==> chapters/bpo/sections/rules/rule_separate_batchsafe.tex <==
\begin{trule}
Let $e$ be a batch-safe expression in statement {\em stmt}. Then,
\begin{sqlindent}
\>\> $stmt$; \hspace{3mm} {\Large $\Leftrightarrow$} \hspace{3mm} $T\ v = e;\ \ stmt'$; \\
where $stmt'=SUBS(stmt, e, v)$ and $T=${\em type-of}$(e)$;
\end{sqlindent}
\caption{Isolating Batch-Safe Expressions}
\end{trule}


==> chapters/bpo/sections/sec_condition.tex <==
\section{Applicability of Transformation Rules}
\label{sec:batchability:chap:bpo}
\input{chapters/bpo/examples/example_noloop.tex}
Our program transformation algorithm succeeds in rewriting fairly complex
programs for batched bindings. However, it may not be always be possible to
rewrite a program to batch the invocation of a specific operation. As an
example, consider the program and its DDG shown in
\reffig{fig:example-noloop}. We can batch the query invocation in statement
{\tt s2} but not the one in statement {\tt s1}.  The query invocation in
statement {\tt s1} lies on the true-dependence cycle {\tt s1} $\fdep$ {\tt
s4} $\ta{LFD}$ {\tt s1} and hence we cannot reorder the statements so as to
satisfy the pre-conditions of Rule-2.  Similarly, in the DDG of
\reffig{fig:sampleddg}, the query invocation in statement {\tt s8} is
batchable, whereas the one in statement {\tt s10} is not batchable.

Flow dependencies that result from control-dependencies (Rule 4) must be
taken into account while checking for the presence of a true-dependence
cycle.  For instance, statement {\tt s2} in the code fragment of
\reffig{fig:case3b} lies on true-dependence cycle after converting the
control dependence of {\tt s2} on {\tt s0} into a flow dependence.
Intuitively, an operation cannot be batched if the execution of the
operation in any iteration depends on the value it returned in a
previous iteration. 

\begin{figure}[ht]
\begin{center}
\begin{minipage}{0.8\textwidth}
{\small
\ordinalg{
s0: \> while(x $<$ n) loop \\
s1: \>     \> y $=$ y $-$ 1; \\
s2: \> \> {\bf x $=$ q(y);} \\ % $\longrightarrow$ Not batchable \\
\> end loop; 
}
}
\end{minipage}
\end{center}
\caption{True-Dependence Cycle Created Due to Control-Dependency}
\label{fig:case3b}
\end{figure}

\input{chapters/bpo/sections/theorem.tex}



==> chapters/bpo/sections/sec_controlalgo.tex <==
\section{Control Algorithm for Rule Application}
\label{sec:control-algo:chap:bpo}
Rewriting a program for set-orientation involves the following steps:  {\em
(i)} identify iteratively invoked query execution statements, {\em (ii)}
decide whether it is beneficial to batch the query execution and the
ancestor loop (in the hierarchy of loops enclosing the statement) with
respect to which the statement must be batched and {\em (iii)} rewrite the
program by {\em systematically} applying the transformation rules presented
in the previous section.

\eat{
\begin{enumerate}
\item Identify iteratively invoked query execution statements 
\item Decide whether it is beneficial to batch the query execution and
      the ancestor loop (in the hierarchy of loops enclosing the
      statement) with respect to which the statement must be batched.
\item Rewrite the program by {\em systematically} applying the transformation 
      rules presented in this chapter.
\end{enumerate}
}
\input{chapters/bpo/algos/algo_main.tex}

Identifying the query execution statements in a loop is usually straight
forward. However, the decision on whether a statement should be batched and
the level in the loop hierarchy up to which the statement must be batched,
requires a cost-based analysis. Cost-based analysis is a future direction
for our work and some of the parameters needed for cost-based analysis are
discussed in \refchap{chap:concl}.  In this section, we assume these two
inputs (the query invocation to be batched and the ancestor loop up to which
the query must be batched) are available from the user. Given a query
execution statement and a loop with respect to which the statement must be
batched, the transformation rules presented in this chapter can be used to
rewrite the program. However, it is important to apply the rules in a
systematic way so as to achieve the goal of batching the given statement. 

In \reffig{fig:control-algo} we give the procedure for applying the rules so
as to batch a given query execution statement {\em w.r.t.} a given ancestor
loop enclosing it. The procedure {\em batch} recursively pulls out the given
statement, starting from the inner most loop enclosing it.  Procedure {\em
do-batching} performs the actual task of rewriting by applying the rules.
First, we apply Rule-3 on the statement and ensure the RHS contains only the
query execution expression. We then convert all the control-dependencies to
flow-dependencies by applying Rule-4.  This allows us to treat the entire
body of the loop as a {\em basic block} (a straight-line sequence of
statements with no branches into or out of the sequence). We perform a
reordering of the statements (if needed) to satisfy the pre-conditions for
Rule-2, and then use Rule 2 to split the loop at the program points which
immediately precede and succeed the query execution statement. This leaves
the query execution statement in a loop by itself - a form in which we can
apply Rule-1 or Rule-6 and make use of the batched form. Rule-1 gets applied
for the inner most loop enclosing the statement and Rule-6 gets applied for
the higher level loops.

\subsection*{Reordering Statements to Enable Loop Splitting}
\label{reorder}
As described in \refsec{subsec:rule5}, to facilitate splitting of a loop, it
may be necessary to reorder the statements within a loop. A loop can be
split using Rule-2 only if there are no loop-carried flow dependencies that
cross the split boundaries. \refsec{subsec:rule5} gives an example and
specifies the basic transformations (Rule 5) that enable reordering of
statements. The basic transformations specified in Rule 5 must be applied in
an appropriate sequence to achieve the desired reordering of statements in a
loop. We now give an algorithm to do so. The goal is to reorder the
statements such that no loop-carried flow dependencies cross the desired split
boundaries. We make use the following definition in the description to
follow.
\begin{definition}
\label{defn:true-dep-path-cycle}
A true-dependence path (or cycle) in a data dependence graph is a directed
path (or cycle) where each edge represents either a flow-dependence (FD) or
a loop-carried flow-dependence (LCFD).

\noindent
{\em Note that a true-dependence path excludes anti, output, loop-carried
anti and loop-carried output dependence edges.}
\end{definition}

\input{chapters/bpo/algos/algo_reorder.tex}

\begin{figure}[ht]
\begin{minipage} {1.0\textwidth}
\begin{center}
\includegraphics[width=4.5in,height=2.3in]{chapters/bpo/fig/reorder.eps}
\caption{Cases for Reordering Statements}
\label{fig:reorder-cases}
\end{center}
\end{minipage}
\end{figure}

The algorithm {\em reorder}, shown in \reffig{fig:reorder}, works as follows.
For each loop-carried flow dependence edge that crosses the split boundaries
(the two program points in the basic block that immediately precede and
succeed the statement to batch), the algorithm decides the statement to move,
and its target position. There are four cases to consider while deciding the
statement to move and its target position. The cases are shown in
\reffig{fig:reorder-cases}.  The way in which we choose the {\em stmtToMove}
and {\em targetStmt} ensures the following. If $s_q$, the statement to be
batched, does not lie on a true-dependency cycle, then there exists no
true-dependence path from the {\em stmtToMove} to the {\em targetStmt}. We
then compute two sets {\em srcDeps} and {\em tgtDeps}. {\em srcDeps} is the
set of statements present between {\em stmtToMove} and {\em targetStmt}, and
which have a path of flow-dependence edges from {\em stmtToMove}. {\em
tgtDeps} is the set of statements present between {\em stmtToMove} and {\em
targetStmt}, and from which there exists a path of flow-dependence edges to the
{\em targetStmt}. Note that the two sets will be disjoint. Each statement in
{\em srcDeps} is then moved past the {\em targetStmt} using the {\em
moveAfter} procedure. The procedure {\em moveAfter} (shown in
\reffig{fig:movedirect}) performs the required reordering by swapping pairs of
adjacent statements.  While doing so, the procedure resolves any anti and
output dependencies by creating stub statements, which make use of temporary
variables. 

\input{chapters/bpo/algos/algo_movedirect.tex}
\input{chapters/bpo/examples/reorder-examples.tex}

Figures \ref{fig:reorder-ex1} through \ref{fig:reorder-ex3} show examples
illustrating statement reordering. \reffig{fig:reorder-ex3-ddg} shows the
data dependence graph for the original and reordered code of
\reffig{fig:reorder-ex3}. In \reffig{fig:reorder-ex3-ddg}, for each
flow-dependence (FD) edge from $x$ to  $y$, there exists a corresponding
loop-carried anti-dependence (LCAD) edge from $y$ to $x$ but these edges are
not shown. Similarly, AD and OD edges have corresponding LCFD and LCOD edges
respectively, which are not shown. In this example, $s1$ is the
statement containing the query to batch. The LCFD edge from $s4$ to $s1$
crosses the split boundary and hence $s1$ must be moved past $s4$. As can be
seen in \reffig{fig:reorder-ex3-ddg}, after the reordering, no LCFD 
edges cross the split boundary. The LCAD edges crossing the split boundary
do not prohibit splitting of the loop, because these will be removed by the
introduction of the {\em loop local table} while splitting the loop.



==> chapters/bpo/sections/sec_define.tex <==
\section{Rewriting for Batched Bindings} 
\label{sec:define:chap:bpo}
In order to exploit the benefits of batching, we must have an efficient {\em
batched form} of the operation being invoked, and a way of using the {\em
batched form} in place of repeated invocations of the operation.  In this
section, we formally define {\em batched forms} of operations and introduce
the problem of rewriting loops so as to make use of the {\em batched forms}
of expensive operations invoked within them. We also consider the issues in
batching invocations of operations that have side-effects. Finally, we
introduce the problem of generating {\em batched forms} of complex
procedures.

\subsection{Batched Forms of Operations}
Informally, the batched form of an operation takes a batch (or set) of
parameters at once and processes them. Batched forms of operations are
typically more efficient than iterative invocation of the corresponding
non-batched forms. For example, a database bulk load operation can be
thought of as a batched form of the {\em insert} operation, assuming
logging can be ignored. Similarly, a
relational {\em join} can be thought of as a batched form of relational {\em
selection} with a parameterized predicate. Note that we model a batch as a
{\em set} and not a {\em sequence}. This is due to the fact that most
batched forms do not guarantee the order in which the elements in the batch
are processed, and this is an important reason for their efficiency.  We now
define the batched forms formally.

\subsubsection*{Batched Forms of Pure (Side-Effect Free) Functions}
Let $f:D \rightarrow R$ be a side-effect free function, where $D$ is the
domain and $R$ is the range of $f$. A function $fb:BD \rightarrow BR$ is
considered a batch form of $f$ if the following are true.

\begin{enumerate}
\addtolength{\itemsep}{-5pt}
    \item The domain {\em BD} is the power set of {\em D}
    \item The range {\em BR} is the power set of $D \times R$
    \item $\forall b \in BD, fb(b) = \bigcup_{b_i \in b} \{(b_i, f(b_i))\}$
\end{enumerate}

\noindent
{\bf Example:} Consider the square function defined as $sq(x) = x^2$.  The
corresponding batched form can be defined as $sqb(sx) = \{(x, x^2) : x \in
sx\}$ \\

Intuitively, the batched form of a function takes a set of parameters and
returns a set comprising of all the results.  To establish the correlation
between a parameter and the corresponding result we require the batched form
to return the parameter value along with the result.

\subsubsection*{Batched Forms of Parameterized Relational Queries}
Relational queries are pure functions that return (multi)sets of tuples.
Though we can use the above definition of batched forms for queries, it
makes the return type of batched queries violate the first normal form
(1NF) as queries may have set-valued return type. We desire the first normal
form on batched queries so as to be able to make our techniques easily
implementable in existing relational query processing systems. Hence we use
a slightly modified definition for the batched form of a query. 

Let $q(p_1, p_2, \ldots, p_n)$ be a query with $n$ parameters. Let $v_1, v_2,
\ldots, v_m$ be the attributes in the result-set that $q$ returns.  The
batched form $qb$ of $q$ takes a set $p$ of {\em n-tuples} as its parameter
(each {\em n-tuple} gives a binding for the parameters $p_1, p_2, \ldots,
p_n$). The result-set of $qb$ contains the union of $q$'s results for all
the parameter tuples in $p$. Each tuple in {\em qb's} result-set contains $n
+ m$ attributes $p_1, p_2,\ldots, p_n, v_1, v_2, \ldots, v_m$. Often only a
subset of the parameters are sufficient to establish the correlation with
the corresponding results. However, for simplicity, we assume the batched
form returns all the parameter values along with the results.  Formally, 
% as in short paper
%\[qb(p) = \bigcup_{p_t \in p} \{\{p_t\} \times q(p_t)\}\]
\[ qb(p) = \bigcup_{p_t \in p} 
           \left \{ 
              \begin{array}{ll} 
                \{\{p_t\} \times q(p_t)\}  & \mbox{if}\ q(p_t) \neq \phi \\
                \{\{p_t\} \times  \{ \mbox{{\small null-m}} \}\}  & 
                  \mbox{otherwise}
              \end{array} 
           \right. 
\]

\noindent When the result of $q$ is an empty set for any parameter 
binding, the result-set of $qb$ contains a tuple corresponding to the
specific parameter binding but the attributes $v_1, v_2, \ldots, v_n$ will
be set to null. 

\singlespace
\noindent {\bf Example:} 
Consider the following parameterized select-project query:
\[ 
q(custid)=\Pi_{ordrid}(\sigma_{customer\text{-}id=custid}(\text{ORDERS}))
\]
The corresponding batched form can be defined as:
\\
{\small $qb(\text{cs}) = \Pi_{(custid, ordrid)}(\text{cs} \LOJoin_{custid=customer\text{-}id}\text{ORDERS})$}, \\
\ \ \  where {\em cs} is the parameter relation having the attribute {\em custid}. \\
\doublespace

\eat{
\begin{floatexample}
\ \\
Consider a parameterized query (expression): \\
$q(custid)=\Pi_{ordrid}(\sigma_{customer\text{-}id=custid}(\text{ORDERS}))$ \\
\\
The corresponding batched form can be defined as:
\\
{\small $qb(\text{cs}) = \Pi_{(custid, ordrid)}(\text{cs} \LOJoin_{custid=customer\text{-}id}\text{ORDERS})$}, \\
\ \ \  where {\em cs} is the parameter relation attribute custid. 
\label{ex:simple-batch-form}
\caption{Batched Form of a Select-Project Expression}
\end{floatexample}
}

Batched forms of relational queries have been used in the context of query
decorrelation~\cite{SPL96,KIM82,GAL01,DAYAL87}. As shown in the above
example, batched forms of simple SPJ queries use a join or an outer join.
Batched forms of aggregate queries either use grouping followed by join or
an outer-join followed by grouping.  The details of deriving correct 
batched forms of {\small SQL} queries can be found in the
literature on decorrelation. \refex{ex:udf-co-batched-queries} shows
the batched forms of queries q1 and q2 used inside the {\small
UDF} of \refex{ex:udf-count-offers} in \refchap{chap:intro}.
\input{chapters/bpo/examples/simple_example_batched_queries.tex}

Most database systems also support batched bindings for basic data
manipulation operations like insert, delete and update. The {\em insert
into} $\ldots$ {\em select from} $\ldots$ construct can be used as the
batched form of {\em insert} operation. For updates, we can use the {\em
merge} construct of {\small SQL:2003} (or the {\em update} $\ldots$ {\em
from} $\ldots$ construct of {\small SQLServer}), as the batched form.
Batched forms of these operations employ various techniques such as
set-oriented index update and set-oriented integrity checks to offer
increased efficiency over the corresponding non-batched operations.

\subsubsection*{Operations having Side-Effects}
An operation with side-effects, in addition to returning a value, modifies
the system state. Further, the return value may be a function of not only
the arguments (parameters) but also the system state. We can model such an
operation with a pair of functions, $fv: S \times D \rightarrow R$ and $fs:
S \times D \rightarrow S$, where $S$ is the set of all possible system
states, $D$ is domain of parameters and $R$ is the domain of result values.
Since we assume batched forms are free to process the arguments in any
order, we can define the batched forms for only a restricted class of
side-effect causing operations. We call this restricted class of operations,
for which the batched forms are defined, as {\em batch-safe} operations. We
call an operation {\em batch-safe} if the following conditions hold:

\noindent When processing a set of arguments,
\begin{enumerate}
     \item the operation's return value, for any parameter, is independent of 
           the order in which the parameters are processed. \\
           $\forall s \in S, \forall x,y \in D, fv(S, x) = fv(fs(S, y), x)$

    \item the final system state is
          independent of the order in which the arguments are processed. \\
          $\forall s \in S, \forall x, y \in D$,
          $fs(fs(s, x), y) = fs(fs(s, y), x)$
\end{enumerate}

For example, an INSERT operation on a table that has no constraints defined,
is {\em batch-safe}. However, in the presence of table constraints ({\em
e.g.,} a unique column), the INSERT operation may or may not be {\em
batch-safe} depending on the exact set of parameters. Operations that write
to an external file/device or communicate with other systems may or may not
be {\em batch-safe} depending on the specific application.  If the
programmer has enclosed an operation inside a loop that gives no guarantee
of order, {\em e.g.,} iteration over the result set of a query without
order-by clause, we may treat the operation as {\em batch-safe}. Such
analysis for {\em batch-safety} of an operation can be extended further, but
is beyond the scope of this work. Also, in this chapter, we assume that
operations with side-effects do not have a return value, they just 
cause a change in the system state.


\subsection{Rewriting Loops to Use Batched Forms}
\label{sec:sec3-2}
Consider a statement that invokes operation $q$ inside loop $L$ of a program
$P$. We say that the invocation of $q$ is {\em batchable} {\em w.r.t} loop
$L$ if it is possible to rewrite $P$ into an equivalent program $P'$ by
removing the invocation of $q$ from the body of the loop and making a single
invocation of the batched form of $q$ ({\em i.e., qb}) outside the loop. As
an example, consider the query in \refex{ex:udf-count-offers}, which invokes
a UDF.  A program corresponding to the {\em iterative plan} for this query
is shown in \refex{ex:udf-co-iter-plan}. 

\input{chapters/bpo/examples/simple_example_loop.tex}

In this example, both the queries inside the body of the UDF can be batched
{\em w.r.t} the enclosing loop. \refex{ex:udf-co-batched} shows a rewritten
form of the query and the {\small UDF} in \refex{ex:udf-count-offers}.  The
rewritten query makes used of a batched form of the {\small UDF}, which is
called {\em count$\_$offers$\_$batched}.  The batched form of the {\small
UDF}, shown in \refex{ex:udf-co-batched}, takes a table-valued
parameter. The table-valued parameter (or the batch) is constructed from all
the distinct parameter values with which the non-batched form of the
function would be invoked by the original query.  The {\small UDF} {\em
count$\_$offers$\_$batched}, makes use of a temporary table $r2$. Note that
all the updates performed by the {\small UDF} are only on the 
temporary table. The {\small UDF} {\em count$\_$offers$\_$batched} in turn
makes use of the set-oriented forms the queries {\em q1} and {\em q2 }.
These set-oriented forms called {\em q1b} and {\em q2b} were shown in
\refex{ex:udf-co-batched-queries}. The {\small UDF} uses the {\small SQL}
{\small MERGE} construct to merge the results of the set-oriented queries
with the temporary table $r2$, which stores the values of all the local
variables and function parameters.  In the batched version we still have an
iterative loop (the only loop in the body of {\em
count$\_$offers$\_$batched}), but it contains only inexpensive operations.
It is possible to pull even such operations out of the loop, we discuss
about this in \refchap{chap:concl}.

\input{chapters/bpo/examples/simple_example_batched.tex}

Even if an operation is {\em batch-safe}, it may not always be possible to
batch a given invocation of the operation {\em w.r.t} a loop, because of
side effects within the loop.  In \refsec{sec:rules:chap:bpo} we provide a
set of program transformation rules that allow batching the invocations of
an operation when the program satisfies certain conditions. 

\subsection{Generating Batched Forms of Procedures}
\label{sec:gen-batched-form}
To speed up applications or queries that make repeated calls to stored
procedures or UDFs we need efficient batched forms of these procedures.
However, batched forms of complex operations like stored procedures and UDFs
are (as far as we know) not available unless implemented by the programmers
manually.  We therefore consider the problem of automatically generating
batched forms of stored procedures and UDFs. Our goal is to generate
efficient batched forms by batching the expensive operations within the body
of the procedure/UDF.

\begin{figure}[t]
%\begin{center}
\begin{minipage}{1.0\textwidth}
{\small
\ordinalg{
{\em fb-trivial(pt)} $\Longleftrightarrow$ {\em Apply(pt, f)} \\
where the function {\em Apply} is defined as : \\
\\
\> {\bf {\em Apply(pt, f):}} \\
\> $r=\{\}$ ;\\
\> for each $t$ in {\em pt} \\
\>   \> $<$ {\em body of f with parameters bound from attributes of t} $>$ \\
\>    \> {\em rf} $=$ {\em return value of f}; \\
\>    \> {\em r.addRecords}$(\{$t$\}$ $\times$ {\em rf}$)$; \\
\> return $r$; 
}
}
\end{minipage}
%\end{center}
\caption{Trivial Batched Form of a Procedure}
\label{fig:trivial-batched-form}
\end{figure}

Given any side-effect free function or {\em batch-safe} operation (which
could be a stored procedure) {\em f}, we can generate its trivial batched
form as shown in \reffig{fig:trivial-batched-form}.  Batched form of any
procedure can thus be generated by enclosing it in a loop that iterates over
the parameter set and executes the statements inside the procedure
repeatedly.  However, such a rewriting is not of significant benefit as {\em
cost(fb-trivial)} for a batch size of $k$ is nearly same as $k \times${\em
cost(f)}; Such a rewriting can still be useful in reducing round-trip delays
in client server environments. More interesting batched rewrites are the
ones that use specialized and efficient strategies for batch processing,
{\em e.g.,} batched {\em selection} within the procedure can be processed as
a {\em join}, while a query in the procedure which performs a selection
followed by an aggregate would have a batched form that employs grouping
followed by join.

To generate an efficient batched form of a procedure, we can start with the
trivial batched form of the procedure and try to batch each expensive
sub-operation in the body of the procedure {\em w.r.t.} to the enclosing
loop. To do so, the sub-operation must be taken out of the enclosing loop
and substituted by its batched equivalent. If the sub-operation is a query,
its batched form may be known. If the sub-operation is a procedure call, we
recursively invoke the method to generate the batched form of the called
procedure. 

\eat{
\begin{figure}[t]
{\small
\begin{codefrag}
{\bf GenerateBatchedForm($q$) }\\ 
{\bf BEGIN} \\
    \> {\bf IF} $q$ has a known batched form {\em qb} \\
    \>  \> output {\em qb}; \\
    \> {\bf ELSE} \\
    \> \> Write the trivial batched form of $q$ as: \\
    \> \> {\em tb} $=$ {\em Apply (pt, q)}. Let $L$ be the loop of the {\em Apply} op.  \\
    \> \> {\bf FOR EACH} expensive operation $q_i$ inside the body of {\em tb} \\ 
    \> \> \> {\bf IF} $q_i$ can be batched {\em w.r.t.} $L$ \\ 
    \> \> \> \>  $qb_i=${\em GenerateBatchedForm($q_i$)}; \\
    \> \> \> \>  Re-write {\em tb} to batch $q_i$ {\em w.r.t} $L$ (make use of $qb_i$) \\
{\bf END}  \\
\end{codefrag}
}
\caption{Generating Batched Forms of Procedures}
\label{gen-batched-form}
\end{figure}
}

As we can see, generating batched form of a complex procedure reduces to the
task of batching selected operations {\em w.r.t.} a loop (see
\refsec{sec:sec3-2}).  We address this problem in
\refsec{sec:rules:chap:bpo} after introducing some preliminaries in
\refsec{sec:prelims:chap:bpo}.




==> chapters/bpo/sections/sec_discuss.tex <==
\section{Discussion}
\label{sec:discuss:chap:bpo}

\noindent{\bf Implementation of Parameter Batches}: The $L$-tables, 
discussed in \refsec{sec:rules:chap:bpo}, serve to hold the
parameter batch with which the {\em batched form} of an operation is
invoked. Though small batches can be held in memory, in general we may need
to materialize the batches and the cost of materialization must be taken
into account while deciding to batch an operation. However, for procedures
that run entirely inside the database engine ({\em e.g.,} UDFs) it may be
possible to avoid materialization of batches by constructing a single
dataflow containing both relational and {\em procedural nodes}. Our loop
splitting transformation is designed to facilitate such an approach.
Appendix~\ref{appendix3} contains few additional rules that can be used for
(i) avoiding creation of intermediate batches by passing a relational
expression, instead of a table, to the batched forms and (ii) mapping
program statements that perform simple and inexpensive operations ({\em
e.g., expression evaluation and variable assignment}) to operators that work
on sets. The later of these helps in eliminating loops such as the one left
over in~\refex{ex:udf-co-batched}.  When a single dataflow is thus
built, code that cannot be mapped to relational operators is executed by
{\em procedural nodes} in the dataflow.  Variable bindings inside such nodes
are obtained from input tuples.  Depending on the specific code, each {\em
procedural node} may be blocking or non-blocking.  The $L$-tables
become streams in the pipeline. 

\noindent{\bf Cost-Based Choice of Queries to Batch}:
The operations to batch must be chosen taking into account the potential
benefits and costs associated with the transformed code. Our current
implementation requires the user to specify which operations to consider for
batching. The important parameters on which this decision depends include
(i) cost model for the operation as a function of batch size, (ii) expected
number of iterations of the program loop and (iii) branch probabilities for
the branching statements {\em (if-then-else)} in the program.  Automating
the choice of operations to batch is a future work.

\eat{
\noindent{\bf Multiset Batches}:
Though batched forms of pure functions need to process only a {\em set} of
parameters, the batched forms of operations that have side-effects must
consider a {\em multi-set} of parameters. This however, creates a duplicate
record problem while correlating the results back. In this report , as we
assume no return value for operations with side-effects, the required
equivalence rules work correctly even for multi-sets.
}

%\input{chapters/bpo/sections/completeness.tex}

% ********** Extra details - may be useful for techrep **************
\eat{
\subsubsection{Avoiding the Batch Materialization for Queries with UDFs}
For queries that invoke UDFs it may be possible to avoid materialization of
batches by constructing a single dataflow. Consider the sample code and its
translation shown in \reffig{fig:example-dataflow}. For the translated
program a single dataflow can be constructed as shown in
\reffig{fig:dataflow}. To enable such an approach the query execution engine
must support procedural operator nodes as part of the query evaluation plan.
The procedural operator nodes, shown with label {\em P} in
\reffig{fig:dataflow}, can execute a specified code over the input tuples.
Depending on the specific code, a procedural node can be blocking or
non-blocking.

\input{single_dataflow.tex}

\begin{figure}[t]
\begin{center}
\includegraphics[height=2.5in]{fig/dataflow.eps}
\caption{Dataflow Tree for the Query and UDF in \reffig{fig:example-dataflow}}
\label{fig:dataflow}
\end{center}
\end{figure}

\subsubsection*{Set-Oriented Evaluation in the Presence of Cyclic
                Flow-Dependencies}
Even when an invocation of a side-effect free operation lies on a
flow-dependency cycle (see Conjecture \ref{conj:main}), it may be possible
to have set-oriented evaluation of the function. Instead of trying to deduce
the exact parameter set, we may evaluate the function over a super set of
the parameter set. Such an approach allows us to avoid iterative invocation
of the function even when there is a cyclic flow-dependency involving the
function call. Hence the condition in Conjecture \ref{conj:main} is only a
sufficient condition and not necessary.
%Consider the example in \reffig{fig:example-noloop} of \refsec{sec:rules}.

\noindent{\bf Avoiding the Overheads of Loop Split}:
Loop splitting can be expensive when there are large number of variables
that are written in one partition and read in the other. Each such variable
becomes a table attribute and we remember as many values as there are
iterations of the loop. In certain cases, it may be possible to avoid loop
splitting altogether and still use batching.  The approach is to execute the
loop twice. In the first execution, all the side-effect causing operations
are removed from the body of the loop and the queries to batch are replaced
with statements that collect the parameter values and build a batch. Once
the batch is ready, we invoke the batched form of the query and store the
results. We then execute the loop a second time where the query execution
statements are replaced by statements that look up the stored result of the
batched query execution. Such an approach is feasible when the query to
batch does not have a dependency on another such query and also on any
side-effect causing operation.
}


==> chapters/bpo/sections/sec_perf.tex <==
\section{Experimental Results} 
\label{sec:perf:chap:bpo}
Our rewrite rules can conceptually be used with any language.  However, to
implement the rules we need to perform dataflow analysis of a program and
build the data dependence graph. For our implementation, we chose
Java, since tools for its dataflow analysis are available in public domain.
Our implementation uses the {\em SOOT} optimization framework~\cite{soot}.
{\em SOOT} uses an intermediate code representation called {\em Jimple} and
provides dependency information on  {\em Jimple} statements. Our
implementation transforms the {\em Jimple} code using the dependence
information. Finally, the {\em Jimple} code is translated back into a Java
program. 

Our current implementation requires that queries and updates be performed
using our API layer built on top of JDBC. During rewrite we recognize these
calls and transform them for batched bindings when possible. We have not yet
implemented query rewriting to get batched forms and this step is done
manually.  The techniques for deriving batched forms of queries are well
known and we expect the implementation to be straight-forward.  Tables
(batches) used in the rewritten procedures are constructed in-memory and
transferred to the database before evaluating the batched queries.
Nest/unnest and merge operations are performed on these in-memory tables.

There are no benchmarks for procedural SQL that we could use for our
experiments.  However, we had seen three real-world applications
which were facing serious performance problems due to non-set-oriented
execution, which were affecting their usability.  We use these scenarios for
our experiments. Our current implementation does not support all the
transformation rules presented in this chapter. Hence, in some cases part of
the rewriting was performed manually in accordance to the transformation
rules. We do not have access to the actual data used in these applications
and hence we used synthetic data. In one case we used TPC-H data as it
matched the scenario. As we cannot report timings on the actual application
code, we used independent programs having only the code required for the
specific scenarios.  The experiments were performed on a widely used
commercial database system (we call it SYS1) running on an Intel P4 (HT) PC
with 1GB of RAM. 

\subsection*{Experiment 1: Traversal of Category Hierarchy}

\begin{figure}[ht]
\begin{minipage} {1.0\textwidth}
\begin{center}
\includegraphics[angle=270,width=3.9in]{chapters/bpo/fig/plots/travcat/travcat.eps}
\caption{Performance Results for Experiment 1}
\label{fig:travcat-mssql}
\end{center}
\end{minipage}
\end{figure}

For this experiment, we used a program, which is a slight variant of the UDF
in~\refex{ex:udf-travcat}. The program finds the item (part) with maximum
size under a given category (including all its sub-categories) by performing
a DFS of the category hierarchy. For each node (category) visited, the
program queries the {\em item} table.  The TPC-H {\em part} table, augmented
with a new column {\em category-id} and populated with 2 million rows, was
used as the {\em item} table. The {\em category} table had 1000 rows - 900
leaf level, 90 middle level and 10 top level categories (approximately). A
clustering index was present on the {\em category-id} column of the {\em
category} table and a secondary index was present on the {\em category-id}
column of the {\em item} table. All relevant statistics were built.
\reffig{fig:travcat-mssql} shows the performance of the program before and
after rewrite. 

For the non-batched query on the {\em item} table, SYS1's default choice was
to use the secondary index.  This plan results in a lot of random IO, and
we found an alternative plan, which performs a sequential scan takes less
time since the entire relation is brought into memory on the first
invocation, and there is no IO on subsequent invocations.  Since this plan
was found to be cheaper, we enforced it using optimizer hints.
% The default plan performed extremely poorly (compared to the batched
% query) even for batch size of 1 due to a large number of random IOs. We
% found that the best choice for the original (iterative) program is to use
% a sequential scan in the inner loop. Also, with a large buffer pool (as in
% our setup) this plan required no IOs after the first iteration of the
% loop.  
\reffig{fig:travcat-mssql} compares the time taken by the best plan for the
original program with the batched version.
% Even with 100\% cache hit for iterations $>$ 1, The original program
% performs poorly for larger batch sizes due to the CPU overheads of
% repeated predicate evaluation. 
The batched version, in this case, performed a {\em group-by} followed by a
join, whereas the original program repeatedly executed a query that
performed selection followed by group by; as a result the batched version
showed much better performance. In this experiment, the performance of the
batched form was almost independent of the batch size because the group-by
query computed the results for all the parameters in each case.

In transforming the program, Rule-5 (reordering), Rule-2 (loop splitting)
and Rule-1 (batching) were applied in that order.  There was a 12.5\%
increase in the program size (lines of code) due to the transformation.

\subsection*{Experiment 2: ESOP Management Application}
\label{subsec:exp2}
\begin{figure}[ht]
\begin{minipage} {1.0\textwidth}
\begin{center}
\includegraphics[angle=270,width=4.3in]{chapters/bpo/fig/plots/polaris/pol.eps}
\caption{Performance Results for Experiment 2}
\label{fig:pol}
\end{center}
\end{minipage}
\end{figure}
For this experiment, an application used for managing stock option grants of
multiple organizations was considered. During each {\em upload} operation, a
large number of records from a delimited file were processed.  The
application performed a mix of queries, inserts and updates. A brief outline
of the program logic is given below to indicate the complexity of
control-flow involved.

For each record read from the input file, the program performs validation
and pre-processing of the fields and then queries the {\em options} table to
check if a record for the person already exists. The query predicate is
parameterized on the values read from the input record.  If a record is
present, the old values of the various fields and the {\em internal-emp-id}
are obtained as part of the same query.  Further, the {\em contactinfo}
table is queried using the {\em internal-emp-id} to obtain contact info
fields. If the input record being processed has empty values for any of the
fields, the old values (when present) are copied to those fields.  Finally,
new records are inserted or existing records updated in both {\em options}
and {\em contactinfo} tables.  \reffig{fig:proc2} in
Appendix~\ref{appendix1} shows the procedure.

The rewritten program used an outer join in place of iterative selections,
and performed batched updates and inserts. \reffig{fig:pol} compares the
performance of the rewritten program with the original program for varying
number of input records.

In transforming the program, Rule-4 (control-dependencies to
flow-dependencies), Rule-5 (reordering), Rule-2 (loop splitting) and Rule-1
(batching) were applied.  After transformation there was a 17\% increase in
the program size.
%The increase in program size due to the transformation was 17\%.

\subsection*{Experiment 3: Value Range Expansion}
\label{subsec:exp3}
%(Only Inserts)}
\begin{figure}[ht]
\begin{minipage} {1.0\textwidth}
\begin{center}
\includegraphics[angle=270,width=4.5in]{chapters/bpo/fig/plots/nic/nic.eps}
\caption{Performance Results for Experiment 3}
\label{fig:nic-mssql}
\end{center}
\end{minipage}
\end{figure}

In this application, data about {\em forms} issued to various agents would
arrive in the format {\em (agent-id, start-form-number, end-form-number)}.
The program (shown in \reffig{fig:nicproc} of Appendix~\ref{appendix1})
would iterate over all the {\em form issue} records, expand the {\em issue}
range and populate the {\em forms-master} table with entries corresponding
to each individual form. The purpose was to be able to update and track the
status of each individual form subsequent to its issue.  The original
program had an outer loop iterating over the {\em form issue} records and an
inner loop iterating over the range {\em (start-form-number,
end-form-number)}. An INSERT operation was performed inside the inner loop.
The transformed program could pull the {\em insert} operation out of both
the loops and perform a batched insert.  The running times of the original
and transformed program are shown in~\reffig{fig:nic-mssql}.  The batched
version performs much better for large batch sizes.  For small batch sizes
(less than 1K) the computational overheads due to batch creation and
nest/unnest operations cause the batched version to perform marginally
slower than the original program.

In transforming the program, Rule-5 (reordering), Rule-2 (loop splitting),
Rule-1 and Rule-6 (batching) were applied. The increase in program size 
was 16.5\%.

\eat{
For each record read from the input file:
\begin{itemize}
\addtolength{\itemsep}{-5pt}
\item Perform validation and pre-processing of the fields 
\item The {\em options} table is queried to check if an old record 
for the person already exists. The query predicate is parameterized
on the values read from the input record.
%{\em client-id} and {\em emp-id} values from the input record. 
If a record is present, the old values of the various fields and 
the {\em internal-emp-id} are obtained as part of the same query.
\item If an old record was present, the {\em contactinfo} table is queried 
using the {\em internal-emp-id} to obtain contact info fields.
\item If the input record being processed has empty values for any of 
the fields, the old values (when present) are copied to those fields.
\item New records are inserted or existing records updated 
%(if a record was present already) 
in both {\em pmaster} and {\em contactinfo} tables.
\end{itemize}
}

\eat{
\subsection*{Experiment 4: Effect of Batch Size}
\begin{figure}[t]
\begin{minipage} {0.5\textwidth}
\begin{center}
\includegraphics[angle=270,width=3.0in]{chapters/bpo/fig/plots/jdbc-batch-update.eps}
\caption{Performance Results for Experiment 4}
\label{fig:jdbc-batched-update}
\end{center}
\end{minipage}
\end{figure}

To see the effect of batch size on inserts and updates, we used a JDBC 
program to populate the TPC-H lineitem table with 6 million rows. 
Commits were performed for every 10,000 rows. We varied the batch size 
from 1 to 10,000 and the total time for the load operation with various 
batch sizes are plotted in Figures \ref{fig:jdbc-batched-update}.
}

%\vspace{-0.3in}
\subsection*{Time Taken for Program Transformation} 
Although the time taken for program transformation is usually not a concern
(as it is a one-time activity), we note that, in our experiments the program
transformation took very little time (less than a second). 
%The increase in code size due to the transformation was 12.5\% in
%experiment-1, 17\% in experiment-2 and 16.5\% in experiment-3.


==> chapters/bpo/sections/sec_prelims.tex <==
\section{Background for Our Work} 
\label{sec:prelims:chap:bpo}
In this section, we formally outline the language constructs we support and
provide background material on the terminology used in this chapter.

\subsection{Language Constructs}
For our illustration, we use a simple procedural language.  The language
offers expressions, assignment, conditional \- branching and looping. The
supported language constructs are briefly described below.

\begin{itemize}
\addtolength{\itemsep}{-3pt}
\item {\em while loops} are of the form {\em while}{\em {\tt (predicate)}}
      {\em loop} $\ldots$ {\em end loop;}.  

\item {\em cursor loops} are of the form {\em for each} {\tt record} 
      {\em in} {\tt query/table} {\em loop} $\ldots$ {\em end loop;} 
      An {\em order by} clause can be present if the iteration is over 
      a table. When present, the {\em order by} is assumed to be 
      {\em ascending} by default. Unlike the more general and
      powerful {\em while loops}, the cursor loops iterate over the result
      of a query and hence their iteration space is known once the query is
      evaluated.

\item Branching is possible through {\em if-then-else} having the syntax
      {\em if} {\tt (predicate)} $\{ \ldots \}$ {\em else} $\{ \ldots \}$.  

\item Scalar variables: we consider only scalar variables in our discussion.
      However, our techniques can be easily extended to handle arrays,
      records and collection types.  Each looping block can have variables
      local to the block.  Statements can access variables local to their
      block or variables defined in any of the ancestor blocks. 

\item 
      Result of scalar queries (queries that return exactly one tuple) can
      be assigned to variables. \\ {\em e.g.,} $v_1, v_2, \ldots, v_n = $
      {\em select} $c_1, c_2, \ldots, c_n$ {\em from} $\ldots$; \\ Note that
      a single assignment can be used to simultaneously assign values to
      multiple variables.  Set-valued queries can be used only in the
      context of {\em cursor loops}.
\end{itemize}

We also use a few additional constructs in the transformed code. We assume
these constructs are not available for the end-user and hence cannot be
present in the input program. 
\begin{itemize}
\addtolength{\itemsep}{-4pt}
    \item  The TABLE type is used to construct the parameter
           batches. The TABLE type can be implemented so as 
           to make use of both main memory and disk. 
           %We discuss this in more detail in \refsec{sec:discuss:chap:bpo}.
    \item Updatable cursor loops are of the form 
          {\em for each} {\tt record} {\em by ref} {\em in} 
          {\tt table} {\em loop} $\ldots$ {\em end loop;}
          Any updates to the record modify the underlying table variable. 
    \item The transformed program may use 
          relational operators such as selection, projection and join. 
\end{itemize}

\section*{Assumptions}
We make the following assumptions about the program.
\begin{enumerate}
\addtolength{\itemsep}{-4pt}
    \item Unconditional control transfer 
          statements like GOTO, EXIT and CONTINUE are not used.
    \item Statements have no hidden side-effects. Information about all 
          reads and writes performed by a statement (either on memory 
          locations or on external resources like files and databases) 
          are captured in the {\em data dependence graph} (explained in 
          the next section).
\end{enumerate}

\subsection{Data Dependence Graph}
The {\em Data Dependence Graph} (DDG), sometimes referred to as Program
Dependence Graph~\cite{MUCHNICK,PDG87}, of a program is a directed
multi-graph in which program statements are nodes (vertices) and the edges
represent data dependencies between the statements. The different types of
data dependence edges are explained below.

\begin{itemize}
\addtolength{\itemsep}{-4pt}
\item A {\em flow-dependence} edge ($\fdep$) exists from statement (node)
      $s_a$ to statement $s_b$ if $s_a$ writes a location that $s_b$ may
      read, and $s_b$ follows $s_a$ in the forward control-flow. 

\item An {\em anti-dependence} edge ($\adep$) exists from statement $s_a$ to
      statement $s_b$ if $s_a$ reads a location that $s_b$ may write, and
      $s_b$ follows $s_a$ in the forward control flow.

\item An {\em output-dependence} edge ($\od$) exists from statement $s_a$ to
      $s_b$ if both $s_a$ and $s_b$ may write to the same location, and $s_b$
      follows $s_a$ in the forward control flow. 

\item A {\em loop-carried flow-dependence} edge ($\lcfd{L}$) exists from
      $s_a$ to $s_b$ if $s_a$ writes a value in the $i^{th}$ iteration of a
      loop $L$ and $s_b$ may read the value in a later iteration ($j^{th}$
      iteration where $j>i$). 

\item Similarly, there are loop carried counter parts of {\em anti} and {\em
      output} dependencies and are denoted by ($\lcad{L}$) and ($\lcod{L}$)
      respectively.
\end{itemize}

The data dependence graph for the sample UDF of \refex{ex:udf-travcat}
is shown in \reffig{fig:sampleddg}. 

\section*{External Dependencies}
Statements may have dependencies not only through program variables but also
through the database and other external resources like files. For example,
we have $s_1 \fdep s_2$ if $s_1$ writes a value to the database, which $s_2$
may read subsequently. Though standard dataflow analysis performed by
compilers considers only dependencies through program variables, it is not
hard to extend the techniques to consider external dependencies, at least in
a conservative manner. For instance, we could model the entire database (or
file system) as a single program variable and thereby assume every
query/read operation on a database/file to be conflicting with an
update/write of the database/file. In practice, it is possible to perform a
more accurate analysis on the external writes and reads.  When referring to
external dependencies explicitly, we use {\em E} as a superscript to the
corresponding type of dependence edge {\em e.g.,} $s_1 \extfdep s_2$.

\begin{figure} [ht]
\centerline{\psfig{file=chapters/bpo/fig/ddg-small.eps,width=12cm,height=9cm}}
\caption{A Subgraph of the Data Dependence Graph for the UDF in \refex{ex:udf-travcat}}
\label{fig:sampleddg}
\end{figure}



==> chapters/bpo/sections/sec_relwork.tex <==
\section{Related Work}
\label{sec:relwork:chap:bpo}
Queries such as those shown in ~\refex{ex:udf-count-offers} and
\refex{ex:udf-travcat} can be thought of as nested queries with complex
inner blocks. The inner block in such cases contains subqueries embedded in
procedural code. Known decorrelation techniques such as
~\cite{KIM82,GAN87,SPL96,GAL01,DAYAL87,GAL07} cannot be used to unnest such
queries.  The techniques proposed in this chapter make it possible to
rewrite a procedure so as to enable set-oriented evaluation of the embedded
sub-queries through batched bindings. This is an essential step in
decorrelation~\cite{SPL96}.  Further optimizations, such as pipelining the
output of the expression that produces the parameter batch into the
expression that consumes it, are possible and should be considered for
future work.  Graefe~\cite{GRA03} highlights the benefits of batched
bindings for speeding up index nested loops joins. Batched bindings not only
help in performing IO efficiently, but can also make it possible to employ a
set-oriented strategy at the operator level.  {\em Magic sets}
decorrelation~\cite{SPL96} employs parameter batches for decorrelation of
nested queries. Our techniques can be thought of as extending this approach
for complex procedures.  Our work is a step towards combining query
optimization with program analysis and transformation techniques; we believe
this combination will give significant benefits for database applications.

Lieuwen and DeWitt~\cite{LIEUWEN92} consider the problem of optimizing set
iteration loops in database programming languages.  Their techniques can
convert nested set iteration loops into joins. However, their work does not
address the issue of batching procedure calls. 
%Their transformation rules work on a restricted syntax. 
The program transformation rules in this chapter can work with complex
control-flow including {\em if-then-else} and {\em while} loops. Rule-2 in
this chapter is a more general version of Rule T4 in \cite{LIEUWEN92}.  An
earlier work similar to \cite{LIEUWEN92} is \cite{SHOPIRO80}. It describes a
programming language called Theseus for manipulating relational databases,
and proposes optimization transformations, some of which are special forms
of those presented in \cite{LIEUWEN92}.  To the best of our knowledge,
reordering of statements in a loop to facilitate batched invocations of
queries is not considered before.  The works of Katz and Wong \cite{KATZ82},
and Demo and Kundu \cite{DEMO85} address the problem of converting programs
which make use of CODASYL FIND-statements into equivalent programs using
relational queries. Similar to our work, their solution employs dataflow
analysis. The aim of dataflow analysis in their work is to find dependencies
between CODASYL FIND-statements so as to group the statements that access
the same logically definable set of records.  Fegaras~\cite{LEO99} addresses
query optimization in object oriented databases, in the presence of object
identity and in-place updates.  Poulovassilis and Small~\cite{POUL96}
consider algebraic optimization of declarative, functional database
programming languages.  Their work considers a computationally complete
functional language and addresses issues such as termination, infinite data
structures, but does not consider imperative language constructs and
side-effects. Ceri and Widom \cite{CERI91} address the problem of deriving
production rules for incremental maintenance of materialized views. The
generated rules are set-oriented in the sense that they can process a set of
changes performed on the base tables at once. In their work, the view 
definitions are assumed to be in {\small SQL} without any procedural 
constructs.

Some of the program transformation techniques we employ are derived from
those proposed in the area of parallelizing
compilers~\cite{KENEDY90,PAUDUA95,FORT87}. However, the problem of batching
differs from the problem of parallelizing in the following ways: {\em (i)}
presence of flow-dependencies (described in \refsec{sec:prelims:chap:bpo})
does not allow parallelization.  However, batching is possible even if the
order of two operations cannot be changed due to flow-dependencies, and {\em
(ii)} as the aim of batching is to improve the performance of expensive IO
bound queries and other database operations, it may be acceptable for the
transformations to introduce additional {\small CPU} operations or use extra
memory to make batching possible. However, such approaches do not generally
yield significant benefits in the context of parallelizing the instructions
and are not considered to the best of our knowledge.



==> chapters/bpo/sections/sec_rules.tex <==
\section{Program Transformation}
\label{sec:rules:chap:bpo}
Recall from \refsec{sec:sec3-2} that an invocation of an operation $q$
inside a loop $L$ is said to be {\em batchable} {\em w.r.t} loop $L$ if it
is possible to rewrite the program into an equivalent program where the
invocation of $q$ is removed from the body of the loop and a single
invocation of the batched form {\em qb} is made outside the loop. For such a
rewrite, it is necessary that the operation should be {\em batch-safe}.
However, the data and control dependencies between program statements may
make it impossible to batch a statement that invokes an operation even if
the operation is {\em batch-safe}. In this section, we present a set of
program transformation rules, which enable us to batch a statement {\em
w.r.t.} a loop when the program satisfies certain conditions. 

The program transformation rules we present, like the equivalence rules of
relational algebra, allow us to repeatedly refine a given program. Applying
a rule to a program involves substituting a program fragment that matches
the antecedent ({\small LHS}) of the rule with the program fragment
instantiated by the consequent ({\small RHS}) of the rule.  Some rules
facilitate the application of other rules and together achieve the goal of
batching a desired statement {\em w.r.t.} a loop.  Applying any rule results
in an equivalent program and hence the rule application process can be
stopped at any point.

\input{chapters/bpo/sections/notation.tex}

\input{chapters/bpo/sections/rules/rule1.tex}
\subsection{Rewriting Set Iteration Loops (Rule 1)}
In the simplest case, the loop contains a single statement that invokes the
operation we want to batch. In this rule, we consider cursor update loops -
the loop iterates over a set of tuples and the values returned by the
operation to be batched are assigned back to the attributes of the tuple
associated with current iteration. Rules 1A through 1C 
%shown in \reffig{fig:rule1} 
are the basic rules that allow replacing a loop by a batched invocation.
Rule 1D and all the other rules presented in this section help us transform
the program so as to enable the application Rules 1A, 1B or 1C.

In Rule-1A, $q$ can be any batch-safe operation (with or without
side-effects).  Note the use of projection without duplicate elimination
($\Pi^{d}$) for constructing the parameter multiset. However, in rules 1B
and 1C, we require $q$ to be a {\em pure} function returning exactly one
tuple ({\em e.g., a scalar query}). In rules 1B and 1C we construct a
duplicate-free parameter set using the standard relational projection.  This
avoids the duplicate record problem while merging back the results of the
batched invocation.

For brevity, in rules 1B and 1C we omit the form with loop invariant
parameters.  In rules 1B and 1C we deal only with assignments to cursor
attributes and not variables. The reason for this will be clear when we
describe rules 2 and 3. For now, it suffices to know that the later
transformations bring the program into a form in which we can apply one of
the rules described in this section.

\subsection{Splitting a Loop (Rule 2)}
In general, the body of a loop may contain several statements along with the
query execution statement(s) we are interested in batching.  In such a case,
we try to split the loop into multiple loops, such that the statement we are
interested in batching appears in a loop by itself.  Consider the examples
in Figures~\ref{fig:loop-split-ex1} and \ref{fig:loop-split-ex2}.  The
statements to be batched are shown in bold.  As shown in the figures, we
split the loop into multiple set-iteration loops.  The aim is to have the
statement to be batched appear in a loop by itself, a form in which we can
apply Rule 1.  For example, in the rewritten code of
\reffig{fig:loop-split-ex1}, the loop containing a single {\small INSERT}
statement can be replaced by a batched invocation, by first removing the
{\em order by} using Rule 1D and then applying Rule 1A(i).

\input{chapters/bpo/examples/case1.tex}
\input{chapters/bpo/examples/case1b.tex}
\input{chapters/bpo/sections/rules/rule2.tex}

If the sequence of statements {\em ss} in a loop is made up of two
consecutive sub-sequences $ss_1, ss_2$ ({\em i.e.,} $ss=ss_1+ss_2$), and if
there are no loop-carried flow dependencies from any statement in $ss_2$ to
any statement in $ss_1$ or to the loop predicate, then the loop can be split
such that $ss_1$ and $ss_2$ appear in separate loops. 

Unlike cursor loops, the iteration space for general {\em while} loops
cannot be known upfront~\cite{PAUDUA95} and is constructed dynamically. In
general, the loop splitting transformation, for the case of {\em while}
loops, can be expressed as Rule 2\footnote{
In the interest of readability, the earlier examples in 
Figures~\ref{fig:loop-split-ex1} and \ref{fig:loop-split-ex2} 
contained minor variations from the construction in Rule 2.}.
%shown in in \reffig{fig:rule2}.  

We call a variable as {\em split variable} if it is involved in a
loop-carried anti or output dependency that crosses the split boundaries.
While splitting a loop we introduce a table-valued variable, which has
attributes corresponding to each of the split variables.  Each loop in the
original program, if required to be split, introduces exactly one table. The
table essentially serves to break the loop-carried anti and output
dependencies.  We call the table associated with loop $L$ in the original
program as the $L$-table.  Note that after the split, the newly formed loops
that iterate on the $L$-table must have an {\small ORDER BY} clause.
The {\small ORDER BY} clause can then be eliminated using Rule 1D if the 
statements inside the loop are batch-safe. 


Although we succeed in splitting a loop by breaking loop-carried anti and
output dependencies, loop-carried flow dependencies prohibit splitting of
the loop (see precondition (a) of Rule-2). For example, if a statement in
$ss_2$ wrote a variable whose value is read in $ss_1$ or by the loop
predicate, then Rule 2 does not apply. However, later in this chapter we
shall see that in some cases it is possible to reorder the statements within
a loop so as avoid such loop-carried flow dependencies. All types of
loop-carried external dependencies prohibit splitting the loop (see 
preconditions (a) and (b) of Rule-2). Recall that external dependencies
are data dependencies through external resources like files. 
%{\em Loop local tables}, when small enough, can be held in memory but this
%may not always be possible.  We discuss the implementation issues of {\em
%loop-local} tables in \refchap{chap:concl}.
Rule 2 generalizes rule T4 of Lieuwen and DeWitt~\cite{LIEUWEN92}. We compare
our work with \cite{LIEUWEN92} in \refsec{sec:relwork:chap:bpo}.

\eat{
The need for conditions (\smallbf{c1}) and (\smallbf{c2}) in Rule 2A is
straight forward. The need for (\smallbf{c3}) arises due to the way in which
we construct the $L$-tables. Only the variables local to loop $L$ are made
attributes of the $L$-table.  Any variable defined in an ancestor block
$L_p$ of $L$ becomes an attribute of the $L_p$-table. Constructing the
$L$-tables in this way avoids redundant space consumption and more expensive
updates of redundant information by giving normalized representation of the
$L$-tables. By introducing an extra split variable, we can make a loop
satisfy condition (\smallbf{c3}) even if it did not satisfy it originally.
The extra split variable preserves the value of the non-local variable
for each iteration.  For brevity, we omit the transformation rule for this
step.
}

\eat{  % Extra matter
Consider the example in \reffig{fig:case-nonlocal} in which, a non-local
variable {\em max} is being written and subsequently used as a query
parameter inside the loop. This prohibits splitting the loop as it violates
condition (\smallbf{c3}).  In such a case, we first apply an auxiliary rule,
which introduces an extra {\em local} variable in the loop. The local
variable acts as a copy of the non-local variable and when converted to an
attribute of the $L$-table by Rule-2, it preserves multiple
values of the non-local variable and thus enables batching of $q$.  In the
transformed code of \reffig{fig:case-nonlocal}, note that we can apply
Rule-1 and replace the final loop containing {\em q(r.localmax)} with a
single batched invocation.
}

\eat{
When condition (\smallbf{c3}) is not satisfied, we apply an auxiliary rule,
which introduces an extra local variable in the loop that acts as a copy of
the non-local variable. This transformation, illustrated with the example in
\reffig{fig:case-nonlocal}, enables the application of Rule 2 by making the
loop satisfy condition (\smallbf{c3}). The auxiliary rule is straight
forward and we omit its formal specification.
}

\subsection{Separating Batch-Safe Operations (Rule~3)}
\eat{
Assignment operation is not batch-safe unless the target location ({\small
LHS}) is different for each argument ({\small RHS}) ({\em i.e.,} there is no
loop carried self-output dependency for the statement). Loop carried
self-output dependencies are eliminated when we convert local variables of a
loop into table attributes during loop split. However, for non-local
variables this is not true. We therefore decouple assignments to non-local
variables as shown in the example of \reffig{fig:case4a}.  Further,
references to non-local variables may need to be changed so that condition
{\bf (c3)} for Rule 2 is satisfied. \reffig{fig:case4b} shows an example.
The transformations rule is formally expressed below.
}
A program statement may contain the expression we want to batch in
combination with other non batch-safe operations.  In such a case, we
isolate the batch-safe operation by introducing an extra variable.
\reffig{fig:separate-batch-safe} shows an example and Rule 3 expresses the
transformation formally.

\input{chapters/bpo/examples/case4a.tex}
\input{chapters/bpo/sections/rules/rule_separate_batchsafe.tex}

%\newpage
Variable assignment is not batch-safe in general, {\em e.g.,} assignment to
a global variable. However, assignments to different locations, {\em e.g.,}
different rows of a cursor loop, can be performed in any order and hence
batch-safe in the context of split variables that are converted to
attributes of the $L$-table by Rule 2. If the return value of a query is
assigned to a non-local variable, applying Rule 3 introduces a new split
variable and thus enables batching the query.


\subsection{Control to Flow Dependencies (Rule 4)}
\noindent Conditional branching ({\em if-then-else}) and {\em while} loops
lead to control dependencies.  If the predicate evaluated at a conditional
branching statement $s1$ determines whether or not control reaches statement
$s2$, then $s2$ is said to be control dependent on $s1$.  During loop split,
it may be necessary to convert the control dependencies into flow
dependencies~\cite{KENEDY90}. \reffig{fig:control-to-flow} shows an example.
Rule 4 specifies the transformation formally.
\input{chapters/bpo/examples/case3.tex}
\input{chapters/bpo/sections/rules/rule3.tex}

\eat{
Converting control dependencies to data dependencies is also required when
checking if an operation is {\em batchable}. For instance, statement s2 in
the code fragment of \reffig{fig:case3b} is not batchable due to the
flow-dependency cycle that results after converting the control dependency
of s2 on s0 into a data dependency.  Intuitively, an operation cannot be
batched if the $i^{th}$ execution of the operation depends in some way on
the value it returned in a previous execution.

\begin{figure}[t]
\begin{center}
\begin{minipage}{0.8\textwidth}
{\small
\ordinalg{
s0: \> while(x $<$ n) loop \\
s1: \>     \> y $=$ y $-$ 1; \\
s2: \> \> {\bf x $=$ q(y);} $\longrightarrow$ Not batchable \\
\> end loop; 
}
}
\end{minipage}
\end{center}
\caption{Cyclic Flow-Dependencies Due to Control-Dependency}
\label{fig:case3b}
\end{figure}
}


\subsection{Reordering Statements (Rule 5)}
\label{subsec:rule5}
\input{chapters/bpo/examples/example-revdep.tex}
Consider the example in \reffig{fig:example-revdep}. Suppose we want to batch
the query invocation {\bf q(category)} in statement s1.  We cannot directly
split the loop so as to batch s1 because there are loop-carried
flow-dependencies from s3 to s1 and to the loop predicate, which
violate pre-condition (a) of Rule 2.  Statement s3, which appears after s1,
writes a value and statement s1 reads it in a subsequent iteration.  We
therefore reverse the order of statements s1 and s3 before splitting the
loop (\reffig{fig:example-revdep}). Intuitively, we first collect all the
categories in the hierarchy and then perform a batched invocation of the
query that computes the item counts for the categories. The basic rules that
allow us to reorder statements are specified in Rule 5. To be able to split
a loop so as to batch the desired statement, multiple applications of Rule 5
may be needed. It is important that Rule 5 be applied in a carefully chosen
sequence so as to achieve the desired reordering.  We will return to this
issue in \refsec{reorder}, where we give an algorithm to reorder statements
such that the pre-conditions for Rule 2 are met.

\input{chapters/bpo/sections/rules/rule5.tex}

\eat{
Reversing the order of statements can be non-trivial as shown in the example
of \reffig{fig:example-revdep-complex}.  \reffig{fig:ddg-complex-ord-rev}
shows the backward flow dependencies before and after the order reversal.
\input{chapters/bpo/examples/example-revdep-complex.tex}

\begin{figure}[t]
\centerline{\psfig{file=chapters/bpo/fig/complex-ord-rev.eps}}
\caption{Back Edges Before and After Order Reversal for the Example of \reffig{fig:example-revdep-complex}}
\label{fig:ddg-complex-ord-rev}
\end{figure}

\noindent The intuition behind this claim is illustrated with the examples
in Figures \ref{fig:swap-ex1}, \ref{fig:swap-ex2} and
\ref{fig:swap-ex2-ddg}.

\input{chapters/bpo/examples/swap-example1.tex}
\input{chapters/bpo/examples/swap-example2.tex}

\begin{figure}[t]
\centerline{\psfig{file=chapters/bpo/fig/ord-rev.eps}}
\caption{DDG Changes for the Example in \reffig{fig:swap-ex2}}
\label{fig:swap-ex2-ddg}
\end{figure}
}


\subsection{Batching Across Nested Loops (Rule 6)}
\label{subsec:rule6}
Loops in a program may be nested within other loops and form a hierarchy.
The query or update operation we are interested in batching may lie anywhere
in the loop hierarchy. It is often desirable to batch the query or update
operation {\em w.r.t.} as many ancestor loops as possible. The aim here is
to make fewest possible calls to the expensive operation, in other words, to
make the size of the batch in each invocation as large as possible. 

Consider a loop $L_c$ nested under loop $L_p$ and a query $q$ inside $L_c$.
When the child loop ($L_c$) is split using Rule 2, a TABLE valued local
variable, $L_c$-table, is introduced in the parent loop ($L_p$).
With the application of Rule 1, $q$ is pulled out of $L_c$ and is replaced
by $qb$ that lies directly inside $L_p$. In turn, when the parent loop is
split, the $L_c$-table (of the child loop) becomes a TABLE valued
attribute (nested table) in the parent's $L_p$-table. We now
perform a second level batching of $qb$ {\em w.r.t.} $L_p$ by unnesting the
$L_p$-table.  Rule~6 enables this transformation.
Intuitively, we first try to pull the statement out of the inner most loop
enclosing it and then out of the next (higher) level loops. 
\reffig{fig:final-udf2} in Appendix~\ref{step-by-step-trans} gives
a complete example of batching a statement across nested loops.

In {\rm Rule 6} we make use of the {\em nest}($\nu$) and {\em unnest}($\mu$)
operators of nested relational algebra~\cite{COLBY89,BINCAO05}.  Below we give
a brief description of these operators and refer to~\cite{COLBY89} for the
formal definitions. 

\noindent {\bf Nest}: The {\em nest} operator ($\nu_{S \rightarrow s}(r)$)
groups the tuples of $r$ on attributes {\em schema(r)} $-$ $S$, then for
each group forms a single tuple with a relation valued attribute $s$
containing the $S$ values of the tuples grouped together.  \\

\noindent {\bf Unnest}: The {\em unnest} operator ($\mu_{s}(r)$), where $s$
is a relation valued attribute of $r$, performs the inverse operation of
{\em nest}. \\ $\mu_{s}(r)=\bigcup_{t \in r}(\Pi_{R} \{t\} \times t.s)$,
where $R$ is the set of all attributes in {\em schema(r)} excluding $s$.

\noindent 
Though we use a nested relational model for the $L$-tables, our
techniques are easy to implement on any RDBMS by storing the nested tables
separately.

\input{chapters/bpo/sections/rules/rule6.tex}

\eat{
Note that assignments to tuples of the parent iteration need to be converted
to UPDATE statements because when the loops are combined each parent tuple
would get duplicated as many times as there are tuples in the child
iteration.  So when a parent tuple is updated all the copies must be
updated. Finally, we project the combined iteration table on the attributes
of the outer iteration table and assign it back to the outer iteration
table.  \reffig{fig:example-dataflow} in \refsec{sec:discuss:chap:bpo} shows a
detailed example of how the loop combining transformation works.
}

\subsection{Correctness of Transformation Rules}
We give here a brief description of our approach for proving the correctness
of the program transformation rules. Appendix~\ref{appendix3} gives 
formal proofs of correctness.

Let $P_L$ be a program fragment that matches the {\small LHS} of a rule and
$P_R$ be the program fragment instantiated by the corresponding {\small
RHS}.  Let $p$ be the program position at which $P_L$ begins. Let $(G,S)$ be
the pair of {\em any} valid program and system states at $p$. The program
state $G$ comprises of values for all variables accessible at the program
position $p$ and the system state $S$ comprises of the state of all external
resources like database and file system. To prove the correctness of a
transformation rule, we must show the following. If the execution of $P_L$
on $(G,S)$ results in the state $(G', S')$ then the execution of $P_R$ on
$(G, S)$ will also result in the state $(G', S')$. Note that we assume
intermediate program and system states are not observable. This is a valid
assumption in many practical applications.  The correctness of many rules
directly follows from the definition of {\em batch-safe} operation and that
of {\em batched forms}.  In some cases, we need to show the multiset
equivalence of the $L$-tables, which is being updated, at the
end of the execution of $P_L$ and $P_R$.  The proof of correctness of {\em
Rule 2} uses an argument on the values seen by each statement in the
$i^{th}$ iteration $(1 \leq i \leq n$), where $n$ is the number of loop
iterations.
%\input{condition.tex}
%\input{completeness.tex}


==> chapters/bpo/sections/sec_summary.tex <==
\section{Summary}
\label{sec:summary:chap:bpo}
In this chapter we considered parameter batching as a means to improve
performance of iteratively invoked database procedures and user-defined
functions. We presented a technique, based on program analysis and
transformation, to automate the generation of batched forms of procedures
and to replace calls to stored procedures within imperative program loops
with a call to the batched form.  Our implementation and performance study
show the practicality and usefulness of the the proposed techniques. 

Procedural extensions to SQL offer new challenges and opportunities for
query optimization.  To deal with these challenges query optimization must
be augmented with program analysis and transformation techniques.  Our work
is a step towards combining query optimization with program analysis and
transformation techniques; we believe this combination will give significant
benefits for database applications.


==> chapters/bpo/sections/theorem.tex <==
\subsection*{Condition for Batching}
In this sub-section, we state and prove the condition under which procedure
{\em reorder} can reorder the statements in a loop such that a given
statement $s_q$ can be batched. Before presenting the theorem and its proof,
we introduce some useful terms and prove a supporting lemma.

Let $b$ be the basic block of statements containing $s_q$, the statement to be
batched.  Let $C$ be the set of {\small LCFD} edges that cross the split
boundaries of $s_q$ in the given basic block $b$. Let $T$ be the set of
{\small LCFD} edges $(v_1, v_2)$ such that both $v_1$ and $v_2$ succeed $s_q$
in $b$.  For example, in \reffig{fig:proof-ct-sets}, $C = \{(s_2, s_1),
(s_3, s_q)\}$ and $T = \{(s_3, s_2)\}$. 

\begin{figure}[ht]
\begin{center}
\includegraphics[width=2.5in,height=1.7in]{chapters/bpo/fig/proof-CT-sets.eps}
\caption{Example of Dependence Edges in the $C$ and $T$ Sets}
\label{fig:proof-ct-sets}
\end{center}
\end{figure}

\noindent We now state and prove a lemma, which characterizes
the behavior of procedure {\em moveAfter}.
\begin{lemma}
\label{lemma:move-cond}
Each call to procedure moveAfter(s, t), made from procedure reorder,
satisfies the following pre-conditions and post-conditions.

\noindent {\bf Pre-conditions for procedure moveAfter(s, t)} 
    \begin{enumerate}[(R.1)]
    \addtolength{\itemsep}{-3mm}
        \item t = targetStmt (the original target statement assigned in
                  procedure reorder)
        \item No true-dependence path from $s$ to $t$ exists.
        \item No statement between $s$ and $t$ has a true-dependence path
              from $s$.
    \end{enumerate}

\noindent {\bf Post-conditions for procedure moveAfter(s, t)} 
    \begin{enumerate}[(T.1)]
    \addtolength{\itemsep}{-3mm}
        \item $|srcDeps|$ decreases by at least 1 if s was in srcDeps.
        \item $|C|+|T|$ does not increase when $s \neq stmtToMove$, and  
              $|C|+|T|$ decreases by at least 1 when $s=stmtToMove$ 
              (here, stmtToMove is the original statement to be 
               moved past the targetStmt, and is assigned in procedure 
               reorder)
        \item Program correctness is preserved.
        \item The procedure terminates, and $s$ is moved past $t$.
    \end{enumerate}
\end{lemma}

\input{chapters/bpo/sections/proof_prepost_cond.tex}

%\newpage
\noindent We now state and prove our main theorem.
% Main theorem
\begin{theorem}
\label{lemma:revorder}
Given a basic block of code $b$ and statement $s_q$ in $b$ such that 
$s_q$ does not lie on a true-dependence cycle in the DDG, procedure
reorder terminates, reordering the statements of $b$ such that:
    \begin{enumerate}[(a)]
        \addtolength{\itemsep}{-3mm}
        \item No LCFD edges cross the program points that immediately 
              precede and succeed $s_q$.
        \item Program correctness is preserved ({\em i.e.}, the reordered 
              block is equivalent to the original)
    \end{enumerate}
\end{theorem}

\begin{proof}
First, we prove that procedure {\em reorder} terminates. 

\begin{enumerate}
\item %The inner {\em while} loop of procedure {\em reorder} terminates: 
      The inner {\em while} loop of procedure {\em reorder} executes until
      the set {\em srcDeps} is empty. In each iteration, a call to procedure
      {\em moveAfter} is made, with an element of {\em srcDeps} being passed
      as the parameter $s$. From the post-condition {\em (T.1)} of 
      Lemma~\ref{lemma:move-cond}
      we know that, after each call to {\em moveAfter}, the
      size of {\em srcDeps} decreases by at least 1.  Hence, the inner {\em
      while} loop of procedure {\em reorder} must terminate.

\item %The outer {\em while} loop of procedure {\em reorder} terminates: 
      The outer {\em while} loop of procedure {\em reorder} executes until
      $|C|=0$.  In each iteration of the outer {\em while} loop, the last
      call to procedure {\em moveAfter} is made with $s$ being set to
      $stmtToMove$. Hence, from the post-condition {\em (T.2)} of
      Lemma~\ref{lemma:move-cond} we know that $|C|+|T|$ decreases by at
      least 1 at the end of each iteration of the outer {\em while} loop.
      None of the other calls to the procedure {\em moveAfter} cause any
      increase in $|C|+|T|$ (follows from the post-condition {\em (T.2)} of
      Lemma~\ref{lemma:move-cond}). Hence, the outer {\em while} of
      procedure {\em reorder} must terminate.

\item Each call to procedure {\em moveAfter}, made from procedure
      {\em reorder}, terminates (post-condition {\em (T.4)} in 
      Lemma~\ref{lemma:move-cond}).
\end{enumerate}

\noindent
\noindent From 1, 2 and 3 above, it is straight-forward to observe
that procedure {\em reorder} terminates.

Any reordering of statements within the basic block $b$ are performed
by procedure {\em moveAfter} and not directly by procedure {\em reorder}.
Hence, the post-condition {\em (T.3)} of Lemma~\ref{lemma:move-cond}
suffices to prove that procedure {\em reorder} preserves program
correctness.

When procedure {\em reorder} terminates, no LCFD edges cross the 
program points that immediately precede and succeed $s_q$. This 
directly follows from the termination condition, $|C|=0$, of the 
outer {\em while} loop of procedure reorder.

\noindent
This completes the proof of Theorem~\ref{lemma:revorder}
\end{proof}


==> chapters/concl/chap_concl.tex <==
\chapter{Conclusions and Future Work}
\label{chap:concl}
In this thesis we looked at ways to speed up iterative execution of queries,
user-defined functions and stored procedures.  Iterative execution can
happen either because known decorrelation techniques do not apply, for
instance when the nested block is a complex procedure, or because an
iterative plan has the least expected cost amongst the alternatives
available to the query optimizer. We took a two pronged approach to address
the problem. First, we looked at exploiting ordered parameter bindings to
speed up iterative plans and presented extensions to a cost-based optimizer for
choosing efficient sort orders. Next, we showed how to achieve set-oriented
execution of queries and updates within complex procedures through parameter
batching enabled by program rewrite.

In \refchap{chap:nqo} we showed how state retention of operators allows us
to exploit sorted parameter bindings to improve the efficiency of iterative
query plans. We then showed how a Volcano style cost-based query optimizer
can be extended to take into account state retention and effects of sorted
parameter bindings. An important problem, which arises in optimizing both
nested queries as well as queries containing joins, grouping and other set
operations is that of deciding the optimal sort order of parameters and
inputs. We addressed this problem in \refchap{chap:eio}. We showed that even
a simplified version of the problem of choosing optimal sort orders is {\em
NP-Hard} and gave principled heuristics, which take into account partially
available sort orders and attributes common to multiple join predicates. We
presented experimental results, carried out by forcing plans generated by
our optimizer extensions on widely used database systems. The results showed
significant improvements in actual query execution time due to the proposed
techniques when compared to the default plans chosen by the respective
systems.
Although it is difficult to quantify the percentage of real-world queries that
can benefit from the proposed techniques, our experiments carried on queries
taken from the TPC-H benchmark and a financial application, and our experience
with ETL tasks in data warehousing indicate that a significant number of
queries can benefit from the proposed techniques.

In \refchap{chap:bpo} we considered iterative execution involving complex
user-defined functions and stored procedures, which use a mix of procedural
constructs and {\small SQL}. We proposed a program analysis and
transformation based approach to enable set-oriented execution of queries
and updates inside such procedures. The approach consists of a set of
program transformation rules, which are used to {\em (i)} automatically generate
the batched form of a given procedure and {\em (ii)} replace iterative calls to
the procedure with code to construct a parameter batch and invoke the
batched form. Our program transformation rules can deal with a rich set of
language constructs such as looping, conditional control transfer and
assignments. With the help of our implementation of the rewrite rules for a
subset of Java, we carried out an experimental study on cases chosen from
three real-world applications. The results are very promising, and show
up to 75\% improvement in the actual execution time.

With increasing use of procedural extensions to {\small SQL} and emergence
of language integrated querying paradigms ({\em e.g.,} Microsoft
LINQ~\cite{LINQ}), combined optimization of application code and database
queries/updates becomes more and more important for improving the
application performance.  Our work is a step towards this goal. 

The proposed program rewrite techniques are useful in two broad scenarios:
(a) to transform programmer written loops with database access into
potentially more efficient code and (b) to automatically generate batch
processing routines from routines that were developed for one at a time
request processing.  There is a large body of code in languages like 
{\small PL/SQL}
and Java, in the former category. For our experiments we considered two
such examples (Experiment 1 and 3 in \refchap{chap:bpo}) from real-world
applications\footnote{Due to confidentiality reasons we cannot name the
applications and organizations.}.  Although it is hard to quantify the number
of cases which have the second requirement, we have come across two cases in
which many stored procedures were required to be rewritten for batch
processing.  One such example is considered in Experiment 2 of Chapter 4. 
%We did not have access to additional procedures and the data.

\eat{
Whether batching a specific query invocation yields significant benefits
depends on the number of iterations, data characteristics and the physical
design of the database. The decision on whether to batch a query invocation
must therefore be made in a cost-based manner. The scope of program rewrite
techniques presented in this thesis is to present a set of equivalence rules
and characterize the query invocations that can be batched. Cost-based
optimization is a future work.
}
Whether batching a specific query invocation yields significant benefits
depends on the number of iterations, data characteristics and the physical
design of the database. Applying the program transformation rules presented 
in this thesis in a cost-based manner is a future work.

%---------------------------------------------------
\subsection*{Future Work}

There are several interesting challenges ahead to fully realize the goal of
optimizing iterative invocation of complex procedural blocks and iterative
invocation of queries/updates from application code. We briefly discuss
some directions for future work.

\subsubsection*{Sort Orders from Secondary Indices}
In \refchap{chap:eio}, while computing the set of approximate favorable orders
on base relations, we consider only the clustering index and secondary
indices that cover the given query. Although it is possible to use non query
covering secondary indices to get ordered tuples (by traversing the index
leaf pages), it is usually very inefficient due to random IO. However, if
the actual tuple fetch can be deferred until a point where the extra
attributes are needed in the query plan, it is possible that the approach
can perform better.  If a highly selective filter discards many rows before
the extra attributes are needed, only a few tuple fetches happen.
Evaluating such alternatives in a cost-based manner is an interesting future
work.

\subsubsection*{Cost-Based Choice of Queries to Batch}
Our current implementation requires manual input on which operations to
consider for batching. An interesting and important problem is to make a
cost-based decision on which queries/updates to batch. The important
parameters on which this decision depends include {\em (i)} cost model for
the operation as a function of batch size, {\em (ii)} expected number of
iterations of the program loop {\em (iii)} branch probabilities for the
branching statements {\em (if-then-else)} in the program and {\em (iv)}
overheads of the transformed code. 

%Automating the choice of operations to batch is an interesting future work.

\subsubsection*{Pipelined Execution of Queries Inside a UDF}
The $L$-tables, discussed in \refsec{sec:rules:chap:bpo}, serve to hold the
parameter batch with which the batched form of a procedure is invoked.
Though small batches can be held in memory, in general we may need to
materialize the batches and the cost of materialization must be taken into
account while deciding to batch an operation. However, for procedures that
run entirely inside the database engine ({\em e.g.,} UDFs) it may be
possible to avoid materialization of batches by constructing a single
dataflow containing both relational and procedural nodes. Our loop
splitting transformation is designed to facilitate such an approach.
Appendix~\ref{appen:extra-rules} contains a few additional rules that 
can be used
for {\em (i)} avoiding creation of intermediate batches by passing a relational
expression, instead of a table, to the batched forms and {\em (ii)} mapping
program statements that perform simple and inexpensive operations ({\em
e.g.,} expression evaluation and variable assignment) to operators that work
on sets. The later of these helps in eliminating loops such as the one left
over in \refex{ex:udf-co-batched}.  When a single dataflow is thus built,
code that cannot be mapped to relational operators is executed by procedural
nodes in the dataflow.  Variable bindings inside such nodes are obtained
from input tuples.  
%Depending on the specific code, each procedural node may be blocking or
%non-blocking.  The $L$-tables become streams in the pipeline.  operators.

\eat{
\subsubsection*{Avoiding the Batch Materialization for Queries with UDFs}
For queries that invoke UDFs it may be possible to avoid materialization of
batches by constructing a single dataflow. Consider the sample code and its
translation shown in \reffig{fig:example-dataflow}. For the translated
program a single dataflow can be constructed as shown in
\reffig{fig:dataflow}. To enable such an approach the query execution engine
must support procedural operator nodes as part of the query evaluation plan.
The procedural operator nodes, shown with label {\em P} in
\reffig{fig:dataflow}, can execute a specified code over the input tuples.
Depending on the specific code, a procedural node can be blocking or
non-blocking.
}

\subsubsection*{Set-Oriented Evaluation in the Presence of 
                Cyclic Flow-Dependencies}
The program transformation rules presented in \refchap{chap:bpo} and the
rule application algorithm guarantee that a query execution statement $s$
can be batched {\em w.r.t.} a loop if $s$ does not lie on a true-dependence
cycle in the DDG (Theorem \ref{lemma:revorder}). Intuitively, the only
statements we fail to batch are the statements whose execution in an
iteration of the loop depends on the result of their own execution in 
a previous iteration. In such cases, the set of parameters for a query
execution statement cannot be computed up front (without invoking the 
query itself). 

However, in certain cases, it may be possible to identify a superset of the
parameter batch even if the query execution statement lies on a
true-dependence cycle.  For example, consider the iterative execution of a
scalar aggregate query with a parameterized equality predicate in its {\em
where} clause. An example of such a query would be: {\small SELECT}
sum(balance) {\small FROM} account {\small WHERE} branch=:branch.  If a
true-dependence cycle makes it impossible to compute the exact set of
parameters (in this example, {\em branches}) for the query, one can compute
the query results for all the possible parameters by using a vector
aggregate query, which for our example would be: {\small SELECT}
sum(balance) {\small FROM} account {\small GROUP BY} branch.  Note that such
an approach can be used only for pure functions and not for operations with
side-effects (even if the operation is batch-safe).

\eat{
\subsubsection*{Avoiding the Overheads of Loop Split}
Loop splitting can be expensive when there are a large number of variables
that are written in one partition of the loop and read in the other. Each
such variable becomes an attribute in the $L$-table and we store as
many values as there are iterations of the loop. In certain cases, it may be
possible to avoid loop splitting altogether and still use batching.  The
approach involves executing the loop twice. In the first execution, all the
side-effect causing operations are removed from the body of the loop and the
queries to batch are replaced with statements that collect the parameter
values and build a batch. Once the batch is ready, we invoke the batched
form of the query and store the results. We then execute the loop a second
time where the query execution statements are replaced by statements that
look up the stored result of the batched query execution. Such an approach
is feasible when the query invocations to be batched do not have a
dependency on other such query invocations and also on any side-effect
causing operation. Such an alternative must be considered by the optimizer
while making a cost-based decision.
}



==> chapters/eio/chap_eio.tex <==
%\chapter{Optimization with Interesting Orders}
\chapter{Sort Order Selection}
\label{chap:eio}
The previous chapter showed the use of sort orders (of sub-query parameters)
in improving the efficiency of iterative execution plans. Sort orders, in
general, play an important role in query evaluation.  Algorithms that rely
on sorted inputs are widely used to implement joins, grouping, duplicate
elimination and other set operations.  The notion of {\em interesting
orders}~\cite{SEL79} has allowed query optimizers to consider plans that
could be locally sub-optimal, but produce ordered output beneficial for
other operators, and thus produce a globally optimal plan.  However, the
number of interesting orders for most operators is factorial in the number
of attributes involved. For example, all possible sort orders on the set of
join attributes are of interest to a merge join. Considering the
exhaustive set of interesting orders is prohibitively expensive as the input
sub-expressions must be optimized for each interesting sort order and the
corresponding plan must be memoized. 

Deciding a practical set of interesting sort orders is a crucial step in
query optimization. The variation in plan cost due to the choice of
different sort orders could be very high. A plan with carefully chosen sort
orders, which exploit clustering/covering indices and commonalities between
order requirements of multiple operators, can perform significantly better
than a plan with na\"ively chosen orders, due to the reduction in sorting
cost. Sorting cost in a plan can also be reduced by exploiting partially
available sort orders. For example, a primary index on a subset of
attributes involved in the join predicate partially fulfills the sort order
requirement of merge-join, and can greatly reduce the cost of the
intermediate sorting stage. The optimizer must therefore consider partial
sort orders while choosing interesting orders.  Sorting based algorithms for
binary operators such as join and union, although agnostic to the exact sort
order of their inputs, require a matching order from the two inputs. These
factors make the problem of choosing sort non-trivial. 

In this chapter we address the problem of choosing interesting sort orders.
We use join expressions for our description. However, the solution can be
used for choosing input sort orders for any sorting based operator as well
as for choosing sort orders on sub-query/{\small UDF} parameters. 

The rest of this chapter is organized as follows.  \refsec{sec:pso:chap:eio}
describes how partial sort orders can be exploited during sorting and
proposes extensions to a cost-based optimizer to account for their benefits
during plan generation. In \refsec{sec:nphard:chap:eio} we show that a
special case of the problem of selecting globally optimal sort orders is
NP-hard and give a 1/2-benefit approximation algorithm to handle the case. Although
the problem is intractable, the knowledge of available indices and sort
order propagation properties of physical operators allows us to provide a
good heuristic approach, which we describe in \refsec{sec:favord:chap:eio}.
\refsec{sec:favord-to-pso:chap:eio} shows how the solution can be used to
obtain interesting parameter sort orders for nested sub-expressions.  We
present our experimental results in \refsec{sec:perf:chap:eio}.  We discuss
related work in \refsec{sec:relwork:chap:eio} and summarize the work in
\refsec{sec:summary:chap:eio}.

\input{chapters/eio/sections/sec_pso.tex}
\input{chapters/eio/sections/sec_nphard.tex}
\input{chapters/eio/sections/sec_favord.tex}
\input{chapters/eio/sections/sec_favord_to_pso.tex}
\input{chapters/eio/sections/sec_perf.tex}
\input{chapters/eio/sections/sec_relwork.tex}
\input{chapters/eio/sections/sec_summary.tex}
%\input{chapters/eio/ack.tex}


==> chapters/eio/sections/pathalgo.tex <==
\begin{figure*}[ht]
\begin{minipage}{1.0\textwidth}
%\algsize{
\ordinalg{
\large{Procedure PathOrder} \\
{\bf Input:} 
s[n]  : array of attribute sets \\
{\bf Output:} 
p[n]  : array of permutations or sort orders \\
{\bf Data Structures:} \\
\>  benefit[n][n], split[n][n] : arrays of integers \\
\>  commons[n][n] : array of attribute sets \\
%\>  split[n][n]   : array of integers \\
\>  apermute(s)   : Function that returns an arbitrary permutation of attribute set s \\
BEGIN \\
\>    for i=1 to n \\
%\>    for i=1; i$\leq$n; i++) $\{$ \\
\>\>        benefit[i][i] = 0; p[i] = $\epsilon$; commons[i][i] = s[i]; split[i][i] = -1; \\
%\>\>        commons[i][i] = s[i]; \\
%\>\>        split[i][i]   = -1; \\

\>   for j=1 to n-1  \>\>\>\>\>\>\>\> // Consider path segments of length j \\
%\>   for (j=1; j $\leq$ n-1; j++) $\{$ \\
\>\>        for i = 1 to n-j  \>\>\>\>\>\>\> // Consider path segment (i, i+j) \\
%\>\>        for (i = 1; i $\leq$ n-j; i++) $\{$ \\
\>\>\>            Let k be the index such that i $\leq$ k $<$ (i+j) and 
                  benefit[i][k]+benefit[k+1][i+j] \\ 
\>\>\>            is maximum \\
\>\>\>            commons[i][i+j] = commons[i][k] $\cap$ commons[k+1][i+j]; \\
\>\>\>            benefit[i][i+j] = benefit[i][k] + benefit[k+1][i+j] + 
                                    $f(|$commons[i][i+j]$|)$; \\
\>\>\>            split[i][i+j] = k; \\
%\>\>        $\}$ \\
%\>    $\}$ \\
\\
\>    Call MakePermutation(1, n); \>\>\>\>\>\>\>\>// Form the attribute permutations \\
END PROC  \\
 \\
\noindent
// Procedure to construct attribute permutations from the memo structure, 
   in which \\
// the optimal split point and common attributes are remembered. \\
\large{Procedure MakePermutation(i, j)} \\
BEGIN \\
\>    Let ca = commons[i][j];  // Attributes common to all the vertices from i to j \\
\>    Let cp = apermute(ca);   // An arbitrarily chosen permutation of ca. \\
\>    for k=i to j \\
\>\>        Append cp to p[k]; \\
\>   if (i = j) \\
\>\>        return; \\
\>    // Remove the common attributes from all subpaths of (i,j), so that the \\
\>    // attributes do not repeat. \\
\>    For all i', j' s.t. $i' \geq i$ and $j' \leq j$  \\
\>\>      commons[i'][j'] = commons[i'][j'] $-$ ca; \\
\>    // Construct the permutations of remaining attributes for the two subpaths, \\
\>    // to the left and right of the the split point. \\
\>    m = split[i][j]; \\
\>    MakePermutation(i, m); \\
\>    MakePermutation(m+1, j); \\
%\>   $\}$ \\
%$\}$\\
END PROC  \\
}
%}
\end{minipage}
\caption{Optimal Benefit Sort Orders for a Path}
\label{fig:pathalgo}
\end{figure*}


==> chapters/eio/sections/sec_favord.tex <==
\section {Optimization with Favorable Orders}
\label{sec:favord:chap:eio}
The benefit model we presented in the previous section, does not take into
account factors such as the physical sort order of a relation, available
indices and size of base relations and intermediate results.  Moreover, we
assumed that the join order is fixed.  In this section, we present a two
phase approach to address the more general problem.  In phase-1, which occurs
during plan generation, we use the information about available indices and
properties of physical operators to efficiently compute a small set of
promising sort orders to try. We formalize this idea through the notion of
{\em favorable orders}.  Phase-2, is a plan refinement step and occurs after
the optimizer makes its choice of the best plan. In phase-2, the sort orders
chosen by the optimizer are refined further to reap extra benefit from the
attributes common to multiple joins.  Phase-2 uses the 1/2 benefit 
approximation algorithm of \refsec{subsec:approxalgo}

\subsection {Favorable Orders}
\label{subsec:favord}
Given an expression $e$, we expect some sort orders (on the result of $e$)
to be producible at much lesser cost than other sort orders.  Available
indices, indexed materialized views, specific rewriting of the expression
and choice of physical operators determine what sort orders are easy to
produce. To account for such orders, we introduce the notion of {\em
favorable} orders. In the discussion that follows, we use the following 
notations:

%\vspace{-5pt}
\begin{itemize}
\onlythesis{\addtolength{\itemsep}{-3mm}}
%{\small
\item {\em cbp}$(e, o)$ : Cost of the best plan for expression $e$
      with $o$ being the required output sort order
\item $o_R$ : The clustering order of relation $R$ 
\item {\em idx}$(R)$ :  Set of all indices over $R$
\item $o(I)$ : Order (key) of the index $I$ 
\item $\langle s \rangle$ : An arbitrarily chosen permutation of set $s$
\item $P(s)$  : Set of all permutations of set $s$ 
%\item $o \wedge s$ : Longest prefix of $o$ such that each attribute
%      in the prefix belongs to the attribute set $s$ 
\item {\em schema}$(e)$ : The set of attributes in the output of $e$
%}
\end{itemize}

\noindent We first define the {\bf {\em benefit}} of a sort order $o$ {\em
w.r.t.} an expression $e$ as follows:

\vspace{0.1in}
{\em benefit}$(o, e) = cbp(e, \epsilon)+coe(e, \epsilon, o)-cbp(e, o)$ 

\noindent Intuitively, a positive benefit implies the sort order can be
obtained with lesser cost than a full sort of unordered result. For
instance, the clustering order of a relation $r$ will have a positive {\em
benefit} for the expression $\sigma_{p}(r)$.  Similarly, query covering
secondary indices and indexed materialized views can yield orders with
positive benefit.  We call the set of all orders, on $schema(e)$, having a
positive benefit {\em w.r.t.} $e$ as the {\em favorable order set} of $e$
and denoted it as {\em ford(e)}. 

\vspace{0.1in}
{\em ford(e)}$=\{$ {\em o: benefit(o, e)}$>0\ \}$ 

\subsubsection{Minimal Favorable Orders}
The number of favorable orders for an expression can be very large.  For
instance, every sort order having the clustering order as its prefix is a
favorable order. We call a sort order $o \in$ {\em ford(e)} as a 
{\em minimal favorable order} if the following two conditions hold.
\begin{enumerate}
\onlythesis{\addtolength{\itemsep}{-2mm}}
    \item $\not \exists$ $o'$ $\in$ {\em ford(e)} such that $o' \leq o$ and
          {\em cbp}$(e, o')$ $+$ {\em coe}$(e, o', o)$ $=$ {\em cbp}$(e, o)$.
          Intuitively, sort order $o$ is minimal only if there does not
          exists a sort order $o'$ such that the cost of obtaining order $o$
          equals the cost of obtaining sort order $o'$ followed by an
          explicit sort to obtain order $o$.
    \item $\not \exists$ $o''$ $\in$ {\em ford(e)} such that $o \leq o''$
          and {\em cbp}$(e, o'') =$ {\em cbp}$(e, o)$. Intuitively, sort
          order $o$ is minimal only if there does not exists a sort order
          $o''$ subsuming order $o$ and available at the same cost as $o$.
\end{enumerate}

We call the set of all minimal favorable orders of an expression $e$ as the
{\em minimal favorable order set} of $e$ and denote it by {\em ford-min(e)}.
Conditions 1 and 2 above, ensure that when a relation has an index that
provides sort order $o$ efficiently, orders that are prefixes of $o$ and
orders that have $o$ as their prefix are not minimal favorable orders.

\noindent We define favorable orders of an expression {\em w.r.t.} a set of
attributes $s$ as: {\em ford(e, s)}$=\{o \wedge s$: $o\in$ {\em
ford(e)}$\}$.  Intuitively, {\em ford(e, s)} is the set of orders on $s$ or
a subset of $s$ that can be obtained efficiently.  Similarly, the {\em
ford-min} of an expression {\em w.r.t.} a set of attributes $s$ is defined
as: {\em ford-min(e, s)}$=\{o \wedge s$ : $o\in$ {\em ford-min(e)}$\}$ 


\subsubsection{Heuristics for Favorable Orders}
\label{subsec:compfavord}
Note that the definition of favorable orders uses the cost of the best plan
for the expression. However, we need to compute the favorable orders of an
expression {\bf before} the expression is optimized and without requiring to
expand the physical plan space. Further, the size of the
exact {\em ford-min} of an expression can be prohibitively large in the
worst case.  In this section, we describe a method of computing approximate
{\em ford-min}, denoted as  {\em afm}, for {\em SPJG} expressions.  We
compute the {\em afm} of an expression bottom-up. For any expression {\em
e}, {\em afm(e)} is computable after the {\em afm}  is computed for all of
{\em e}'s inputs.

\begin{enumerate}
%\addtolength{\itemsep}{-1mm}
\item $e=R$, where $R$ is a base relation or materialized view.  We include
      the clustering order of $R$ and all secondary index orders such that 
      the index covers the query. \\
      {\em afm}$(R)=\{o: o=o_R$ or $o=o(I), I \in idx(R)$ and $I$ covers 
      the query$\}$

\item $e=\sigma_{p}(e_1)$, where $e_1$ is an arbitrary expression. \\
      {\em afm}$(e)=\{o: o \in $ {\em afm($e_1$)} $\}$

\item $e=\Pi_{L}(e_1)$, where $e_1$ is any expression. We include longest 
      prefixes of input favorable orders such that the prefix has only the 
      projected attributes. \\
     {\em afm}$(e)=\{o: \exists o'\in$ {\em afm($e_1$)} and $o=o'\wedge L\}$

\item $e=e_1 \Join e_2$ with join attribute set $S=\{a_1, a_2, \ldots, a_n\}$. 
      Noting that nested loops joins propagate the sort order of one of the 
      inputs (outer) and merge join propagates the sort order chosen for join 
      attributes, we compute the {\em afm} as follows: first, we include all 
      sort orders in the input {\em afms}, next, we consider the longest 
      prefix of each input favorable order having attributes only from the 
      join attribute set and extend it to include an arbitrary permutation 
      of the remaining join attributes.  \\
      Let $\mathcal{T}=${\em afm}$(e_1)\ \cup$ {\em afm}$(e_2)$ \\
      Then,
      {\em afm}$(e_1 \Join e_2)=\mathcal{T}\cup\ \{o:o' \in 
      \mathcal{T}\cup\{\epsilon\}\ and\ o=o' \wedge S\ + 
      \ \langle S-${\em attrs}$(o'\wedge S)\rangle \}$ 

      Note that, for the join attributes not involved in an input favorable
      order prefix ({\em i.e.,} $S-${\em attrs}$(o' \wedge S)$), we take an
      arbitrary permutation. An exact {\em ford-min} would require us to
      include all permutations of such attributes.  In the post-optimization
      phase, we refine the choice made here using the benefit model and
      algorithm of \refsec{subsec:approxalgo}.

\item $e=_{L}\mathcal{G}_{F}(e_1)$ \\
{\em afm}$(e)=$ 
      $\{o:o' \in $ {\em afm($e_1$)}$\cup \{\epsilon\}$ {\em and } 
      $o=o' \wedge L\ + \ \langle L-${\em attrs}$(o'\wedge L)\rangle \}$\\
      Intuitively, for each input favorable order we identify the longest
      prefix with attributes from the projected group-by columns and extend
      the prefix with an arbitrary permutation of the remaining attributes.
\end{enumerate}
\eat{
Computing {\em afms} requires a single pass of the query tree. At each node
of the query tree the only significant operation performed is computation of
the longest common prefix {\em lcp} of an order {\em w.r.t.} a set, {\em
i.e.,} $o \wedge s$.  The number of {\em lcp} operations performed at a node
is at most the number of input favorable orders for that node. Let $m$ be
the average number of favorable orders for base relations. If the query
involves a join of $n$ relations the worst-case number of {\em lcp}
operations performed at any node is $O(2^n m)$.  Typically $m$ is very small
($\leq 2$) and hence even the worst-case number of {\em lcp} operations is
within acceptable limits. However, in most practical cases, the number of
{\em lcp} operations performed is far below the worst-case.
}

\subsection {Optimizer Extensions}
\label{subsec:optext}
We make use of the approximate favorable orders during plan generation
(phase-1) to choose a small set of promising {\em interesting orders} for
sort-based operators. We describe our approach taking merge join as an
example but the approach is applicable to other sort based operators. In
phase-2, which is a post-optimization phase, we further refine the chosen
sort orders.

\subsubsection{Plan Generation (Phase-1)}
\label{subsec:plangen}
Consider an optimization goal of expression $e=e_l \Join e_r$ and required
output sort order $o$. When we consider merge-join as a candidate algorithm,
we need to generate sub-goals for $e_l$ and $e_r$ with the required output
sort order being some permutation of the join attributes. 

Let $S$ be the set of attributes involved in the join predicate. We consider
only conjunctive and equality predicates.  We compute the set
$\mathcal{I}(e, o)$ of interesting orders as follows.  \\ 
\\

\noindent {\bf Steps to compute $\mathcal{I}(e, o)$}:
\begin{enumerate}
\item Collect the favorable orders of inputs plus the required output
      order \\ $\mathcal{T}(e, o) = ${\em afm}$(e_l, S)\ \cup\ ${\em
      afm}$(e_r, S)\ \cup\ {o \wedge S}$, where {\em afm}$(e, S)=\{o'
      \wedge S: o'\in $ {\em afm}$(e)\}$ 

\item Remove redundant orders \\ If $o_1, o_2 \in \mathcal{T}(e,o)$ and
    $o_1 \leq o_2$, remove $o_1$ from $\mathcal{T}(e,o)$ 
    
\item Compute the set $\mathcal{I}(e,o)$ by extending each order in
      $\mathcal{T}(e,o)$ to the length of $|S|$; the order of extra attributes
      can be arbitrarily chosen \\ $\mathcal{I}(e,o)=\{o : o'\in
      \mathcal{T}(e,o)\ and\ o=o'\ + \ \langle S-attrs(o')\rangle \}$
\end{enumerate}

We then generate optimization sub-goals for $e_l$ and $e_r$ with each order
$o'\in\mathcal{I}(e,o)$ as the required output order and retain the cheapest
combination.

\paragraph{An Example:}
Consider \onlythesis{\refex{query:carcatalog}}
\onlyjournal{\refquery{query:carcatalog}} of \refsec{sec:pso:chap:eio}. For
brevity, we refer to the two catalog tables as {\em ct1} and {\em ct2}, the
rating table as {\em rt}, and the columns with their starting letters.  The
{\em afms} computed as described in \refsec{subsec:compfavord} are as
follows:

\noindent
{\em afm}$(ct1)=\{(y)\}$, {\em afm}$(ct2)=\{(m)\}$, {\em afm}$(rt)=\{(m)\}$,
{\em afm}$(ct1 \Join ct2) =$ $\{(y), (m),$ $(y, co, c, m)$, $(m, co, c, y)\}$, 
{\em afm}$((ct1 \Join ct2) \Join rt)=\{(y), (m),$ $(y, co, c, m)$, 
$(m, co, c, y)$, $(y, m)$, $(m, y)\}$

For $(ct1 \Join ct2) \Join rt$ we consider two interesting sort orders
$\{(y,m), (m,y)\}$ and for $ct1 \Join ct2$ we consider four sort orders
$\{(y,co,c,m),(m,co,c,y),(y,m,co,c),$ \- $(m,y,co,c)\}$. As a result the
optimizer will consider the plan shown in \reffig{fig:optplan}.

\paragraph{A Note on Optimality:}
If the set $\mathcal{I}(e,o)$ is computed using the exact 
set of minimal favorable orders ({\em ford-min}), then it must 
contain an optimal sort order, {\em i.e.}, a sort order, which
produces the optimal merge join plan in terms of overall
plan cost. 

\begin{theorem}
\label{theorem:optorder}
The set $\mathcal{I}(e,o)$ computed with exact ford-min contains an optimal
sort order $o_p$ for the optimization goal $e=(e_l \Join e_r)$ with $(o)$ as
the required output sort order, under Assumption A.
\end{theorem}

\noindent {\em Assumption A :}
If $o_1$, $o_2$ are two sort orders on the same set of attributes 
({\em i.e.,} attrs$(o_1) =$ attrs$(o_2)$), then the {\small CPU} cost
of sorting the result of an expression {\em e} to obtain $o_1$ will
be same as that for $o_2$, {\em i.e.,} cpu-cost$(e, o_1)=$ cpu-cost$(e,
o_2)$.

\noindent 
The theorem essentially states the following: to identify an optimal sort
order, it is sufficient to consider only the minimal favorable orders and
not the full set of favorable orders.  Appendix \ref{appen:proof-opt-order}
gives the proof of Theorem~\ref{theorem:optorder}.

\subsubsection{Plan Refinement (Phase-2)}
During the plan refinement phase, for each merge-join node in the plan tree,
we identify the set of {\em free attributes}, the attributes which were not
part of any of the input favorable orders. Note that for these attributes we
had chosen an arbitrary permutation while computing the {\em afm}
(\refsec{subsec:compfavord}).  We then make use of the 1/2 benefit approximation
algorithm for trees (described in \refsec{subsec:approxalgo}) and rework the
permutations chosen for the {\em free attributes}. 

Formally, let $p_i$ be the permutation chosen for the join node $v_i$. Let
$q_i$ be the order such that $q_i \in $ {\em afm}$(v_i.${\em left-input}$)$
$\cup$ {\em afm}$(v_i.${\em right-input}$)$ and $|p_i \wedge q_i|$ is the
maximum. Intuitively, $q_i$ is the input favorable order sharing the longest
common prefix with $p_i$.  Let $f_i=${\em attrs}$(p_i - (p_i \wedge q_i))$;
$f_i$ is the set of {\em free attributes} for $v_i$. 

We now construct a binary tree, where each node $n_i$ corresponding to
join-node $v_i$ is associated with the attribute set $f_i$. The attribute
permutations for the nodes are chosen using the 1/2 benefit approximation algorithm;
the chosen sort order for free attributes is then appended to the sort order
chosen during plan generation ({\em i.e.,} $p_i \wedge q_i$) to get a
complete order.

The reworking of the sort orders will be useful only if the adjacent nodes
share the same prefix, i.e., $p_i \wedge q_i$ was the same for adjacent
nodes.  This condition however certainly holds when the inputs for joins
have no favorable orders.

\reffig{fig:postpassexample} illustrates the post-optimization phase. Assume
all relations involved ($R_1, \ldots, R_4$) are clustered on attribute $a$ and
no other favorable orders exist. {\em i.e.,} {\em afm}$(R_i)=\{(a)\}$, for
$i=1$ to $4$. The orders chosen by the plan generation phase are shown
besides the join nodes with {\em free attributes} being in {\em italics}.
The reworked orders after the post-optimization phase are shown underlined.

\begin{figure}[ht]
\onecolonly{
\centerline{\includegraphics[angle=0,width=3.5in]{chapters/eio/fig/postpassexample.eps}}
}
\twocolonly{
\centerline{\includegraphics[angle=0,width=2.8in]{chapters/eio/fig/postpassexample.eps}}
}
\caption{Post-Optimization Phase}
\label{fig:postpassexample}
\end{figure}



==> chapters/eio/sections/sec_favord_to_pso.tex <==
%\section{Computing Interesting Parameter Sort Orders}
\section{Application to Nested Queries}
\label{sec:favord-to-pso:chap:eio}
The problem of choosing interesting sort orders on sub-query parameters,
discussed in \refsec{sec:optext:chap:nqo}, is similar to the problem of
choosing sort orders on inputs. We now briefly describe how the techniques
presented in this chapter can be used to compute interesting sort orders 
on sub-query parameters.

Let $e_2$ be an expression nested below expression $e_1$ and $S$ be be the
set of parameters bound by $e_1$ that are used inside $e_2$. First, we
compute the approximate favorable orders of appropriate sub-expressions in
$e_2$ and deduce the corresponding sort order on parameters. As an example,
consider a sub-expression $\sigma_{p}(e_3)$ in $e_2$. We compute {\em
afm}$(e_3)$ and then deduce the corresponding sort orders on parameters by
mapping each attribute to the parameters it is equated to in predicate $p$.
Next, we compute the favorable orders for the outer expression {\em w.r.t.}
to the set of parameters it binds, {\em afm}$(e_1, S)$.  The final set
of interesting parameter sort orders is formed by taking the union of 
interesting parameter sort orders obtained from all the inner
sub-expressions and the favorable orders of the outer sub-expression.

Intuitively, our approach considers plans that sort the outer tuples to
match a sort order favorable to the inner expression(s), and also plans that
sort the inner relations to match a sort order favorable to the outer
expression.


==> chapters/eio/sections/sec_nphard.tex <==
\section{Choosing Sort Orders for a Join Tree}
\label{sec:nphard:chap:eio}
Consider a join expression $e = e_1 \Join e_2$, where $e_1, e_2$ are input
subexpressions and the join predicate is of the form:
$(e_{1}.a_{1}=e_{2}.a_{1}$ {\em and} $e_{1}.a_{2}=e_{2}.a_{2} \ldots $ {\em
and} $e_{1}.a_{n}=e_{2}.a_{n})$. Note that, {\em w.l.g.}, we use the same
name for attributes being compared from either side and we call the set
$\{a_1, a_2, \ldots, a_n\}$ as the join attribute set. In this case, the
merge join algorithm has potentially $n!$ interesting sort orders on inputs
$e_{1}$ and $e_{2}$\hspace*{-1mm}~\footnote{We assume merge-join requires
sorting on all attributes involved in the join predicate. We do not consider
orders on subsets of join attributes since the additional cost incurred at
merge-join matches the benefit of sorting a smaller subset of attributes.}.
The specific sort order chosen for the merge-join can have significant
influence on the plan cost due to the following reasons: $(i)$ Clustering
and covering indices, indexed materialized views and other operators in the
subexpressions $e_1, e_2$ can make one sort order much cheaper to produce
than another. $(ii)$ The merge-join produces the same order on its output as
the one selected for its inputs. Hence, a sort order that helps another
operator above the merge-join can help eliminate a sort or just have a
partial sort. In this section we show that a special case of the the problem
of choosing optimal sort orders for a tree of merge-joins is {\em NP-Hard}
and provide a 1/2 benefit approximation algorithm for the problem\exceptjournal{\footnote{The work
was carried out in collaboration with Ajit A. Diwan and Ch. Sobhan Babu.}}. 
In the next section, we describe our heuristics for a more general setting
of the problem in which we make use of the proposed 1/2 benefit
approximation algorithm.

\subsection{Finding Optimal is NP-Hard}
We now show that the problem of choosing optimal sort orders is NP-Hard by
considering a special case of the problem.  Let $ e = R_1 \Join R_2 \Join
R_3 \ldots \Join R_n$ be a join expression with conjunctive join predicates
on $n$ relations, where $n$ is a power of 2.  Let $T$ be a balanced join
order tree for $e$.  \reffig{fig:jointree} shows an example. For each join
node $v$ in $T$, we assign an attribute set $L_v$ (called {\em
representative join attribute set}), which is constructed as follows. If
$a_i$ is an attribute involved in the join predicate of $v$ then
$\mathcal{H}(a_i) \in L_v$, where $\mathcal{H}(a_i)$ is the {\em
representative} of the attribute equivalence class in the result of $e$. Two
attributes $a_i$ and $a_j$ belong to the same attribute equivalence class if
they are equated directly or transitively in the join predicates of $e$. The
{\em representative} of an equivalence class is an arbitrarily chosen
attribute belonging to the equivalence class.  For example, if the predicate
$R_1.a_1=R_2.a_2 \wedge R_2.a_2=R_3.a_3$ is part of the join predicates of
$e$, then $R_1.a_1, R_2.a_2$ and $R_3.a_3$ belong to the same attribute
equivalence class, and we will have
$\mathcal{H}(R_1.a_1)=\mathcal{H}(R_2.a_2)=\mathcal{H}(R_2.a_2) = R_1.a_1$.
In \reffig{fig:jointree} we have shown the representative join attribute
sets for each join node. For brevity, we omit the relation name qualifiers
for attributes.

\begin{figure}[ht]
\begin{center}
\onecolonly{
\includegraphics[angle=0,width=3.4in]{chapters/eio/fig/jointree.eps}
}
\twocolonly{
\includegraphics[angle=0,width=3.0in]{chapters/eio/fig/jointree.eps}
}
\end{center}
\caption{A Join Tree with Representative Join Attribute Sets}
\label{fig:jointree}
\end{figure}

Now, suppose all the base relations and intermediate results in $T$ are
of the same size and no indices are present on the base relations. The
problem of choosing optimal sort orders for each join requires us to choose
permutations of representative join attribute sets such that we minimize the
cost of intermediate sorts. The cost of sorting depends on the sort order
already present on the input and the sort order required.  In general, the
sort cost on any edge $(v_i, v_j)$ of the tree is a monotonically decreasing
function of the length of common prefix between attribute permutations
chosen for $v_i$ and $v_j$. For example, see our cost model for sort
presented in \refsec{subsec:optchangepso}. We define the benefit of a
solution to be $\sum_{v_iv_j\in E} f(|p_i \wedge p_j|)$, where $E$ is the
set of edges in the tree, $p_i, p_j$ are attribute permutations chosen by
the solution for vertices $v_i, v_j$ and $f$ is any monotonically increasing
function in the length of the common prefix ($|p_i \wedge p_j|$), with 0 at
origin ({\em i.e.,} $f(0)=0$).  Minimizing the sorting cost requires
maximizing the total benefit.

\begin{figure}[ht]
\begin{center}
\onecolonly{
\includegraphics[angle=0,height=2.3in,width=4.4in]{chapters/eio/fig/tree.eps}
}
\twocolonly{
\includegraphics[angle=0,width=3.2in]{chapters/eio/fig/tree.eps}
}
\end{center}
\caption{A Special Case of Choosing Globally Optimal Sort Order}
\label{fig:tree}
\end{figure}

%As a special case, let us consider $f(p_i, p_j) = |p_i \wedge p_j|$.  In
%this case, the problem requires us to find attribute permutations so as to
%maximize the sum of lengths of common prefixes of permutations chosen for
%adjacent nodes. 
\reffig{fig:tree}, shows an example along with a solution, which maximizes
the total benefit assuming $f(|p_i \wedge p_j|) = |p_i \wedge p_j|$. The
representative join attribute set for each join node is shown in curly
braces besides the node. Permutations chosen by the solution are indicated
with angle brackets and the number on each edge shows the benefit for that
edge. Below we state the problem formally.

\noindent
%\newtheorem{eioproblem}{Problem}

%\vspace{-2pt}
\begin{eioproblem}
\label{problem1}
(Common Prefix Problem)
Let $T$ be a tree having $n$ vertices, the vertex set being $V(T)$ and the
edge set being $E(T)$.  Each vertex $v_i$ $(i=1,\ldots, n)$ is associated
with an attribute set $s_i$. Let $f$ be any non-decreasing function with
$f(0)=0$.  Find a set of attribute permutations $p_1,p_2 \ldots, p_n$, where
$p_i$ is a permutation of set $s_i$, such that the benefit function
%$\mathcal{F}$ is maximized.
$\mathcal{F} = \sum_{\forall v_iv_j\in E(T)} f(|p_i \wedge p_j|)$ is maximized.
%\[ \mathcal{F} = \sum_{\forall v_iv_j\in E(T)} f(|p_i \wedge p_j|) \]
\end{eioproblem}
%\[ \mathcal{F} = \sum_{\forall v_iv_j\in E(T)} f(p_i, p_j) \]
%where $f$ is a non-decreasing function of
%$|p_i \wedge p_j|$ and $f(p_i, p_j) = 0$ if $|p_i \wedge p_j| = 0$.


\noindent 
We prove that \refproblem{problem1} is NP-Hard even for binary trees.  To do
so we consider the special case where $f(|p_i \wedge p_j|) = |p_i \wedge
p_j|$. \\ 
Before giving a proof for this theorem, we will study some well
known NP-Hard problems, which are reducible to the Common Prefix Problem.

%We give a reduction from the known {\em NP-Hard} problem 
%{\em Sum-Cut}~\cite{DIAZ02}.

\begin{eioproblem}
\label{problem-sumcut}
(Sum-Cut)~\cite{DIAZ02}
{\em
Given a graph $G$ with $m$ vertices, number the vertices of $G$ as
$1,\ldots, m$ such that  $\sum_{1\leq i \leq m} c_i$ is minimized, where
$c_i$ is the number of vertices numbered $\leq i$ that are adjacent to at
least one vertex numbered greater than $i$.
}
\end{eioproblem}

\noindent The Sum-Cut problem can be rephrased as follows: given a graph $G$
with $m$ vertices, number the vertices of $G$ as $1,\ldots, m$ such that
$\sum_{1\leq i \leq m} \bar{c_i}$ is maximized, where $\bar{c_i}$ is the
number of vertices numbered $\leq i$ that are adjacent to no vertex numbered
greater than $i$. Let $G'$ be the complement graph of $G$.  The complement
graph $G'$ of $G$ contains an edge $(v_i,v_j)$ {\em iff} $(v_i,v_j)$ is not
present in $G$. On the complement graph $G'$, it is straight-forward to see
that the Sum-Cut problem is equivalent to \refproblem{problem2} given below.

\begin{eioproblem}
\label{problem2}
(Mod-Sum-Cut)
{\em 
Given a graph $H$ with $m$ vertices, number the
vertices of $H$ as $1,2,\ldots,m$ such that $\sum_{1\leq i \leq m} q_i$ is
maximized, where $q_i$ is the number of vertices that are adjacent to {\em
all} the vertices numbered greater than $i$.
}
\end{eioproblem}

First, we reduce the {\em Mod-Sum-Cut} problem to the Common Prefix Problem
on star trees. A {\em star tree} or simply a {\em star} of $n$ vertices is a
tree with a root and $n-1$ leaf vertices.

\begin{lemma}
The Common Prefix Problem is NP-Hard for stars.
\end{lemma}
\begin{proof}
We reduce the {\em Mod-Sum-Cut} problem to the Common Prefix Problem on
stars, with the function $f$ set to $|p_i \wedge p_j|$ ({\em i.e.,} the
length of the longest common prefix). Let graph $G$ with $m$ vertices be the
given instance of Mod-Sum-Cut problem. Let $v_1, \ldots, v_m$ be the
vertices of $G$. We construct an instance of the Common Prefix Problem on
stars as follows: let $S$ be a star having $m+1$ vertices, with $u_r$ as as
its root and $u_1,\ldots,u_m$ as its leaves. The attribute set of root $u_r$
is chosen to be the set of all vertices in $G$ ({\em i.e.}, $\{v_1, \ldots,
v_m\}$), and the attribute set of each leaf $u_i$ is chosen to be {\em
adj}$(v_i)$, where {\em adj}$(v_i)$ is the set of all vertices adjacent to
$v_i$ in graph $G$. A pictorial illustration of the construction is shown in
\reffig{fig:common-prefix-star}.

\begin{figure}[ht]
\begin{center}
\onecolonly{
\includegraphics[angle=0,width=3.4in]{chapters/eio/fig/common-prefix-star.eps}
}
\twocolonly{
\includegraphics[angle=0,width=3.0in]{chapters/eio/fig/common-prefix-star.eps}
}
\end{center}
\caption{Reducing Mod-Sum-Cut to Common Prefix on Star}
\label{fig:common-prefix-star}
\end{figure}


Now, we show that there exists a solution of value $k$ for 
Mod-Sum-Cut on $G$ {\em iff} there exists a solution of value $k$
for the Common Prefix Problem on $S$.

Suppose there exists a solution of value $k$ for Mod-Sum-Cut on $G$. Let the
order of vertices in the solution be $v_{g(1)}, v_{g(2)}, \ldots,
v_{g(m)}$, where $g$ is a permutation on $1, \ldots, m$ ({\em i.e.,} a
one-to-one function from $\{1, \ldots, m\}$ to $\{1, \ldots, m\}$). We
construct the solution for the corresponding Common Prefix Problem (for star
$S$) as follows: for the root vertex $u_r$, we choose the attribute
permutation to be $o_r=v_{g(m)}, v_{g(m-1)}, \ldots, v_{g(1)}$. For each
leaf vertex $u_i$, we choose a permutation $o_i$ of its attribute set
{\em adj}$(v_i)$ such that the length of the longest common prefix $|o_i
\wedge o_r|$ is maximum.

In the solution ordering for Mod-Sum-Cut, let $l_i$ be the smallest
integer such that $v_i$ is adjacent to all vertices in the set $v_{g(l_i+1)},
\ldots, v_{g(m)}$. This implies the following: {\em (i)} in the solution
value for Mod-Sum-Cut, vertex $v_i$ will be counted $m-l_i$ times, {\em
i.e.,} $k=\sum_{v_i}(m-l_i)$, and {\em (ii)} in the corresponding Common
Prefix Problem, there exists a common prefix of length $m-l_i$ between
the permutations chosen for $u_i$ and the root $u_r$. This shows there exists
a solution of value $k$ for the corresponding Common Prefix Problem.

Now, suppose there exists a solution of value $k$ for the Common Prefix
Problem on $S$.  In the solution, let the attribute permutation chosen for
the root vertex $u_r$ be $o_r=v_{h(1)}, v_{h(2)}, \ldots, v_{h(m)}$, where
$h$ is a permutation on $1, \ldots, m$.  Now, we construct the
solution for Mod-Sum-Cut on $G$ by reversing the order of attributes in
$o_r$, {\em i.e.,} by ordering the vertices of $G$ as $v_{h(m)}, v_{h(m-1)},
\ldots, v_{h(1)}$. 

In the solution for the Common Prefix Problem on $S$, let $o_i$ be the
permutation (of set {\em adj}$(v_i)$) chosen for leaf $u_i$. Let $l_i$
denote the length of the longest common prefix between $o_i$ and $o_r$, {\em
i.e.,} $l_i=|o_i \wedge o_r|$. We observe that, the solution value
$k=\sum_{1 \leq i \leq m}(l_i)$. In the corresponding solution for
Mod-Sum-Cut on $G$, $l_i$ will be the smallest integer such that vertex
$v_i$ is adjacent to all vertices in the set $v_{h(m)}, \ldots,
v_{h(m-l_i+1)}$.  Hence, in the solution value for Mod-Sum-Cut on $G$,
vertex $v_i$ will be counted $l_i$ times. Therefore, the solution for
Mod-Sum-Cut will have a value of $\sum_{1 \leq i \leq m}(l_i) = k$.
\end{proof}

\begin{theorem}
\label{theorem-nphard}
\refproblem{problem1} is NP-Hard even for binary trees.
\end{theorem}

\begin{proof}
We reduce the Common Prefix Problem on stars to the Common Prefix Problem on
binary trees. Let $S$ be a star with $u_r$ as its root and $u_1, \ldots,
u_m$ as its leaves. Let $a_r$ denote the set of attributes associated with
$u_r$ and $a_1, a_2, \ldots, a_m$ denote the set of attributes associated
with vertices  $u_1, u_2, \ldots, u_m$ respectively. We now construct an
instance of the Common Prefix Problem on binary trees as follows: let $T$ be
a binary tree with $2m$ vertices, with $r_1, r_2, \ldots, r_m$ as its internal
vertices and $w_1, w_2, \ldots, w_m$ as its leaves. Let the edge set $E(T)$
be $\{r_ir_{i+1} : 1 \leq i < m\} \cup \{r_iw_{i}: 1 \leq i \leq m\}$.  Each
internal vertex $r_i$ is assigned the attribute set $\mathcal{A}=a_r \cup
\mathcal{L}$, where $\mathcal{L}$ is an arbitrarily chosen set of attributes
of size $ > m\times |a_r|$ and is disjoint from $a_r \cup a_1 \cup \ldots
\cup a_m$. Each leaf vertex $w_i$ is assigned the attribute set $a_i$.
\reffig{fig:common-prefix-tree} pictorially illustrates the construction.
In the figure, the attribute sets $a_r$ and $a_1, \ldots, a_m$ for the star
are assumed to be as in \reffig{fig:common-prefix-star}.

\begin{figure}[ht]
\begin{center}
\onecolonly{
\includegraphics[angle=0,width=3.4in]{chapters/eio/fig/common-prefix-tree.eps}
}
\twocolonly{
\includegraphics[angle=0,width=3.0in]{chapters/eio/fig/common-prefix-tree.eps}
}
\end{center}
\caption{Reducing the Common Prefix Problem on Stars to the Common Prefix Problem on Binary Trees}
\label{fig:common-prefix-tree}
\end{figure}


\noindent Let $\mathcal{Z}=(m-1) \times |\mathcal{A}|$.

First, we show that if there exists a
solution of value $k$ for the Common Prefix Problem on $S$ then there exists
a solution of value $k+\mathcal{Z}$ for the Common Prefix Problem on $T$.

Suppose there exists a solution of value $k$ for the Common Prefix Problem
on $S$. Let the $o_r$ be the attribute permutation assigned for $u_r$ and
$o_i$ be the attribute permutation assigned for each $u_i$, $1 \leq i \leq
m$. We construct a solution for $T$ as follows: for each intern vertex
$r_i$, we assign the permutation $o_r + o_l$, where $o_l$ is a fixed
permutation of $\mathcal{L}$, chosen arbitrarily. For each leaf 
vertex $w_i$, we assign the permutation $o_i$. Since the same permutation
is chosen for all the internal vertices, each of the $(m-1)$ pairs of 
adjacent internal vertices will have a common prefix of length 
$|\mathcal{A}|$. Further, each of the $m$ pairs of internal 
and leaf vertices that are adjacent to each other will have a 
common prefix of length $|o_i \wedge o_r|$. As $k=\sum_{1\leq i \leq m}
(|o_i \wedge o_r|)$, we conclude the solution value for $T$ is 
$k + \mathcal{Z}$.

Next, we show that if there exists a solution of value $k$ for the Common
Prefix Problem on $T$ then there exists a solution of value $k-\mathcal{Z}$
for the Common Prefix Problem on $S$. To do so, we make use two supporting
lemmas, Lemma~\ref{lemma:identical-permutation} and
Lemma~\ref{lemma:begin-with-ar}. Below we state and prove these lemmas and
then continue with the proof of Theorem~\ref{theorem-nphard}.

\begin{lemma}
\label {lemma:identical-permutation}
In any optimal solution for the Common Prefix Problem on $T$, 
all the internal vertices are assigned an identical permutation $p$.
\end{lemma}

\begin{proof}
%Without loss of generatlity we assume $|\mathcal{L}| > m \times |a_r|$. 
Let $T_{opt}$ be an optimal solution for $T$. In the optimal solution, let
$p_1, \ldots, p_m$ be the permutations assigned to internal vertices $r_1,
\ldots, r_m$ respectively. We prove that $|p_i \wedge p_{i+1}| =
|\mathcal{A}|$ for $1 \leq i < m$, which essentially proves this lemma. 

\noindent
{\bf Case 1:} Suppose $|p_i \wedge p_{i+1}| < |a_r|$ for some $i$, 
              $1 \leq i < m$. \\
This implies, the total benefit of $T_{opt}$, {\em Ben}$(T_{opt}) < (m-2)
\times |\mathcal{A}| + (m+1) \times |a_r|$.  Since $|\mathcal{L}| > m \times
|a_r|$, we have $|\mathcal{A}| > (m+1) \times |a_r|$. Therefore, {\em
Ben}$(T_{opt}) < (m-1) \times |\mathcal{A}|$.  However, we know that there
exists a solution for $T$ with benefit of at least $(m-1) \times
|\mathcal{A}|$. This is because each of the internal vertices have the same
attribute set of size $|\mathcal{A}|$. This contradicts the given fact that
$T_{opt}$ is optimal. Therefore, we conclude that our assumption: $|p_i
\wedge p_{i+1}| < |a_r|$ for some $i$, $1 \leq i < m$, cannot be true. \\

\noindent
{\bf Case 2:} Suppose $|p_i \wedge p_{i+1}| \geq |a_r|$ for all $1 \leq i <
m$, but $|p_i \wedge p_{i+1}| < |\mathcal{A}|$ for some $i$, $1 \leq i < m$. \\
Given a permutation $p$, we use the notation $p[j]$ to denote the
attribute at the $j^{th}$ position, where $1 \leq j \leq |p|$.
The condition for Case 2 implies the following: 
\begin{enumerate}[(a)]
\onlythesis{\addtolength{\itemsep}{-2mm}}
    \item $p_1[j] = p_2[j] = \ldots = p_m[j]$ for $1 \leq j \leq |a_r|$.
    \item in $T_{opt}$, the total benefit of edges incident between internal
          vertices $\sum_{1 \leq i < m}(|p_i \wedge p_{i+1}|)$ must be
          less than $|\mathcal{A}| \times (m-1)$. 
\end{enumerate}

Now, consider a solution $T_{opt}'$ for $T$ in which each leaf vertex is
assigned the same permutation as in $T_{opt}$ and all the internal vertices
are assigned an identical permutation $p$ constructed as follows: 
the first $|a_r|$ attributes of $p$ are chosen in the same order as 
the first $|a_r|$ attributes in $p_i$ for any $1 \leq i \leq m$ 
({\em i.e.,} $p[j] = p_i[j], 1 \leq j \leq |a_r|$), and the next 
$|\mathcal{A} - a_r|$ attributes are chosen an in an arbitrary order.

We observe that in both $T_{opt}'$ and $T_{opt}$ the total benefit of 
edges incident from internal vertices to leaf vertices remains the same.
However, in $T_{opt}'$, the total benefit of edges incident between 
internal vertices will be $|\mathcal{A}| \times (m-1)$ (this is
because all internal vertices are assigned an identical permutation).
This implies, the total benefit of $T_{opt}'$ is larger than
that of $T_{opt}$, which contradicts the given fact that $T_{opt}$
is optimal. Therefore, we conclude the assumption made for Case 2
cannot be true.

We thus conclude in every optimal solution $T_{opt}$, all the internal 
vertices are assigned an identical permutation, completing the proof
of Lemma~\ref{lemma:identical-permutation}.
\end{proof}

\noindent Next, we state and prove our second supporting lemma.
\begin{lemma}
\label{lemma:begin-with-ar}
There exists an optimal solution for $T$ such that, in the permutation 
$p$ chosen for the internal vertices, every attribute
in set $a_r$ occurs before any attribute in set $\mathcal{L}$ occurs.
\end{lemma}

\begin{proof}
Let $T_{opt}$ be an optimal solution for $T$. In $T_{opt}$, let $p_1,
\ldots, p_m$ be the permutations assigned to the internal vertices $r_1,
\ldots, r_m$ respectively. From Lemma \ref{lemma:identical-permutation} 
we know that all the internal vertices are assigned an identical
permutation; let $p_1 = p_2 = \ldots = p_m = p$. 

Suppose there exist $x,y$ such that $x < y$, $p[x] \in \mathcal{L}$ and
$p[y] \in a_r$.  We now modify $p_1, \ldots, p_m$ as follows: in each $p_i$,
we swap $p_i[x]$ with $p_i[y]$. Since there is no attribute common to the
set $\mathcal{L}$ and the attribute sets associated with the leaf vertices,
this modification cannot decrease the total benefit of $T_{opt}$. This 
modification can be repeated until all the attributes in $a_r$ appear
before the attributes in $\mathcal{L}$ in the permutation $p$.
\end{proof}

From Lemmas~\ref{lemma:identical-permutation} and
~\ref{lemma:begin-with-ar}, we can make the following statement: if there
exists a solution of value $k$ for the Common Prefix Problem on $T$, then
there exists a solution $T_{opt}$ of value at least $k$, in which, all
internal vertices are assigned an identical permutation $p$ and $|p \wedge
a_r|=|a_r|$.

We now construct a solution for the star $S$ as follows: for the root vertex
$u_r$ we assign the permutation $p \wedge a_r$. For each leaf vertex
$u_i$, we assign the permutation chosen for the corresponding leaf $w_i$ in
the solution $T_{opt}$. In $T_{opt}$, the maximum benefit which can be
contributed by edges incident between internal vertices of $T$ is
$\mathcal{Z}$. Therefore we conclude the corresponding solution on $S$ should
have a benefit of at least $k-\mathcal{Z}$.
\end{proof}


%% The following text gives a direct reduction from Mod-Sum-Cut to
%% common prefix on binary trees. This is replaced by the above 2-step
%% reduction via stars.
\eat{
\noindent First, we will reduce \refproblem{problem2} (Mod-Sum-Cut) 
to \refproblem{problem1} (Common Prefix Problem) on stars. Next, 

In the Common
Prefix Problem, we assume the benefit function to be an identity
function of the length of the common prefix, {\em i.e.,}
$f(|p_i \wedge p_j|) = |p_i \wedge p_j|$.

Given an instance of the {\em Mod-Sum-Cut} problem, we construct
an instance of the Common Prefix Problem as follows.
Let the $m$ vertices
of the graph be labeled $u_1, \ldots, u_m$. We construct the binary tree by
choosing a vertex set $V(T)$ of size $2m$, $\{v_1,v_2 \ldots, v_{2m}\}$.
$v_1, \ldots, v_m$ are internal vertices and $v_{m+1}, \ldots, v_{2m}$ are leaf
vertices.  Let the edge set $E(T)$ be $\{v_iv_{i+1} : 1 \leq i < m\} \bigcup
\{v_iv_{m+i}: 1 \leq i \leq m\}$.  Attribute set $s_i$ of internal vertex
$v_i$ is $V(G) \cup \mathcal{L}$, where $\mathcal{L}$ is an arbitrarily
large set disjoint from $V(G)$, for $1 \leq i \leq m$.  Attribute set $s_i$
of leaf vertex $v_i$ is $\{w: w\in V(G)$ and $wu_{i-m}\in E(G)\}$, for $m <
i \leq 2m$.
}

\subsection{A Polynomial Time Algorithm for Paths}
\label{subsec:pathalgo}
We now present an efficient algorithm for solving the Common Prefix Problem,
when the tree is a path. The algorithm employs dynamic programming.  Note
that left-deep and right-deep join plans result in problem instances on 
paths. \onlyjournal{The algorithm relies on the following theorem.}

\begin{theorem}
Let $v_1, v_2, \ldots, v_n$ be a path, where each vertex $v_i$ is associated
with an attribute set $s_i$. The optimal solution of Common Prefix Problem
for any segment $(i, j)$ of the path, {\small OPT$(i, j)$ = max$\{$ OPT$(i,
k) + $OPT$(k+1, j) + f(c(i, j))$ $\}$} over all $i\leq k<j$, where $c(i, j)$
is the number of common attributes for the segment $(i, j)$.  
\end{theorem}

\begin{proof}
\ \\
{\bf Case 1:} Let $c(i, j) = 0$, {\em i.e.}, there exists no 
attribute common to all vertices $v_i, v_{i+1}, \ldots, v_j$.  Consider an
optimal solution for the path $v_i, \ldots, v_j$.  Let $p_x$ be the attribute
permutation assigned by the optimal solution to vertex $v_x$, $i \leq x
\leq j$.  The optimal solution must contain two vertices $v_k, v_{k+1}$ such
that the benefit for the edge $(v_k, v_{k+1})$ is 0, {\em i.e.}, $|p_k
\wedge p_{k+1}|=0$. This directly follows from the assumption of Case 1,
$c(i, j) = 0$. Now, the problem can be independently solved for the two
segments $(v_i, v_k)$ and $(v_{k+1}, v_j)$ and $OPT(i, j) = OPT(i, k) +
OPT(k+1, j)$.

\noindent
{\bf Case 2:} Let $c(i, j) \neq 0$.  Let $s(i, j)$ be the set of attributes
common to all vertices $v_i, \ldots, v_j$. Note that the cardinality $|s(i,
j)| = c(i, j)$. Let $o_s$ be an arbitrarily chosen permutation of set $s(i,
j)$.  We claim that there exists an optimal solution \onlyjournal{$S_{opt}$}
such that, for every
vertex $v_x$ ($i \leq x \leq j$) the attribute permutation $p_x$ chosen by
the optimal solution has $o_s$ as its prefix. To see this, consider an
optimal solution in which $o_s$ is not a prefix of some $p_x$. We can then
reorder the permutations assigned to the vertices, without a decrease in the
total benefit $OPT(i, j)$, so as to have $o_s$ as the prefix of each $p_x, i
\leq x \leq j$.

\onlyjournal{
In the above optimal solution $S_{opt}$, there must exist an edge $v_i
}

\onlythesis{
Let $v_i', \ldots, v_j'$ be a path where each vertex $v_x'$ is associated
with the attribute set $s_x - s(i, j)$, {\em i.e.}, $v_x'$ has all the 
attributes of $v_x$ except those in $s(i, j)$. We can see that the value 
of the optimal solution $OPT(v_i, v_j)$ is given by Equation~\ref{eqn:eq1}.
%
%--------- Equation (1) -----------
%
\begin{equation}
\label{eqn:eq1}
OPT(v_i, v_j) = OPT(v_i', v_j') + (j-i) \times f(c(i, j))
\end{equation}
%
%
\noindent Now, consider the path $v_i', \ldots, v_j'$. From our construction 
of the path, we know there are no attributes common to all the vertices
of $v_i', \ldots, v_j'$. Therefore, we have: 
%
%--------- Equation (2) -----------
%
\onecolonly{
\begin{equation}
\label{eqn:eq2}
OPT(v_i', v_j') = OPT(v_i', k') + OPT(v_{k+1}', v_j')\ \text{for some}\ k', 0 \leq k' \leq n. 
\end{equation}
}
\twocolonly{
\begin{eqnarray}
\label{eqn:eq2}
OPT(v_i', v_j') & = & OPT(v_i', k') + OPT(v_{k+1}', v_j') \nonumber\\
                &   & \text{for some}\ k'\ \text{such that}, 
                      0 \leq k' \leq n. 
\end{eqnarray}
}
%
%--------- Equation (3) -----------
%
\noindent From the construction of the path $v_i', \ldots, v_j'$, we have:
\begin{equation}
\label{eqn:eq3}
OPT(v_i', v_k') = OPT(v_i, v_k) - (k - i) \times f(c(i, j))
\end{equation}
%
%--------- Equation (4) -----------
%
\begin{equation}
\label{eqn:eq4}
OPT(v_{k+1}', v_j') = OPT(v_{k+1}, v_j) - (j - k - 1) \times f(c(i, j))
\end{equation}
%
\noindent Substituting from Equations~\ref{eqn:eq3} and \ref{eqn:eq4} in 
Equation~\ref{eqn:eq2}, we get:
%
%--------- Equation (5) -----------
%
\onecolonly{
\begin{equation}
\label{eqn:eq5}
OPT(v_i', v_j') = OPT(v_i, v_k) + OPT(v_{k+1}, v_j) 
                  - (j - i - 1) \times f(c(i, j)) \ \\
                  \text{ for some}\ k', 0 \leq k' \leq n.
\end{equation}
}
\twocolonly{
\begin{eqnarray}
\label{eqn:eq5}
OPT(v_i', v_j') & = & OPT(v_i, v_k) + OPT(v_{k+1}, v_j)  \nonumber\\
                &   & - (j - i - 1) \times f(c(i, j)) \nonumber \\
                &   & \text{for some}\ k'\ \text{such that}, 
                    0 \leq k' \leq n.
\end{eqnarray}
}
%
\noindent Substituting Equation~\ref{eqn:eq5} in Equation~\ref{eqn:eq1}, 
we get:
%
%--------- Equation (6) -----------
%
\onecolonly{
\begin{equation}
\label{eqn:eq6}
OPT(v_i, v_j) = OPT(v_i, v_k) + OPT(v_{k+1}, v_j) + f(c(i, j))
\ \text{for some}\  k', 0 \leq k' \leq n.
\end{equation}
}
\twocolonly{
\begin{eqnarray}
\label{eqn:eq6}
OPT(v_i, v_j) & = & OPT(v_i, v_k) + OPT(v_{k+1}, v_j) + f(c(i, j)) \nonumber\\
              &    & \text{for some}\  k'\ \text{such that}, 
                     0 \leq k' \leq n. 
\end{eqnarray}
}
%
\noindent Hence the proof.
}
\end{proof}

%% Description of the top-down approach
\eat{
The dynamic programming algorithm starts by identifying the set $s(1,n)$ of
common elements for all vertices $v_1, \ldots, v_n$. These elements are
removed from the attribute set $s_i$ of every vertex $v_i$ $(1 \leq i \leq
n)$ and the set $s(1, n)$ is remembered. For every value of $k$, $1 \leq k
< n$, a recursive invocation of the algorithm is made for path segments
$v_1, \ldots, v_k$ and $v_{k+1}, \ldots, v_n$. Let $k_{max}$ be the value of
$k$ that maximizes $OPT(1, k) + OPT (k+1, n)$. The optimal solutions for the
sub-problems $(v_1, v_k)$ and $(v_{k+1}, v_n)$ are then used to construct
the solution for the whole problem $(v_1, v_n)$ by prefixing the attribute
permutations $p_i$ chosen for each vertex $v_i$ with $o_s$, an arbitrarily
chosen permutation of the common elements $s(1,n)$. The recursive invocation
of the algorithm terminates when the path segment is of length $0$ 
({\em i.e.}, a single vertex), for which, an arbitrarily chosen permutation 
of the attribute set is returned as the solution with solution benefit 0.
}

Procedure {\em PathOrder} in \reffig{fig:pathalgo} computes optimal
attribute permutations for any path $(1, n)$, where each vertex $i$, $1 \leq
i \leq n$, is associated with an attribute set $s[i]$. The procedure uses
dynamic programming and computes solutions bottom up starting from path
segments of length 0 (single vertices). The procedure begins by assigning a
benefit of $0$ to all path segments $(i, i)$, $1 \leq i \leq n$.  It then
constructs solutions for paths of increasing length. For each path $(i,
i+j)$, of length $j$, $1 \leq j \leq n-1$, the value of $k$, which maximizes
{\em ben}={\em benefit}$(i, k)+${\em benefit}$(k+1, i+j)$ is identified. The
values of $k$, {\em ben} and the attributes common to all the vertices of
path $(i, i+j)$ are remembered (memoized). Finally, the sub-procedure {\em
MakePermutation} is used to construct the attribute permutations $p[1],
\ldots, p[n]$ using the memo structure.  The first call to procedure {\em
MakePermutation} is made with parameter $i$ set to $1$ (the first vertex on
the path) and $j$ set to $n$ (the last vertex on the path), and each of the
attribute permutations $p[1], \ldots, p[n]$ initialized with an empty sort
order.  Procedure {\em MakePermutation} constructs the attribute permutation
for each of the vertices $i, i+1, \ldots, j$ as follows: a permutation {\em
cp} of {\em commons(i, j)} ({\em i.e.,} the set of attributes common to all
the vertices from $i, \ldots, j$) is chosen at arbitrary.  {\em cp} is then
appended to each of $p[i], \ldots, p[j]$. The common attributes for segment
$(i, j)$ are then removed from the common attributes of all subpaths of
$(i,j)$. The optimal split point $m$ for the path segment $(i,j)$ is read
from the memo structure, and the construction of the permutations continues
recursively on subpaths $(i, m)$ and $(m+1, j)$, until $i=j$ ({i.e.,} 
a single vertex). The overall time complexity of procedure {\em PathOrder}
is $O(n^3)$.

\input{chapters/eio/sections/pathalgo.tex}

\subsection{A 1/2 Benefit Approximation Algorithm for Binary Trees}
\label{subsec:approxalgo}
For binary trees we propose an approximation with benefit at least half that
of an optimal solution. Note that our approximation guarantee implies at least 
half the best possible {\em improvement} over the worst case sort cost. 
This however, does not imply a 2-approximation on the total cost.

We split the tree into two sets of paths, $P_o$ and $P_e$. $P_o$ has the
paths formed by edges incident from odd levels and $P_e$ has those formed by
edges incident from even levels, \reffig{fig:treeapprox} shows an example.
We then find an 
%use the procedure {\em PathOrder} to find 
optimal solutions for each of the two sets of paths. Note that this gives us
two solutions for the complete tree, because each set of paths covers all
the vertices of the tree (for any left over vertices at the leaf level or
the root, we choose an arbitrary permutation).  Let the optimal
solutions for the two sets of paths be $S_o$ and $S_e$ and the corresponding
benefits be {\em ben($S_{o}$)} and {\em ben($S_{e}$)}. Let the set of edges
included in $P_o$ and $P_e$ be denoted by $E_{o}$ and $E_e$ respectively.
Consider an optimal solution {\em $S_T$} for the whole tree. In the optimal
solution, let the sum of benefits of all edges in $E_{o}$ be {\em
odd-ben($S_T$)} and that of edges in $E_{e}$ be {\em even-ben($S_T$)}.  Note
that  {\em ben($S_o$)} $\geq$ {\em odd-ben($S_T$)} and {\em ben($S_e$)}
$\ge$ {\em even-ben($S_T$)}. Since the total benefit of the optimal solution
{\em ben($S_T$)} $=$ {\em odd-ben($S_T$)} $+$ {\em even-ben($S_T$)}, we have
{\em ben($S_o$)} $+$ {\em ben($S_e$)} $\geq$ {\em ben($S_T$)}.  Hence at
least one of {\em ben($S_o$)} or {\em ben($S_e$)} is $\geq 1/2$ {\em
ben($S_T$)}.  There may be vertices not included in the chosen solution,
e.g., the even level split in \reffig{fig:treeapprox} does not include the
root and leaf nodes. For these left over vertices arbitrary permutations can
be chosen.  Kenkre and Vishwanathan~\cite{SREK08} have subsequently 
improved upon our result and have given a 
${log\ log\ n}\over{1\ +\ log\ log\ n}$ factor approximation.
\begin{figure} [t]
\begin{center}
\onecolonly{
\includegraphics[width=4.5in,height=1.2in]{chapters/eio/fig/treeapprox.eps}
}
\twocolonly{
\includegraphics[angle=0,width=3.0in]{chapters/eio/fig/treeapprox.eps}
}
\end{center}
\caption{A 1/2 Benefit Approximation for Binary Trees}
\label{fig:treeapprox}
\end{figure}



==> chapters/eio/sections/sec_perf.tex <==
\section{Experimental Results} 
\label{sec:perf:chap:eio}
We performed experiments to evaluate the benefits due to the proposed ideas.
For comparison, we use PostgreSQL (version 8.1.3) and two widely used
commercial database systems (we call them SYS1 and SYS2). All tests were run
on an Intel P4 (HT) PC with 512 MB of RAM. We used TPC-H 1GB dataset and
additional tables as specified in the individual test cases. For each table,
a clustering index was built on the primary key. Additional secondary
indices built are specified along with the test cases. All relevant
statistics were built and the optimization level for one of the systems,
which supports multiple levels of optimization, was set to the highest.

\eat{
The tables used and the number of tuples in each table are summarized
in \reffig{table:perftables}.

\begin{figure}[t]
\center
{ \small
\begin{tabular}{|c|c|c|c|} \hline
{\bf Name} & lineitem & part & supplier \\
\hline
{\bf Tuples} & 6,000,000 & 200,000 & 10,000 \\
\hline
\hline
{\bf Name} & partsupp & orders & customer\\
\hline
{\bf Tuples} &  800,000 & 1,500,000 &  150,000 \\
\hline
\end {tabular}
}
\caption{Tables used for the Experiments}
\label{table:perftables}
\end{figure}
}

%We used the TPC-H dataset of 1 GB for our tests. 

\subsection{Modified Replacement Selection}
The first set of experiments evaluate the benefits of exploiting partial
sort orders. External sort in PostgreSQL employs the standard replacement
selection (SRS) algorithm~\cite{KNUTH} suitably adapted for variable length
records.  We modified this implementation to exploit partial sort orders
available on the input (as described in \refsec{sec:pso:chap:eio}), and we
call it Modified Replacement Selection (MRS).  We now present experiments
comparing the performance of MRS with SRS.

%\noindent {\bf Experiment A1}: \\
\subsubsection*{Experiment A1}
The first experiment consists of a simple ORDER BY of the TPC-H {\em
lineitem} table on two columns {\em (l$\_$suppkey, l$\_$partkey)}. 

\onlythesis{
\begin{floatexample}
\begin{sqlindent}
\\
SELECT \>\> l$\_$suppkey, l$\_$partkey \\
FROM   \>\> lineitem \\
ORDER  \>\> BY l$\_$suppkey, l$\_$partkey;
\end{sqlindent}
\label{query:lisort}
\caption{An Order-By Query on Two Columns (Query 1)}
\end{floatexample}
}

\onlyjournal{
\begin{query}
%ORDER-BY on lineitem
\label{query:lisort}
%\vspace{-5pt}
\begin{tabbing}
xxxxxxxxxx\=xxxxxxxxx\=xxxxxxxxx\=\kill
\\
SELECT \> l$\_$suppkey, l$\_$partkey \\
FROM   \> lineitem \\
ORDER  \> BY l$\_$suppkey, l$\_$partkey;
\end{tabbing}
\end{query}
}

A secondary index on {\em l$\_$suppkey} was available that covered the query
(included the {\em l$\_$partkey} column)\footnote{On systems not supporting
indexes with included columns, we used a table with only the desired two
columns, clustered on {\em l$\_$suppkey}}.  On all three systems, the order
by on {\em (l$\_$suppkey, l$\_$partkey)} took almost the same time as an
order by on {\em (l$\_$partkey, l$\_$suppkey)} showing that the sort
operator of these systems did not exploit partial sort orders effectively.
We then compared the running times with our implementation that exploited
partial sort order {\em (l$\_$suppkey)} and the results are shown in
\reffig{fig:perf-pso}. 

For SYS1 and SYS2, as we did not have access to their source code, we
simulated the partial sorting using a correlated rank query. The subquery
sorted the index entries matching a given {\em l$\_$suppkey} on {\em
l$\_$partkey} and the subquery was invoked with all {\em suppkey} values so
as to obtain the desired sort order of {\em (l$\_$suppkey, l$\_$partkey)}. 
%Further, on all three systems (with their default sort), an order by on 
%{\em (l$\_$partkey, l$\_$suppkey)} took almost the same time as an order 
%by on {\em (l$\_$suppkey, l$\_$partkey)} showing that the systems by
%default did not exploit partial sort orders effectively.

\begin{figure*}[ht]
%\hspace{-3ex}
\begin{tabular}{c@{}c@{}c}
\begin{minipage}{0.5\textwidth} 
\includegraphics[angle=270,totalheight=2.2in,width=4.0in]{chapters/eio/fig/perf/plots/lisort.eps}
\caption{Performance Results for Experiment A1} 
\label{fig:perf-pso}
\end{minipage}
&
\begin{minipage}{0.5\textwidth}
\includegraphics[angle=270,totalheight=2.2in,width=4.0in]{chapters/eio/fig/perf/plots/rate_time_y.eps}
\caption{Rate of Output}
\label{fig:perf-rate}
\end{minipage}
\end{tabular}
\end{figure*}

By avoiding run generation I/O and making reduced comparisons, MRS performs
3-4 times better than SRS. 

\subsubsection*{Experiment A2}
The second experiment shows how MRS is superior in terms of its ability to
produce records early and uniformly.  Table $R_3$ having 3 columns $(c1, c2,
c3)$ was populated with 10 million records and was clustered on $(c1)$.  The
query asked an order by on $(c1, c2)$. \reffig{fig:perf-rate} shows the plot
of number of tuples produced vs.  time with cardinality of $c1=10,000$.

MRS starts producing the tuples without any delay after the operator
initialization where as SRS produces its first output tuple only after
seeing all input tuples.  By producing tuples early, MRS speeds up the
pipeline significantly. Such early output behavior is highly desirable
for Top-K queries.

\subsubsection*{Experiment A3}
The third experiment shows the effect of {\em partial sort segment size} on
sorting. 8 tables $R_0, \ldots, R_7$, with identical schema of 3 columns
$(c1, c2, c3)$ were each populated with 10 million records and average
record size of 200 bytes.  Each table was clustered on $(c1)$. Table $R_{i}$
had $10^i$ tuples for each distinct value of $c1$ ({\em i.e.,} uniform
distribution over $10^{7-i}$ distinct values of $c1$), resulting in a partial
sort segment size of $200\times 10^i$ bytes. Thus $R_0$ had a sort segment
of size 1 tuple or 200 bytes, and $R_7$ had a sort segment of size 10
million tuples or 2GB.  The query had an order by on $(c1, c2)$.  The
running times with default and modified replacement selection on PostgreSQL
are shown in \reffig{fig:perf-pgvaryselect}.

\begin{figure*}[ht]
\onecolonly{
\includegraphics[angle=270,width=5.0in]{chapters/eio/fig/perf/plots/pgvaryselect_logscale_new.eps}
}
\twocolonly{
\centerline{
\includegraphics[angle=270,width=0.75\textwidth]{chapters/eio/fig/perf/plots/pgvaryselect_logscale_new.eps}
}
}
\caption{Effect of Partial Sort Segment Size}
\label{fig:perf-pgvaryselect}
\end{figure*}

When the partial sort segment size is small enough to fit in memory (up to
10MB or 50K records), SRS produces a single sorted run on disk and does not
involve merging of runs. The modified replacement selection (MRS) gets the
benefit of avoiding I/O and reduced number of comparisons. When the partial
sort segment size becomes too large to fit in memory, we see a sudden rise
in the time taken by SRS.  This is because replacement selection will have
to deal with merging several runs. MRS however deals with merging smaller
number of runs initially as each partial sort segment is sorted separately.
As the partial sort segment size increases, the running time of MRS rises
and becomes same as that of SRS at the extreme point where all records have
the same value for $c1$.

\subsubsection*{Experiment A4}
To see the influence of MRS on a query with joins and aggregates, we
considered the query shown in \refex{query:pslijoin}. The query finds the
number of lineitems and available quantity for each supplier, part pair.
The supplier and part key columns were common to the join, group-by and the
order-by clauses.  Two indices, {\em lineitem(l$\_$suppkey)} and  {\em
partsupp(ps$\_$supp\-key)}, were present and covered the query.  The indices
were thus useful to obtain part of the desired sort order {\em (suppkey,
partkey)}.

%The {\em partsupp} table was clusterd on {\em ps$\_$suppkey} and a
%secondary index {\em lineitem(l$\_$suppkey)} that covered the query
%supplied the partial sort order.

\onlythesis{
\begin{floatexample}
\begin{sqlindent}
\\
SELECT \>\> ps$\_$suppkey, ps$\_$partkey, ps$\_$availqty, count(l$\_$partkey) \\
FROM   \>\> partsupp, lineitem \\
WHERE  \>\> ps$\_$suppkey=l$\_$suppkey AND ps$\_$partkey=l$\_$partkey \\
GROUP BY ps$\_$suppkey, ps$\_$partkey, ps$\_$availqty \\
ORDER BY ps$\_$suppkey, ps$\_$partkey;
\end{sqlindent}
\caption{Number of lineitems for each (supplier, part) pair (Query 2)}
\label{query:pslijoin}
\end{floatexample}
}

\onlyjournal{
\begin{query}
\label{query:pslijoin}
Number of lineitems for each (supplier, part) pair
\begin{tabbing}
xxxxxxxxxx\=xxxxxxxxx\=xxxxxxxxx\=\kill
SELECT \> ps$\_$suppkey, ps$\_$partkey, ps$\_$availqty, \\
       \> count(l$\_$partkey) \\
FROM   \> partsupp, lineitem \\
WHERE  \> ps$\_$suppkey=l$\_$suppkey AND \\
       \> ps$\_$partkey=l$\_$partkey \\
xxxxxxxxxxxxx\=xxxxxxxxx\=xxxxxxxxx\=\kill
GROUP BY \> ps$\_$suppkey, ps$\_$partkey, ps$\_$availqty \\
ORDER BY \> ps$\_$suppkey, ps$\_$partkey;
\end{tabbing}
\end{query}
}

On PostgreSQL the query took 63 seconds to execute with SRS, and 25 seconds 
with MRS. The query plan used in both cases was the same: a merge join
of the two relations on {\em (suppkey, partkey)} followed by aggregation.
%\reffig{fig:perf-pslijoin} shows the running times of the query with SRS
%and MRS on PostgreSQL. 

\eat{
\begin{figure*} [t]
\includegraphics[angle=270,width=3.3in]{chapters/eio/fig/perf/plots/pslijoin.eps}
\caption{Join of partsupp and lineitem} 
\label{fig:perf-pslijoin}
\end{figure*}
}

\subsection{Choice of Interesting Orders}
We extended our Volcano-style cost based optimizer, which we call PYRO, to
consider partial sort orders and to use the proposed method for choosing
sort orders for merge joins and aggregation. We compare the plans produced
by the extended implementation, which we call PYRO-O, with those of
PostgreSQL, SYS1 and SYS2. 
%The optimization overheads due to the extensions were negligible. 

\subsubsection*{Experiment B1} 
For this experiment we used the query shown in \refex{query:outofstock}
below, which lists parts for which the outstanding order quantity is
more than the stock available at the supplier.

\onlythesis{
\begin{floatexample}
\begin{sqlindent}
\\
SELECT \>\> ps$\_$suppkey, ps$\_$partkey, ps$\_$availqty, sum(l$\_$quantity) \\
%AS total$\_$required \\
FROM  \>\>  partsupp, lineitem  \\
WHERE \>\> ps$\_$suppkey=l$\_$suppkey AND ps$\_$partkey=l$\_$partkey AND l$\_$linestatus='O' \\
GROUP  BY ps$\_$availqty, ps$\_$partkey, ps$\_$suppkey \\
HAVING  sum(l$\_$quantity) $>$ ps$\_$availqty ORDER BY ps$\_$partkey;
\end{sqlindent}
\caption{Parts Running Out of Stock (Query 3)}
\label{query:outofstock}
\end{floatexample}
}

\onlyjournal{
\begin{query}
\label{query:outofstock}
Parts Running Out of Stock
\begin{tabbing}
xxxxxxxxx\=\kill
SELECT \> ps$\_$suppkey, ps$\_$partkey, ps$\_$availqty, \\
       \> sum(l$\_$quantity) \\
FROM  \>  partsupp, lineitem  \\
WHERE \> ps$\_$suppkey=l$\_$suppkey AND ps$\_$partkey=\\
      \> l$\_$partkey AND l$\_$linestatus='O' \\
GROUP  BY ps$\_$availqty, ps$\_$partkey, ps$\_$suppkey \\
HAVING  sum(l$\_$quantity) $>$ ps$\_$availqty \\
ORDER BY ps$\_$partkey;
\end{tabbing}
\end{query}
}

Table {\em partsupp} had clustering index on its primary key {\em
(ps$\_$partkey, ps$\_$suppkey)}.  Two secondary indices, one on
$ps\_suppkey$ and the other on $l\_suppkey$ were also built on the {\em
partsupp} and {\em lineitem} tables respectively.  The two secondary indices
covered all attributes needed for the query. 

The experiment shows the need for cost-based choice of interesting orders.
The choice of interesting orders for the join and aggregate are not obvious
in this case for the following reasons:

\begin{enumerate}
\item The order-by clause favors the choice of a sort order
   where {\em partkey} appears first.
\item The clustering index on {\em partsupp} favors the choice of 
   {\em (partkey, suppkey)}.
\item The secondary indices favor the choice of 
   {\em (suppkey, partkey)} that can be obtained by using a low
   cost partial sort.  Note that this option can be much cheaper 
   due to the size of the {\em lineitem} relation.
\end{enumerate}

Therefore, the optimizer must make a cost-based decision on the sort order
to use.  Figures \ref{fig:perf-query1fig1} and \ref{fig:perf-query1fig2}
show the plans chosen by PostgreSQL, PYRO-O, SYS1 and SYS2. 

All plans except the hash-join plan of SYS1 and the plan produced by PYRO-O
use an expensive full sort of 6 million lineitem index entries on {\em
(l$\_$partkey, l$\_$suppkey)}. Further, PostgreSQL uses a hash aggregate where
a sort-based aggregate would have been much cheaper as the required sort
order for the group-by was available from the output of merge-join. Note
that the sort order {\em (ps$\_$partkey, ps$\_$suppkey,
ps$\_$availability)}, required by the group-by, can be inferred from the
sort order {\em (ps$\_$partkey, ps$\_$suppkey)}, available on the result of
merge-join, due to the presence of the functional dependency {\em
$\{$ps$\_$partkey, ps$\_$suppkey$\} \rightarrow\{$ps$\_$availqty$\}$}.  On
SYS1, it was possible to force the use of a merge-join instead of hash-join
and the plan chosen is shown in \reffig{fig:perf-query1fig2}(b).

\begin{figure*} [ht]
\centerline{\includegraphics[angle=0,width=5.0in]{chapters/eio/fig/perf/plans/query1fig1.eps}}
\caption{Plans for Query 3 (PostgreSQL and PYRO-O)} 
\label{fig:perf-query1fig1}
\end{figure*}


\begin{figure*} [t]
\centerline{\includegraphics[angle=0,width=5.0in]{chapters/eio/fig/perf/plans/query1fig2.eps}}
\caption{Plans for Query 3 (SYS1 and SYS2)} 
\label{fig:perf-query1fig2}
\end{figure*}

We compared the actual running time of PYRO-O's plan with those of
PostgreSQL and SYS1 by forcing our plan on the respective systems.  Figures
\ref{fig:q2q3postgres} and \ref{fig:q2q3mssql} show the execution times.  It
was not possible for us to force our plan on SYS2 and make a fair comparison
and hence we omit the same.  The only surprising result was the default plan
chosen by SYS1 performed slightly poorer than the forced merge-join plan on
SYS1. In all cases, the forced PYRO-O plan performed significantly better
than the other plans. The main reason for the improvement was the use of a
partial sort of {\em lineitem} index entries as against a full sort. The
final sort on {\em partkey} was not very expensive as only a few tuples
needed to be sorted.

For Query 3 (Example~\ref{query:outofstock}) the plan generation phase
(phase-1) was sufficient to select the sort orders and phase-2 does not make
any changes.  We shall now see a case for which phase-1 cannot make a good
choice and the sort orders get refined by phase-2.


\begin{figure*}[ht]
\centering
\begin{tabular}{@{}c@{}c}
\begin{minipage}{0.5\textwidth}
\includegraphics[angle=270,width=3.4in]{chapters/eio/fig/perf/plots/q2q3-postgres.eps}
\caption{Performance on PostgreSQL}
\label{fig:q2q3postgres}
\end{minipage}
&
\begin{minipage}{0.5\textwidth}
\includegraphics[angle=270,width=3.4in]{chapters/eio/fig/perf/plots/q2q3-mssql.eps}
\caption{Performance on SYS1}
\label{fig:q2q3mssql}
\end{minipage}
\end{tabular}
\end{figure*}

\subsubsection*{Experiment B2}
This experiment uses the query shown in \refex{query:r1-r3}, which has two
full outer joins with two common attributes between the joins.  We performed
this experiment to see whether the systems we compare with are designed to
exploit attributes common to multiple sort-based operators. 

\onlyjournal{
\begin{query}
\label{query:r1-r3}
Attributes common to multiple joins
\begin{tabbing}
xxxx\=xxxxx\=xxxxx\=\kill
SELECT * FROM R1 \\
\> FULL OUTER JOIN R2 \\
\> \> ON (R1.c5=R2.c5 AND R1.c4=R2.c4 AND \\
\> \> \>  R1.c3=R2.c3) \\
\> FULL OUTER JOIN R3 \\
\> \> ON (R3.c1=R1.c1 AND R3.c4=R1.c4 AND \\
\> \> \>  R3.c5=R1.c5);
\end{tabbing}
\end{query}
}

\onlythesis{
\begin{floatexample}
\begin{sqlindent}
\\
SELECT * FROM R1 \\
\>\> FULL OUTER JOIN R2 \\
\>\> \>\> ON (R1.c5=R2.c5 AND R1.c4=R2.c4 AND R1.c3=R2.c3) \\
\>\> FULL OUTER JOIN R3 \\
\>\> \>\> ON (R3.c1=R1.c1 AND R3.c4=R1.c4 AND R3.c5=R1.c5);
\end{sqlindent}
\caption{A query with attributes common to multiple joins (Query 4)}
\label{query:r1-r3}
\end{floatexample}
}

The tables R1, R2 and R3 were identical and each populated with 100,000
records. No indexes were built. As shown in
\reffig{fig:perf-r1-r3-sys1-pg-pyro}(a), both SYS1 and PostgreSQL chose sort
orders that do not share any common prefix. The plan chosen by PYRO-O is
shown in \reffig{fig:perf-r1-r3-sys1-pg-pyro}(b).  In the plan chosen by
PYRO-O, the two joins share a common prefix of {\em (c4, c5)}, and thus the
sorting effort is expected to be significantly less.  SYS2, not having an
implementation of full outer join, chose a union of two left outer joins.
The two left outer joins used to get a full outer join used different sort
orders making the union expensive, illustrating a need for coordinated
choice of sort orders. The execution timings for Query 4 on PostgreSQL and
SYS1 are shown in Figures \ref{fig:q2q3postgres} and \ref{fig:q2q3mssql}
respectively.

\eat{
The plan chosen by SYS2 is shown in \reffig{fig:perf-r1-r3-sys2}. SYS2, not
having an implementation of full outer join, choose a union of two left
outer joins.  The two left outer joins between R1 and R2 use different sort
orders. This, not only takes away the opportunity of reusing intermediate
results (sorted R1 and R2) but also makes the the UNION operator more
expensive. Note that a one-pass merge UNION requires the same sort order
from both inputs. 
}

\begin{figure*}
\begin{center}
\includegraphics[angle=0,height=2.4in,width=5.5in]{chapters/eio/fig/perf/plans/perf-r1-r3-mssql-pg-pyro.eps}
\end{center}
\caption{Plans for Query 4} 
\label{fig:perf-r1-r3-sys1-pg-pyro}
\end{figure*}

\subsubsection*{Experiment B3}
In this experiment we compare our approach of choosing orders, PYRO-O, with
the exhaustive approach, and a heuristic used by PostgreSQL.  PostgreSQL
uses the following heuristic: for each of the $n$ attributes involved in the
join condition, a sort order beginning with that attribute is chosen; in
each order, the remaining $n-1$ attributes are ordered arbitrarily. We
implemented PostgreSQL's heuristic in PYRO along with the extensions to
exploit partial sort orders and we call it PYRO-P.  The exhaustive approach,
called PYRO-E, enumerates all $n!$ permutations and considers partial sort
orders. In addition, we also compare with baseline PYRO, which chooses an
arbitrary sort order, and a variation of PYRO-O, called PYRO-O$^-$ that
considers only exact favorable orders (no partial sort).
\reffig{fig:perf-plancost} shows the estimated plan costs. Note the logscale
for y-axis. The plan costs are normalized taking the plan cost with
exhaustive approach to be 100. In the figure, Q3 and Q4 stand for Query 3
(Example ~\ref{query:outofstock}) and Query 4 (Example~\ref{query:r1-r3}) of
Experiments B1 and B2. Q5 and Q6 stand for Query 5 and Query 6, and are
shown below as Examples~\ref{query:ibank-trans} and
~\ref{query:ibank-basket} respectively.  For Q3 and Q4, as very few
attributes were involved in the join condition, PostgreSQL's heuristic along
with extensions to exploit partial sort orders, produced plans which were
close to optimal. However, for more complex queries the heuristic does not
perform well since it makes an arbitrary choice for secondary orders. 

\onlythesis{
{\small
\begin{floatexample}
\begin{sqlindent}
\\
SELECT T1.UserId, T1.BasketId, T1.ParentOrderId, T1.WaveId, T1.ChildOrderId, \\
 \>\> (T1.Quantity * T1.Price) as OrderValue, \\
 \>\> SUM(T2.Quantity * T2.Price) as ExecValue \\
FROM TRAN T1, TRAN T2 \\
WHERE T1.UserId=T2.UserId AND T1.ParentOrderId=T2.ParentOrderId AND \\
 \>\> T1.BasketId=T2.BasketId AND T1.WaveId=T2.WaveId AND \\
 \>\> T1.ChildOrderId=T2.ChildOrderId AND T1.TranType='New' AND \\
 \>\> T2.TranType='Executed' \\
GROUP BY T1.UserId, T1.BasketId, T1.ParentOrderId, T1.WaveId, T1.ChildOrderId;
\end{sqlindent}
\caption{Total value executed for a given order (Query 5)}
\label{query:ibank-trans}
\end{floatexample}
}
}

\onlyjournal{
\begin{query}
\label{query:ibank-trans}
Total value executed for a given order
\begin{tabbing}
xxxxxxxxx\=xxx\=\kill
SELECT \> T1.UserId, T1.BasketId, T1.ParentOrderId, \\
       \> T1.WaveId, T1.ChildOrderId, \\
       \> (T1.Quantity * T1.Price) as OrderValue, \\
       \> SUM(T2.Quantity * T2.Price) as ExecValue \\
FROM TRAN T1, TRAN T2 \\
WHERE \> T1.UserId=T2.UserId AND \\
      \> T1.ParentOrderId=T2.ParentOrderId AND \\
      \> T1.BasketId=T2.BasketId AND \\
      \> T1.WaveId=T2.WaveId AND \\
      \> T1.ChildOrderId=T2.ChildOrderId AND \\
      \> T1.TranType='New' AND \\
      \> T2.TranType='Executed' \\
GROUP BY \>\> T1.UserId, T1.BasketId, T1.ParentOrderId, \\
         \>\> T1.WaveId, T1.ChildOrderId;
\end{tabbing}
\end{query}
}

\onlyjournal{
\begin{query}
\label{query:ibank-basket}
Basket Analytics
\begin{tabbing}
xxxxxxxxx\=xxxxx\=\kill
SELECT * FROM BASKET B, ANALYTICS A \\
WHERE \> B.ProdType = A.ProdType AND \\
      \> B.Symbol = A.Symbol AND \\
      \> B.Exchange = A.Exchange;
\end{tabbing}
\end{query}
}
\onlythesis{
\begin{floatexample}
\begin{sqlindent}
SELECT * FROM BASKET B, ANALYTICS A \\
WHERE \>\> B.ProdType = A.ProdType AND B.Symbol = A.Symbol AND \\
      \>\> B.Exchange = A.Exchange;
\end{sqlindent}
\caption{Basket Analytics (Query 6)}
\label{query:ibank-basket}
\end{floatexample}
}

\begin{figure*}[ht]
%\hspace{-3ex}
\begin{tabular}{@{}c@{}c}
\begin{minipage}{0.5\textwidth}
\centerline {\includegraphics[angle=270,totalheight=2.0in,width=3.4in]{chapters/eio/fig/perf/plots/all-pyro-plancost.eps}}
\caption{Evaluating Different Heuristics} 
\label{fig:perf-plancost}
%\vspace{-10pt}
\end{minipage}
&
\begin{minipage}{0.5\textwidth}
\centerline{\includegraphics[angle=270,totalheight=2.0in,width=3.4in]{chapters/eio/fig/perf/plots/all-pyro-opttime.eps}}
\caption{Optimizer Scalability}
\label{fig:perf-opttime}
\end{minipage}
\end{tabular}
\end{figure*}

\subsection {Optimization Overheads}
The optimization overheads due to the proposed extensions were negligible.
During plan generation, the number of sort orders we try at each join or
aggregate node is of the order of the number of indices that are useful for
answering the query, which in most practical case is expected to be small.
\reffig{fig:perf-opttime} shows the scalability of the three heuristics.
For this experiment a query that joined two relations on varying number of
attributes was used. Though PYRO-P and PYRO-O take the same amount of time
in this experiment, in most cases, the number of favorable orders is much
less than the total number of attributes involved and hence PYRO-O generates
fewer interesting orders than PYRO-P. 

The plan-refinement algorithm presented in \refsec{subsec:approxalgo} was
tested with trees up to 31 nodes (joins) and 10 attributes per node. The
time taken was negligible in each case. The execution of plan refinement
phase took less than 6 ms even for the tree with 31 nodes.

Both the optimizer extensions and the extension to external-sorting (MRS)
were straight forward to implement.  The optimizer extensions neatly
integrated into our existing Volcano style optimizer.



==> chapters/eio/sections/sec_pso.tex <==
\section{Exploiting Partial Sort Orders} 
\label{sec:pso:chap:eio}
Often, sort order requirements of operators are partially satisfied by
indices or other operators in the input subexpressions. A prior knowledge of
partial sort orders available from inputs allows us to efficiently produce
the required (complete) sort order more efficiently. When operators have
flexible order requirements, it is thus important to choose a sort order
that makes maximum use of partial sort orders already available. We motivate
the problem with an example. \onlythesis{Consider the query shown
in~\refex{query:carcatalog}.} \onlyjournal{Consider
~\refquery{query:carcatalog} shown below.} Such queries frequently arise in
consolidating data from multiple sources, {\em e.g.,} in
extract-transform-load ({\small ETL}) tasks. The join predicate between the
two {\em catalog} tables involves four attributes and two of these
attributes are also involved in another join with the {\em rating} table.
Further, the order-by clause asks for sorting on a large number of columns
including the columns involved in the join predicate. 

\onecolonly{
\begin{floatexample}
%\noindent A query with complex join condition
\begin{sqlindent}
\\
SELECT \>\> c1.make, c1.year, c1.city, c1.color, c1.sellreason, 
            c2.breakdowns, r.rating \\
FROM  \>\> catalog1 c1, catalog2 c2, rating r \\
WHERE \>\> c1.city=c2.city AND c1.make=c2.make AND c1.year=c2.year AND \\
       \>\> c1.color=c2.color AND c1.make=r.make and c1.year=r.year  \\
ORDER BY c1.make, c1.year, c1.color, c1.city,
         c1.sellreason, c2.breakdowns, r.rating;
\end{sqlindent}
\label{query:carcatalog}
\caption{A Query with Many Join and Grouping Attributes}
\end{floatexample}
}

\twocolonly{
\begin{query}
\label{query:carcatalog}
\begin{tabbing}
xxxxxxxxx\=xxx\=\kill
\\
SELECT \> c1.make, c1.year, c1.city, c1.color, \\
       \> c1.sellreason, c2.breakdowns, r.rating \\
FROM  \> catalog1 c1, catalog2 c2, rating r \\
WHERE \> c1.city=c2.city {\small AND} c1.make=c2.make {\small AND} \\
      \> c1.year=c2.year {\small AND} c1.color=c2.color {\small AND} \\
      \> c1.make=r.make and c1.year=r.year  \\
ORDER BY \>\> c1.make, c1.year, c1.color, c1.city, \\
         \>\> c1.sellreason, c2.breakdowns, r.rating;
\end{tabbing}
\end{query}
}

\begin{figure*}[ht]
\begin{tabular}{@{}c@{}c}
\begin{minipage}{0.5\textwidth}
\centerline{\includegraphics{chapters/eio/fig/naiveplan-mod.eps}}
\caption{A Na\"ive Merge-Join Plan}
\label{fig:naiveplan}
\end{minipage}
&
\begin{minipage}{0.5\textwidth} 
\centerline{\includegraphics{chapters/eio/fig/betterplan-mod.eps}}
\caption{Optimal Merge-Join Plan}
\label{fig:optplan}
\end{minipage}
\end{tabular}
\end{figure*}

The two catalog tables contain 2 million records each, and have average
tuple sizes of 100 and 80. We assume a disk block size of 4K bytes and 10000
blocks (40 MB) of main memory for sorting.  The table {\em catalog1} is
clustered on {\em year} and the table {\em catalog2} is clustered on {\em
make}. The {\em rating} table has a secondary index on the {\em make}
column, and the index includes the {\em year} and {\em rating} columns in
its leaf pages ({\em i.e.,} the index covers the query).
Figures~\ref{fig:naiveplan} and ~\ref{fig:optplan} show two different plans for
the example query. Numbers in the parentheses indicate estimated cost of the
operators in number of I/Os (CPU cost is appropriately translated into I/O
cost units). Edges are marked with the number of tuples expected to flow on
that edge and their average size.  For brevity, the input and output orders
for the sort enforcers are shown using only the starting letters of the
column names. Though both plans use the same join order and employ
sort-merge joins, the second plan is expected to perform significantly
better than the first.

\subsection{Changes to External Sort}
\label{subsec:extsort}
External sorting algorithms have been studied extensively but in isolation.
The standard replacement selection~\cite{KNUTH} for run formation well
adapts with the extent to which input is presorted. In the extreme case,
when the input is fully sorted, it generates a single run on the disk and
avoids merging altogether. \eat{Per-{\AA}ke} Larson~\cite{PAUL} revisits run
formation in the context of query processing and extends the standard
replacement selection to handle variable length keys and to improve locality
of reference. Estivill-Castro and Wood~\cite{WOOD}
provide a survey of adaptive sorting algorithms. The technique we propose in
this section to exploit partial sort orders is a specific optimization in
the context of multi-key external sorting. We observe that, by exploiting
prior knowledge of partial sort order of input, it is possible to eliminate
disk I/O altogether and have a completely pipelined execution of the sort
operator. 

\noindent We use the following conventions: $o, o_1, o_2$ {\em etc.} refer
to sort orders. A sort order of size $n$ is a sequence of attributes/columns
$(a_1, a_2, \ldots, a_n)$. Sort direction (ascending/descending) is
ignored; our techniques are applicable independent of the sort direction. 

\begin{itemize}
%\addtolength{\itemsep}{-5pt}
%{\small
\item $\epsilon$  : Empty (no) sort order
\item {\em attrs}$(o)$ : The set of attributes in sort order $o$
\item $|o|$ : Number of attributes in the sort order $o$
\item $o_1 \leq o_2$  : Order $o_2$ subsumes order $o_1$ ($o_1$ is a 
      prefix of $o_2$)
\item $o_1 < o_2$   : Order $o_1$ is a strict prefix of $o_2$ 
%}
\end{itemize}

Consider a case where the sort order to produce is $(col_1, col_2)$ and the
input already has the order $(col_1)$. Standard replacement-selection writes
a single run with all the tuples to the disk and reads it back again; this
breaks the pipeline and incurs substantial I/O for large inputs. It is not
difficult to see how the standard replacement selection can be modified to
exploit the partial sort orders. Let $o=(a_1, a_2, \ldots, a_n)$ be the
desired sort order and $o'=(a_1, a_2, \ldots, a_k)$, $k < n$ be the partial
sort order known to hold on the input. At any point during sorting we need
to retain only those tuples that have the same value for attributes $a_1,
a_2, \ldots, a_k$. When a tuple with a new value for these set of attributes
is read, all the tuples in the heap (or on disk if there are large number of
tuples matching a given value of $a_1, a_2, \ldots, a_k$) can be sent to the
next operator in sorted order. Thus in most cases, partial sort orders allow
a completely pipelined execution of the sort. Exploiting partial sort orders
in this way has several benefits:

\begin{enumerate}
\item Let $o=(a_1, a_2, \ldots, a_n)$ be the desired sort order and $o'=(a_1,
a_2, \ldots, a_k)$, $k < n$ be the partial sort order known to already hold
on the input. We call the set of tuples that have the same value for
attributes $(a_1, a_2, \ldots, a_k)$ as a {\em partial sort segment}. If each
{\em partial sort segment} fits in memory (which is quite often the case in
practice), the entire sort operation can be completed without any disk I/O.

\item Exploiting partial sort orders allows us to output tuples early (as
soon as a new segment starts). In a pipelined execution this can have large
benefits. Moreover, producing tuples early has immense benefits for Top-K
queries and situations where the user retrieves only some result tuples.

\item Since sorting of each {\em partial sort segment} is done
independently, the number of comparisons are significantly reduced. Note
that we empty the heap every time a new segment starts and hence insertions
into heap will be faster. In general, independently sorting $k$ segments
each of size $n/k$ elements, has the complexity $O(n\ log(n/k))$ as against
$O(n\ log(n))$ for sorting all $n$ elements.  Further, while sorting each
{\em partial sort segment} comparisons need to be done on fewer attributes,
$(a_{k+1},\ldots, a_n)$ in the above case.
\end{enumerate}

Our experimental study presented in \refsec{sec:perf:chap:eio} confirms that
the benefits of exploiting partial sort orders can be substantial, and yet
none of the systems we evaluated exploited the partial sort orders. 

\eat{
For commercial systems we confirmed our claim by using special nested rank
queries to partially sort multiple groups of tuples and comparing the time
taken with an equivalent sort on the same system. For PostgreSQL (version
8.1.3) the source code was available and confirmed our claim.
}

\subsection{Optimizer Extensions for Partial Sort Orders}
\label{subsec:optchangepso}
In this section we assume operators have fixed sort order requirements, and
we focus only on incorporating partial sort orders. We deal with flexible
sort order requirements of operators in subsequent sections.

\noindent We use the following notations: 
\begin{itemize}
\onlythesis{\addtolength{\itemsep}{-3mm}}
\item $o_1 \wedge o_2$ : Longest common prefix between sort orders $o_1$ 
                         and $o_2$
\item $o \wedge s$     : Longest prefix of sort order $o$ such that 
                         each attribute
                         in the prefix belongs to the attribute set $s$ 
\item $o_1 + o_2$      : Sort order obtained by concatenating $o_1$ and $o_2$
\item $o_1 -  o_2$     : Sort order $o'$ such that $o_2 + o' = o_1$ 
                         (defined only when $o_2 \leq o_1$)
\item {\em coe}$(e, o_1, o_2)$  : The cost of enforcing order $o_2$ on the
                         result of expression $e$ which already has order $o_1$ 
\item $N(e)$           : Expected size, in number of tuples, of the 
                         result of expression $e$
\item $B(e)$           : Expected size, in number of blocks, of the
                         result of expression $e$
\item $D(e, s)$        : Distinct values for attribute(s)
                         $s$ of expression $e$. 
                         {\small $D(e, s)=N(\Pi_{s}(e))$}
\item $cpu\_cost(e, o)$ : CPU cost of sorting the result of $e$ to get order $o$
\item $M$              : Number of memory blocks available for sorting
\end{itemize}


The {\em Volcano} optimizer framework~\cite{GRA93} assumes that an algorithm 
(physical operator) either guarantees a required sort order fully or it 
does not. Further, a physical property enforcer (such as sort) only knows 
the property to be enforced and has no information about the properties 
that hold on its input. The optimizer's cost estimate for the enforcer 
thus depends only on the required output property (sort order).
In order to remedy these deficiencies we extended the optimizer in the 
following way: 
consider an optimization goal $(e, o)$, where $e$ is the expression 
and $o$ the required output sort order. If the physical operator 
being considered for the logical operator at the root of $e$ guarantees
a sort order $o' < o$, then the optimizer adds a partial sort enforcer 
{\em enf} to enforce $o$ from $o'$.  We use the following cost model
to account for the benefits of partial sorting.

\eat{
{\bf Cost Model} \\
We estimate the cost of sorting the result of expression $e$ with a memory 
of $M$ blocks to obtain an order $o$ as follows:
}

{\small
\[coe(e, \epsilon, o) = 
            \left \{ 
            \begin{array}{ll}
               \mbox{\em {cpu-cost}}(e, o)  & \mbox{if $B(e)\leq M$} \\
                          B(e)(2\lceil log_{M-1} (B(e)/M)\rceil + 1) & 
               \mbox{otherwise}
            \end{array}
            \right. \]
}

\noindent
If $e$ is known to have the order $o_1$, we estimate the cost of obtaining
an order $o_2$ as follows:

\noindent
$coe(e, o_1, o_2)$ $=\ D(e,\ ${\em attrs}$(o_s)) * coe(e', \epsilon, o_r)$,
where $o_s=o_2 \wedge o_1$, $o_r=o_2-o_s$ and $e'=\sigma_{p}(e)$, where $p$
equates attributes in $o_s$ to an arbitrary constant. Intuitively, we
consider the cost of sorting a single {\em partial sort segment}
independently and multiply it by the number of segments.  Note that we
assume uniform distribution of values for {\em attrs}$(o_s)$. Therefore, we
estimate $N(e')=\lceil N(e)/D(e,\ ${\em attrs}$(o_s)) \rceil$ and
$B(e')=\lceil B(e)/D(e,\ ${\em attrs}$(o_s)) \rceil$.  When the actual
distribution of values is available, a more accurate cost model that does
not rely on the uniform distribution assumption can be used.



==> chapters/eio/sections/sec_relwork.tex <==
\section{Related Work} 
\label{sec:relwork:chap:eio}
Both System R~\cite{SEL79} and Volcano~\cite{GRA93} optimizers consider
plans that could be locally sub-optimal but provide a sort order of interest
to other operators, and thus yield a better plan overall. However, both
System R and Volcano assume that operators have one or few {\em exact} sort
orders of interest. This is not true of operators like merge-join,
merge-union, grouping and duplicate elimination, which have a factorial number
of interesting orders.  Heuristics such as the PostgreSQL heuristic, are
commonly used by optimizers. Details of the heuristics are publicly
available only for PostgreSQL. Further, System R and Volcano optimizers
consider only those sort orders as useful that completely meet an order
requirement. Plans that partially satisfy a sort order requirement are not
handled.  In this \onlythesis{chapter}\onlyjournal{paper} we addressed 
these two issues.

The seminal work by Simmen et.al.~\cite{MALK96} describes techniques to
infer sort orders from functional dependencies and predicates applied, and
thereby avoids redundant sort enforcers in the plan. Simmen
et.al.~\cite{MALK96} briefly mention the problem of non-exact sort order
requirements and mentions an approach of propagating an order specification
that allows any permutation on the attributes involved.  Though such an
approach is possible for single input operators like group-by, it cannot be
used for operators such as merge-join and merge-union for which the order
guaranteed by both inputs must match.  Moreover, the paper does not make it
clear how the flexible order requirements are combined at other joins and
group-by operators.  Simmen et.al.~\cite{MALK96} also note that the approach
of carrying a flexible order specification increases the complexity of the
code significantly. Our techniques do not use flexible order specifications
and hence can be incorporated into an existing optimizer with minimal
changes.  Further, our techniques work uniformly across all types of
operators that have a flexible order requirement.  

Claussen et.al.~\cite{CLAUS:VLDBJ00} explore early-sorting as a means to
reduce sorting cost in query plans. The key idea is to avoid sorting of
large intermediate join results by pushing sorting to base relations, and
using order preserving hash joins.  There has been significant work on
avoiding redundant sorting by inferring sort orders and groupings using
functional dependencies \cite{MALK96,MITCH:VLDB03,MOER:VLDB04,MOER:ICDE04}.
These techniques are complementary to our work.


==> chapters/eio/sections/sec_summary.tex <==
\section{Summary}
\label{sec:summary:chap:eio}
In this \onlythesis{chapter}\onlyjournal{paper} we addressed the problem of
choosing efficient sort orders for sort-based operators such as merge-join
and sort-based grouping.  We showed that even a simplified version of the
problem is {\em NP-Hard}, and proposed principled heuristics for choosing
interesting orders. Our heuristics are guided by the notion of favorable
orders.  We take into account important issues such as partially matching
sort orders and attributes common to multiple operators.  We then explained
how the solution can be used for choosing efficient parameter sort orders
for nested queries. We presented a detailed experimental study on widely
used database systems, and the results showed significant performance
improvements due to the proposed techniques for several queries. 


==> chapters/intro/chap_intro.tex <==
\chapter{Introduction}
\label{chap:intro}
Database applications with complex queries have become commonplace.  For
example, nested queries, queries containing complex joins and grouping, and
queries that make use of procedural extensions to {\small SQL} are
frequently encountered in database applications. Applications also make use
of stored procedures, which use a mix of procedural language constructs and
{\small SQL}.

In such applications, queries and updates to a database are often executed
repeatedly, with different values for their parameters. Repeated invocations
of queries and updates can occur due to several reasons. For example,
consider a nested query in which a sub-query or inner query would be nested
below an outer query block. \refex{ex:q1} shows a nested query on the TPC-H
schema~\cite{TPCH}. The query retrieves {\em orders} none of whose {\em
lineitems} were shipped on the day the order was placed. 

\begin{floatexample}
\begin{sqlindent}
\\
SELECT \>\> o$\_$orderkey, o$\_$orderdate FROM ORDERS \\
WHERE  \>\> o$\_$orderdate NOT IN ( 
             \>\>\>\>\ \  SELECT l$\_$shipdate FROM LINEITEM \\
       \>\>  \>\>\>\>\ \  WHERE l$\_$orderkey = o$\_$orderkey);
\end{sqlindent}
\caption{A Nested Query}
\label{ex:q1}
\end{floatexample}

Sub-queries can use parameters whose values are bound by the outer query
block as illustrated in \refex{ex:q1}.  The default way of executing nested
queries is to iteratively invoke the sub-query for each parameter binding
produced by the outer query block. Similarly, when a query makes use of a
user-defined function ({\small UDF}) in its {\small WHERE/SELECT} clause,
the {\small UDF} will be invoked multiple times with different values for
its parameters. As a result, queries used inside the {\small UDF} get
executed repeatedly.  External programs that perform batch processing are
another important reason for repeated invocation of queries/updates.  Such
programs call database stored-procedures repeatedly by iterating over a set
of parameters, and as a result, cause repeated invocations of queries and
updates contained in the body of the stored-procedure. Application programs,
stored-procedures and user-defined functions can also make explicit use of
looping constructs, such as {\small FOR/WHILE/CURSOR} loops, and invoke
queries/updates inside the loop.

\section{Problem Overview and Motivation} 
Iterative execution plans for queries and updates are often very inefficient
and result in poor application performance.  Lack of opportunity for sharing
of work ({\em e.g.}, disk IO) between multiple invocations of the
query/update is a key reason for the inefficiency of iterative plans. Random
disk IO and network round-trip delays also degrade the performance of
iterative plans.  Consider the query shown in \refex{ex:q1}.  A na\"\i ve
nested iteration plan for the query would invoke the sub-query on the
LINEITEM table for every tuple of the ORDERS relation. If a useful index is
not present to answer the sub-query, the LINEITEM table would be scanned
once for each invocation of the sub-query. In practice, an index on
the {\em o$\_$orderkey} column is expected to exist and the sub-query can be
evaluated with an index lookup. However, repeated index lookups
result in a large number of random IOs and can lead to poor performance.

An important technique used to address poor performance of nested queries is
query decorrelation, also known as query unnesting\cite{KIM82,KIE84,GAN87,
DAYAL87,MUR89, SPL96,GAL01,GAL07}. Query decorrelation aims at rewriting a
given nested query as an equivalent non-nested query by making use of set
operations such as joins and outer-joins.
\refex{ex:q1decorr}\footnote{Standard SQL does not provide a construct for
anti semi-join. The syntax used here is merely to illustrate the internal
representation after decorrelation} shows a decorrelated form of the query
in \refex{ex:q1}.

\begin{floatexample}
\begin{sqlindent}
\\
SELECT \>\> o$\_$orderkey, o$\_$orderdate \\
FROM   \>\> ORDERS ANTI SEMI JOIN LINEITEM ON \\
       \>\> o$\_$orderdate=l$\_$shipdate AND o$\_$orderkey=l$\_$orderkey;
\end{sqlindent}
\caption{A Decorrelated Form of the Nested Query in \refex{ex:q1}}
\label{ex:q1decorr}
\end{floatexample}

By rewriting nested queries using set operations, decorrelation expands the
space of alternative execution strategies, which otherwise would be
restricted only to iterative execution plans. The query optimizer, can now
consider set-oriented strategies, such as hash-join and merge-join to answer
a nested query.  The query optimizer estimates the cost of alternative
plans, including the iterative execution plans, and chooses the one with the
least expected cost. 

\input{chapters/intro/examples/udf-count-offers.tex}

Although decorrelation techniques are applicable for a wide variety of
nested queries, iterative execution of queries and updates can still occur 
due to the following reasons:

\begin{enumerate}
\item  For several queries, even when decorrelation is applicable, an 
       iterative execution plan might be the most efficient of the 
       available alternatives~\cite{GRA03,JUN98}.

\item  Known decorrelation techniques are not applicable for complex nested
       blocks such as those containing procedural code. For example,
       consider the query shown in \refex{ex:udf-count-offers}. The
       user-defined function {\em count-offers} used in the {\em where}
       clause of the query forms a nested block with procedural code and
       sub-queries inside it.  Decorrelation techniques proposed till date
       are not applicable to such queries, except in special cases when the
       body of the {\small UDF} is very simple. 

\item  Decorrelation is also not applicable when queries and updates 
       are invoked from imperative loops ({\em e.g.,} a {\em while} loop) 
       of external programs and user-defined functions or stored procedures.
\end{enumerate}

The focus of this thesis is to develop query evaluation, optimization and
program transformation techniques to improve the performance of repeatedly
invoked parameterized sub-queries, updates, stored-procedures and
user-defined functions. To this end we make the following contributions.

\section{Summary of Contributions}
%The focus of this thesis is to develop query evaluation, optimization and
%program transformation techniques to improve the performance of repeatedly
%invoked parameterized sub-queries, updates, stored-procedures and
%user-defined functions. To this end we make the following contributions.

\begin{enumerate}
\item We propose new query evaluation techniques, which make use of {\em sort
      order} of parameter bindings and {\em state retention} across calls, 
      to speed up the evaluation of nested queries. These alternative
      techniques augment the optimizer's plan space with improved nested 
      iteration plans.  We show how to extend a cost-based query optimizer 
      so that the effects of sorted parameter bindings and state retention
      are taken into account. 

\item We address the problem of choosing optimal sort orders during 
      query plan generation. The problem of choosing optimal
      sort orders is important not only for nested queries, but also for
      queries containing joins, aggregates and other set operations. 

%\item We develop program transformation rules that enable set-orientation 
%      of complex iterative programs through batching of parameter bindings. 
\item We address the problem of efficient evaluation of repeatedly called
      user-defined functions and stored-procedures, which contain {\small
      SQL} queries and updates embedded within procedural code. We present
      an approach, based on program analysis and transformation, to
      automatically generate batched forms of procedures. Batched forms of
      procedures work with a set of parameter bindings and thereby enable
      set-oriented processing of queries/updates inside the procedure
      body. 
\end{enumerate}

\noindent We provide details of each of these contributions, below.

\subsection{Improved Iterative Execution with Parameter Sorting}
Parameterized sub-queries being pure (side-effect free) functions, it is
possible to reorder their invocations without affecting the results. Ordered
(sorted) parameter bindings provide several opportunities for speeding up
the sub-query evaluation.  For example, it is known~\cite{GRA03} that
ordered parameter bindings reduce random disk access and yield better cache
hit ratio. We propose additional query evaluation techniques, which exploit
sorted parameter bindings by retaining state across calls.

\noindent 
{\em Restartable Scan:} 
Nested sub-queries or queries inside user-defined functions often select
tuples from a relation, one of whose columns matches the parameter value.
The selection predicate involving the parameter is called {\em correlation
predicate}. In the query of \refex{ex:q1}, the selection predicate {\em
l$\_$orderkey=o$\_$orderkey} in the sub-query is a correlation predicate. A
relation referenced by the sub-query is called an inner relation. If the
inner relation is stored sorted (clustered) on the column appearing in the
correlation predicate, making the sub-query invocations in the sorted order
of parameter values allows the following: at the end of each invocation, the
scan for the inner relation can remember its position in the relation
and restart from that point in the next invocation. Thus, the 
restartable scan enables us to achieve the efficiency of set-oriented
algorithms like merge-join to situations where a merge-join is not
directly applicable.  

\noindent {\em Incremental Computation of Aggregates:} 
Nested queries where the sub-query computes an aggregate value are often
encountered in practice and are known as nested aggregate queries.  For
nested aggregate queries having non-equality correlation predicates ($<,
\leq, >$ or $\geq$), known query processing strategies are very inefficient.
We describe a strategy, which by employing a combination of restartable
scan and a state retaining aggregate operator, computes the result of the
nested aggregate query very efficiently.

\noindent {\em Plan Generation:}
While considering alternative plans for a given query, it is imperative that
the query optimizer must take into account query execution plans that
exploit ordered parameter bindings and estimate their cost appropriately. We
present a cost-model of operators, which takes into account the effect of sorted
parameter bindings. We then address the problem of extending a cost-based
query optimizer to take into account state retention of operators and the
effect of sorted parameter bindings. We have implemented the proposed
ideas and present experimental results, which show significant benefits
for several classes of queries.

A key challenge in optimizing queries by taking parameter sort orders into
account, is to decide the optimal sort order of parameters. This problem is
important not only for nested queries, but also for queries containing
joins, aggregates and other set operations.  We describe it next.



\subsection{Choosing Sort Orders in Query Optimization}
For a given set of sub-query parameters, several sort orders are possible.
Different sort orders can result in different plan costs and the query
optimizer must make a judicious choice of sort orders to use.  Sort orders,
in general, play an important role in query processing. Algorithms that rely
on sorted inputs are widely used to implement joins, grouping, duplicate
elimination and other set operations. The notion of {\em interesting
orders}~\cite{SEL79} has allowed query optimizers to consider plans that
could be locally sub-optimal, but produce ordered output beneficial for
other operators, and thus be part of a globally optimal plan.  However, the
number of interesting orders for most operators is factorial in the
number of attributes involved. For example, all possible sort orders on the
set of join attributes are of interest to a merge-join.  Considering
the exhaustive set of sort orders is prohibitively expensive as the input
sub-expressions must be optimized for each of these sort orders.  The
following factors make the problem of choosing sort orders non-trivial.

\begin{itemize}
\item Clustering and secondary indices that cover the query (an index is
said to cover a query if it includes all the attributes required to answer
the query) make it possible to produce some sort orders at much lesser cost
than others.

\item Partially available sort orders can greatly reduce the cost of
intermediate sorting step. For example, if the input is sorted on attribute
$a$, it is more efficient to obtain the sort order $(a,b)$ as compared to the
sort order $(b,a)$.

\item Attributes common to multiple joins, group-by and set operations must
be taken into account for choosing globally optimal sort orders.  For
example, consider the following query.
%in \refex{ex:q2}. 

\singlespace 
{\em
%\begin{floatexample}
\begin{sqlindent}
%\\
SELECT \>\> R.a, S.b, T.c FROM  R, S, T \\
WHERE  \>\> R.a = S.a AND R.b = S.b AND S.b = T.b AND S.c = T.c\\
GROUP BY R.a, S.b, T.c;
\end{sqlindent}
}
\doublespace
%\caption{}
%\label{ex:q2}
%\end{floatexample}

A good query execution plan makes a coordinated choice of sort orders for
the two joins and the group-by, so that the cost of intermediate sorting
steps is minimized.

%For a globally optimal plan, a coordinated choice of sort orders for the two
%joins and the group-by is necessary. Such a choice must minimize the cost of
%intermediate sorting steps.

\item Binary operators like merge-join, can accept any sort order on
the attributes involved, but require a matching sort order from their 
two inputs. 
\end{itemize}

Previous work on sort orders has mainly focused on inferring sort orders from
functional dependencies and predicates in the input sub-expression.
Simmen et.al.~\cite{MALK96} highlight the importance of choosing good sort
orders for operators like group-by, which have flexible order requirements.
But their approach cannot be used for binary operators such as merge-join,
which require a matching sort order from their two inputs.

We show that even a simplified version of the problem of choosing sort
orders is {\em NP-Hard}. 
\eat{
The simplified version of the problem is equivalent
to \refproblem{problem1} stated below.

\noindent
\begin{eioproblem}
\label{problem1}
Let $T$ be a binary tree of order $n$, with vertex set $V(T)$ and edge set
$E(T)$.  Each node $v_i$ $(i=1,\ldots n)$ is associated with an attribute
set $s_i$.  Find a sequence of permutations $p_1,p_2 \ldots p_n$, where
$p_i$ is a permutation of set $s_i$, such that the benefit function
$\mathcal{F}$ is maximum.
\[ \mathcal{F} = \sum_{\forall v_iv_j\in E(T)} |p_i \wedge p_j|\]
\[\text{where } |p_i \wedge p_j| \text{ denotes the length of the longest}
\text{ common prefix between } p_i \text { and } p_j.
\]
\end{eioproblem}

We give a polynomial time algorithm to solve \refproblem{problem1}, when the
tree is a path. Solving the problem for paths is important as left-deep and
right-deep join plans result in a problem instance on paths. Further, we
give a 1/2-factor approximation to \refproblem{problem1} by making use of
the algorithm for paths. 
}
We then give an approach to address the general
case of the problem of choosing sort orders. 

\begin{enumerate}
\item We introduce the notion of {\em favorable} orders, which
      characterizes the set of sort orders easily producible on the
      the result of an expression.  The notion of favorable 
      orders allows us to consider promising sort orders during plan 
      generation. 

\item We show how a cost-based query optimizer can be extended to
      identify favorable orders and make use them to choose good 
      sort orders during plan generation. Our optimizer extensions
      also take into account plans that may not completely 
      produce a required sort order but produce only a part (prefix) 
      of the required sort order. When a sort order is partly
      available, a partial sort operator is
      used to obtain the complete (desired) sort order. The 
      partial sort operation uses a modified version of the 
      standard external-sorting algorithm.

\item We introduce a plan refinement phase in which the sort orders 
      chosen during plan generation are further refined to take into
      account attributes common to different operators, and thus reduce
      the cost of intermediate sorts further, when possible. 
      %For this, we 
      %make use of the 1/2-approximation algorithm for \refproblem{problem1}.
\end{enumerate}

We have implemented the proposed techniques in a cost-based query optimizer, 
and we carry out a performance comparison of the plans generated by our
optimizer with those of two widely used database systems. The results
show performance benefits up to 50\%.


\subsection{Rewriting Procedures for Batched Bindings}
Several data retrieval and update task need more expressive power than what
standard {\small SQL} offers. Therefore, many applications perform database
queries and updates from within procedural application code. Database
systems also support stored procedures and user-defined functions ({\small
UDF}s), which can use a mix of procedural constructs and {\small SQL}.
Repeated execution of {\small UDF}s and stored procedures can occur if
queries make use of {\small UDF}s in their {\small WHERE} or {\small SELECT}
clause, or if a stored procedure is invoked from external batch processing
applications.  In \refex{ex:udf-count-offers}, the function {\em
counter$\_$offers} gets invoked for every tuple in the {\em sellorders}
table. This in turn results in multiple invocations of queries inside the
function body. Known decorrelation techniques do not apply to such cases and
hence most database systems are forced to choose iterative execution plans.

%\input{../chapters/bpo/examples/udf-travcat.tex}
%\input{udf-travcat.tex}

An important technique to speed up repeated invocation of such
procedures/functions is parameter batching. Parameter batching allows the
choice of efficient set-oriented plans for queries and updates. For example,
the the {\em batched form} of the {\small UDF} {\em count$\_$offers} would
take a set of triplets {\em (itemcode, amount, curcode)} and return a set
comprising of the function's results for each triplet. By working with a set
of parameters, the batched form can avoid repeated calls to the queries
contained inside the function body. For instance, the batched form of the
{\small UDF} {\em count$\_$offers}, can issue a single join query to obtain
the exchange rates for all the required currencies. Assuming the set of
parameters to the {\small UDF} is available in a temporary relation {\em
pbatch}, the query issued by the batched form of {\em count$\_$offers} can
be as follows:

\singlespace 
{\em
\begin{sqlindent}
SELECT pb.curcode, cx.exchrate FROM curexch cx, pbatch pb \\
WHERE  cx.ccode = pb.curcode; 
\end{sqlindent}
}
\doublespace

\noindent The two key challenges in exploiting batching lie in developing
techniques to
\begin{enumerate}
\item automatically rewrite a given procedure to work with a batch of
      parameters bindings. In other words, to generate the {\em batched
      form} of a given procedure.  It is possible for an application
      developer to manually create the batched form of a procedure,
      but the process is time consuming and error prone. 
\item automatically rewrite a program, which iteratively invokes a database
      procedure from within an imperative loop, such as a {\em while}
      loop, so that the rewritten program makes a single invocation
      of the batched form of the procedure.
\end{enumerate}

We present an approach, based on program analysis, to automate the
generation of batched forms of procedures and replace iterative calls by
code to create parameter batch and then call the batched form.  The approach
comprises of a set of program transformation rules, which make use of
conditions on the data dependence graph of the given program. The data
dependence graph gives information about various types dependencies between
program statements and is obtained through program analysis. 

To the best of our knowledge no previously published work addresses the
problem of rewriting procedures to accept batched bindings. Lieuwen and
DeWitt\cite{LIEUWEN92} consider the problem of optimizing set iteration
loops in database programming languages. The goal of their work is to
convert nested set iteration loops arising in object-oriented database
languages into joins, and they propose a program transformation based
approach to achieve this. The rewrite rules proposed in our thesis share
some similarities with their work, but are designed to address the problem
of batching database calls made from programs written in general procedural
languages.  Our rewriting technique can be used with complex
programs, written using a rich set of language constructs such as
set-iteration (or cursor) loops, {\em while} loops, control flow statements
({\em if-then-else}) and assignment statements. Our rewrite rules make use
of some of the techniques, such as {\em loop splitting}, known in the
context of parallelizing compilers~\cite{KENEDY90}. 

In many situations, the inter-statement data dependencies within a program
may not permit set-oriented evaluation of a specific query inside the
program body. We show that by appropriately reordering the program
statements and by introducing temporary variables, we can enable
set-oriented evaluation in large number of cases. 

Our rewrite rules can conceptually be used with any language.  We have
prototyped the rewrite techniques for a subset of Java.  We present our
performance study on examples taken from three real-world applications.  The
results are very promising and show performance benefits up to 75\% due to
the proposed rewriting techniques.

\section{Organization of the Thesis}
This thesis is organized as follows. \refchap{chap:nqo} describes our work
on optimizing nested queries by exploiting parameter sort orders.  This is
followed by \refchap{chap:eio}, which addresses the problem of choosing
interesting sort orders.  \refchap{chap:bpo} addresses the problem of
parameter batching for procedure calls. \refchap{chap:concl} concludes the
thesis with some comments on possible directions for future work.



==> chapters/nqo/algos/algo.tex <==
\begin{figure}[ht]
\begin{minipage}{1.0\textwidth}
\algsize{
\ordinalg{
Procedure {\bf PhysDAGGen} \\
Inputs: \>\> {\em e}, logical equivalence node for the expression \\
        \>\> {\em p}, physical property required on the output \\
        \>\> {\em s}, sort order guaranteed on the parameter bindings \\
Output: \>\> Generates the physical plan space and returns the physical 
             equivalence node \\
BEGIN \\
\>    If a physical equivalence node $n_{p}$ exists for {\em e, p, s} in 
      the memo structure \\
\>\>        return $n_{p}$ \\
\>    Create an equivalence node $n_{p}$ for {\em e, p, s} and add it 
      to the memo structure \\
\>    For each child logical operation node {\em o} of {\em e} \\
\>\>        If({\em o} is an instance of {\em ApplyOp}) \\
\>\>\>            ProcApplyNode({\em o}, {\em s}, $n_{p}$) \\
\>\>        else \\
\>\>\>            ProcLogicalOpNode({\em o}, {\em p}, {\em s}, $n_{p}$) \\
\>    For each enforcer {\em f} that generates property {\em p} \\
\>\>        Create an enforcer node $o_{f}$ under $n_{p}$ \\
\>\>        Set the input of $o_{f}$ = PhysDAGGen({\em e}, $\epsilon$, {\em s}) \\
\>    return $n_{p}$ \\
END
}
}
\end{minipage}
\caption{Main Algorithm for Physical Plan Space Generation}
\label{fig:PhyAlgo}
\end{figure}



==> chapters/nqo/algos/get_int_orders.tex <==
\begin{figure}[t]
\begin{minipage}{0.5\textwidth}
\algsize{
\ordinalg{
Set$<$Order$>$ {\bf GetInterestingOrders}(LogEqNode {\em e}, \\
\>\>\>\>Map {\em plm}, int {\em l}) \\ %$\{$ \\
\>    If the set of interesting orders {\em i$\_$ords} for ({\em e},{\em plm}) \\
\>    is already found \\
\>\>        return {\em i$\_$ords} \\
\>    Create an empty set {\em result} of sort orders for ({\em e},{\em plm})\\
\>    For each logical operation node {\em o} under {\em e} \\ %$\{$\\
\>\>        For each algorithm {\em a} for {\em o} \\ %$\{$ \\
\>\>\>            Let $s_{a}$ be the sort order of interest  \\
\>\>\>            to {\em a} on the unbound parameters in {\em e} \\
\>\>\>            If $s_{a}$ is a valid order under {\em plm} and $s_{a}$ $\notin$ {\em result} \\ 
\>\>\>\>                Add $s_{a}$ to {\em result} \\
\>\>\>            For each input logical equivalence node \\
\>\>\>            $e_{i}$ of {\em a} \\ %$\{$ \\
%\>\>\>\>                {\em childOrd} = GetInterestingOrders($e_{i}$) \\
\>\>\>\>                If ({\em o} is an {\em Apply} operator AND \\
\>\>\>\>\>                $e_{i}$ is a {\em use} input) \\ %$\{$ \\
%\>\>\>\>\>                  // Augment the parameter-level map \\
\>\>\>\>\>                  {\em newLevelMap} = clone({\em plm}) \\
%\>\>\>\>\>                  {\em bindPLM} = GetParamNestLevel(\\
%\>\>\>\>\>\>\>                              {\em o.bindInput}, $l$) \\
%\>\>\>\>\>                  Add each mapping in {\em bindPLM} \\
%\>\>\>\>\>                  to {\em newLevelMap} \\
%\>\>\>\>\>                  Let $ll$ be the highest level number in \\
%\>\>\>\>\>                  {\em newLevelMap}\\
\>\>\>\>\>                  For each variable {\em v} bound by {\em o.bindInput} \\ %$\{$ \\
\>\>\>\>\>\>                    newLevelMap.add({\em v}, {\em l}) \\
%\>\>\>\>\>                  $\}$\\
\>\>\>\>\>                {\em childOrd} = GetInterestingOrders($e_{i}$, \\
\>\>\>\>\>\>\>                             {\em newLevelMap}, $l+1$) \\
%\>\>\>\>\>\>\>                             {\em newLevelMap}, $ll+1$) \\
\>\>\>\>\>                 {\em childOrd} = GetAncestorOrders(\\
\>\>\>\>\>\>\>                 {\em childOrd}, {\em o.bindInput}) \\
%\>\>\>\>                $\}$ \\
\>\>\>\>                Else \\ %$\{$ \\
\>\>\>\>\>                {\em childOrd} = GetInterestingOrders($e_{i}$, \\
\>\>\>\>\>\>\>\>                                     {\em plm}, {\em l}) \\
%\>\>\>\>                $\}$ \\
\>\>\>\>                {\em result} = {\em result} $\cup$ {\em childOrd} \\
%\>\>\>            $\}$\\
%\>\>        $\}$\\    
%\>    $\}$\\
\>    return {\em result} \\
%$\}$
end proc
}
}
% \end{minipage}
% \caption{Get Interesting Sort Orders}
% \label{fig:GetOrdersAlgo}
% \end{figure}
% 
% 
% \begin{figure}[ht]
% \begin{minipage}{0.5\textwidth}

% Ravi: For VLDB moved the following to a separate figure
\eat{
{\small
\ordinalg{
Set$<$Order$>$ {\bf GetAncestorOrders}(Set$<$Order$>$ {\em i$\_$ords}, \\
\>\>\>\>\>\> LogEqNode {\em e}) \\ %$\{$ \\
\>  Initialize {\em a$\_$ords} to be an empty set of sort orders \\
\>  For each {\em ord} $\in$ {\em i$\_$ords} \\ %$\{$ \\
\>\>  {\em newOrd} = Empty vector;  \\
\>\>  For ($i=1$; $i<=$length({\em ord}); $i=i+1$) \\ %$\{$ \\
\>\>\>	 If {\em ord[i]} is NOT bound by {\em e} \\
\>\>\>\>	append({\em ord[i]}, {\em newOrd}) \\
\>\>\>   Else \\
\>\>\>\>        break; \\
\>\>  $\}$\\
\>\>  add {\em newOrd} to {\em a$\_$ords} \\
\> $\}$\\
\> return {\em a$\_$ords} \\
$\}$\\
}
}
}
\algsize{
\ordinalg{
Set$<$Order$>$ {\bf GetAncestorOrders}(Set$<$Order$>$ {\em i$\_$ords}, \\
\>\>\>\>\>\> LogEqNode {\em e}) \\ %$\{$ \\
\>  Initialize {\em a$\_$ords} to be an empty set of sort orders \\
\>  For each {\em ord} $\in$ {\em i$\_$ords} \\ %$\{$ \\
\>\>  {\em newOrd} = Empty vector;  \\
\>\>  For ($i=1$; $i<=$length({\em ord}); $i=i+1$) \\ %$\{$ \\
\>\>\>	 If {\em ord[i]} is NOT bound by {\em e} \\
\>\>\>\>	append({\em ord[i]}, {\em newOrd}) \\
\>\>\>   Else \\
\>\>\>\>        break; \\
%\>\>  $\}$\\
\>\>  add {\em newOrd} to {\em a$\_$ords} \\
%\> $\}$\\
\> return {\em a$\_$ords} \\
%$\}$\\
end proc
}
}
\end{minipage}
% \caption{Get Ancestor Orders}
% \label{fig:GetAncestorOrder}
% \end{figure}

\caption{Get Interesting Sort Orders}
\label{fig:GetOrdersAlgo}
\end{figure}



==> chapters/nqo/algos/get_local_orders.tex <==
\begin{figure}[t]
\begin{minipage}{0.5\textwidth}
\algsize{
\ordinalg{
Set$<$Order$>$ {\bf GetLocalOrders}(Set$<$Order$>$ {\em i$\_$ords}, \\
\>\>\>\>\>\> LogEqNode {\em e}) \\ %$\{$ \\
\>  Initialize {\em l$\_$ords} to be an empty set of sort orders \\
\>  For each {\em ord} $\in$ {\em i$\_$ords} \\ %$\{$ \\
\>\>  {\em newOrd} = Empty vector;  \\
\>\>  For ($i=$length({\em ord}); $i>0$; $i=i-1$) \\ %$\{$ \\
\>\>\>	 If {\em ord[i]} is bound by {\em e} \\
\>\>\>\>	prepend({\em ord[i]}, {\em newOrd}) \\
\>\>\>   Else \\
\>\>\>\>        break; \\
%\>\>  $\}$\\
\>\>  add {\em newOrd} to {\em l$\_$ords} \\
%\> $\}$\\
\> return {\em l$\_$ords} \\
%$\}$\\
end proc
}
}
\end{minipage}
\caption{Get Local Orders}
\label{fig:GetLocalOrder}
\end{figure}



==> chapters/nqo/algos/proc_apply_node.tex <==
\begin{figure}[ht]
\begin{minipage}{0.5\textwidth}
%\renewcommand{\baselinestretch}{0.95}
\algsize{
\ordinalg{
Procedure {\bf ProcApplyNode} \\
Inputs: \>\> {\em o}, logical operation node corresponding to the {\em Apply} 
             operator in the LQDAG \\
        \>\> {\em s}, sort order guaranteed on the parameter bindings \\
        \>\> {\em e}, the physical equivalence node for the plans generated \\
Output: \>\> Expanded physical plan space. New plans are created 
             under {\em e}. \\
BEGIN \\
\>  Form the set {\em i$\_$ords} of valid interesting orders on parameters 
    by considering all the input \\
\>  sub-expressions of {\em o}. \\

\>  From the set {\em i$\_$ords}, create the set {\em l$\_$ords} by extracting 
    sort order prefixes of attributes bound \\
\>  by {\em o.bindInput}. \\
    
\>    For each order {\em ord} in {\em l$\_$ords} and the empty sort order $\epsilon$ \\% $\{$ \\
\>\>        // Generate plans for the {\em bind} expression \\
\>\>        Let $l_{eq}$ = PhysDAGGen({\em o.bindInput, ord, s}) \\
\>\>        Let {\em newParamOrd} =  concat({\em s}, {\em ord}) \\
\>\>        Let {\em iterOp} = New iterator physical op for {\em Apply} \\
\>\>        {\em iterOp.bindInput} = $l_{eq}$ \\
\>\>        For each {\em use} input {\em u} of {\em o} \\% $\{$ \\
\>\>\>        Let $u_{eq}$ = PhysDAGGen({\em u, $\epsilon$, newParamOrd}) \\
\>\>\>        Add $u_{eq}$ as a {\em use} input of {\em iterOp} \\
\>\>        Add {\em iterOp} as a child of $e$ \\
END
}
}
\end{minipage}
\caption{Plan Generation at an {\em Apply} Node}
\label{fig:ApplyAlgo}
\end{figure}



==> chapters/nqo/algos/proc_logop_node.tex <==
\begin{figure}[ht]
\begin{minipage}{1.0\textwidth}
\algsize{
\ordinalg{
Procedure {\bf ProcLogicalOpNode} \\
Inputs: \>\> {\em o}, a logical operation node in the LQDAG \\
        \>\> {\em p}, physical property required on the output \\
        \>\> {\em s}, sort order guaranteed on the parameter bindings \\
        \>\> {\em e}, the physical equivalence node for the new plans \\
Output: \>\> Expanded physical plan space. New plans are created 
             under {\em e}. \\
BEGIN \\
\>    For each algorithm {\em a} such that {\em a} implements {\em o},
      ensures physical property {\em p} on the output \\
\>    and requires a sort order $s'$ on the parameters, where $s'$ is 
      subsumed by {\em s} \\%$\{$ \\
\>\>        Create an algorithm node $o_{a}$ under $e$ \\
\>\>        For each input {\em i} of $o_{a}$ \\%$\{$ \\
\>\>\>            Let $o_{i}$ be the $i^{th}$ input (logical equivalence
node) of $o_{a}$ \\
\>\>\>            Let $p_{i}$ be the physical property required from input 
                      {\em i} by algorithm {\em a} \\
\>\>\>            Set input {\em i} of $o_{a}$ = PhysDAGGen($o_{i}$, $p_{i}$, 
                            {\em s}) \ \   // Main plan generation procedure \\
                            \hspace*{3.7in} // shown in \reffig{fig:PhyAlgo}\\
END
}
}
\end{minipage}
\caption{Plan Generation at a Non-Apply Node}
\label{fig:ChildAlgo}
\end{figure}



==> chapters/nqo/chap_nqo.tex <==
%\chapter{Parameter Sorting}
\chapter{Iterative Plans with Parameter Sorting}
\label{chap:nqo}
%\vspace{-6mm}
In many cases of iterative execution, such as those involving sub-queries or
functions, the order of calls to the nested sub-query or the function does
not affect the end result. Ordering the query/function invocations on the
parameter values gives several opportunities for improving the efficiency.
For example, System R\cite{SEL79} caches and reuses inner sub-query
results for duplicate parameter bindings, and it uses sorted parameter
bindings so that only a single result of the inner sub-query is required to
be held in memory at any given time. Graefe~\cite{GRA03} emphasizes the
importance of nested iteration plans, and highlights sorting of outer tuples
as an important technique to improve buffer effects.

This chapter describes additional query evaluation techniques that exploit
sort order of parameter bindings.  The task of a query optimizer is to
consider alternative plans for a given query and choose the best, {\em
i.e.}, the least cost plan.  The optimizer must therefore consider iterative
plans that exploit sort order of parameters, and estimate their cost
appropriately. The second part of this chapter address the problem of
extending a cost-based query optimizer to consider iterative plans
exploiting parameter sort orders.

The rest of this chapter is structured as follows. After stating some
basic definitions in \refsec{sec:prelim:chap:nqo}, in
\refsec{sec:epso:chap:nqo} we illustrate how to make use of ordered parameter
bindings to improve the efficiency of iterative query execution plans.
\refsec{sec:optext:chap:nqo} illustrates how a Volcano style cost-based
optimizer~\cite{GRA93} can be extended to consider the proposed techniques,
and \refsec{sec:perf:chap:nqo} presents experimental results and analysis.
We discuss related work in \refsec{sec:relwork:chap:nqo}, and summarize our
work in \refsec{sec:summary:chap:nqo}.

\input{chapters/nqo/sections/sec_sortorder.tex}
\input{chapters/nqo/sections/sec_epso.tex}
\input{chapters/nqo/sections/sec_optext.tex}
\input{chapters/nqo/sections/sec_perf.tex}
\input{chapters/nqo/sections/sec_relwork.tex}
\input{chapters/nqo/sections/sec_summary.tex}



==> chapters/nqo/examples/udf-turnaroundtime.tex <==
\begin{floatexample}
{\em 
Find the turn around time for high priority orders. The turn around time of
an order is calculated as the maximum of the differences between the ship
date and placement date of all its line items, if the order price is $<$
2000 and it is calculated as the maximum of the differences between the
commit date and placement date otherwise.}

%{\footnotesize
\begin{tabbing}
xxxxxxxxx\=xxxxxxxxxxxxxxxx\=xxxxxxxxx\=\kill
SELECT \> o$\_$orderkey, {\bf turn$\_$around$\_$time}(o$\_$orderkey, o$\_$totalprice, o$\_$orderdate) \\
FROM   \> ORDERS WHERE  o$\_$orderpriority='HIGH'; 
\end{tabbing}
%}

%{\footnotesize
\begin{tabbing}
xxxxxxxxx\=xxxx\=xxxxxxxxxxx\=\kill
DEFINE \>{\bf turn$\_$around$\_$time}(@orderkey, @totalprice, 
                                                 @orderdate) $\{$ \\
xxxx\=xxxx\=xxxxxxxx\=\kill
    \>IF (@totalprice $<$ 2000) \\
    \> 	\>SELECT max(l$\_$shipdate $-$ @orderdate) FROM LINEITEM \\
	\> 	\>WHERE l$\_$orderkey$=$@orderkey; \\
    \>ELSE \\
    \>	\>SELECT max(l$\_$commitdate$-$@orderdate) FROM LINEITEM \\
	\>	\>WHERE  l$\_$orderkey$=$@orderkey; \\
$\}$
\end{tabbing}
%}
\label{ex:udf-turnaroundtime}
\caption{Query Used in Experiment 4}
\end{floatexample}



==> chapters/nqo/sections/index-cost.tex <==
\subsubsection*{Cost of Clustered Index Lookups with Sorted Parameters}
%This section shows the advantages of sorted correlation bindings for
%clustered index scans. We consider the cost estimate of nested iteration
%plans with and without sorting.
For ease of illustration, we assume the outer query block references a
single relation {\em R} and the inner block references a single relation
{\em S}. We assume the following statistics are available for the optimizer.

{\footnotesize
\begin{itemize}
\itemsep0pt
    \item Number of blocks occupied by the outer relation = $B_{r}$ 
    \item Number of tuples in the outer relation = $N_{r}$
    \item Number of blocks occupied by the inner relation = $B_{s}$
    \item Number of tuples in the inner relation = $N_{s}$
    \item Tuples per block for the inner relation = $F_{s}$
    \item Number of distinct values for the attribute of {\em S}
          involved in the correlation predicate = $d$.
    \item Number of inner relation tuples that match each value 
          of the correlation variable = $C_{s}$. \\
          Assuming uniform distribution, $C_{s}=N_{s}/d$. 
    \item Combined selectivity of all the simple predicates in the 
          outer block = $S_{o}$
    \item $t_t$: Transfer time for a block, default value 0.1 msec for a 
          4K block at 40 MB/s
    \item $t_s$: Seek time, default value 4 msec
\end{itemize}
}

\noindent
{\bf Cost Estimate Without Sorting} \\
When the correlation bindings that act as the lookup keys for the clustered
index are not guaranteed to follow any order, each record fetch can
potentially require a disk I/O. The number of records from the inner
relation that match each correlation binding is $C_s$. Since the inner
relation is clustered on the lookup column the records to be fetched would
be stored contiguously, and hence occupy $\lceil C_s/F_s \rceil$ contiguous
blocks. Let $k$ be the average number of cache misses on index nodes 
for each lookup. Then the estimated cost of each lookup and fetch is given by: 
\[C_l = t_t(\lceil C_{s}/F_{s}\rceil\ + k) + t_s(k+1)\]
The total estimated cost (across all the iterations) would thus be 
$N_{r} \times S_{o} \times C_l$. 

%The total estimated cost (across all the iterations) 
%across all iterations will be: \[N_{r} \times S_{o}(t_t(\lceil C_{s}/F_{s}
%\rceil\ + k) + t_s(k+1)) \]. 

\noindent
{\bf Cost Estimate With Sorting} \\
We consider two cases: 
\begin{enumerate} 
\item When the outer predicate is such that the correlation bindings contain
all the values in an interval of the index ({\em e.g.}, an outer predicate
on the correlation attribute, which is also a foreign key of the inner
relation), the inner relation records accessed over all the iterations lie
on a set of contiguous blocks. Thus multiple lookups can be served from a
single block fetch. The total number of records from the inner relation
accessed over all the iterations will be $A_s=N_{r} \times S_{o} \times C_{s}$.
As the records are stored contiguously, the total inner relation access 
cost will be: $t_t(\lceil A_{s}/F_{s} \rceil) + t_s $. 

Assuming $N_{r}=100,000,\ S_{o}=0.5,\ C_{s}=10$ and $F_{s}=100$, the
expected number of inner relation's blocks accessed (across all iterations)
with sorted correlation bindings will be 5000, and we pay only a transfer
cost for each.  On the other hand the expected number of blocks accessed
without sorting will be 50,000 (ten times higher) even with no cache misses
for the index pages ({\em i.e.,} $k=0$). When the correlation bindings are
not sorted multiple fetches can occur for the same block of the inner
relation due to the interleaved access with other blocks. This is the reason
for the higher estimated cost (which assumes a worst case cache behavior) 
when the correlation bindings are not sorted.

\item When the predicates of the outer query block are on attributes different 
from the ones used as correlation variables,
%(e.g., the query in Example 2),
the correlation bindings will be from disjoint intervals. 
Let $j$ be the expected number of times the inner query block is evaluated
($j$ is the number of distinct correlation bindings generated from the
$N_{r} \times S_{o}$ tuples that qualify the outer predicates).
%Let $k=N_{r} \times S_{o}$ be the number of outer tuples for which the
%inner block is evaluated.  
Let $q=\lceil F_{s}/C_{s} \rceil$. $q$ denote the number of distinct values
for the attribute of $S$ involved in the correlation predicate, which are
stored on each block. Recall that $d$ is the total number of distinct values
for the attribute of $S$ that is involved in the correlation predicate. 
We can estimate the number of inner relation's blocks accessed as 
follows: a block of the inner relation will be accessed if any of the
$q$ distinct values in it is part of the $j$ distinct correlation 
bindings. Therefore,
the probability that a block of $S$ gets accessed is given by $p=(1 -
\frac{^{d-q}C_{j}}{^dC_{j}})$, where $^mC_{n}$ is the notation for choosing
$n$ from $m$, i.e., $\frac{m!}{(m-n)!n!}$.  

Therefore, the expected number of blocks read, {\em num\_blocks} will
be: $p \times B_{s}$.

The cost estimate will thus be $min(scantime, (t_s+t_t) num\_blocks)$ where
{\em scantime} is the time to scan the complete table ($t_s + B_{s}\times
t_t$). 

\end{enumerate}



==> chapters/nqo/sections/sec_epso.tex <==
%\section{Parameter Sort Orders in Query Evaluation}
\section{Query Evaluation with Ordered Parameters}
\label{sec:epso:chap:nqo}
Query evaluation algorithms for standard relational operators, such as
selection, join and grouping are well studied \cite{ACM:QEVAL}.  For example,
a relational selection can be implemented as a table scan or an index
lookup, and a relational join can use hashing, sorting or repeated index lookups
(index nested loops join).  A query execution plan comprises of operators,
each of which implements such an algorithm. In the case of iterative
execution of query plans, the operators are initialized with a different
parameter in each iteration and then executed, which gives no opportunities for
reordering or sharing of disk IO.  In this section, we illustrate how the
standard query evaluation techniques can be extended for improved
performance by making use of the sort order of query parameters.

\subsection{Restartable Table Scan}
Nested sub-queries or queries inside user-defined functions often select
tuples from a relation, one of whose columns matches the parameter value.
The selection predicate involving the parameter is called the {\em correlation
predicate}. In the query of \refex{ex:q1}, the selection predicate {\em
l$\_$orderkey=o$\_$orderkey} in the sub-query is a correlation predicate. A
relation referenced by the sub-query is called an inner relation.  In
\refex{ex:q1}, {\small LINEITEM} is an inner relation. 

Consider an inner relation, which is stored sorted on the column that
appears in an equality correlation predicate. For instance, if the {\small
LINEITEM} table in \refex{ex:q1} has a clustering index on the {\em
l$\_$orderkey} column, it would be stored sorted on the {\em l$\_$orderkey}
column.  Now, if the sub-query invocations are made in the order of the
parameter values, we can employ a {\em restartable table scan} for the inner
relation. The {\em restartable table scan} works as described next. In the
following description we assume the parameter bindings to be duplicate free.
For the first value of the parameter, the scan starts from the beginning of
the relation (or the first matching tuple in the clustering index) and
returns all the records that match the equality correlation predicate. The
scan stops on encountering a record that does not satisfy the correlation
predicate. The scan {\em remembers} this position. For subsequent bindings
of the parameter, the scan continues from the remembered position, {\em
i.e.,} the position at which it left off in the previous binding. This
allows the complete query to be evaluated with at most one full scan of the
inner relation. In the above explanation, we assumed the parameter bindings
to be duplicate free. Duplicate parameter values can be handled in two ways:
(a) Cache the sub-query result and reuse it for subsequent invocations with
the same parameter value, thus avoiding re-execution of the subquery with
the same parameter values. When the parameter values are sorted, at most one
result needs to be cached at any given time~\cite{SEL79}, and (b) remember
the most recent parameter value {\em (v)} and two positions {\em segstart}
and {\em segend} for the inner relation scan - {\em segstart} positioned at
the first tuple which matched the parameter value and {\em segend}
positioned at the last tuple that matched the parameter value. If a new call
has the same parameter value {\em (v)}, continue the scan from {\em
segstart}, otherwise continue the scan from {\em segend}. In general, the
approach of caching the sub-query result is more efficient unless the
subquery result for each invocation is too large to fit in memory.

Apart from clustering index, {\em query covering} secondary indices also
allow the use of {\em restartable table scan}. An index is said to {\em
cover} a query, if the index leaf pages contain all the columns required to
answer the query. By having additional columns (columns in addition to the
index key) in the index leaf pages, the index supports reading tuples in the
index key order without incurring random IO to fetch data pages.  Thus query
covering indices make it possible to efficiently obtain alternative sort
orders for the same relation, and are being used increasingly in read
intensive applications.

\subsubsection*{Cost Model}
Given an iterative plan, traditional query optimizers estimate the plan
cost as follows. The plan cost for the inner and outer sub-plans are
computed independently by adding the individual operator costs.  The cost of
the inner sub-plan is then multiplied by the estimated number of times it is
invoked, which is the number of distinct parameter values bound from the
outer query block. With operators such as restartable scan, which retain
state across calls, such a model of computing the plan cost cannot be
used. The solution is to cost a plan for $n$ invocations at once.
Accordingly, each operator in the plan must have a cost function, which
takes into account the number of invocations.

Thus, the cost of restartable scan for $n$ invocations with parameterized 
selection predicate $p$ on relation $r$ having $B_r$ disk blocks is computed 
as follows.

\[ \textrm{restart-scan::cost}(r, p, n) =  
        \left \{ 
                \begin{array}{ll} 
                    B_r   & \mbox{if}\ r\  
                            \mbox{is sorted to support}\ p \\
                    INF     & \mbox{otherwise. (the operator cannot be used)}
                \end{array} \right. 
\]

On the other hand, if a plain relation scan were to be employed, the
relation would be scanned $n$ times over all the iterations, amounting
to a cost of $n \times B_r$.

A plan that employs ordered parameter bindings and restartable scan has
the following advantages over a plan that employs \naive iterative index
lookups.
\begin{enumerate}
\item Performs sequential reads and hence incurs reduced seek time and 
      permits prefetching of disk blocks.
\item If more than one record from the same data page are needed, parameter
      sorting guarantees that the page is accessed exactly once irrespective 
      of the buffer replacement policy.
\end{enumerate}

However, if a query requires very small number of tuples from the inner
relation, an index lookup plan is generally more efficient than the
restartable scan. In such cases the index lookup plan avoids reading most of
the relation while the restartable scan has to perform a complete scan of
the relation.  The iterative index lookup plan can however benefit from
sorted parameter bindings as we shall see in \refsec{subsec:idxscan-with-pso}.

The effect produced by a restartable scan is similar to that of a merge
join. In essence, the restartable scan extends the benefits of merge-join to
iterative plans. This is important since merge-join is not directly
applicable to complex nested blocks such as user-defined functions with
embedded queries.

\subsection{Clustered Index Scan with Parameter Sorting}
\label{subsec:idxscan-with-pso}
If a clustering index exists for the inner relation on the column that is
involved in the correlation predicate and if the query requires a small
number of tuples from the inner relation, it is often more efficient to
employ iterative index lookups as against a restartable scan. However, a
\naive iterative index lookup plan leads to random IO.  Performance of
clustered index lookups in the evaluation of correlated nested queries can
be greatly improved by producing the parameter bindings in sorted
order~\cite{GRA03}. Sorting ensures sequential I/O and therefore permits
prefetching. Further, sorting of parameters ensures each data page is
fetched at most once irrespective of the buffer replacement policy. 
In this section, we derive a cost model for iterative clustered index
lookups with sorted keys. An accurate cost-model, which takes into 
account the benefits of parameter sorting, is essential for the optimizer
to pick the overall best plan.

\input{chapters/nqo/sections/index-cost.tex}

\eat{
Appendix ~\ref{sec:apdxa} shows the advantages of sorted correlation
bindings for clustered index scans by deducing the cost formula.
}


\subsection{Incremental Computation of Aggregates}
\label{subsec:incragg}
We now describe an efficient technique to evaluate nested aggregate queries
having non-equality correlation predicates, using the restartable scan.
%The technique illustrated in the previous section is applicable only when
%the correlation predicate in the inner subquery is an equality predicate.
%We now show how the {\em restartable table scan} can be employed for
%non-equality predicates, when the inner subquery has an aggregate.
Decorrelation is often very expensive for such queries. Consider the SQL
query shown in \refex{ex:q2}.  The query lists days on which the sales
exceeded the sales seen on any day in the past.

\begin{floatexample}
\begin{sqlindent}
\\
SELECT \>\> day, sales  FROM  DAILYSALES DS1 \\
WHERE  \>\> sales $>$ (SELECT MAX(sales) FROM DAILYSALES DS2 \\
       \>\>       \>\ \ \ \ WHERE  DS2.day $<$ DS1.day); 
\end{sqlindent}
\caption{A Nested Aggregate Query with Inequality Predicate}
\label{ex:q2}
\end{floatexample}

A na\"\i ve nested iteration plan for the above query employs a 
sequential scan of the {\small DAILYSALES} table for both the outer and the
inner block.  Assuming the inner block scans an average of half of the table
for each outer tuple, the cost of this plan would be $t_t(B_{ds} +
N_{ds}\times B_{ds}/2) + t_s(1+N_{ds})$, where $B_{ds}$ is the number of
blocks occupied by {\small DAILYSALES} table, $N_{ds}$ is the number of
tuples in the same table, and $t_t$ and $t_s$ are the block transfer time
and seek time respectively.

Now, suppose the {\small DAILYSALES} relation (or materialized view) is stored,
sorted on the {\em day} column.  If the plan for the outer query block
generates the bindings for the correlation variable ({\small
DAILYSALES}.day) in non-decreasing order, we can see that the tuples that
qualify for the aggregate ({\small MAX}) operator's input in the $i^{th}$
iteration will be a superset of the tuples that qualified in the
$(i-1)^{th}$ iteration.  The {\small MAX} operator, in its state, can retain
the maximum value seen so far and use it for computing the maximum value for
the next iteration by looking at only the additional tuples. So, the scan needs
to return only those additional tuples that qualify the predicate since its
previous evaluation.  The technique proposed here is applicable for $<,
\leq, >$ and $\geq$ predicates and the aggregate operators {\small MIN, MAX,
SUM, AVG and COUNT}.  The maximum cost of such a plan would be $2 \times
B_{ds} \times t_t + 2 \times t_s$, which is significantly lesser than the
cost of the na\"\i ve nested iteration plan.

When there are {\small GROUP BY} columns specified along with the aggregate,
the aggregate operator has to maintain one result for each group. The
aggregate operator can maintain its state in a hash table; the key for the
hash table being the values for the {\small GROUP BY} columns and the value
against each key being the aggregate computed so far for the corresponding
group.

\eat {
\subsection{Sorting Parameters on their Physical Order}
In the previous sections we assumed the relation referenced by the 
inner subquery to be sorted on the attribute that appears in the 
correlation
predicate. This restriction can be relaxed for attributes with {\em unique}
constraint. The key idea is to sort the parameters as per their physical 
order instead of their value. Consider the query shown in Example 6.

\noindent
{\footnotesize 
\begin{tabbing}
xxxxxxxx\=xxxxxxx\=xxxxxxxxx\=\kill
{\bf Example 6} \\
SELECT \> R1.a  \\
FROM   \> R1 \\
WHERE  \> R1.b IN \> (SELECT \> R2.c \\
       \>         \>  FROM   \> R2 \\
       \>         \>  WHERE  \> R2.d = R1.e); \\
\end{tabbing}
}

{\bf Case 1:} R2 is physically sorted on R2.d. In this case, the 
{\em Restart Scan} operator is directly applicable for the scan of 
R2 and the entire query can be evaluated with one scan of R1 and
one scan of R2.

{\bf Case 2:} R2 is physically sorted on some column R2.f. Now, let $T =
\pi_{f,d}(R2)$. We take an outer join of R1 with T and sort the result of
this outer join on R2.f, {\em nulls} being sorted high. From this result we
produce the correlation bindings for R1.e. This allows us to use the {\em
Restart Scan} operator for the inner relation as the bindings for R1.e are
generated as per their physical order in R2.  However, we note that this
technique gives the correct result for all types of nested queries only if
R2.d has no duplicates.

This technique is very effective when there is an index on R2.d that covers
R2.f. Such an index allows us to compute the outer join of R1 with
$\pi_{f,d}(R2)$ without touching the data pages of R2.
}




==> chapters/nqo/sections/sec_optext.tex <==
%\section{Extensions to a Cost-Based Optimizer}
\section{Parameter Sort Orders in Query Optimization}
\label{sec:optext:chap:nqo}
A query optimizer considers alternative execution plans for a given query,
estimates the cost of each plan and chooses the plan with the least expected
cost. To estimate the cost of an iterative plan, traditional optimizers
first identify the best plan for the nested sub-query independently and
multiply its cost by the expected number of iterations. Clearly, this
approach does not take into account plans that exploit ordered parameter 
bindings. The optimizer must consider different sort orders on the 
sub-query parameters. For each sort order,
there is an associated benefit for the sub-query plan that exploits
the sort order and a cost for the outer query plan to generate the parameters
in the required order. The optimizer must choose the optimal plan for the
query by considering benefits and cost of various possible sort orders.

\eat{
A nested sub-query block can use one or more parameters whose values are
bound in any of its {\em ancestor} blocks. For a given nested sub-query,
several execution plans are possible, each having an estimated cost and a
sort order requirement on the sub-query parameters. The plan cost for the
outer (parent) query block depends on the order in which the parameter
bindings are to be generated. The optimizer, must therefore consider the
various alternative sort orders for the sub-query parameters and decide on
the overall best plan. 
}

The Volcano query optimization framework~\cite{GRA93} is a state of the art
cost-based query optimizer.  This section illustrates how a Volcano style
query optimizer can be extended to take into account plans that make use of
parameter sort orders.  The rest of this section is organized as follows.
\refsec{subsec:optframework} briefly describes the Volcano optimizer
framework. \refsec{subsec:ext-overview} proposes extensions to the
optimizer's high-level interface to support optimization of parameterized
expressions. \refsec{subsec:logrep} describes the logical representation we
adopt for nested queries.  The changes to the to plan space
and search algorithm are described in \refsec{subsec:phyplan} and
\refsec{subsec:search} respectively.

\subsection{The Optimizer Framework}
\label{subsec:optframework}
In this section we briefly describe the {\small PYRO} cost-based optimizer
framework over which we propose our extensions.  {\small PYRO} is an
extension of the Volcano optimizer~\cite{GRA93}. A detailed description 
of the {\small PYRO} optimizer can be found in in~\cite{ROY01} and 
~\cite{ROY00}.

\noindent The optimizer performs three main tasks.

\begin{enumerate}
\item Logical Plan Space Generation \\
In this first step the optimizer, by applying logical transformations such
as join associativity and pushing down of selections through joins,
generates all the semantically equivalent rewritings of the input query.

\item Physical Plan Space Generation \\ 
This step generates several possible execution plans for each rewriting
produced in the first step. An execution plan specifies the exact algorithm
to be used for evaluating each logical operator in the query.  Apart from
selecting algorithms for each logical operation, this step also considers
{\em enforcers} that help in producing required {\em physical properties}
(such as sort order of tuples) on the output. Physical property requirements
arise due to two reasons {\em (i)} the user/application may specify a
physical property requirement as part of the query, {\em e.g.,} an order-by
clause and {\em (ii)} algorithms that implement operations such as join and
duplicate elimination may require their inputs to satisfy a sort order or
grouping property.  The {\em algorithms} for relational operators and the
{\em enforcers} of physical properties are collectively referred to as {\em
physical operators} as against the logical operators of the logical plan
space.

\item Finding the Best Plan \\
Given the cost estimates of different algorithms that implement the logical
operations and the enforcers, the cost of each execution plan is estimated.
The goal of this step is to find the plan with minimum cost.
\end{enumerate}

The above three steps can either be executed in a depth-first order or in a
breadth-first order~\cite{ROY00}. For the purpose of our explanation we
consider the breadth-first order, in which each step is performed completely before
the next step is started. However, in our actual implementation, physical
plan generation and search for the best plan are combined in a single phase.

An {\small AND-OR} graph representation called Logical Query {\small DAG}
({\small LQDAG}) is used to represent the logical plan space, {\em i.e.,}
all the semantically equivalent rewritings of a given query. The {\small
LQDAG} is a directed acyclic graph whose nodes can be divided into {\em
equivalence nodes} and {\em operation nodes}; the equivalence nodes have
only operation nodes as children and the operation nodes have only
equivalence nodes as children. An operation node in the {\small LQDAG}
corresponds to an algebraic operation, such as join $(\Join)$ or select
$(\sigma)$. It represents the expression defined by the operation and its
inputs. An equivalence node in the {\small LQDAG} represents the equivalence
class of logical expressions (rewritings) that generate the same result set,
each expression being defined by a child operation node of the equivalence
node and its inputs. An example {\small LQDAG} is shown in
\reffig{fig:lqdag}\footnote{This figure is taken from~\cite{ROY00}.}.

\begin{figure} [ht]
%\centerline{\psfig{file=chapters/nqo/fig/lqdag.eps}}
\center \includegraphics[height=2.0in,width=2.8in]{chapters/nqo/fig/lqdag.eps}
\caption{A Logical Query DAG for A $\Join$ B $\Join$ C}
\label{fig:lqdag}
\end{figure}

Once all the semantically equivalent rewritings of the query are generated,
the Volcano optimizer generates the {\em physical plan space} by considering
different algorithms for each logical operation and {\em enforcers} to
generate required physical properties. In some optimizers, such as
Cascades~\cite{GRA95} and SQL Server~\cite{GF04:sqlserveropt}, the logical
and physical plan space generation stages are intermixed.  The physical plan
space is represented by an {\small AND-OR} graph called {\small PQDAG} which
is a refinement of the {\small LQDAG}. Given an equivalence node {\em e} in
the {\small LQDAG}, and a physical property {\em p} required on the result
of {\em e}, there exists an equivalence node in the {\small PQDAG}
representing the set of physical plans for computing the result of {\em e}
with the physical property {\em p}. A physical plan in this set is
identified by a child operation node of the equivalence node and its input
equivalence nodes.  The equivalence nodes in a {\small PQDAG} are called
{\em physical equivalence nodes} to distinguish them from the {\em logical
equivalence nodes} of the {\small LQDAG}. Similarly, the operation nodes in a
{\small PQDAG} are called {\em physical operation nodes} to distinguish them
from the {\em logical operation nodes} of the {\small LQDAG}.

The optimizer framework we use models each of the logical operators,
physical operators and transformation rules as separate classes, and this
design permits the extensions we propose to be easily incorporated.


\subsection{Extensions to the Optimizer Interface}
\label{subsec:ext-overview}
Both Volcano~\cite{GRA93} and {\small PYRO}~\cite{ROY00} optimizers take the
initial query (expression), a set of physical properties (such as sort
order) required on the query result and a cost limit (the upper bound on
plan cost) as inputs and return the execution plan with least expected cost.
The following method-signature summarizes the Volcano optimizer's input and
output.

\vspace{0.02in}
\ordinalg{
Plan {\bf FindBestPlan} (Expr {\em e}, PhyProp {\em p}, CostLimit c);
}

\noindent The optimizer makes an assumption that if the expression is
evaluated multiple times the cost gets multiplied accordingly. This
assumption ignores advantageous buffer effects due to sorted parameter
bindings and the benefits due to state retention techniques proposed in the
previous section.  When the parameter bindings are sorted, the cost of
evaluating an expression {\em n} times can be significantly lesser than {\em
n} times the cost of evaluating the expression once.  In order to consider
these factors, we propose a new form of the {\em FindBestPlan} method. The
following method-signature summarizes the new form of the {\em FindBestPlan}
method.

\ordinalg {
Plan {\bf FindBestPlan} (Expr {\em e}, PhysProp {\em p}, CostLimit {\em c},
     SortOrder {\em pso}, int {\em callCount});
}

The new {\em FindBestPlan} procedure takes two additional parameters. The
first of these, is the sort order guaranteed on the
parameters (outer variables) used by {\em e}.  The second parameter, termed
{\em callCount}, tells the number of times the expression is expected to be
evaluated. The cost of the returned plan is the estimated cost for {\em
callCount} invocations.  Note that the original Volcano algorithm's 
interface can be thought of as a special case of this enhancement, where
the expression {\em e} is assumed to have no unbound references (parameters)
and the callCount is 1. 

\subsection{Logical Representation of Nested Queries}
\label{subsec:logrep}
We now describe the way in which we represent nested queries in the LQDAG.
A nested query, in the simplest case, contains two query blocks - an {\em
outer} query block and an {\em inner} query block. The inner query block
uses parameters whose values are bound from the tuples obtained by
evaluating the outer query block.  
\eat{
The inner sub-query, in general, returns a set of tuples for each
invocation.  An iterative execution plan for such a nested query contains
two {\em sub-plans}, one for evaluating the outer query block and the other
for evaluating the inner query block. 
}
We adopt a variant of the {\em Apply} operator proposed in~\cite{GAL01} for
representing nested queries. In its simplest form, the {\em Apply} operator
has two sub-expressions: the {\em bind} sub-expression corresponds to the
outer query block and the {\em use} sub-expression corresponds to the
parameterized inner query block.  Conceptually, the {\em Apply} operator
evaluates the use sub-expression for every tuple in the result of the bind
sub-expression. After each evaluation of the use sub-expression, the {\em
Apply} operator combines the tuple from the bind sub-expression and
the result of the use sub-expression. Combining may involve evaluating a
predicate such as {\small IN} or {\small NOT IN} that check for set
membership, {\small EXISTS} or {\small NOT EXISTS} that check for set
cardinality, a scalar comparison ($=, \neq, >, \geq, <, \leq$), or a
comparison of a scalar with members of a set: {\em relop} {\small ANY}
or {\em relop} {\small ALL}, where {\em relop} is one of the
comparison operators. \reffig{fig:applyexample} shows the logical 
representation of the query given in \refex{ex:q1} of \refchap{chap:intro}. 

\begin{figure} [ht]
\center \includegraphics[height=1.2in,width=3.3in]{chapters/nqo/fig/applyexample.eps}
\caption{Example of Representing a Nested Query using {\em Apply} ($\mathcal{A}$)} 
\label{fig:applyexample}
\end{figure}

\eat{
The {\em Apply} operator, instead of evaluating a predicate, can evaluate a
scalar valued user-defined function in the select clause.  It is also
possible to use the results of the use sub-expression for each tuple in the
bind sub-expression and output a nested relation. We return to this issue in
\refsec{sec:sec6}. 

\reffig{fig:apply} depicts the {\em Apply} operator pictorially. 

\begin{figure} [ht]
\center \includegraphics[height=1.7in,width=2.5in]{chapters/nqo/fig/apply.eps}
\caption{The {\em Apply} Operator}
\label{fig:apply}
\end{figure}
}

We refer to the {\em bind} sub-expression of an {\em Apply} operator as its
{\em left} sub-expression and the {\em use} sub-expression as its {\em
right} sub-expression.  In general, an {\em Apply} operator can have
multiple {\em use} expressions that represent multiple sub-queries nested at
the same level.  In a complex multi-level nested query a sub-expression $e$
may use some variables and bind other variables.  The variables that $e$
binds may be passed on to the {\em use} sub-expressions of parent or
ancestor {\em Apply} operators; $e$ must be in the left-most subtree of such
{\em Apply} operators.  The variables that $e$ uses must be defined at
parent or ancestor {\em Apply} operators;  $e$ must be in a use-subtree,
{\em i.e.}, non-left-most subtree, of such {\em Apply} operators.  

\eat{
When the nested block is
a complex user-defined function, containing both queries and procedural
statements, we represent only the queries and their nesting structure,
ignoring the procedural statements. For instance, the query in
\refex{ex:udf-count-offers} is represented as shown in
\reffig{fig:udfexample}. This representation suffices to identify efficient
execution plans that exploit parameter sort orders.

\begin{figure} [ht]
\center \includegraphics[width=3.3in]{chapters/nqo/fig/udfexample.eps}
\caption{Example of Representing a Complex Nested Block using {\em Apply}} 
\label{fig:udfexample}
\end{figure}
}

\subsection{Physical Plan Space Generation}
\label{subsec:phyplan}
The physical plan space generation involves generating alternative execution
plans for a given logical expression and representing them in the {\small
PQDAG}. In {\small PYRO}, two query execution plans $p_1$ and $p_2$ are
considered equivalent ({\em i.e.,} they belong to the same physical
equivalence class) {\em iff} the following conditions are met: {\em (i)}
$p_1$ and $p_2$ evaluate the same logical expression $e$, and {\em (ii)}
$p_1$ and $p_2$ produce the result of $e$ in the same sort order.

We redefine the notion of equivalence of execution plans in {\small PYRO} to
include the parameter sort orders required by the plans. Two plans $p_1$ and
$p_2$ belong to the same equivalence class {\em iff} $p_1$ and $p_2$
evaluate the same logical expression, guarantee the same physical
properties on their output and require the same sort order on the parameter
bindings, when invoked iteratively.  Thus, for a given logical expression
{\em e} and physical property {\em p}, there exists a set of physical
equivalence nodes in the {\small PQDAG}.  Each equivalence node in this set
corresponds to a distinct sort order requirement on the parameters used in
{\em e}. 

The physical plan space generation step therefore involves the following:
given a logical equivalence node {\em e}, a physical property {\em p}
required on the result of {\em e} and a sort order {\em s} known to hold on
the parameters in {\em e}, generate all the evaluation plans and
representing them in the {\small PQDAG}.  The search phase of optimization
then takes the {\small PQDAG} and a {\em call count} as its inputs and finds
the best plan.

\subsubsection{Generating Plans for Non-Apply Operators}
The plan generation step in PYRO works as follows. The LQDAG is traversed,
and at each logical operation node, all the applicable algorithms
(physical operators) are considered. A physical operator is applicable if it
implements the logical operation and ensures the required physical
properties on the output. 

\input{chapters/nqo/algos/proc_logop_node.tex}

To take into account the sort order of parameters, we need a minor
modification to the plan generation step. For a given logical operation, we
consider only those physical operators (algorithms) as applicable, whose
sort order requirement on the parameters is subsumed by the sort order known
to hold (guaranteed) on the parameters.  As an example, consider a selection
logical operator $\sigma_{R1.a=p_{1}}(R1)$, where $p_{1}$ is a correlation
(outer) variable.  Suppose two algorithms, a plain table scan requiring no
sort order and a state retaining scan requiring a sort order $(p_{1})$ on
the parameters, are available. Now, if the parameter sort order guaranteed by
the parent block subsumes $(p_{1})$, both the algorithms (physical
operators) are applicable.  However, if the parameter sort order guaranteed
by the parent block does not subsume $(p_1)$, then only the plain table scan
is applicable. \reffig{fig:ChildAlgo} shows the plan generation steps 
at a {\em Non-Apply} logical operator.

% To reduce the number of candidate plans it is possible to adopt a heuristic:
% consider only the physical operator(s) that requires the strongest parameter
% sort order less than the guaranteed sort order. If this heuristic is adopted
% in the above example, when the parameter sort order guaranteed from the
% parent block is $(p_1)$ only the state retaining scan is considered and the
% plain table scan is dropped. Procedure {\em ProcLogOpNode} in

\subsubsection{Plan Generation for an Apply Operator}
Earlier work on {\em Apply} operator~\cite{GAL01} attempts to rewrite the
{\em Apply} operator using joins, outer-joins or semi-joins before plan
generation. Our goal here is to expand the plan space to include efficient
iterative plans for the {\em Apply} operator. This involves two steps.

\begin{enumerate}
\item Identify a set of useful and valid sort orders on the sub-query 
      parameters.
\item Generate iterative plans in which the plan for the sub-query 
      makes use of the sort order of parameters produced by the plan for 
      the outer-block.
%\item Generating iterative plans in which the plan for the sub-query 
%      exploits a sort order and the plan for the outer block guarantees
%      the same sort order on the parameters.
\end{enumerate}

\noindent {\bf Identifying Valid Interesting Sort Orders} \\
If sub-query has $n$ parameters, there are potentially $n!$ sort orders
on the parameters.
Considering all possible sort orders of parameters used in an expression is
prohibitively expensive. Only few sort orders on the parameters are expected
to be useful. To consider selected sort orders in the optimization process,
System R~\cite{SEL79} introduced the notion of {\em interesting orders}. We
extend this notion to sort orders of parameters and call them as {\em
interesting parameter sort orders}.  Our algorithm to generate the physical
plan space creates physical equivalence nodes for only {\em interesting}
parameter sort orders.

Intuitively, interesting parameter sort orders are the ones that are useful
for efficient evaluation of one or more nested blocks ({\em use} expressions
of an apply operator). Typically, the clustering order and query covering
indices on base relations used inside the nested block(s) decide the
interesting parameter sort orders. However, the optimizer must also consider
plans that explicitly sort a relation in the inner block to match the sort
order easily available from the outer block. The problem of identifying
interesting orders is common to both nested queries and joins and deserves
special attention. We address this problem in \refchap{chap:eio}. In the
rest of this chapter we assume that the set of interesting sort orders on
unbound parameters of an expression, is available to us.

Every interesting sort order on the parameters may not be {\em valid}
(feasible) under the given nesting structure of query blocks. For example,
consider a query with two levels of nesting; $q_a(q_b(q_c))$, $q_a$ is the
outer-most query block and $q_c$ is the inner most. Assume $q_c$ uses two
parameters $a$ and $b$, where $a$ is bound by $q_a$ and $b$ is bound by
$q_b$. Now, the sort order $(a, b)$ is a valid interesting order for $q_c$
but not the sort order $(b, a)$. As block $q_b$ that binds parameter $b$ is
nested below the block $q_a$ that binds parameter $a$, the sort order $(b,
a)$ cannot be generated and hence invalid.

\begin{definition}
\label{defn:valid-sort-order}
{\bf Valid Interesting Sort Orders}\\
A sort order $s=(a_{1}, a_{2}, \ldots, a_{n})$ on the parameters of 
a query block $b$ is {\em valid} (feasible) {\em iff} there is a nesting
of query blocks such that the following
two conditions are satisfied:
\begin{enumerate}
\item
$level(a_{i}) \leq level(a_{j})$ for all $i,j\ s.t.\ i < j$, where
$level(a_{i})$ is the level of the query block in which $a_{i}$ is bound.
The level of the outer most query block is considered as 0 and all the query
blocks nested under a {\em level-i} query block have the level $i+1$.

\item 
Let the BindAttrs of a block $b_k$ with respect to a sort order $s$ be defined 
as follows.\\
BindAttrs($b_k$, $s$): Attributes in $s$ that are bound by either block 
$b_k$ or by an ancestor of $b_k$.
% \\ LinkAttrs($b_k$, $s$): Attributes in $b_k$ that are linked with attributes 
% the values of attributes in $s$ with an equality predicate.

Then, for each ancestor block $b_k$ of $b$ at level $k$ such that 
level$(b)$ $> k + 1$ (i.e., excluding the parent block of $b$),
values of BindAttrs$(b_k, s)$ are distinct for any
two invocations of $b_{k+1}$. 
%a candidate key in the schema of $b$, 
\end{enumerate}
\end{definition}

The first condition in Definition~\ref{defn:valid-sort-order} ensures that
attributes bound by an outer query block always precede attributes bound by
an inner query block in any valid sort order. The need for the second
condition is best explained with an example.  Consider a query with two
levels of nesting; $q_a(q_b(q_c))$, $q_a$ being the outer-most query block
and $q_c$ being the inner most. Suppose block $q_c$ makes use of two
parameters: parameter $a$ bound at $q_a$ and parameter $b$ bound at $q_b$.
If $q_a$ generates duplicate values for $a$, then $(a,b)$ is not a valid
parameter sort order for $q_c$. This is because if $q_a$ generates
duplicate bindings for $a$, then even if the plan for $q_b$ produces the
bindings for $b$ in sorted order, $q_c$ cannot see a sorted sequence on
$(a,b)$ across all its invocations; the bindings for attribute $b$ will
cycle back for the same value of attribute $a$.
Now, if $q_a$ is guaranteed to not generate duplicates for $a$, then $(a,
b)$ is a valid parameter sort order for block $q_c$.  However the sort order
$(b)$ is not valid (unless $q_a$ invokes $q_b$ at most once) since even if
the plan for block $q_b$ produces the bindings for $b$ in sorted order,
block $q_c$ will see a sorted sequence of $b$ values for a single invocation
from $q_a$, but may not see a sorted sequence on $b$ across multiple
invocations from $q_a$.\\

\noindent {\bf Generating Plans for the {\em Bind} and {\em Use} 
               Expressions of an Apply Operator} \\ 
Consider a query block $q$ under which blocks $q_{1}, q_{2}, \ldots, q_{n}$
are nested.  This is represented by an {\em Apply} expression with $q$ as
the {\em bind} sub-expression and $q_{1}, q_{2}, \ldots, q_{n}$ as {\em use}
sub-expressions. Generating plans at the {\em Apply} node involves
the following steps:
\begin{enumerate}
\addtolength{\itemsep}{-3mm}
    \item For each use expression $q_i$, identify the set $s_i$ of interesting
          parameter sort orders. Identifying a good set of interesting sort
          orders is a topic of interest not only for nested queries but also
          for queries with joins, group-by and set operations. We address
          this problem in the next chapter.
    \item For the outer query block $q$, identify the set $s_q$ of sort orders
          that are available readily or at a low cost.
    \item Form the set {\em i$\_$ords} as $s_1 \cup \ldots \cup s_n \cup s_q$.
    \item From the set {\em i$\_$ords} discard the sort orders that are 
          not {\em valid}, under the given nesting structure of query blocks. 
          The conditions for validity are specified in 
          definition~\ref{defn:valid-sort-order}.
    \item From the set {\em i$\_$ords} we derive a set {\em l$\_$ords}
          consisting of sort orders that are relevant to the {\em bind}
          expression $q$ of the {\em Apply} operator. Note that the 
          sort orders in {\em
          i$\_$ords} can contain some attributes that are bound higher up in
          the complete query structure.  Deriving {\em l$\_$ords} from {\em
          i$\_$ords} involves extracting the suffix of each order {\em ord}
          $\in$ {\em i$\_$ords} such that the suffix contains only those
          parameters that are bound in $q$. 
\eat{
\reffig{fig:orderprop} illustrates how the parameter sort orders are
propagated. 
\begin{figure} [ht]
\centerline{\psfig{file=chapters/nqo/fig/orderprop.eps}}
\caption{Sort Order Propagation for a Multi-Level Multi-Branch Expression}
\label{fig:orderprop}
\end{figure}
In the figure, we indicate the parameters bound and parameters used at each
expression with the convention B: and U: respectively. Consider the {\em
Apply} operator at the root of sub-expression $e_2$. The set {\em i$\_$ords}
of interesting orders for $e_{22}$ has a single element $(a,c)$, i.e., {\em
i$\_$ords}=$\{(a,c)\}$. From this set we derive the set {\em l$\_$ords} as
$\{(c)\}$ since $c$ is the only parameter bound by the expression $e_{21}$
that is the {\em bind} expression for the {\em Apply} operator in
consideration.
}
    \item For each sort order {\em o} $\in$ {\em l$\_$ords} $\cup$
          $\{\epsilon\}$, where $\epsilon$ stands for the empty sort order,
          we generate plans for the {\em bind} expression by making {\em o}
          as the required physical property on the result (output), and then
          generate plans for all the {\em use} expressions.  We create a
          physical operation node $a$ for the {\em Apply} operation
          depending on the predicate associated with the {\em Apply} node.
          The plans generated for the {\em bind} and {\em use} expressions
          are added as the child plans for $a$. 
\end{enumerate}

\begin{figure} [ht]
\centerline{\psfig{file=chapters/nqo/fig/orderprop.eps}}
\caption{Sort Order Propagation for a Multi-Level Multi-Branch Expression}
\label{fig:orderprop}
\end{figure}

We now illustrate the working of the above steps using the example
expression shown in \reffig{fig:orderprop}. Two sub-expressions
$e_2=(e_{21}$ {\em Apply} $e_{22})$ and $e_3$ are nested under the
outer-most expression $e_1$. In the figure, we indicate the parameters bound
and parameters used by each expression with the convention {\em B:} and {\em
U:} respectively. Consider the outer-most apply operator present at the root
of the expression tree.  In step 1, for each of the {\em use}
sub-expressions {\em i.e.}, for $e_2$ and $e_3$ we identify the set of
interesting parameter sort orders. The interesting parameter sort orders of
an expression depend upon the sort orders of base relations used in the
expression and the correlation predicates.  The details of deriving
interesting orders is the topic of the next chapter.  For now, suppose the
sub-expression $e_2$ has two interesting sort orders $(a)$ and $(a,b)$ on
the parameters it uses, and suppose the sub-expression $e_3$ has one
interesting sort order $(b)$. In step 2, we identify the set of sort orders
available at low cost on the output of expression $e_1$. Such sort orders
are called {\em favorable} sort orders and the details of finding the
favorable sort orders are given the next chapter. For this example, suppose
there exists a single favorable sort order $(a)$ for expression $e_1$. In
step 3, we compute the set {\em i$\_$ords} as $\{(a), (a,b), (b)\}$. In step
4, we check for the validity of these sort orders as per Definition 2.3. All
the three sort orders are valid in this case. We then derive the set {\em
l$\_$ords} in step 5, by extracting the sort order suffix relevant to the
{\em bind} expression $e_1$.  $e_1$ being the outer-most block, {\em
l$\_$ords} will be same as {\em i$\_$ords}.  In step 6, we generate plans
for the {\em use} expression $e_1$ with each of the three sort orders $(a)$,
$(a,b)$ and $(b)$ as the required output sort order, and also generate the
plans for the {\em use} expressions with each of these sort orders as the
guaranteed sort order on the parameter bindings. The corresponding plans of
the {\em bind} and {\em use} expressions are then paired as child plans of a
physical apply operator. Note how the set {\em l$\_$ords} is computed for
the apply operator at the root of sub-expression $e_2=(e_{21}$ {\em Apply}
$e_{22})$. The set {\em i$\_$ords} of interesting orders for $e_{22}$ has a
single element $(a,c)$, {\em i.e.}, {\em i$\_$ords}=$\{(a,c)\}$. From this
set we derive the set {\em l$\_$ords} as $\{(c)\}$ since $c$ is the only
parameter bound by the expression $e_{21}$, which is the {\em bind} expression
for the {\em Apply} operator in consideration.

Procedure {\em ProcApplyNode} in \reffig{fig:ApplyAlgo} shows the plan
generation steps at an {\em Apply} operator node.
The top level procedure for generating the physical plan space is given in
Figure~\ref{fig:PhyAlgo}, and it makes use of the two procedures {\em
ProcLogicalOpNode} and {\em ProcApplyNode}.  For simplicity, we omit the
cost based pruning from our description and return to it later. As a
result the {\em callCount} parameter does not appear in the algorithm. 
Figures \ref{fig:lqdag-apply} and \ref{fig:pqdag-apply} show the logical
query DAG and the resulting physical query DAG (assuming a very limited
collection of algorithms) for the example of \reffig{fig:applyexample}.
%\input{chapters/nqo/algos/get_int_orders.tex}
%\input{chapters/nqo/algos/get_local_orders.tex}

\eat{
A procedure to generate interesting orders, {\bf GetInterestingOrders}, is
shown in Figure~\ref{fig:GetOrdersAlgo}.  The procedure makes use of an
auxiliary procedure {\bf GetAncestorOrders} which takes a set of interesting
orders and a node, and returns sort orders defined by ancestors of the
specified node.  Procedure {\bf GetLocalOrders}, shown in
Figure~\ref{fig:GetLocalOrder}, takes a set of interesting orders and a node
(the bind sub-expression of an apply operator) and returns the interesting order
suffixes that are defined by the specified node.
}
\input{chapters/nqo/algos/proc_apply_node.tex}
\input{chapters/nqo/algos/algo.tex}

\begin{figure} [ht]
%\centerline{\psfig{file=chapters/nqo/fig/lqdag.eps}}
\center \includegraphics[height=2.0in,width=2.8in]{chapters/nqo/fig/lqdag-apply.eps}
\caption{LQDAG for the Example of \reffig{fig:applyexample}}
\label{fig:lqdag-apply}
\end{figure}
\begin{figure} [ht]
%\centerline{\psfig{file=chapters/nqo/fig/lqdag.eps}}
\center \includegraphics[height=2.0in,width=4.4in]{chapters/nqo/fig/pqdag-apply.eps}
\caption{PQDAG for the Example of \reffig{fig:applyexample}}
\label{fig:pqdag-apply}
\end{figure}
\eat{
We assume that physical operator(s) corresponding to the {\em Apply}
operator do not guarantee any sort orders on the output\footnote{Though the
{\em Apply} operator passes through the physical properties of its {\em
bind} expression to its output, for simplicity we do not consider it here}.
Therefore if any sort order needs to be guaranteed on the output of the {\em
Apply} operator an enforcer plan is generated. 
}

To check if a sort order is valid, we need a mapping from each parameter to
the level number of the block in which the parameter is bound.  In the
logical query DAG (LQDAG), due to the sharing of common sub-expressions, the
mapping of parameters to the level of the query block that binds it cannot
be fixed statically for each logical equivalence node.  In fact, a single
logical equivalence node can get different level numbers because of the {\em
level altering} transformations such as: 
\[ 
(R\ \mathcal{A}_{EXISTS} (\sigma_{S.c2=R.c1}(S)
 \mathcal{A}_{EXISTS} (\sigma_{T.c3=R.c1} T))) \]
\[ \Longleftrightarrow 
((R \SemiJoin_{R.c1=S.c2}S) \mathcal{A}_{EXISTS} (\sigma_{T.c3=R.c1} T))
\]

In the LHS of the above equivalence rule relation $T$ gets a level number
two levels higher than $R$, whereas 
in the RHS $T$ gets a level number one level higher than $R$. This happens
because the RHS uses an outer join to remove the nesting of $S$ within $R$.
\reffig{fig:levelalter} gives a pictorial illustration.

\begin{figure} [ht]
\center \includegraphics{chapters/nqo/fig/levelalter.eps}
\caption{An Example of Level Altering Transformation}
\label{fig:levelalter}
\end{figure}

In general with such transformations, a sub-expression can see a 
different mapping of parameters to levels depending on which expression 
is chosen above it in a logical plan.  We can thus get multiple 
interesting parameter sort orders, corresponding to the different nesting
structures.
In our implementation, we address this issue by carrying along a
map of parameters to levels when recursively traversing the LQDAG to find
valid interesting sort orders.  A node in the LQDAG could be traversed 
more than once, if there are alternative nesting structures above.
Interesting sort orders computed at a node can be memoized against 
the nesting structure to avoid repeated computation.

\subsection{Search for Best Plan and Cost-Based Pruning}
\label{subsec:search}
At the end of physical plan space generation we will have a physical query
{\small DAG} with a root physical equivalence node.  The best plan for the
{\small PQDAG} is computed recursively by adding the cost of each physical
operator to the cost of the best plans for its inputs and retaining the
cheapest combination. 

While computing the plan cost we take into account the fact that the {\em
use} sub-expressions of an {\em Apply} operator are evaluated as many times
as the cardinality of the {\em bind} sub-expression of the {\em Apply}
operator. If caching of sub-query results is employed, then the number of
distinct correlation bindings will be used in place of cardinality. Each
physical operator's cost function is enhanced to take an integer $n$ as a
parameter and return the cost for {\em n} invocations of the operator.
Memoization of the best plan is done for each 4-tuple (expression, output
physical properties, input parameter sort order, call count). This is
required since the best plan may be different for different call counts.  
%Call counts do not affect the physical DAG generation except by pruning
%parts of the DAG.

Optimization with different call counts can potentially increase the cost of
optimization.  However, if the plan is the same for two different call
counts, we can assume that it would be the same for all intermediate call
counts.  The same plan can then be reused for all calls with an intermediate
call count, with no further memoization required.  Results from parametric
query optimization \cite{ARU03} indicate that the number of different plans
can be expected to be quite small.  This helps in reducing both the  number
of plans memoized and the number of optimization calls.  We apply all simple
(non-nested) predicates before the nested predicate is applied.  This
further reduces the number of distinct call counts with which an expression
is optimized. 
\nocite{JOE94,SURAJIT96}

\eat{
We apply all simple (non-nested) predicates before the nested predicate is
applied.  This further reduces the number of distinct call counts with which
we optimize an expression.  And finally, if as a heuristic, nested calls are
made only after all other join predicates have been applied, we will have
exactly one call count for the nested expression. Adopting this heuristic,
however, may not always be a good
strategy~\cite{JOE94,SURAJIT96}.
}

\noindent {\bf Cost-Based Pruning} \\
\label{subsec:pruning}
In our description, we ignored cost-based pruning for simplicity and
separated the physical DAG generation and the search phases.  In our actual
implementation, the generation of the physical plan space and search for the
best plan take place in a single phase. While generating the physical plan
space, the cost of each plan is calculated and the best plan seen so far is
memoized. We perform cost-based pruning as in the original Volcano
algorithm~\cite{GRA93}.

\eat{
\noindent {\bf Semantics of Cost Limit} \\
\label{subsec:costlimit}
As described in \refsec{subsec:ext-overview}, the optimizer takes a cost limit
as one of its inputs and returns the best plan only if its estimated cost is
lesser than the given cost limit. When no plan with cost less than the given
cost limit can be found the optimizer remembers the cost for which the
optimization failed. Any future request for optimizing the same query with a
new cost limit triggers re-optimization only if the new cost limit is
greater than the cost limit at which the optimization had failed earlier.
With the modified optimizer method to deal with unbound parameters in the
query, the optimizer returns a {\em set} of plans each requiring a different
parameter sort order.  Hence, it is possible that for a given cost limit
some plans may be found and for a higher cost limit more plans with more
relaxed parameter sort orders would be found. To avoid frequent
re-optimizations we redefine the meaning of the cost limit as the cost limit
for the plan with the weakest parameter sort order (null). i.e., the
optimizer returns a set of plans for a given cost limit only if the cost of
the plan that requires no parameter sort order is less than the given cost
limit. The assumption here is that the plan requiring the weakest parameter
sort order would be the costliest of all plans.
}

\eat{
\subsection{Containment Differential}
\refsec{subsec:incragg} showed how nested aggregate queries can benefit
from sorted parameter bindings. In Example 5, we showed how a
state-retaining aggregate can work in conjunction with a restartable scan to
efficiently evaluate an aggregate sub-query having a non-equality predicate.
The aggregate values computed are incrementally updated in each invocation
of the sub-query, thus avoiding multiple scans of the relation referenced in
the sub-query.  In general, the input to the aggregate can be the result of a
parametrized sub-expression.

The state-retaining aggregate operator requires that, logically, its input
with the $i^{th}$ parameter value (in the specified parameter sort order) be
a superset of the input with the $(i-1)^{th}$ parameter value; further,
physically, the input with the $i$th parameter value should be just the
delta {\em w.r.t.} to the tuples seen till the ${i-1}^{th}$ parameter value.
In the optimizer we model this requirement on the input of the
state-retaining aggregate operator as a new physical property termed {\em
containment differential}. A state-retaining aggregate is applicable only
when its input satisfies the {\em containment differential} property for a
specified parameter sort order, that is, it returns only the differential
tuples when invoked with successive parameter values.  

Note that unlike the {\em sort order} physical property, where a plan that
guarantees some sort order can be used in a place where no sort order is
expected, a plan that satisfies the {\em containment differential} property
can be used only when the containment-differential property is expected from
the parent operator.
}


==> chapters/nqo/sections/sec_perf.tex <==
\section{Experimental Results}
\label{sec:perf:chap:nqo}
We implemented the state-retention techniques in {\small PostgreSQL}
%~\cite{POSTGRES} 
and carried out a performance study. The optimization techniques 
were implemented in our Volcano-style optimizer called PYRO, and these
plans were forced on PostgreSQL bypassing it optimizer.
We considered three algorithms: nested
iteration({\small NI}), magic decorrelation({\small MAG})~\cite{SPL96} and
nested iteration with state retention({\small NISR}). In the case of nested
iteration ({\small NI}) a suitable index was assumed to be present and used.
Whenever a relation was assumed to be sorted, the NI plan used a clustered
index. Magic decorrelation~\cite{SPL96} involves partially evaluating the
outer query block so as to identify the full set of parameters with which
the subquery is to be executed. The partial result of the outer query block
is called a {\em supplementary} table.  The correlated subquery is then
rewritten as a non-nested query by using an appropriate type of join with
the supplementary table.  The rewritten query produces the sub-query results
for the set of parameters from the supplementary table.  A join of the
rewritten sub-query and the supplementary table to evaluate the remaining
outer predicates gives the final result. For a more detailed description of
the magic decorrelation technique we refer the reader to ~\cite{SPL96}. In
our experiments, the plans employing magic decorrelation were composed with
the supplementary table materialized. 

%While performing the decorrelation of
%{\small NOT IN} queries we assumed the availability of sort-merge anti-join.
%When an implementation of anti-join is not available, decorrelation is not
%applicable and only nested iteration with indexing will be a candidate to
%compare with the plan generated by our algorithms.

{\small PostgreSQL} did not automatically decorrelate any of the queries 
we considered, and it always used a simple nested iteration plan. Hence, the
results noted for the nested iteration (NI) algorithm also act as the
baseline {\small PostgreSQL} measures. The plans employing state-retention
techniques and magic decorrelation were forced through code changes, 
bypassing the {\small PostgreSQL's} optimizer.

For our experiments, we used the {\small TPC-H}~\cite{TPCH} dataset on
1{\small GB} scale, and an additional relation, {\em dailysales} which had 2,500
records. The experiments are described below.

\eat{
The tables used for our experiments and the number of
tuples in each table are shown in \reffig{table:perftables}. 

\begin{figure}[ht]
\center
{ \small
\begin{tabular}{|c|c|c|c|} \hline
{\bf Name} & {\em orders} & {\em lineitem} & {\em part}  \\
\hline
{\bf Tuples} &  1,500,000 &  600,000 & 200,000 \\
\hline
\hline
{\bf Name} & {\em supplier} & {\em partsupp} & {\em dailysales} \\
\hline
{\bf Tuples} &  10,000 &  800,000 & 2,500 \\
\hline
\end {tabular}
}
\caption{Tables used for the Experiments}
\label{table:perftables}
\end{figure}
}

\subsubsection*{Experiment 1}
For this experiment, we used the query shown in \refex{query:nqoexp1},
which is a minor variant of the query given in \refex{ex:q1} of 
\refchap{chap:intro}. The query in \refex{ex:q1} uses a {\small NOT IN}
predicate whose decorrelated form requires an implementation of 
anti-join, which is not available in {\small PostgreSQL}. Hence, we 
changed the predicate to an {\small IN} predicate.

\begin{floatexample}
\begin{sqlindent}
\\
SELECT \>\> o$\_$orderkey, o$\_$orderdate FROM ORDERS \\
WHERE  \>\> o$\_$orderdate IN ( 
             \>\>\>\ \  SELECT l$\_$shipdate FROM LINEITEM \\
       \>\>  \>\>\>\ \  WHERE l$\_$orderkey = o$\_$orderkey);
\end{sqlindent}
\caption{Query Used in Experiment 1}
\label{query:nqoexp1}
\end{floatexample}

\begin{figure}[ht]
\centering
\includegraphics[angle=270,width=3.0in]{chapters/nqo/fig/NoAggEq.eps}
\caption{Performance Results for Experiment 1}
\label{fig:Query1}
\end{figure}

Figure~\ref{fig:Query1} shows the execution times for this query. Magic
decorrelation performs poorly because there are no outer
predicates and no duplicates. This leads to a large redundant join in the
plan produced by magic decorrelation.  Indexed nested loops join performs
significantly better but is still less efficient than nested iteration with
state retention. This is due to the overhead of index lookups. This overhead
is significant even though most of the index pages above the leaf level are
cached in memory.  
%A sort-merge anti-join implementation if present and used
%would perform exactly same as NISR and hence we have not consider it here
%explicitly. However, note that a sort-merge anti-join cannot be used if the
%correlated query block is part of a procedure or function where as NISR can
%be used in this case.

\eat{
\begin{figure}[ht]
\centering
\begin{tabular}{@{}c@{}c}
\begin{minipage}{0.5\textwidth} 
\includegraphics[angle=270,width=3.0in]{chapters/nqo/fig/NoAggEq.eps}
\caption{Performance Results for Experiment 1}
\label{fig:Query1}
\end{minipage}
&
\begin{minipage}{0.5\textwidth}
\includegraphics[angle=270,width=3.0in]{chapters/nqo/fig/AggNEq.eps}
\caption{Performance Results for Experiment 2}
\label{fig:Query2}
\end{minipage}
\end{tabular}
\end{figure}
}

\subsubsection*{Experiment 2}
For our second experiment we used the query shown in \refex{ex:q2} of
\refsec{subsec:incragg}. The query lists the days on which the sales exceeded
the maximum daily sales seen in the past.  Figure~\ref{fig:Query2} shows
the execution times for the plans.

\begin{figure}[ht]
\centering
\includegraphics[angle=270,width=3.0in]{chapters/nqo/fig/AggNEq.eps}
\caption{Performance Results for Experiment 2}
\label{fig:Query2}
\end{figure}

\noindent
For this query, nested iteration with state retention completely outperforms
magic decorrelation and plain nested iteration. Due to the presence of a
non-equality correlation predicate the cost of both magic decorrelation and
plain nested iteration increase very rapidly with the increase in the number
of outer block tuples. Nested iteration with state retention performs a
single scan of the inner and the outer relations as described in
\refsec{subsec:incragg}.

\subsubsection*{Experiment 3}
For our third experiment we used a query which is a modified version of the
{\small TPC-H} min cost supplier query shown in \refex{ex:tpch-mincost}
below.

\begin{floatexample}
\begin{sqlindent}
\\
SELECT \>\> s$\_$sname, s$\_$acctbal, s$\_$address, s$\_$phone \\
FROM   \>\> PARTS, SUPPLIER, PARTSUPP \\
WHERE  \>\> s$\_$nation='FRANCE' AND p$\_$size=15 AND p$\_$type='BRASS' AND \\
       \>\> p$\_$partkey=ps$\_$partkey AND s$\_$suppkey=ps$\_$suppkey AND \\
       \>\> ps$\_$supplycost =  \\
       \>\>	 \>\> (   SELECT min(PS1.ps$\_$supplycost) \\
       \>\>  \>\> \ \ FROM   PARTSUPP PS1, SUPPLIER S1 \\
       \>\>	 \>\> \ \ WHERE  p$\_$partkey=PS1.ps$\_$partkey AND \\
       \>\>	 \>\> \>\>     S1.s$\_$suppkey=PS1.ps$\_$suppkey AND \\
       \>\>	 \>\> \>\>     S1.s$\_$nation='FRANCE'); 
\end{sqlindent}
\caption{Query Used in Experiment 3}
\label{ex:tpch-mincost}
\end{floatexample}

The results are shown in figure~\ref{fig:Query3}(a). Magic decorrelation
performs the best because of the low selectivity of the outer predicates.
There were only 108 distinct tuples satisfying the outer predicates. Restart
scan performs poorly in this case as the entire relation is scanned where
only small fraction of it was required. However, as the selectivity of the
outer predicates increases, {\small NISR} becomes more attractive.  This is
evident from a second experiment that we carried out by dropping the
predicate "p$\_$size=15".  As can be seen in \reffig{fig:Query3}(b), {\small
NISR} performs better in this case.

\begin{figure}[ht]
%\vspace{-0.1in}
\begin{center}
\mbox{
	\subfigure[With all outer predicates]{\includegraphics[angle=270, width=3.0in]{chapters/nqo/fig/1Tpch.eps}} 
	\subfigure[Dropping `p$\_$size=15']{\includegraphics[angle=270, width=3.0in]{chapters/nqo/fig/2Tpch.eps}}
}
\caption{Performance Results for Experiment 3}
\label{fig:Query3}
\end{center}
\vspace{-5mm}
\end{figure}

\input{chapters/nqo/examples/udf-turnaroundtime.tex}

\subsubsection*{Experiment 4}
The query used in our fourth experiment is shown in
\refex{ex:udf-turnaroundtime}.  For this query, we compare only {\small NI}
with {\small NISR} since decorrelation techniques are not directly
applicable. The nested iteration plan employed a clustered index lookup on
the {\em lineitem} table, where as {\small NISR} employed two restartable
scans.  As can be seen in \reffig{fig:Query4}, {\small NISR} performs
significantly better than {\small NI}; this is because the inner relation
({\em lineitem}) is scanned at most twice with {\small NISR}, whereas
{\small NI} performs an indexed lookup of the inner relation for each tuple
in the outer relation.

\eat{
The fourth query is the query given in Example 2 of \refsec{sec:sec2}. The
query finds the turn around time for all high priority orders. As this query
invokes a user-defined function decorrelation techniques are not directly
applicable.
}
\begin{figure} [ht]
\center \includegraphics[angle=270,width=3in]{chapters/nqo/fig/FuncQ.eps}
\caption{Performance Results for Experiment 4}
\label{fig:Query4}
\end{figure}

\eat {
For Query 3, {\small MAG} perform the best since it applies all the
predicates of the outer query block to get the {\em binding relation} which
will be joined with the inner relations. Since there were only 108 distinct
tuples satisfying the outer predicates the extra cost incurred by {\small
NI} for the join of whole outer relation is reduced. Also since only a small
portion of the inner relations are touched, {\small NISR} performs badly
over the other techniques.

To study this behavior further, we evaluated query 3, dropping the predicate
''p$\_$size = 15''. This time since the selectivity of the outer predicates
increases (5684 invocations), the relative difference between the costs of
{\small NI} and {\small MAG} reduce. Also for the same reason, {\small NISR}
performs better.
}

\subsubsection*{Optimization Overheads}
The optimization overheads due to the proposed extensions in the 
Volcano optimizer were negligible. We measured the optimization 
time for complex nested queries, with up to 10 levels of nesting,
and observed no measurable overheads.





==> chapters/nqo/sections/sec_relwork.tex <==
\section{Related Work} 
\label{sec:relwork:chap:nqo}
Since early '70s, there has been extensive work in query optimization. An
excellent survey of query optimization techniques
is~\cite{SURAJIT-SURVEY98}.  Nested queries in particular, have received
significant interest; however, most of the emphasis so far has been on
decorrelation
techniques~\cite{KIM82,KIE84,GAN87,DAYAL87,MUR89,SPL96,GAL01,GAL07}.
Decorrelation of queries on XML databases with XQuery as the query language
is addressed in~\cite{MOER06}.  Decorrelation techniques try to rewrite a
given nested query into a form that does not use the nested subquery
construct.  Decorrelation techniques allow an optimizer to consider
alternative set oriented plans such as merge join or hash join for
evaluating a nested query, and in most cases these methods perform better
than the na\"\i ve nested iteration method. The techniques we proposed to
speed up nested iteration are orthogonal to decorrelation, and a cost-based
optimizer should consider both decorrelated evaluation and the
improved nested iteration methods while choosing the best plan. In this
chapter, we show several cases where the improved nested iteration methods
can perform significantly better than the plans generated by decorrelation
techniques.

Techniques for improving the performance of nested iteration have been
proposed by Selinger et.al.~\cite{SEL79} and Graefe~\cite{GRA03}. 
System R~\cite{SEL79} uses the idea of caching the
inner subquery result for distinct values of correlation variables and
sorting the outer tuples which allows caching of only one result of the
inner query at any point in time.  Graefe~\cite{GRA03} emphasizes the
importance of nested iteration plans and discusses asynchronous IO, caching
and sorting of outer tuples as techniques that can improve the performance
of nested iteration. Asynchronous IO as a means to improve iterative query
execution plans is also considered by Elhemali et.al.~\cite{GAL07} and
Iyengar et.al.~\cite{IYENGAR08}. Rao and Ross~\cite{JUN98} propose an
approach of improving the efficiency of iterative plans by identifying and
reusing invariants (sub-expressions within the nested sub-query, which are
not correlated to the outer query). The invariants can be computed just
once, in the first invocation, and reused for subsequent invocations of the
nested sub-query.  Akinde and B{\"o}hlen~\cite{AKINDE03} argue that
decorrelation techniques may not {\em always} produce the most efficient
plans, especially for complex {\small OLAP} queries, and propose generalized
multi-dimensional join ({\small GDMJ}) operator as an alternative means for
efficient evaluation of several types of {\small OLAP} queries.

The techniques we propose in this paper for improving the nested iteration
method augment the techniques proposed in \cite{SEL79} and \cite{GRA03}.
Sorting in System R is purely to ensure the cached result can be kept in
memory (only one cached result needs be retained). Graefe~\cite{GRA03}
describes sorting of outer tuples to produce advantageous buffer effects in
the inner query plan.  Both~\cite{SEL79} and \cite{GRA03} do not discuss the
changes required in the optimizer to consider these options and generate an
overall best plan.  Database systems such as Microsoft SQL Server consider
sorted correlation bindings and the expected number of times a query block
is evaluated with the aim of efficiently caching the inner query results
when duplicates are present, and to appropriately estimate the cost of
nested query blocks~\cite{GF04:sqlserveropt}. To the best of our knowledge,
the state-retention techniques and optimization of multi-branch, multi-level
correlated queries considering parameter sort orders have not been proposed
or implemented earlier.

\eat{
The Microsoft SQL Server query optimizer (which is also based on the
Volcano optimizer),
has an extension to the {\em findBest} procedure (their equivalent to our
FindBestPlan procedure), which passes it ``context'' information
\cite{GF04:sqlserveropt}.  The information in the context includes the
parameters, their sort order, number of rows required, and number of
expected executions.  The parameter sort order and number of expected
executions information is used to cost plans appropriately, taking cache
effects in index lookups into account, and to decide what results to
materialize.  The number of rows required is orthogonal to nested iteration,
and is used for top-K queries and for {\small EXISTS} sub-queries.   The same
subtree may be optimized under different contexts; however, further details
are not available to us.  As far as we are aware they cannot infer and use
interesting sort orders for parameters, and they do not handle state
retention.
}


==> chapters/nqo/sections/sec_sortorder.tex <==
\section{Definitions}
\label{sec:prelim:chap:nqo}

\begin{definition} 
{\bf Sort Order} \\
Let $s$ be a relational schema having $n$ attributes, $a_1, \ldots, a_n$. A
sort order {\em o} on schema $s$ is an ordered sequence of attributes from
any subset of $\{a_1, \ldots, a_n\}$.
\end{definition}

\noindent
We denote sort orders by enclosing the sequence of attributes in parentheses
as in $(a_1, a_4, a_5)$. A sort order $s=(a_{s1}, a_{s2}, \ldots, a_{sk})$ is
said to hold on a sequence of tuples conforming to schema $s$, if the
sequence has the tuples sorted on attribute $a_{s1}$ and for a given value
of $a_{s1}$ the tuples are sorted on $a_{s2}$, and so on up to $a_{sk}$.
Note that we ignore the sort direction (ascending/descending) in our
description. Sort direction can be represented by using the complement
notation, {\em e.g.}, $(a_1, \bar{a_2})$ can be used to represent a sequence
sorted in non-decreasing order on attribute $a_1$ and then in non-increasing
order on attribute $a_2$. The techniques we propose in this chapter are
applicable independent of the sort direction, and hence we omit the sort
direction in all our description.

\begin{definition} 
{\bf Subsumption of Sort Orders} \\
Sort order $o_1$ is said to subsume sort order $o_2$ iff $o_2$ is a prefix
of $o_1$.
\end{definition}
\noindent 
For example, sort order $(a,b,c)$ subsumes sort order $(a,b)$.
Note that the subsumption relation forms a partial order on the set of sort 
orders.



==> chapters/nqo/sections/sec_summary.tex <==
\section{Summary}
\label{sec:summary:chap:nqo}
In this chapter we revisited iterative execution plans for nested queries
and showed how sort order of parameter bindings can be exploited through
state retention to improve their execution time.  For several queries, even
when decorrelation is applicable, an iterative execution plan might be the
most efficient of the available alternatives and hence the optimizer's
search space should include these improved nested iteration plans and the
optimizer must estimate their cost appropriately.  We showed how a Volcano
style cost-based optimizer can be extended to take into account state
retention of operators and effects of parameter sort orders.  We presented a
performance study based on our implementation of the proposed techniques and
the results show significant benefits for several types of queries, with no
noticeable overheads in the optimization time. 


